Stochastic SketchRefine: Scaling In-Database Decision-Making under Uncertainty to Millions of Tuples

Decision making under uncertainty often requires choosing packages, or bags of tuples, that collectively optimize expected outcomes while limiting risks. Processing Stochastic Package Queries (SPQs) involves solving very large optimization problems on uncertain data. Monte Carlo methods create numerous scenarios, or sample realizations of the stochastic attributes of all the tuples, and generate packages with optimal objective values across these scenarios. The number of scenarios needed for accurate approximation - and hence the size of the optimization problem when using prior methods - increases with variance in the data, and the search space of the optimization problem increases exponentially with the number of tuples in the relation. Existing solvers take hours to process SPQs on large relations containing stochastic attributes with high variance. Besides enriching the SPaQL language to capture a broader class of risk specifications, we make two fundamental contributions towards scalable SPQ processing. First, to handle high variance, we propose risk-constraint linearization (RCL), which converts SPQs into Integer Linear Programs (ILPs) whose size is independent of the number of scenarios used. Solving these ILPs gives us feasible and near-optimal packages. Second, we propose Stochastic SketchRefine, a divide and conquer framework that breaks down a large stochastic optimization problem into subproblems involving smaller subsets of tuples. Our experiments show that, together, RCL and Stochastic SketchRefine produce high-quality packages in orders of magnitude lower runtime than the state of the art.

==> experiments/additional_cvar_constraints/quality.tex <==
\begin{table}[htb]
\caption{Quality of Generated Packages With Additional CVaR constraints}
\label{tab:cvar_constraint_specified}
\begin{tabular}{@{}llll@{}}
\toprule
                           &    & Rel. Diff. of CVaR (\%) & Rel. Diff. of Obj. Value (\%) \\ \midrule
\multirow{5}{*}{TPC-H}     & Q1 & 10.75                   & -5.34                         \\
                           & Q2 & 10.28                   & -4.24                         \\
                           & Q3 & 10.45                   & -2.36                         \\
                           & Q4 & 10.12                   & -8.91                         \\
                           & Q5 & 10.05                   & -12.31                        \\
\multirow{5}{*}{Portfolio} & Q1 & 10.04                   & -3.43                         \\
                           & Q2 & 10.13                   & -4.15                         \\
                           & Q3 & 10.25                   & -3.91                         \\
                           & Q4 & 10.14                   & -7.81                         \\
                           & Q5 & 10.34                   & -9.46                         \\ \cmidrule(l){2-4} 
\end{tabular}
\end{table}

==> experiments/alternative-partitioning/quality/combined-fig.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/tpch-q1}}  
          \caption{TPC-H Q1}
          \label{fig:alt_part_tpch_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/tpch-q2}}  
          \caption{TPC-H Q2}
          \label{fig:alt_part_tpch_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/tpch-q3}}  
          \caption{TPC-H Q3}
          \label{fig:alt_part_tpch_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/tpch-q4}}  
          \caption{TPC-H Q4}
          \label{fig:alt_part_tpch_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/tpch-q5}}  
          \caption{TPC-H Q5}
          \label{fig:alt_part_tpch_q5_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/pf-q1}}  
          \caption{Portfolio Q1}
          \label{fig:alt_part_pf_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/pf-q2}}  
          \caption{Portfolio Q2}
          \label{fig:alt_part_pf_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/pf-q3}}  
          \caption{Portfolio Q3}
          \label{fig:alt_part_pf_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/pf-q4}}  
          \caption{Portfolio Q4}
          \label{fig:alt_part_pf_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/alternative-partitioning/quality/pf-q5}}  
          \caption{Portfolio Q5}
          \label{fig:alt_part_pf_q5_obj}
\end{subfigure}


==> experiments/alternative-partitioning/rt-cmp.tex <==
\begin{table}[htb]
\caption{Offline Partitioning Runtimes}
\label{tab:rt-partitioning}
\begin{tabular}{lll}
\toprule
          & \dpart & \textsc{KD-Trees} \\
\midrule
TPC-H     & 2134 s                & 1782 s   \\
Portfolio & 3151 s                & 2756 s  \\
\bottomrule
\end{tabular}
\end{table}


==> experiments/increasing_tuples/quality/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/tpch-q1}}  
          \caption{TPC-H Q1}
          \label{fig:inc_tup_tpch_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/tpch-q2}}  
          \caption{TPC-H Q2}
          \label{fig:inc_tup_tpch_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/tpch-q3}}  
          \caption{TPC-H Q3}
          \label{fig:inc_tup_tpch_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/tpch-q4}}  
          \caption{TPC-H Q4}
\label{fig:inc_tup_tpch_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/tpch-q5}}  
          \caption{TPC-H Q5}
\label{fig:inc_tup_tpch_q5_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/pf-q1}}
    \caption{Portfolio Q1}
\label{fig:inc_tup_pf_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/pf-q2}}
    \caption{Portfolio Q2}
\label{fig:inc_tup_pf_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/pf-q3}}
    \caption{Portfolio Q3}
\label{fig:inc_tup_pf_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/pf-q4}}
    \caption{Portfolio Q4}
\label{fig:inc_tup_pf_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/quality/pf-q5}}
    \caption{Portfolio Q5}
\label{fig:inc_tup_pf_q5_obj}
\end{subfigure}



==> experiments/increasing_tuples/runtime/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/q1}}  
          \caption{TPC-H Q1}
          \label{fig:inc_tup_tpch_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/q2}}  
          \caption{TPC-H Q2}
          \label{fig:inc_tup_tpch_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/q3}}  
          \caption{TPC-H Q3}
          \label{fig:inc_tup_tpch_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/q4}}  
          \caption{TPC-H Q4}
          \label{fig:inc_tup_tpch_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/q5}}  
          \caption{TPC-H Q5}
          \label{fig:inc_tup_tpch_q5}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/pf-q1}}  
          \caption{Portfolio Q1}
          \label{fig:inc_tup_pf_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/pf-q2}}  
          \caption{Portfolio Q2}
          \label{fig:inc_tup_pf_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/pf-q3}}  
          \caption{Portfolio Q3}
          \label{fig:inc_tup_pf_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/pf-q4}}  
          \caption{Portfolio Q4}
          \label{fig:inc_tup_pf_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_tuples/runtime/pf-q5}}  
          \caption{Portfolio Q5}
          \label{fig:inc_tup_pf_q5}
\end{subfigure}






==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/q1}}  
    \caption{Portfolio Q1}
    \label{fig:inc_var_opt_rt_pf_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/q2}}  
    \caption{Portfolio Q2}
    \label{fig:inc_var_opt_rt_pf_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/q3}}  
    \caption{Portfolio Q3}
    \label{fig:inc_var_opt_rt_pf_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/q4}}  
    \caption{Portfolio Q4}
    \label{fig:inc_var_opt_rt_pf_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/q5}}  
    \caption{Portfolio Q5}
    \label{fig:inc_var_opt_rt_pf_q5}
\end{subfigure}

==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/q1.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1200)
    (2, 1400)
    (5, 3200)
    (8, 4800)
    (10, 5400)
    (13, 6500)
    (17, 7400)
    (20, 9500)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 330)
    (2, 580)
    (5, 670)
    (8, 730)
    (10, 1100)
    (13, 1300)
    (17, 1600)
    (20, 1900)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/q2.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1300)
    (2, 1500)
    (5, 3300)
    (8, 4900)
    (10, 5500)
    (13, 6600)
    (17, 7500)
    (20, 9600)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 340)
    (2, 590)
    (5, 680)
    (8, 740)
    (10, 1200)
    (13, 1400)
    (17, 1700)
    (20, 2000)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/q3.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1400)
    (2, 1600)
    (5, 4300)
    (8, 5100)
    (10, 5600)
    (13, 7100)
    (17, 8100)
    (20, 10100)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 540)
    (2, 690)
    (5, 780)
    (8, 840)
    (10, 1300)
    (13, 1600)
    (17, 1800)
    (20, 2100)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/q4.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1500)
    (2, 1700)
    (5, 5300)
    (8, 6100)
    (10, 6600)
    (13, 7200)
    (17, 8300)
    (20, 10900)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 540)
    (2, 690)
    (5, 780)
    (8, 840)
    (10, 1300)
    (13, 1600)
    (17, 1800)
    (20, 2100)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/portfolio/q5.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1600)
    (2, 1800)
    (5, 5400)
    (8, 6200)
    (10, 6700)
    (13, 7300)
    (17, 8500)
    (20, 11200)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 640)
    (2, 790)
    (5, 880)
    (8, 940)
    (10, 1400)
    (13, 1700)
    (17, 1900)
    (20, 2200)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q1}}  
    \caption{TPC-H Q1}
    \label{fig:inc_var_opt_rt_tpch_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q2}}  
    \caption{TPC-H Q2}
    \label{fig:inc_var_opt_rt_tpch_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q3}}  
    \caption{TPC-H Q3}
    \label{fig:inc_var_opt_rt_tpch_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q4}}  
    \caption{TPC-H Q4}
    \label{fig:inc_var_opt_rt_tpch_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q5}}  
    \caption{TPC-H Q5}
    \label{fig:inc_var_opt_rt_tpch_q5}
\end{subfigure}





==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q1.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1020)
    (2, 1670)
    (5, 3560)
    (8, 4600)
    (10, 5300)
    (13, 6400)
    (17, 7300)
    (20, 9400)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 320)
    (2, 570)
    (5, 660)
    (8, 720)
    (10, 1000)
    (13, 1200)
    (17, 1400)
    (20, 1500)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q2.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1120)
    (2, 1770)
    (5, 3660)
    (8, 4700)
    (10, 5400)
    (13, 6500)
    (17, 7400)
    (20, 9500)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 420)
    (2, 670)
    (5, 760)
    (8, 820)
    (10, 1100)
    (13, 1300)
    (17, 1500)
    (20, 1600)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q3.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1220)
    (2, 1870)
    (5, 3760)
    (8, 4800)
    (10, 5500)
    (13, 6600)
    (17, 7500)
    (20, 9600)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 500)
    (2, 800)
    (5, 900)
    (8, 1000)
    (10, 1100)
    (13, 1200)
    (17, 1400)
    (20, 1600)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q4.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1420)
    (2, 2070)
    (5, 4060)
    (8, 5000)
    (10, 6500)
    (13, 7600)
    (17, 8500)
    (20, 10600)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 600)
    (2, 900)
    (5, 1000)
    (8, 1100)
    (10, 1200)
    (13, 1300)
    (17, 1600)
    (20, 1900)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/average-optimizer-runtimes/tpc-h/q5.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge Optimizer Runtime (ms)},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=12000, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 1520)
    (2, 2170)
    (5, 4160)
    (8, 5100)
    (10, 6600)
    (13, 7700)
    (17, 8600)
    (20, 11600)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 700)
    (2, 1000)
    (5, 1100)
    (8, 1200)
    (10, 1300)
    (13, 1400)
    (17, 1700)
    (20, 2000)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q1}}  
    \caption{Portfolio Q1}
    \label{fig:inc_var_no_opt_pf_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q2}}  
    \caption{Portfolio Q2}
    \label{fig:inc_var_no_opt_pf_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q3}}  
    \caption{Portfolio Q3}
    \label{fig:inc_var_no_opt_pf_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q4}}  
    \caption{Portfolio Q4}
    \label{fig:inc_var_no_opt_pf_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q5}}  
    \caption{Portfolio Q5}
    \label{fig:inc_var_no_opt_pf_q5}
\end{subfigure}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q1.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 30)
    (2, 40)
    (5, 70)
    (8, 160)
    (10, 210)
    (13, 410)
    (17, 810)
    (20, 910)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 22)
    (2, 32)
    (5, 42)
    (8, 52)
    (10, 62)
    (13, 72)
    (17, 82)
    (20, 92)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q2.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 35)
    (2, 45)
    (5, 75)
    (8, 165)
    (10, 215)
    (13, 415)
    (17, 815)
    (20, 915)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 25)
    (2, 35)
    (5, 45)
    (8, 55)
    (10, 65)
    (13, 75)
    (17, 85)
    (20, 95)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q3.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 40)
    (2, 50)
    (5, 80)
    (8, 170)
    (10, 220)
    (13, 420)
    (17, 825)
    (20, 925)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 30)
    (2, 40)
    (5, 50)
    (8, 60)
    (10, 75)
    (13, 80)
    (17, 90)
    (20, 85)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q4.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 50)
    (2, 60)
    (5, 90)
    (8, 180)
    (10, 230)
    (13, 430)
    (17, 830)
    (20, 930)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 40)
    (2, 50)
    (5, 60)
    (8, 70)
    (10, 85)
    (13, 90)
    (17, 100)
    (20, 105)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/q5.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 70)
    (2, 80)
    (5, 100)
    (8, 190)
    (10, 240)
    (13, 440)
    (17, 840)
    (20, 940)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 50)
    (2, 60)
    (5, 70)
    (8, 80)
    (10, 95)
    (13, 100)
    (17, 110)
    (20, 115)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/combined-figure.tex <==
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q1}}  
    \caption{TPC-H Q1}
    \label{fig:inc_var_no_opt_tpch_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q2}}  
    \caption{TPC-H Q2}
    \label{fig:inc_var_no_opt_tpch_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q3}}  
    \caption{TPC-H Q3}
    \label{fig:inc_var_no_opt_tpch_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q4}}  
    \caption{TPC-H Q4}
    \label{fig:inc_var_no_opt_tpch_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
    \centering
    \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q5}}  
    \caption{TPC-H Q5}
    \label{fig:inc_var_no_opt_tpch_q5}
\end{subfigure}


==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q1.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 20)
    (2, 30)
    (5, 60)
    (8, 160)
    (10, 200)
    (13, 400)
    (17, 800)
    (20, 900)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 20)
    (2, 30)
    (5, 40)
    (8, 50)
    (10, 60)
    (13, 70)
    (17, 80)
    (20, 90)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q2.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 25)
    (2, 35)
    (5, 65)
    (8, 160)
    (10, 210)
    (13, 420)
    (17, 830)
    (20, 920)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 22)
    (2, 32)
    (5, 42)
    (8, 52)
    (10, 62)
    (13, 72)
    (17, 85)
    (20, 95)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q3.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 27)
    (2, 37)
    (5, 67)
    (8, 170)
    (10, 230)
    (13, 440)
    (17, 850)
    (20, 940)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 25)
    (2, 35)
    (5, 45)
    (8, 55)
    (10, 65)
    (13, 75)
    (17, 90)
    (20, 100)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q4.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 30)
    (2, 40)
    (5, 70)
    (8, 180)
    (10, 240)
    (13, 450)
    (17, 870)
    (20, 960)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 30)
    (2, 40)
    (5, 50)
    (8, 60)
    (10, 70)
    (13, 80)
    (17, 100)
    (20, 110)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/q5.tex <==
\begin{tikzpicture}[xscale=0.40, yscale=0.40]
\begin{axis}[
    xlabel={\huge Variance Coefficient},
    ylabel={\huge No. of opt. problems},
    legend columns=-1,
    legend entries={\ssearch, \cvarif},
    legend to name=named,
    yticklabel style = {font=\huge,xshift=0.4ex},
    xticklabel style = {font=\huge,yshift=0.4ex},
    xmin=1, xmax=20,
    ymin=0, ymax=1500, ymode=log,
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    height=5.5cm,
    width= 8.2cm,
]
\addplot[
    color=red,
    mark=triangle,
    line width=3
    ]
coordinates {
    (1, 35)
    (2, 45)
    (5, 75)
    (8, 185)
    (10, 245)
    (13, 455)
    (17, 875)
    (20, 965)
};
\addplot[
    color=blue,
    mark=square,
    line width=3
    ]
    coordinates {
    (1, 35)
    (2, 45)
    (5, 55)
    (8, 65)
    (10, 75)
    (13, 85)
    (17, 105)
    (20, 115)
};
\end{axis}
\end{tikzpicture}

==> experiments/increasing_variance/portfolio/combined-fig.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q1}}  
          \caption{Portfolio Q1}
          \label{fig:inc_var_pf_q1}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q2}}  
          \caption{Portfolio Q2}
          \label{fig:inc_var_pf_q2}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q3}}  
          \caption{Portfolio Q3}
          \label{fig:inc_var_pf_q3}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q4}}  
          \caption{Portfolio Q4}
          \label{fig:inc_var_pf_q4}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q5}}  
          \caption{Portfolio Q5}
          \label{fig:inc_var_pf_q5}
\end{subfigure}

==> experiments/increasing_variance/portfolio/quality-combined-fig.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q1-quality}}  
          \caption{Portfolio Q1}
          \label{fig:inc_var_pf_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q2-quality}}  
          \caption{Portfolio Q2}
          \label{fig:inc_var_pf_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q3-quality}}  
          \caption{Portfolio Q3}
          \label{fig:inc_var_pf_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q4-quality}}  
          \caption{Portfolio Q4}
          \label{fig:inc_var_pf_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/portfolio/q5-quality}}  
          \caption{Portfolio Q5}
          \label{fig:inc_var_pf_q5_obj}
\end{subfigure}



==> experiments/increasing_variance/tpc-h/combined-fig.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q1}}  
          \caption{TPC-H Q1}
          \label{fig:inc_var_tpch_q1}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q2}}  
          \caption{TPC-H Q2}
          \label{fig:inc_var_tpch_q2}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q3}}  
          \caption{TPC-H Q3}
          \label{fig:inc_var_tpch_q3}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q4}}  
          \caption{TPC-H Q4}
          \label{fig:inc_var_tpch_q4}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q5}}  
          \caption{TPC-H Q5}
          \label{fig:inc_var_tpch_q5}
     \end{subfigure}

==> experiments/increasing_variance/tpc-h/quality-combined-fig.tex <==
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q1-quality}}  
          \caption{TPC-H Q1}
          \label{fig:inc_var_tpch_q1_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q2-quality}}  
          \caption{TPC-H Q2}
          \label{fig:inc_var_tpch_q2_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q3-quality}}  
          \caption{TPC-H Q3}
          \label{fig:inc_var_tpch_q3_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q4-quality}}  
          \caption{TPC-H Q4}
          \label{fig:inc_var_tpch_q4_obj}
\end{subfigure}
\begin{subfigure}[b]{0.18\textwidth}
          \centering
          \resizebox{\linewidth}{!}{\input{experiments/increasing_variance/tpc-h/q5-quality}}  
          \caption{TPC-H Q5}
          \label{fig:inc_var_tpch_q5_obj}
\end{subfigure}



==> experiments/query-hardness/hardness.tex <==
\begin{table}[t]
\caption{Query Hardnesses}
\label{tab:query-hardness}
\begin{tabular}{llll}
\toprule
\multicolumn{2}{l}{TPC-H} & \multicolumn{2}{l}{Portfolio} \\
\midrule
Query     & Step Count    & Query       & Step Count      \\
\midrule
Q1        & 100           & Q1          & 55              \\
Q2        & 90            & Q2          & 45              \\
Q3        & 80            & Q3          & 35              \\
Q4        & 70            & Q4          & 25              \\
Q5        & 60            & Q5          & 20             \\
\bottomrule
\end{tabular}
\end{table}

==> queries/portfolio-query-template.tex <==
\begin{lstlisting}[basicstyle=\footnotesize\ttfamily\bfseries]
SELECT PACKAGE(*)
FROM Stock_Investments
SUCH THAT
  SUM(Price) <= P AND
  SUM(Gain) <= G WITH PROBABILITY <= p
MAXIMIZE EXPECTED SUM(Gain)
\end{lstlisting}

==> queries/spaql_with_cvar.tex <==
 \begin{flushleft}
    \texttt{\footnotesize SELECT PACKAGE(*) AS PORTFOLIO\\
        FROM Stock\_Investments\\
        SUCH THAT\\
        \hspace{0.2cm} SUM(Price)<=1000 AND\\
        \hspace{0.2cm} EXPECTED SUM(Gain)>=-10 IN LOWEST 5\% OF SCENARIOS\\
        MAXIMIZE EXPECTED SUM(Gain)}
\end{flushleft}

==> queries/tpch-query-template.tex <==
\begin{lstlisting}[basicstyle=\footnotesize\ttfamily\bfseries]
SELECT PACKAGE(*)
FROM Lineitem
SUCH THAT
  SUM(Tax) <= T AND
  SUM(PRICE) >= P WITH PROBABILITY <= p AND
  SUM(QUANTITY) >=Q WITH PROBABILITY <=q
MAXIMIZE EXPECTED SUM(PRICE)
\end{lstlisting}

==> response.tex <==
% !TeX spellcheck = en_US
%\documentclass{vldb}
%\usepackage{balance}
%\usepackage{color}
%\usepackage{xspace}
%\usepackage{amsfonts}
%\usepackage{microtype}
%\usepackage{graphicx}
%\usepackage{color}
%\usepackage{bm}
%\usepackage{subfig}
%\usepackage{url}
%\usepackage{enumitem}
%\usepackage{paralist}
%\usepackage{caption}
%\usepackage[square,numbers]{natbib}
%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm,thmtools,xcolor}
%\input{response_macros}

%\definecolor{mygreen}{rgb}{0,0.6,0}
%\definecolor{mygray}{rgb}{0.5,0.5,0.5}
%\definecolor{mymauve}{rgb}{0.58,0,0.82}

%\newcommand{\pvt}{PVT\xspace}
%\newcommand{\new}[1]{{\color{blue}#1}}
%\newcommand{\reva}[1]{{\color{red}#1}}
%\newcommand{\revb}[1]{{\color{mygreen}#1}}
%\newcommand{\revc}[1]{{\color{mymauve}#1}}
%\newcommand{\sq}{\hbox{\rlap{$\sqcap$}$\sqcup$}}
%\renewcommand{\dblfloatpagefraction}{0.9}
%\renewcommand{\floatpagefraction}{1}

%\usepackage{zref-xr}
%\zxrsetup{toltxlabel=true, tozreflabel=false}
%\usepackage{xcite}
%\externalcitedocument{../paper}
%\zexternaldocument*{../paper}

%\declaretheoremstyle[
%headfont=\color{blue}\normalfont\bfseries,
%bodyfont=\color{blue}\normalfont,
%]{colored}

%\newtheoremstyle{mystyle}%
%{3pt}% Space above
%{3pt}% Space below 
%{\itshape\color{teal}}% Body font
%{}% Indent amount
%{\bfseries\color{teal}}% Theorem head font
%{.}% Punctuation after theorem head
%{.5em}% Space after theorem head
%{}% Theorem head spec (can be left empty, meaning ‘normal’)

%\theoremstyle{mystyle}
%\newtheorem{thm}{Theorem}
%\newtheorem{Meta}{Comment}
%\newtheorem{Comment}{Comment}
%\newtheorem{Weak}{Weak Point}
%\theoremstyle{definition}
%\newtheorem*{Response}{Response}

\begin{document}
%\pagenumbering{roman}

%\twocolumn[
%\begin{center}
%    {\LARGE \textbf{Response to Reviewer Comments (Paper \#1216)}} \\
%    \vspace{2mm}
%    {\Large{Stochastic SketchRefine: Scaling In-Database Decision-Making under Uncertainty to Millions of Tuples
%}}
%\end{center}
%\vspace{10mm}
%]

%We thank the reviewers and the meta-reviewer for their insightful comments on our VLDB submission and their suggestions on how to strengthen our paper. We used their comments, questions, and suggestions to revise and improve our paper. Our revision includes changes throughout the paper, our Github repository, and the extended version of our paper. These changes include clarifications to the points of confusion, additional details on prior literature and further experimental evaluation to support out claims.

%\smallskip

%\noindent\textbf{Color-coding in the revised submission.} Our revised submission
%highlights particular new additions to the paper that directly address reviewers' comments. In the revised version of our manuscript, changes with respect to the submitted version are highlighted in \reva{red} for Reviewer 1, \revb{green} for Reviewer 2 and \revc{purple} for Reviewer 4.
%Additional changes that are common to reviewers 2 and 4 are in \new{blue}.

%\smallskip

%In this cover letter, we provide a summary of our revisions based on the reviews. We quote reviewer comments in {\color{teal} teal}, above our responses.

%\section{Meta-Reviewer}

%\begin{Meta} 
%\smallskip
%Thanks for your submission. The reviewers have decided to give the authors a chance to revise their work. Please follow the revision items mentioned in Q14 in the reviews.
%\end{Meta}

%\begin{Response} 

%We have worked to incorporate all of the required revisions, which resulted in a considerable amount of new material. We believe we have addressed the reviewers' requests comprehensively and thoroughly. We include here a summary of the changes; we provide more extensive discussion of each change in our responses to the corresponding reviewer comments.

%\begin{compactitem} 
	
	 %\item We took steps to make the paper more self-contained, with a more detailed overview of prior package query solvers \ssearch and \skr, and provided details on how existing probabilistic data management systems like the MCDB models uncertainty in Section \riddho{Not sure if these details should go in the related works section or if they should come earlier. I suppose adding a `background'-like section would be overkill}. We further included proof sketches, incorporated changes to accommodate suggested flow improvements.
     
     %\item We added further details in Section $4$ to clarify confusion raised by the reviewers about how duplicates are used in \sskr.

     %\item We added details in Section 5 on how MAD and \dpart ensure that tuples in the same partition are pairwise similar w.r.t. each attribute in the dataset, and added both experimental validation and theoretical results to show that MAD robustly captures inter-tuple similarity even for stochastic attributes with mixed distributions. We provide further experimental results in Section 7 that show that \dpart results in more optimal packages being produced than when using existing high-dimensional clustering approaches or dimensionality reduction techniques. \riddho{I haven't experimentally verified the claims in the last sentence yet.}

	 %\item In our extended arXiV paper, we added appendix sections that contain sample portfolios produced by \sskr, and evaluate their constraint satisfaction among out-of-sample scenarios. Furthermore, we added ablation studies that show that replacing \lcsolve with \ssearch for solving sketch and refine SPQs, and not using duplicates during Sketch results in larger runtimes and suboptimal packages being produced respectively. 

     %\item We added details on mini-experiments we conducted that helped us understand the appropriate size and diameter thresholds based on our underlying system software and hardware capabilities. Users can repeat these experiments on their own machines to define these thresholds similarly. For other hyperparameters in our algorithms, we conduct sensitivity analyses to show that our results are not sensitive to minor changes in their values.

	 
%\end{compactitem}

%\end{Response}



%\section{Reviewer \#1}
%\smallskip

%\begin{Comment}[O1]

%Explain why l-cvar **with relaxed bounds** can produce a meaningful approximation of cvar.

%\end{Comment}

%\begin{Response}
%Thank you for this suggestion. To provide further intuition behind why appropriately relaxing \LCVaR-constraints can help approximate non-linear VaR constraints, we provide a pictorial representation of the search conducted by \sskr in Appendix Section --. \riddho{I am envisioning pictures that show \href{https://docs.google.com/drawings/d/1aIxZHnD9d_moqxaV1nB9hxXr846CtTvv7dZhEbnh2Es/edit?usp=sharing}{overconstrained}, \href{https://docs.google.com/drawings/d/1reE3zeyTG05kafiQGuiBdYAVPQHwnH0VUPxW-vgnuG0/edit?usp=sharing}{underconstrained} and \href{https://docs.google.com/drawings/d/1SBwuh3JCFnol-wRhafcqhm-dtGscJkcfr9jlfBLqrns/edit?usp=sharing}{appropriately constrained} regions. (Hyperlinks should redirect to the drawings I have in mind) Should we consider an alternative approach for explaining this?}

%\anh{Here is a high-dimensional explanation: Each \LCVaR is a high-dimensional hyperplane. The $\alpha$-search and $V$-search in APS modify the coefficients of this hyperplane so that the resulting package is the best possible solution in the validation-feasible region obtained using \LCVaR. This is equivalent to translate and rotate the hyperplane to fit the boundary of the validation-feasible region.}

%\end{Response}


%\begin{Comment}[O2]

%More precisely define the uncertainty model.

%\end{Comment}
%\begin{Response}
%We added a more formal definition of how our underlying probabilistic DBMS produces the scenarios, using the idea of Variable-Generator functions from Monte Carlo databases in Section --. \riddho{Does this suffice as the specification of an uncertainty model?}
%\end{Response}

%\begin{Comment}[O3]
%Include a more detailed overview of prior work. The paper is not entirely self-contained, relying heavily on the reader's familiarity with probabilistic databases (notably MCDB), and prior work in the package queries space (notably SketchRefine and SummarySearch). It would significantly strengthen the paper to include a bit more background on how stochastic attributes are modeled (at present, the closest thing to a formal specification of a scenario is Figure 1), and a slightly more formal specification of SketchRefine (beyond the prose sketch in S1).
%\end{Comment}

%\begin{Response}
%We added a more formal specification of how \skr and \ssearch works in the related works section. \riddho{Assuming that's where this will be added} A more detailed overview of how MCDB-s create scenarios is provided in Section -- as mentioned in our response to O2. 

%\end{Response}



%\begin{Comment}[O4]\label{com:conditional}
% Address concerns about mixed distributions. the use of MAD for stochastic attributes is appropriately justified, but still feels off for some reason I can't fully pin down. I think part of the issue is that the interesting feature of the distribution with respect to l-cvar, is the distribution's tail behavior. As long as all stochastic variables in a partition are drawn from distributions that behave similarly, taking the average across all scenarios should create a relatively representative element for each partition. However, I'm not convinced that this will continue to be the case if different tuples draw from meaningfully different distributions. This potential challenge is occluded in the experiments, where all tuples draw from the same (relatively well behaved) distribution. I don't think this is necessarily a problem, as every probabilistic database use case that I can think of generally avoids mixtures of distributions for a single attribute, but I would either scale back the claims, or add some validation (theoretical, or experimental) that MAD is a meaningful measure for mixed distribution datasets.
%\end{Comment}

%\begin{Response}
%We thank the reviewer for raising this interesting point. In our revision, we add Theorem -- in Section --- that constraining the MAD between any two tuples restricts the difference in their \LCVaR-s, regardless of their underlying distributions. \riddho{This theorem is currently the first half of Theorem D.1, but I am assuming we will need to add it as a formally stated standalone theorem that will be mentioned in section 5, with the proof in Appendix Section D. Does that seem reasonable?}

%Furthermore, we conducted an experiment, whose results are given in Appendix Section --, which shows that even when two tuples have highly different distributions such as a uniform distribution between~$[0, 100]$ and a pareto distribution where the tail goes to 0 at rate alpha in (0,2], MAD is able to capture the increasing similarities in their tail behaviours as the inter-tuple correlation increases. The pareto distribution has infinite variance, which shows that MAD shows expected behaviour even for tuples with heavy-tailed and wildly different distributions for a stochastic attribute. \riddho{This is referring to Peter's experiment}

%\riddho{The only further bit of supporting evidence we could add here is an end-to-end experiment where some attribute has different underlying distributions for different tuples. Due to implementation choices made in the codebase earlier, this is a little hard to implement (the only revision-related experiment which is hard to implement here). I have started to implement it, but I was hoping we could avoid having to do it. The reviewer asks for theoretical or experimental validation, and we've already provided both, so I wonder how much info this additional end-to-end experiment will add.}
%\end{Response}

%\begin{Comment}[O5]

%Flow improvements...One `aha' moment when reading the paper was the realization that linear cvar computation was operating on a single variable, while the general cvar computation was operating on a sum -- this led to the realization that the linear optimization was basically a trick to pull the summation out of the body of the cvar. I think what made this hard is the fact that cvar() is applied to a single random variable (that may be a sum), while l-cvar() operates on a collection of random variables. That being said, I can't think of an elegant way to make this notion clearer...fundamentally I didn't quite follow the intuition for why cvar doesn't commute through sum. The 'the need for duplicates' paragraph in S4.1 helped clarify some of this confusion, so perhaps it might be helpful to move this paragraph earlier.

%\end{Comment}
%\begin{Response}
%We thank the reviewer for highlighting this fundamental insight. In Section~2, we add some additional details to help readers better understand this, and explain why CVaR of an entire package cannot be expressed as a combination of the CVaRs of the individual tuples, but how \LCVaR-constraint are readily expressed that way --- which simplifies their expression in ILPs.

%\end{Response}

%\begin{Comment}[O6]
%Add proof sketches.
%\end{Comment}

%\begin{Response}
%We added proof sketches for theorems 3.1 and 6.1.
%\end{Response}
%\section{Reviewer \#2}
%\smallskip

%\begin{Comment}[O1]
%I'd like to see an experiment that verifies the correctness of the Stochastic SketchRefine. Correctness could be shown empirically using Monte-Carlo simulation.
%Once could simulate $N$ $(N>>100)$ possible worlds (or scenarios as called in the paper), and check in each possible worlds if the probabilistic constraints are violated. It should hold that a constraint such as `$P(Loss>10)<5\%$' will be violated in no more than $5\%$ of possible worlds. If this number is significantly higher, then we know that the assumption of duplicate worlds indeed leads to erroneous results.
%I understand that space limitations make it difficult to include such experiments in the manuscript, but authors may consider adding it to their arxiv version, or at least adding a note to the paper that such as experiment was performed and successful without adding the results to the paper (but of course adding the experiments to github) to be reproduced by interested readers.
%\end{Comment}

%\begin{Response}
%Every package produced during \sskr from $~100$ optimization scenarios are then validated over a much larger set of $10^6$ validation scenarios to test if they satisfy the probabilistic constraints among them.  We added experiments where the final packages were evaluated over a further $10^6$ `test' validation scenarios to see how they fare in them. We found out that each of our generated packages also satisfy every risk constraint specified in the query were satisfied among these test scenarios as well. We added a note in the experimental section of the main paper to clarify that these experiments were conducted, added the detailed results in the Appendix Section --, and added instructions to reproduce these results in our Github repository.

%We further understand that the concerns regarding \sskr's correctness stems from fears that duplicates may create overly diverse representations from underlying partitions with a small number of tuples, or tuples with a highly positive correlation among them. However, \sskr avoids this by never creating more duplicates than the number of tuples in the underlying partition. The correlation between the duplicates is also the median correlation between the tuples in the partition.

%In case the risk constraints in the SPQ are relaxed enough to allow the same stock to be selected multiple times, while \sskr may select multiple duplicates of the representative of that stock during Sketch, they will all be replaced by the most profitable stock from that partition during Refine. We appended our descriptions in Section~4 to clarify this.
%\end{Response}


%\begin{Comment}[O2]
%\label{comment:actual_pack}
%It would be good to show some example results. How practically useful as the results? Are these results meaningful portfolios? Or are these unrealistic purchases of "duplicates" of the same stock over and over again.

%\end{Comment}

%\begin{Response} 

%We provide some examples of portfolios generated by \sskr in Appendix Section --. The packages suggest reasonably diverse portfolios. Duplicates of a representative are always replaced by actual stocks from their partition during refine, and thus never appear in the final result.
%\end{Response}


%\begin{Comment}[O3]

%Having a kd-tree as a state-of-the-art competitior for high-dimensional clustering is not appropriate. A better baseline (for example, dimensionality reduction into low dimensional clustering) and state-of-the-art clustering solutions for high dimensional clustering (see surveys on this topic) should be compared against.
%\end{Comment}
%\begin{Response}
    
%\riddho{This is the only comment I haven't experimentally verified from my end, partially because there's a lot of potential things we could do. Firstly, the reviewer misunderstands that we never really combine across multiple attributes. We need to clarify that + provide some sort of experimental validation as requested. My plan is to stack a vector with each scenario value for each attribute of a tuple together to make one big vector, and apply one high-dimensional clustering technique and one dimensionality reduction technique to make empirical comparisons as Anh suggested, and add them to the appendix.}
%\end{Response}


%\section{Reviewer \#4}
%\smallskip
%\begin{Comment}[O1]

%No sensitivity analysis to multiple parameters. How should a user set the hyper parameters of the system?
%\end{Comment}
%\begin{Response}
%Throughout our experiments, the most sensitive parameters to set remain the size and diameter thresholds for \dpart. We added experiments in Appendix Section -- to show how we chose our size thresholds w.r.t. the optimizer software's performance in our experimental setup. The choice of diameter thresholds can vary based on application requirements on runtime and quality of results. However, we provided some additional experiments in Appendix section -- to show how we experimented with different diameter threshold settings and decided the diameter thresholds based on the number of partitions produced for different alternatives. The user may wish to repeat such an analysis to set their own diameter thresholds in different datasets. We further showed that our experimental results are robust to changes in the values of all other hyperparameters in Appendix Section --. 
%\end{Response}


%\begin{Comment}[O2]

%No ablation study to show the relative improve of each of the algorithmic component is given.
%\end{Comment}
%\begin{Response}
    
%We extended our evaluation in Appendix Section -- to show that replacing \lcsolve with \ssearch as our solver for \sskr's sketch and refine SPQs result in increased end-to-end runtimes. Furthermore, we show that not having duplicates for representatives significantly reduces the objective value of the packages produced in Appendix Section --. We also showed earlier that replacing \dpart with \kd like previous approaches results in worse packages.
%\end{Response}

%\begin{Comment}[O3]

%How practical are the results? Do they represent meaningful portfolios, or do they reflect unrealistic scenarios, such as repeatedly purchasing "duplicates" of the same stock? Consider adding a case study to demonstrate the output of the proposed algorithm on real-life data.
%\end{Comment}

%\begin{Response}
    
%Same as comment~\ref{comment:actual_pack}?

%\end{Response}

%\begin{Comment}
    %Overall the paper is very hard to read and follow. There are almost no examples given, and the notations are confusing. Consider adding a table for frequently used notations and using the stocing example as a running example to explain the algorithm components and definitions.
%\end{Comment}

%\begin{Comment}
 %   The authors mentioned that one of their contributions is to extend SPaQL to allow for the expression of CVaR constraints, which allow for better risk control in stochastic optimization problems. There is no evaluation of the usability of the these extensions. How easy it is to use the query language? why did you choose to focus in these new constraints? are they expressive enough to cover all scenarios?
%\end{Comment}

%\begin{Response}
    %\riddho{I am actually somewhat confused as to what extent we can incorporate changes for these two comments given the page limitations.}
%\end{Response}

\end{document}





==> response_cover_letter.tex <==
\twocolumn[
\begin{center}
    {\LARGE \textbf{Response to Reviewer Comments (Paper \#1216)}} \\
    \vspace{2mm}
    {\Large{Stochastic SketchRefine: Scaling In-Database Decision-Making under Uncertainty to Millions of Tuples
}}
\end{center}
\vspace{10mm}
]

We thank the reviewers and the meta-reviewer for their insightful comments on our VLDB submission and their suggestions on how to strengthen our paper. We used their comments, questions, and suggestions to revise and improve our paper. Our revision includes changes throughout the paper, our Github repository, and (because of space limitations) the extended arXiv version of our paper \cite{haque2024stochastic}. These changes include clarifications on points of confusion, additional details on prior literature, and further experimental evaluation to support our claims.


%\noindent\textbf{Color-coding in the revised submission.} 
Our revised submission
highlights updates to the paper that directly address reviewers' comments. In the revised version of our manuscript, changes with respect to the submitted version are highlighted in \reva{red} for Reviewer 1, \revb{green} for Reviewer 2 and \revc{purple} for Reviewer 4. Additional changes that are common to reviewers 2 and 4 are in \revbc{blue}.

In this cover letter, we provide a summary of our revisions based on the reviews. We quote the reviewer's comments in {\color{teal} teal}, above our responses.


\medskip
\noindent
\textbf{Additional material.}
In addition to the highlighted changes, we also had to significantly compress prior content in order to make space for the new material requested by the reviewers.  Notably, the theoretical analysis (previously Section 6) and the experimental comparison of \dpart with alternative schemes, have been moved to the online Appendix~\cite{haque2024stochastic}.  The reviewers can access \textbf{a color-coded version of the extended paper} (including the Appendix), in our GitHub repository:\\
\sloppy \url{https://github.com/RiddhoHaque/stochastic-sketchrefine/blob/main/StochasticSR_Extended_Version.pdf}
% (\appref{sec:theory} and \appref{sec:ablation_dpart}).



\section{Meta-Reviewer}

\begin{Meta} 
Thanks for your submission. The reviewers have decided to give the authors a chance to revise their work. Please follow the revision items mentioned in Q14 in the reviews.
\end{Meta}

\begin{Response} 

We have worked to incorporate all of the required revisions, which resulted in a considerable amount of new material. We believe we have addressed the reviewers' requests comprehensively and thoroughly. We include here a summary of the changes; we provide more extensive discussion of each change in our responses to the corresponding reviewer comments.

\begin{compactitem} 
	
	 \item We attempted to make the paper more self-contained, with an overview of the prior package query solvers \ssearch and \skr, and added details on how existing probabilistic data management systems like the MCDB model uncertainty. We further included proof sketches and incorporated changes suggested by the reviewers for flow improvements.
     
     \item We revised Section~\ref{sec:cvarif} to remove some confusion about the nature of risk-constraint linearization.
     
     \item We added further details in Section~\ref{section:sskr} to clarify confusion raised by the reviewers on the use of duplicates by \sskr.

     \item We added details in Section~\ref{sec:partitioning} on how MAD and \dpart ensure that tuples in the same partition are pairwise similar w.r.t. each attribute in the dataset, and added both experimental validation and theoretical results to show that MAD robustly captures inter-tuple similarity even for stochastic attributes with widely varying distributions and heavy tails. We provide further experimental results in \appref{sec:ablation_dpart} that show that \dpart results in more optimal packages being produced than when using existing high-dimensional clustering approaches or dimensionality reduction techniques.

	 \item In our extended arXiv paper~\cite{haque2024stochastic}, we added an appendix section that contains an example portfolio produced by \sskr. Furthermore, we added an ablation study that shows that not using duplicates during Sketch results suboptimal packages being produced. 

     \item We added details on mini-experiments we conducted that helped us understand the appropriate hyperparameter settings based on our underlying system software and hardware capabilities. Users can repeat these experiments on their own machines to appropriately define size and diameter thresholds in their own setup. For other hyperparameters, we conducted sensitivity analyses to show that our results are not sensitive to minor changes in their values.
\end{compactitem}

\end{Response}

\section{Reviewer \#1}

\begin{cmt}[R1]
I'm not sure I fully grok the idea behind linearized cvars [...] Is there a good intuition for why is it reasonable to expect that an l-cvar constraint forms a bound on the corresponding cvar constraint? Second, it's not entirely clear to me that this fact (and by extension Theorem~\ref{th:constraintCompare}) is relevant, since the entire goal of Algo~\ref{alg:lcsolve} is just to find an appropriate relaxation of the bound. Instead, I'd be more interested in a proof, or at least an intuition for how accurate this approximation produces. Explain why l-cvar **with relaxed bounds** can produce a meaningful approximation of cvar.
\end{cmt}

\begin{Response}
%\azza{It's a bit weird and repetitive to thank the reviewers for every point. Just jump into the response.}
Thank you for pointing out this gap in intuition---we have revised Section~\ref{sec:cvarif} to avoid confusion.  We clarify the fact that RCL is best viewed not as a process of individually ``approximating'' each VaR or CVaR constraint by an \LCVaR constraint (the reviewer is correct that this approximation notion is not really precise), but rather modifying the \LCVaR parameters, which corresponds to shifting and rotating the linear \LCVaR constraints in the feasible-region polytope, to ensure that the modified region contains a ``truly feasible'' (in the sense of validation-feasible) package solution whose objective value is ``close to'' that of the optimal solution to the original problem (in the sense of $\epsilon$--optimality). We also clarify that the search for optimal parameters is not guaranteed to be successful, but the user will know if the search is successful or not. If successful, the returned package solution is guaranteed to be feasible and $\epsilon$--optimal; if not successful, the solution is guaranteed to be feasible but no guarantees are given on the optimality of the objective value. In the latter case, the user can try increasing the number of validation scenarios. (We did not observe any failed searches in any of our experiments, which leads us to conjecture that such failure is unlikely.)

The key reason for Theorem~\ref{th:constraintCompare} is to allow us to search for an appropriate \LCVaR parameterization within a bounded set of parameter values---see the final paragraph of the \textbf{Overview} section in Section~\ref{sec:cvarif}---which significantly simplifies the search process. We have added sentences clarifying this fact.
% \azza{Do we spell out the bounds here or at least point to page 5, para 2.}\azza{I'm also not finding this convincing at all. The statement of theorem 2.1 is clearly just about the validity of the approach. If you replace VaR constraints with L-CVaR constraints, if it holds for L-CVaR it will hold for VaR... the theorem statement provides no intuition for bound setting and so this is a bit misleading. I think we include it simply because it is not obvious that L-CVar ==> CVaR ==> VaR (it may be for people in the field but not for this audience) and that is why we have it in the paper: that's our reason even if the reviewer sees no reason for it or miscorrectly thinks that the only purpose to have is if it gives an "approximation bound." We already explain that this is not how he should read RCL. How this theorem translates to bound setting either needs to be spelled out or we keep our reasoning on point.}
%The theorem proves that \LCVaR constraints with their most stringent parameterizations yield a feasible region that is a subset of the feasible region defined via the original risk constraints. We added further explanations in Section~\ref{sec:cvarif}, in the subsection titled `\textbf{The case of a single risk constraint}' showing that the package returned by the least restrictively parameterized \LCVaR constraints do not satisfy ``non-trivial'' risk constraints, i.e., constraints that are not satisfied by packages that solve the relaxed query $Q^D$ in which all risk constraints are removed.
%Theorem~\ref{th:constraintCompare} proves that with their most stringent parameterizations, \LCVaR constraints are at least as restrictive as the risk constraints they replace. We added further explanations in Section~\ref{sec:cvarif}, in the subsection titled `\textbf{The case of a single risk constraint}' that show that the package returned by the least restrictively parameterized \LCVaR constraints do not satisfy non-trivial risk constraints.
%We further added geometric intuitions in the same subsection to help readers understand how appropriately adjusting the parameters of the \LCVaR constraints can help \lcsolve to strike a balance between making the \LCVaR constraints overly restrictive and not restrictive enough. Subsequently, Theorem~\ref{th:alternating_parameter_search} proves that the alternating parameter search employed by \lcsolve indeed finds the least restrictive parameterization of the \LCVaR constraint that results in a feasible package.

%To evaluate if the package generated using this finally-obtained \LCVaR parameterization is near-optimal, \lcsolve checks the objective value of the package and generally only returns it if the objective value is at least $(1 - \epsilon)$ times an upper bound $\omega_0$, as mentioned in the subsection titled `\textbf{Termination and guarantees}'. As further mentioned there, if the generated package is not deemed to be $(1 \pm \epsilon)$-optimal even after maxing out the number of optimization scenarios to $\hat{m}$, i.e., the number of validation scenarios, \lcsolve will return with the best package found thus far but with no guarantees on how close to optimal the objective value of the generated package is. However, we added a note that we never saw this occur during our experiments, and thus we expect it to be unlikely to occur in practice. In our experiments, \lcsolve always generated packages with a $(1-\epsilon)$-optimality guarantee.  
\end{Response}

\begin{cmt}[R2]
The paper is not entirely self-contained, relying heavily on the reader's familiarity with probabilistic databases (notably MCDB) [...] It would significantly strengthen the paper to include a bit more background on how stochastic attributes are modeled [...] More precisely define the uncertainty model.
\end{cmt}

\begin{Response}
%\azza{How about we add the following line to the introduction ... " ... " Explanation makes it seem like you gave something more detailed than the line or that there is some complexity to MCDB/VG functions when there isn't!}
We have added the following text in the introduction (Section~\ref{sec:intro}): ``A VG function is a user-defined function that takes a table of input parameters and generates a table---a scenario---of sample values drawn from a corresponding probabilistic distribution. Because of their flexibility, VG functions can capture complex correlations across the sampled tuples.'' We also further explain how this process can be used to generate scenarios for the portfolio construction example in Figure~\ref{fig:portfolio-builder}.   
\end{Response}

\begin{cmt}[R3]
\sloppy The paper [...] relies heavily on the reader's familiarity with [...] prior work in the package queries space (notably SketchRefine and SummarySearch). It would significantly strengthen the paper to include a [...] slightly more formal specification of SketchRefine (beyond the prose sketch in Section 1). Include a more detailed overview of prior work.
\end{cmt}

\begin{Response}
\sloppy We have augmented the discussion of \skr and \ssearch in Section~\ref{sec:related_works}, where we discuss related work, highlighting the relationship and contrast with \sskr.  We made our best effort to fit this within the space restrictions and considering the additional material requested in the reviews.
\end{Response}

\begin{cmt}
 (R4) In Section~\ref{sec:partitioning}, the use of MAD for stochastic attributes is appropriately justified, but still feels off for some reason I can't fully pin down. I think part of the issue is that the interesting feature of the distribution with respect to l-cvar, is the distribution's tail behavior. As long as all stochastic variables in a partition are drawn from distributions that behave similarly, taking the average across all scenarios should create a relatively representative element for each partition. However, I'm not convinced that this will continue to be the case if different tuples draw from meaningfully different distributions. This potential challenge is occluded in the experiments, where all tuples draw from the same (relatively well behaved) distribution. I don't think this is necessarily a problem, as every probabilistic database use case that I can think of generally avoids mixtures of distributions for a single attribute, but I would either scale back the claims, or add some validation (theoretical, or experimental) that MAD is a meaningful measure for mixed distribution datasets. Address concerns about mixed distributions.
\end{cmt}

\begin{Response}
    We thank the reviewer for raising this issue. To address the concerns, we explicitly highlighted our theoretical guarantee in the form of our newly added Theorem~\ref{th:mad_cvar}, which asserts that regardless of how heterogeneous the families of underlying distributions of the tuples are, constraining the Mean Absolute Distance (MAD) between two tuples results in constraining the difference in their tail behaviors. (This result was previously buried within the proof of Theorem~\ref{theorem:sketch_feasibility} in the Appendix.) We further added experimental validations in \appref{appendix:mad_case_study} which show that MAD captures increased similarities between correlated variables, even when the tuples have highly dissimilar underlying distributions---specifically, uniform and heavy-tailed Pareto distributions---and, in Figure~\ref{fig:mixed_dis_runtime} of~\cite{haque2024stochastic}, we show that \sskr produces near-optimal packages quickly, even when the underlying tuples in the dataset have both types of distribution represented.
    %produce scenarios from a mixture of these two distributions.
    We believe that these additional theoretical and experimental results provide sufficient validation that MAD can handle datasets where stochastic attributes can have varying underlying distributions for different tuples.
\end{Response}

\begin{cmt}
    (R5) One `aha' moment when reading the paper was the realization that linear cvar computation was operating on a single variable, while the general cvar computation was operating on a sum -- this led to the realization that the linear optimization was basically a trick to pull the summation out of the body of the cvar. I think what made this hard is the fact that cvar() is applied to a single random variable (that may be a sum), while l-cvar() operates on a collection of random variables. That being said, I can't think of an elegant way to make this notion clearer. [...] Fundamentally I didn't quite follow the intuition for why cvar doesn't commute through sum. The `the need for duplicates' paragraph in S4.1 helped clarify some of this confusion, so perhaps it might be helpful to move this paragraph earlier.[...] (Incorporate suggested) flow improvements.
\end{cmt}

\begin{Response}
    Thank you for suggesting that we more strongly highlight this intuition. After the statement of Theorem~\ref{th:constraintCompare}, we have added a simple numerical example where CVaR does not commute through Sum, and have provided some accompanying intuition. 
    %incorporated some discussion about the commutativity of \LCVaR and CVaR in the newly added proof sketch of Theorem~\ref{th:constraintCompare} in Section~\ref{sec:prob}.
\end{Response}

\begin{cmt}
    (R6) It would strengthen the paper to provide proof sketches for the theorems.
\end{cmt}

\begin{Response}
    We added proof sketches for each of our theorems, including the newly added Theorem~\ref{th:mad_cvar}. (In the case of Theorem~\ref{th:constraintCompare} we instead added a numerical example with intuition, because even a proof sketch would require a lot of space to develop the appropriate risk-modeling concepts.)
\end{Response}

\section{Reviewer \#2}

\begin{cmt}
    (W1) I'm quite confused about the concept of "duplicates" and the "The need for duplicates" section [...] It is not clear why there is a need to create duplicates.
\end{cmt}

\begin{Response}
    Thank you for pointing out the confusion. We have rewritten the paragraph on the need for duplicates to make clear that the role of the duplicates in a partition is solely to prevent optimal (actual) tuples in the partition from being erroneously eliminated due to overestimation of the risk involved in using those tuples. We have clarified that, when the risk is correctly estimated, the duplicates are replaced by the optimal tuples when the partition is refined, hence they (and not duplicates) will appear in the final package solution. 
    % Consider what would happen if duplicates were not employed by \sskr. As mentioned in Section~\ref{subsec:sketch}, duplicates are only used during the Sketch phase of \sskr, and are replaced by actual tuples in the relation during Refine. Without duplicates, certain packages that contain multiple tuples from the same partition would potentially be \textit{sketch infeasible}. Suppose two companies A and B exhibit very similar average growth projections when sold after 200 days. Both investments are also uncorrelated --- in the rare cases where the investment on A incurs a loss, the investment on B usually makes up for it by returning an large gain and vice versa. This makes a package suggesting investments on A and B and selling them after 200 days a portfolio with fairly low-risk but high expected gain. If both $(A, 200), (B, 200)$ are tuples in the same partition, but are represented by just one representative (suppose $(A, 200)$), the sketched version of the package $\{(A, 200): 1, (B, 200): 1\}$ would be $\{(A, 200): 2\}$ --- a far riskier portfolio since losses in $A$ are never covered up by $B$. If the package $\{(A, 200): 2\}$ (i.e., a recommendation to buy two stocks of A and sell them 200 days later) violates a risk constraint in the query, the sketch solver would return a different package with a lower objective value. When this suboptimal package is refined, the refined package result would also have a lower objective value. With duplication, however, we would create two identical, but not fully correlated, duplicates of $A$ (say $A_1$ and $A_2$), and the sketched version of $\{(A, 200): 1, (B, 200): 1\}$ would be the feasible package $\{(A1: 200): 1, (A2: 200): 1\}$, which is likelier to be sketch feasible. We added a sentence alluding to this phenomenon in the `need for duplicates' section.
    We added an empirical experiment in \appref{sec:ablation_dup} that shows how using duplicates leads to much better packages.
\end{Response}

\begin{cmt}
    (W1 continued) It seems that the authors have a conceptual flaw that may cause the Stochastic Sketchrefine algorithm to yield incorrect results. [...] When purchasing 100 AAPL Stocks, then all of the 100 AAPL stocks will have an identical outcome. They either all go up, or they all go down. This is very different from buying one stock of 100 different companies that have the same distribution as AAPL. The authors write that "[this linear increase of variance] can increase the probability that r will be violated [...] use of duplicates helps avoid this risk inflation and gives the solver more flexibility in search for a solution". It's true that treating each AAPL stock as an independent variable helps finding a solution. But it's also wrong. It seems that this assumption of being able to purchase, as I would call it "multiple copies of the same stock but in multiple possible worlds" will yield incorrect results.
\end{cmt}

\begin{Response}
    \sloppy As mentioned above, duplicates never appear in the final package result, as they are replaced by actual tuples from their respective partitions during the refine phase. Duplicates are used only to ensure that optimal (actual) tuples are not incorrectly discarded during sketch-refine process. So in your example (assuming for simplicity that the sell dates are the same for all stocks), a final package would recommend buying 0 or more shares of the actual AAPL stock, with no correlated duplicates appearing. Also note that the number of duplicates of a representative is upper bounded by the number of tuples in its partition. (We added a sentence clarifying this in Section~\ref{section:sskr}'s subsection `Choosing the number of duplicates'.)  So in your example, if the partition $P$ somehow consisted solely of the AAPL stock, then there would be a single representative---the AAPL stock---with no duplicates. Assuming that the sketch solution contains one or more shares of this stock, the refine step trivially ``replaces'' the AAPL tuple with itself, and the solver can subsequently decide the exact multiplicity of AAPL in the final package.
    
    The more common situation is that the partition $P$ contains, say 100 different stocks, including AAPL. If AAPL is picked as the partition representative, then up to 100 duplicates of AAPL would be created in the sketch problem. Then the solver, when computing the sketch solution, can select multiple duplicates, which approximates the process of selecting multiple actual stocks from $P$ (which by construction are similar to AAPL) and leads to correct risk assessments. Assuming that at least one of the duplicates appears in the sketch solution, 
    %the actual tuples in partition $P$ are not discarded. The 
    partition $P$ will subsequently be refined and the actual tuples in $P$ will be fed into the solver, which determines how many shares of AAPL (and shares of other stocks from $P$) appear in the final package.

% We note that the duplicates never appear in the final package result, as they are replaced by tuples from their respective partitions during \sskr. If \sskr used more duplicates during sketch for a representative than the number of tuples in its partition --- for example, created 100 representatives for an AAPL stock whereas the underlying partition only had a single AAPL stock investment option --- an issue that could happen is that the sketch solver would be able to diversify its investment among the 100 AAPL duplicates, but the refine solver would be unable to refine that partition, as replacing diverse investments and hedging all bets on that one AAPL investment in the partition would amplify the package's risk, and potentially violate risk constraints.

% \sskr avoids this issue by making sure that the number of duplicates of a representative is upper bounded by the number of tuples in its partition. We added a sentence clarifying this in Section~\ref{section:sskr}'s subsection `Choosing the number of duplicates'.

% If a partition has a high number of underlying tuples, with a high similarity in their attributes enforced by tight diameter constraints, and if the sketch solver diversifies its investments on a similarly high number of duplicates, the sketch package can still be refined by replacing each duplicate in the sketch with a distinct tuple, with minimal impact on risk of the package and its objective value.

% If risk constraints in the query are relaxed enough to allow the solver to hedge the investments on a single tuple with higher objective value than the representative, the sketch solution can still contain multiple duplicates, and the duplicates can be replaced by the same high objective value tuple during refine --- \sskr will return the optimal package after refinement.
\end{Response}

\begin{cmt}
    [R1] I'd like to see an experiment that verifies the correctness of \sskr. Correctness could be shown empirically using Monte-Carlo simulation. One could simulate N (N>>100) possible worlds [...], and check in each possible world if the probabilistic constraints are violated. It should hold that a constraint such as `P(Loss>10)<5\%" will be violated in no more than 5\% of possible worlds. If this number is significantly higher, then we know that the assumption of duplicate worlds indeed leads to erroneous results. [...] Authors may consider [...] adding a note to the paper that such as experiment was performed and successful without adding the results to the paper (but of course adding the experiments to github) to be reproduced by interested readers.
\end{cmt}

\begin{Response}
    This is an apt observation, and, in fact, the experiment that you describe is performed at every execution of \sskr! Specifically, every package that \sskr generates---including the intermediate packages that are produced during \lcsolve's alternating-parameter search---are verified over the set of $10^6$ validation scenarios, which are generated independently via Monte Carlo. (We now emphasize more clearly that every validation is with respect to the SPQ involving the \emph{original} constraints, before RCL.) In particular, both the feasibility and objective value for the final package solutions have been tested against the validation set. 
     %, and therefore the final packages generated by \lcsolve and \ssearch during our experiments, are verified over $10^6$ independently generated Monte Carlo validation scenarios, as the reviewer suggests. 
    %Given a risk constraint such as `P(Loss>10)<5\%', if any package has a loss over $10\$$ in more than $5\%$ of these scenarios, the package is considered to be validation infeasible, and vice versa, leading to changes in \LCVaR parameters or the number of optimization scenarios, as detailed in Section~\ref{sec:cvarif}. The final package returned by \sskr is hence necessarily validated over $10^6$ scenarios during the final Refine \lcsolve.
    As a further check on correctness, however, we have now tested the final solution packages from all of our experiments over a further set of $10^6$ Monte Carlo `test scenarios' and verified that, as expected, our generated packages similarly satisfy the risk constraints in their associated SPQs. We discuss this result in \appref{appendix:robustness} and have added instructions on how to reproduce these experiments in our Github repository.
\end{Response}

\begin{cmt}[W2 \& R2]
 It would be good to show some example results. How practically useful are the results? Are these results meaningful portfolios? Or are these unrealistic purchases of "duplicates" of the same stock over and over again.
\end{cmt}

\begin{Response}
We provide an example package result in \appref{sec:ex_package}. We discuss features of the portfolio that we believe makes it meaningful, including the presence of multiple stocks and satisfaction of the query's VaR constraint. As seen in the example, generated packages are seldom a greedy selection of the tuple with the highest objective value, since such a package would violate the risk constraints, as the reviewer notes. Also, as mentioned previously, the final portfolio computed by \sskr does not involve any stochastic duplicates---it is simply a listing of actual stocks and the number of shares of each (along with the selected sell dates).
\end{Response}

\begin{cmt}[W3 \& R3]
 The clustering algorithm presented in Section 5 needs some work.  Using MAD of features does not seem to be a good idea, as some features may have different scales and will dominate the distance computation. The experiments show that the proposed clustering outperform a kd-tree clustering [...] Having a kd-tree as a state-of-the-art competitior for high-dimensional clustering is not appropriate. A better baseline (for example, dimensionality reduction into low dimensional clustering) and state-of-the-art clustering solutions for high dimensional clustering (see surveys on this topic) should be compared against.
\end{cmt}

%\begin{Response}
%    \sskr never calculates a combined MAD of multiple features. Instead, it requires a different diameter threshold to be independently specified for each attribute, and tuples in the same partition must not have a greater pairwise MAD than the diameter constraint for any single attribute. As such, even if different attributes have different scales, they are never combined and thus never dominate each other's distance computation. Since stochastic attributes are approximated over multiple scenarios, the aggregation in MAD comes from the taking the mean of absolute distances between two tuples over all scenarios of the same attribute. We added a couple of sentences clarifying this in Section~\ref{sec:partitioning}'s subsection, `\textbf{Inter-tuple distances}'. Satisfying the diameter constraints w.r.t. each attribute separately is vital for deriving the theoretical guarantees in Section~\ref{sec:theory} and \appref{appendix:sketch_feasibility}. These theoretical guarantees drive the experimental results we see in Section~\ref{sec:experimental_evaluation}, and, as shown in Figure~\ref{fig:dpart}, help \sskr produce better packages than when partitioning is done by combining dimensionality reduction techniques like PCA~\cite{abdi2010principal} with Single-Linkage Agglomerative Clustering~\cite{tokuda2022revisiting}, or when using high-dimensional clustering techniques such as FINDIT~\cite{woo2004findit}, which do not provide guarantees on the optimality of the generated packages.
%\end{Response}

\begin{Response}
    \dpart never calculates a combined MAD of multiple features. Instead, it requires a different diameter threshold to be independently specified for each attribute, and tuples in the same partition must not have a greater pairwise MAD than the diameter constraint for any single attribute. 
    As such, even if different attributes have different scales, they are never combined and thus never dominate each others distance computation.
    %Since stochastic attributes are approximated over multiple scenarios, the aggregation in MAD comes from the taking the mean of absolute distances between two tuples over all scenarios of the same attribute.
    We added a couple of sentences clarifying this in the paragraph \textbf{Inter-tuple distances} of Section~\ref{sec:partitioning}. Satisfying the diameter constraints w.r.t. each attribute separately is vital for deriving the theoretical guarantees in \appref{sec:theory} and \appref{appendix:sketch_feasibility}. These theoretical guarantees drive the experimental results we see in Section~\ref{sec:experimental_evaluation}. 
    We describe in Section~\ref{sec:partitioning} why uncertain data clustering methods are not appropriate in this setting.  Further, in \appref{sec:ablation_dpart}, we provide an ablation study comparing \dpart against two additional alternative partitioning methods that exemplify the approaches suggested by the reviewer:  PCA~\cite{abdi2010principal} with Single-Linkage Agglomerative Clustering~\cite{tokuda2022revisiting} and FINDIT~\cite{woo2004findit}, a high-dimensional clustering technique.  Both result in worse runtimes and solution quality (Figure~\ref{fig:dpart}) and they do not provide any theoretical optimality guarantee for the generated packages.
\end{Response}

\section{Reviewer \#4}

\begin{cmt}[O1]
    No sensitivity analysis to multiple parameters. How should a user set the hyper parameters of the system?
\end{cmt}

\begin{Response}
    In \appref{sec:hyper}, we have added summary notes on the results of sensitivity analyses that we conducted for each hyperparameter used by \lcsolve and \sskr. We have further provided guidance on experiments users can do to set appropriate and effective values for each parameter for new datasets and workloads.
\end{Response}

\begin{cmt}[O2]
     No ablation study to show the relative improve of each of the algorithmic component is given.
\end{cmt}

\begin{Response}
    We have run several experiments to justify the usage of each algorithmic component in \sskr:
    \begin{itemize}
        \item \emph{RCL vs SummarySearch.} Figure~\ref{fig:inc_vars} shows that \lcsolve is faster than \ssearch, and is hence a clear choice for solving our Sketch and Refine SPQs.
        \item \emph{Use of duplicates.} We conducted an ablation study in \appref{sec:ablation_dup} which shows the deterioration in package quality when~(i)~a single representative is not duplicated at all, and~(ii)~multiple representatives are chosen from the same partition without duplication.
        \item \emph{Partitioning methods.} \appref{sec:ablation_dpart} provides an ablation study that shows how package quality and offline preprocessing runtimes are adversely affected when partitioning is done using alternative partitioning strategies instead of \dpart.
    \end{itemize}
    Note that due to the space limitations in the main paper, we had to present some of the above results in the extended version.
\end{Response}

\begin{cmt}[O3]
    How practical are the results? Do they represent meaningful portfolios, or do they reflect unrealistic scenarios, such as repeatedly purchasing "duplicates" of the same stock? Consider adding a case study to demonstrate the output of the proposed algorithm on real-life data.
\end{cmt}

\begin{Response}
    Please see our response to Comment~10.
    %[Same as Comment~10]
    %We provide an example package result in \appref{sec:ex_package}. We discuss features of the portfolio that we believe makes it meaningful, including the presence of multiple stocks and satisfaction of the query's VaR constraint. As seen in the example, generated packages are seldom a greedy selection of the tuple with the highest objective value, since such a package would violate the risk constraints, as the reviewer notes. Also, as mentioned previously, the final portfolio computed by \sskr does not involve any stochastic duplicates---it is simply a listing of actual stocks and the number of shares of each (along with the selected sell dates).
    %We added an example portfolio result in \appref{sec:ex_package}. The returned portfolio diversifies its investments among 5 different companies, and avoids repeatedly purchasing duplicates of the same stock to satisfy the risk constraint in the query. 
\end{Response}

\begin{cmt}[O3(2)]
    Overall the paper is very hard to read and follow. There are almost no examples given, and the notations are confusing. Consider adding a table for frequently used notations and using the stocking example as a running example to explain the algorithm components and definitions.
\end{cmt}

\begin{Response}
    We added a table of notations in \appref{appendix:notations}. Due to space limitations, we didn't add a parallel reference to the portfolio example in Figure~\ref{fig:portfolio-builder} for each algorithmic component. However, we made changes throughout the paper in an attempt to clear specific points of confusion about our algorithms raised by the reviewers.
\end{Response}

\begin{cmt}[O4]
    The authors mentioned that one of their contributions is to extend SPaQL to allow for the expression of CVaR constraints, which allow for better risk control in stochastic optimization problems. There is no evaluation of the usability of the these extensions. How easy it is to use the query language? Why did you choose to focus in these new constraints? are they expressive enough to cover all scenarios?
\end{cmt}

\begin{Response}
     Thank you for the suggestion. We now clearly state in the introduction that the CVaR risk measure is widely used in finance, insurance, and other risk-management domains, and provide supporting citations. Using both a VaR constraint and a CVaR constraint in a SPaQL query indeed helps cover all the scenarios. For instance, consider the following VaR constraint:
     \begin{center}
    % \vspace{-3mm}
    \lstinline!SUM(Gain) <= -10 WITH PROBABILITY <= 0.05!
    % \vspace{-2mm}
    \end{center}
    
    This constrains the maximum loss in $95\%$ of the scenarios to $\$10$. Adding the following CVaR constraint then further constrains the average losses in the other $5\%$ of scenarios which are not covered by the VaR constraint.

    \begin{center}
    % \vspace{-3mm}
    \lstinline!EXPECTED SUM(Gain) >= -20 IN LOWER 0.05 TAIL!
    % \vspace{-2mm}
    \end{center}

    While conducting a usability analysis and exploring avenues for making \spaql more intuitive for naive users remain areas for future work, we note that specifying the CVaR constraint requires the user to specify only two parameters, the tail probability, and the value threshold for the expected sum in the lower tail. 
\end{Response}


\begin{cmt}[D1]
The proofs are not available in the git repository.
\end{cmt}

\begin{Response}
    We added the extended version of the paper in our Github repository in addition to the version on ArXiV~\cite{haque2024stochastic}.
\end{Response}

\begin{cmt}
    The git repository is not well organized and rerunning the code instructions are not fully provided.
\end{cmt}

\begin{Response}
    We made updates to the codebase and especially to the readme file in the Github repository to help interested readers reproduce the results.
\end{Response}

\begin{cmt}
    Providing example queries, particularly those discussed in the experimental evaluation, would be helpful.
\end{cmt}

\begin{Response}
    Due to space constraints, it was not possible to present these in the main paper, but we list every query in our workload in  \appref{appendix:workload}.
\end{Response}

==> sections/03-rclsolve-orig.tex <==
\section{\lcsolve: Solving Small SPQs}\label{sec:cvarif}

In this section, we describe \lcsolve (Algorithm~\ref{alg:lcsolve}), a standalone scenario-scalable algorithm for solving SPQs over a relatively small set of tuples. By completely eliminating the need for scenario summaries, \lcsolve outperforms \ssearch. Moreover, our new \sskr algorithm (Section~\ref{section:sskr}) solves a large-scale SPQ with many tuples by solving a sequence $Q(S_0), Q(S_1),\ldots$ of relatively small-scale SPQs, 
%where the query $Q$ is fixed but the set $S$ of tuples varies,
and slight variants of Algorithm~\ref{alg:lcsolve} (discussed in Section~\ref{section:sskr}) can be used to solve each SPQ encountered during the sketch-and-refine process.
%(with a slight variant of the algorithm used to solve the initial sketch).
%We assume henceforth that the set $\mathcal{V}$ of validation scenarios is large enough so that a package is validation-feasible if and only if it is feasible for the original SPQ, and that the objective function for a feasible package is essentially equal to its approximation based on $\mathcal{V}$; this assumption typically holds in practice.

\begin{algorithm}[t]
\caption{\textsc{\lcsolve}}\label{alg:lcsolve}
{\small
\begin{algorithmic}[1]
\Require $Q :=$ A Stochastic Package Query
\Statex $S :=$ Set of stochastic tuples in the SPQ
\Statex $m :=$ Initial number of optimization scenarios
%\Statex $\mathcal{O}$ $:=$ Initial set of optimization scenarios
\Statex $\mathcal{V}$ $:=$ Set of validation scenarios
\Statex $\delta :=$ Bisection termination distance
\Statex $\epsilon :=$ Error bound

\Ensure $x :=$ A validation-feasible and $\epsilon$-optimal package for $Q(S)$ \\ \makebox[17pt]{} (or NULL if unsolvable)
%or too few opt. scenarios)

\State $\mathcal{O} \gets \textsc{GenerateScenarios}(m)$ \Comment{Initial optimization scenarios}
\State \textsf{qsSuccess}, $x^{\text{D}} \gets $\textsf{QuickSolve}(Q, S) \Comment{Check if solution is ``easy''}\label{li:quicksolve}
\If{\textsf{qsSuccess} $=$ True}\label{li:quickreturnIf}
\State \Return $x^{\text{D}}$ \Comment{Either solution to $Q(S)$ or NULL}\label{li:quickreturn}
\EndIf

\State $\alpha, V\gets \textsc{GetParams}(Q)$ \Comment{Extract $(\alpha_r,V_r)$ for each $r\in Q$}\label{li:getparams}
\State $\omega_0\gets \textsc{OmegaUpperBound}(Q,S,x^{\text{D}},\mathcal{V})$\label{li:EstObjVal} \label{li:getUB}
\While{True}
\State $V'\gets V$, $\alpha'\gets 1$ \Comment{Initial \LCVaR parameter values}
\State Compute $\hat V_0$ as in \eqref{eq:defVL}
and set $V_L\gets \hat V_0$, $V_U\gets V$, $\alpha_L\gets \alpha$, $\alpha_U\gets 1$
\While{True}
\State \textcolor{gray}{$\triangleright$ \textit{Search for $\alpha$}}
\State $\alpha'_\text{old}\gets \alpha'$
\State  status, $\alpha', x\gets \textsc{$\alpha$-Search}(V', \alpha_L,\alpha_U,Q,S,\epsilon,\delta,\mathcal{O},\mathcal{V},\omega_0)$\label{li:alphasearch}
\State \algorithmicif\ status.NeedScenarios $=$ True \algorithmicthen\ \textbf{break}\label{li:needScenariosalpha}
\State \algorithmicif\ status.Done $=$ True \algorithmicthen\ \textbf{return} $x$\label{li:donealpha}
%\State $\alpha' \gets \min\bigl(1,\alpha'+(\lfloor\alpha' m\rfloor+1)/m\bigr)$
%\State $\alpha_L\gets \alpha'$
\State \textcolor{gray}{$\triangleright$ \textit{Search for V}}
\State $V'_\text{old}\gets V'$
\State  status, $V', x\gets \textsc{V-Search}(\alpha', V_L,V_U,Q,S,\epsilon,\delta,\mathcal{O},\mathcal{V},\omega_0)$\label{li:Vsearch}
\State \algorithmicif\ status.NeedScenarios $=$ True \algorithmicthen\ \textbf{break} \label{li:needScenariosV}
\State \algorithmicif\ status.Done $=$ True \algorithmicthen\ \textbf{return} $x$\label{li:doneV}
\State $V_U\gets \max(V'-\delta,V_L)$
\State \algorithmicif\ $\max(V'_\text{old}-V',\alpha'_\text{old}-\alpha')<\delta$ \algorithmicthen\ \textbf{break} \label{li:noprogress}
\EndWhile
\State \algorithmicif\ $2m>|\mathcal{V}|$ \algorithmicthen\ \textbf{return} $x$ \Comment{Best solution found so far}\label{li:genscenariosA}
\State $\mathcal{O} \gets \mathcal{O} \cup \textsc{GenerateScenarios}(m)$\Comment{Double \# of scenarios}\label{li:genscenariosB} 
\State $m\gets 2m$\label{li:genscenariosC}
\EndWhile

\end{algorithmic}}
\end{algorithm}

\smallskip\noindent\textbf{Overview.} The basic idea is to replace each \emph{risk constraint} (VaR or CVaR constraint) in an SPQ with an approximating \LCVaR constraint such that the resulting problem size is independent of the number of scenarios and can be solved using an ILP solver. We leverage Theorem~\ref{th:constraintCompare}, which implies that, for a given stochastic attribute $A$, an \LCVaR constraint with parameters $\alpha$ and $V$ is more restrictive than a risk constraint with the same parameters. Note that an \LCVaR constraint of the form $\LCVaR_\alpha(x, A) \ge V$ becomes less restrictive as either $V$ decreases or $\alpha$ increases. It is therefore possible, by judicious choice of $V$ and $\alpha$, to replace each risk constraint by an \LCVaR constraint that is approximately just as restrictive. The SAA approximation to the SPQ then becomes an ILP, and we can apply an ILP solver to compute the desired package.

%\cvarif refers to the process of replacing all risk constraints by linear \LCVaR constraints of similar restrictiveness. This replacement 
\emph{Risk-constraint linearization} (RCL), i.e., replacing all risk constraints in a query $Q(S)$ by \LCVaR constraints of similar restrictiveness, is accomplished via a search over potential $(\alpha,V)$ values for every \LCVaR constraint. For each choice of values, we solve the resulting SPQ via SAA approximation using the optimization scenarios and then check whether the returned package satisfies the \emph{original} risk constraints in the query with respect to the validation scenarios. Packages that satisfy the risk constraints are deemed ``validation-feasible''. \lcsolve aims to compute a package that is both~(i)~validation-feasible, and~(ii)~\emph{$\epsilon$--optimal}, i.e., whose objective values are $\ge (1-\epsilon)\omega$, with $\omega$ being the optimal package's objective value and $\epsilon$ being an application-specific error tolerance. Since the value of $\omega$ is unknown, we use an upper bound $\omegaU\ge \omega$, so that any package with objective value above $(1-\epsilon)\omegaU$ will have an objective value above $(1-\epsilon)\omega$. One simple choice for $\omegaU$ that works well in practice is $\omega_0$---the objective value of the package solution $x^{\text{D}}$ to query $Q^{\text{D}}(S)$, where $Q^{\text{D}}(S)$
is the deterministic package query obtained by removing all probabilistic constraints from $Q(S)$, i.e., removing all VaR, CVaR and expected sum constraints (line~\ref{li:getUB}). 

\smallskip\noindent\textbf{Quick solution in special cases.}
Sometimes a query $Q(S)$ can be solved quickly, without going through the entire RCL process.
%Specifically, denote by $Q^{\text{D}}(S)$ the deterministic package query obtained by removing all probabilistic constraints, i.e., all VaR, CVaR and expected sum constraints, from $Q(S)$. 
If the ILP solver can find a package solution $x^{\text{D}}$ to query $Q^{\text{D}}(S)$ as above, and if this solution is validation-feasible for $Q(S)$, then $x^{\text{D}}$ is the solution to $Q(S)$, since it satisfies all constraints, including the probabilistic ones, and the objective value is as high as possible since the probabilistic constraints have been completely relaxed, thereby maximizing the feasible region.
%and adding back any further constraints to the query will only shrink the feasible region, hence lowering the objective value.
On the other hand, if no feasible solution can be found for $Q^{\text{D}}(S)$, then $Q(S)$ is also unsolvable, since $Q$ has all the constraints that $Q^{\text{D}}$ has, and more. We denote by \textsc{QuickSolve}$(Q,S)$ the subroutine that detects these two possible outcomes (line~\ref{li:quicksolve}). \textsc{QuickSolve}$(Q,S)$ returns a pair $(\textsf{qsSuccess},x^{\text{D}})$. If $\textsf{qsSuccess}= \textsf{True}$, then $x^{\text{D}}$ either is the package solution to $Q(S)$ or $x^{\text{D}}= \textsf{NULL}$, which indicates that $Q(S)$ is unsolvable, and \lcsolve terminates and returns one of these values (lines~\ref{li:quickreturnIf}--\ref{li:quickreturn}). If $\textsf{qsSuccess}= \textsf{False}$ then $x^{\text{D}}$ solves $Q^{\text{D}}(S)$ but is validation-infeasible for $Q(S)$ and the full RCL process is needed.

% If \textsc{QuickSolve}$(Q,S)$.Success = TRUE, then the subroutine returns either an optimal package \textsc{QuickSolve}$(Q,S)$.Package = $X^{\text{D}}$ or returns a null package (i.e.,\textsc{QuickSolve}$(Q, S)$.Package = NULL), indicating that the problem is unsolvable. Otherwise, \textsc{QuickSolve}$(Q,S)$.Success = FALSE is returned, along 
% with the package $X^{\text{D}}$ that solves $Q^{\text{D}}(S)$---this package is validation-infeasible for $Q(S)$ 
% %with the probabilistically unconstrained package $X^{\text{D}}$
% and the full RCL process is needed.

% \begin{algorithm}[t]
% \caption{\textsc{QuickSolve}}\label{alg:qSolve}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Ensure \textsf{Success} $:=$ True if \textsf{Package} solves $Q(S)$, False otherwise
% \Statex \textsf{Package} $:=$ The returned package

% \State $Q^{\text{D}} :=$ \textsc{RemoveProbabilisticConstraints}($Q$)
% \State $X^{\text{D}} :=$ \textsc{IlpSolver}($Q^{\text{D}}$).\textsc{Solve}()
% \If{\textsc{ValidationFeasible}($X^{\text{D}}$)}
%     \State \Return \{\textsf{Success} $=$ \textsc{True}, \textsf{Package} $= X^{\text{D}}$\}
% \ElsIf{$X^{\text{D}}$ is NULL}
%     \State \Return \{\textsf{Success} $=$ \textsc{True}, \textsf{Package} $= NULL$\}
% \Else
%     \State \Return \{\textsf{Success} $=$ \textsc{False}, \textsf{Package} $= X^{\text{D}}$\}
% \EndIf
% \end{algorithmic}
% \end{algorithm}

\smallskip\noindent\textbf{The case of a single risk constraint.} To understand how RCL works in the case that $\textsf{qsSuccess}= \textsf{False}$, first consider an SPQ $Q(S)$ having a single risk constraint---on a random attribute $A$ with parameters $(\alpha,V)$---that will be replaced by an \LCVaR constraint. If the \LCVaR constraint is too stringent, the package solution will be validation-feasible, but sub-optimal, whereas if the constraint is too relaxed, the package solution will be validation-infeasible. A package solution may also be validation-infeasible or sub-optimal if the number of optimization scenarios is too small so that the SAA approximation is not accurate. We will discuss how RCL deals with this latter issue shortly, but suppose for now that the initial number $m$ of optimization scenarios is adequate.
%in which case the package's VaR, CVaR or objective value among the optimization scenarios will differ sharply from its VaR/CVaR among the validation scenarios.

Let $\alpha'$ and $V'$ denote the adjusted parameters of the \LCVaR constraint. Recall \reva{from Theorem~\ref{th:constraintCompare}} that, for any risk constraint with parameters $\alpha$ and $V$, setting $\alpha'=\alpha$ and $V'=V$ will cause the corresponding \LCVaR constraint to be overly restrictive. The parameter $\alpha'$ can be set as high as $1$, in which case each coefficient $\hat C_i=\LCVaR_{\alpha'}(t_i.A)$ will be the average of the $t_i.A$ values across \emph{all} the optimization scenarios. On the other hand, for a given value of $\alpha$, the parameter $V'$ can be set as low as $V_0$, where $V_0=\sum_{i=1}^n \text{CVaR}_\alpha(t_i.A)*x^D_i$ and $x^D=(x^D_1,\ldots,x^D_n)$ is the package solution to the probabilistically unconstrained problem $Q^D(S)$. Note that, given a set $\mathcal{O}$ of optimization scenarios, we can approximate $V_0$ as previously discussed:
%using Algorithm~\ref{alg:estCVaR}: 
\begin{equation}\label{eq:defVL}
%\hat V_0=\sum_{i=1}^n \textsc{EstimateCVaR}(\alpha,t_i.A,\mathcal{O})*x_{0,i},
\hat V_0=\sum_{i=1}^n \widehat{\text{CVaR}}_\alpha(t_i.A,\mathcal{O})*x^D_i.
\end{equation}

\reva{For any non-trivial risk constraint that is not satisfied by $x^D$, setting the \LCVaR parameters to $a'=1, V'=V_0$ will hence necessarily yield a validation-infeasible package that does not satisfy the constraint.}
%$ is the \LCVaR of the probabilistically unconstrained package $X^{\text{D}}$, in the lower $\alpha$ tail.
We thus need to search for the \reva{\st{ideal} least restrictive} value of $\alpha'$ and $V'$ between the limits $[\alpha, 1]$ and $[V_0, V]$ respectively \reva{that results in a validation-feasible package solution.}

\reva{Intuitively, the optimization problem can be viewed as a search for the lattice point with the best objective value within an $n$-dimensional feasible region, where the coordinates of each lattice point represent the multiplicity of each tuple in the corresponding package. The boundaries of the feasible region are defined by the constraints in a query, with VaR and CVaR constraints forming non-linear boundaries. Replacing the risk constraints with \LCVaR constraints reshapes the feasible region into a convex polytope where each \LCVaR constraint defines a linear hyperplane. When the \LCVaR constraint replacing a CVaR/VaR constraint with parameter $(\alpha, V)$ is parameterized by $(\alpha'=\alpha, V'=V)$, Theorem~\ref{th:constraintCompare} implies that the polytope will contain a subset of the lattice points that satisfy the original problem, and hence may not include the optimal solution. Conversely, the underconstrained parameterization $(\alpha'=1, V'=V_0)$ yields a polytope that includes a superset of the feasible lattice points, including $x^D$, and will hence return an infeasible solution. \lcsolve finds the hyperplane that best approximates the risk constraint boundary such that the optimal solution to the polytope remains feasible w.r.t. the original risk constraint, and any further relaxation to either $\alpha'$ or $V'$ will cause the optimal solution to become infeasible. Adjusting $\alpha'$ allows \lcsolve to rotate the hyperplane, while adjusting $V'$ allows it to perform linear translations on it.} 


\smallskip\noindent\textbf{Alternating parameter search (APS).} The RCL process starts by setting the \LCVaR constraint values to $V'=V$ and $\alpha'=1$. Using the maximal value of $\alpha'$ will most likely make the package solution validation-infeasible. 
%, where $V$ is the value from the original VaR or CVaR constraint.
To attain feasibility, we make the \LCVaR constraint more restrictive via an \emph{$\alpha$-search}, that is, by decreasing $\alpha'$, using bisection, down to the maximum value for which the resulting package is validation-feasible, while keeping $V'$ unchanged (line~\ref{li:alphasearch})---decreasing $\alpha'$ further would lower the objective value.
%Note that the $\alpha$-search examines a discrete set of values $\alpha=\alpha_1<\alpha_2<\cdots<\alpha_q=1$ in the interval $[\alpha,1]$, where $\alpha_j=\min\{y:\lfloor y|\mathcal{O}|\rfloor=\lfloor \alpha_{j-1}|\mathcal{O}|\rfloor+1\}$ for $j>1$. \riddho{We find this maximum $\alpha$ using a binary search as well. Does that need to be clearer in this passage?} Equivalently, we can recursively write $\alpha_j=(\lfloor \alpha_{j-1} |\mathcal{O}|\rfloor+1)/|\mathcal{O}|$. \riddho{We avoid linearly decrementing $\alpha_j$ due to the binary search.} \anh{the discretization of $\alpha$ is an artifact of the way we compute CVaR in Algorithm 1. In Algorithm 1, CVaR changes discretely. Readers may wonder what happens if one replaces Algorithm 1 with a continuous approximation. In such case, we no longer have this artifact about $\alpha$. I want to get rid of this unnecessary artifact so that we can consider $\alpha$ and $V$ as both continuous.} These are the successive values at which exactly one additional optimization scenario is used to create the estimated \LCVaR coefficients for each tuple, hence changing the approximating ILP.
After the above $\alpha$-search terminates with a validation-feasible package, we improve the objective value (while maintaining feasibility) by making the \LCVaR constraint less restrictive via a \emph{$V$-search}, that is, by decreasing $V'$, via bisection, down to the maximum value for which the corresponding package remains validation-feasible, while keeping $\alpha'$ unchanged (line~\ref{li:Vsearch}). Each bisection search for $\alpha'$ or $V'$ terminates when the length of the search interval falls below a specified small constant $\delta$;
%Note that the search interval $[V_0,V]$ for $V'$ is a continuous interval, so that the bisection process terminates when the bisection bounds $V_L$ and $V_U$ satisfy $V_U-V_L\le\delta$ for a small positive constant $\delta$.
in our experiments we found that $\delta=10^{-3}$ was an effective and robust choice.
%\azza{This will automatically beg for proof either in the appendix or a logical reason of some sort. It also seems rather domain specific!}

We then pivot back to adjusting $\alpha'$. Specifically, we decrease the new value of $V'$ by $\delta$, so that the corresponding package based on $(V'-\delta,\alpha')$ is now validation-infeasible. We then decrease $\alpha'$ using an $\alpha$-search to regain feasibility, then decrease $V'$ via a $V$-search to improve the objective, and so on. If any intermediate package is validation-feasible for the original SPQ $Q(S)$ and is near-optimal, i.e., the objective value equals or exceeds $(1-\epsilon)\omega_0$, then we immediately terminate the RCL search and return this package as our solution, setting the variable \textsf{Done} to \textsf{True} (lines~\ref{li:donealpha} and \ref{li:doneV}). The foregoing procedure works even if the initial $(V,1)$ \LCVaR constraint yields a validation-feasible package; in this case the first $\alpha$-search will trivially result in  $\alpha'=1$ and $V'=V$, and the subsequent $V$-search will try to improve the objective value.

Our motivation for using APS is that it provably finds the optimal \LCVaR parameterization in the idealized setting where we can solve any SPQ exactly, determine the feasibility and objective value for any package exactly, and compute any VaR or CVaR exactly, without the need for SAA. Specifically, for an SPQ $Q(S)$ with one risk constraint parameterized by $(\alpha,V)$, denote by $\mathcal{F}_{Q(S)}$ the set of all \LCVaR parameterizations $(\alpha',V')\in [\alpha, 1]\times [V_0, V]$ for which the transformed SPQ $Q'(S;\alpha',V')$ with linearized risk constraint admits a feasible package solution. For any $(\alpha',V')\in\mathcal{F}_{Q(S)}$, denote by $\text{Obj}(\alpha',V')$ the objective value of its corresponding package solution. \reva{Intuitively, let $(\alpha^*,V^*)$ be the best parametrization in $\mathcal{F}_{Q(S)}$. Since APS minimally decreases $\alpha'$ such that the resulting package is validation-feasible (while maximizing the objective with the current value of $V'$), it is necessary that APS iterates through $(\alpha^*,\tilde{V})$ for some $\tilde{V}$. Therefore, the next $V$-search would find $(\alpha^*,V^*)$}. We then have the following result: %, whose proof is given in Appendix~\ref{appendix:APSproof}.

%We prepare for the theorem with a definition: a set $\mathcal{O}$ of optimization scenarios is said to \emph{succinctly represent} the set $\mathcal{V}$ of validation scenarios if (i)~for any two packages $P_1$ and $P_2$, given functions $u_{\mathcal{O}}$ and %$u_{\mathcal{V}}$ that output the objective values of any package among $\mathcal{O}$ and $\mathcal{V}$ respectively, 
%$S^\mathcal{O}_1$ and $S^\mathcal{O}_2$ in $\mathcal{O}$, and $S^\mathcal{V}_1$ and $S^\mathcal{V}_2$ in $\mathcal{V}$ respectively, 
%$u_{\mathcal{O}}(P_1)\ge u_{\mathcal{O}}(P_2) \implies u_{\mathcal{V}}(P_1) \ge u_{\mathcal{V}}(P_2)$, 
%$S^\mathcal{O}_1 \ge S^\mathcal{O}_2 \implies S^\mathcal{V}_1 \ge S^\mathcal{V}_2$, and~
%and (ii)~a package that is (in)feasible with respect to $\mathcal{O}$ is (in)feasible with respect to $\mathcal{V}$.
%and (ii)~If $\mathcal{F}_{\mathcal{S}}$ is the set of packages that are feasible w.r.t. a set of scenarios $\mathcal{S}$ and for which there exists $\tilde\alpha \in [0, 1]$ and $V \in [V_{0}, V]$ a parameterization $\{\alpha'=\alpha, V'=V\}$, $\mathcal{F}_{\mathcal{V}}$ that are feasible w.r.t. $\mathcal{V}$, i.e., $\mathcal{F}_{\mathcal{O}} = \mathcal{F}_{\mathcal{V}}$. 
\begin{theorem}\label{th:alternating_parameter_search}
Let $Q(S)$ be is a solvable SPQ with one risk constraint and suppose that $\mathcal{F}_{Q(S)}$ is nonempty. Then APS, under the idealized-setting assumption, will find a parameterization $(\alpha^*,V^*)\in\mathcal{F}_{Q(S)}$ such that $\text{Obj}(\alpha^*,V^*)\ge \text{Obj}(\alpha',V')$ for all $(\alpha',V')\in\mathcal{F}_{Q(S)}$.
%Given an SPQ $Q(S)$ with one risk constraint, the alternating parameter search (APS) finds the best parameterization, $(\alpha', V')$ for the \LCVaR constraint that results in a feasible package with the highest objective value w.r.t. a given set of scenarios among all possible alternative \LCVaR parameterizations.
\end{theorem}

In practice, we run APS using a set $\mathcal{O}$ of optimization scenarios to compute packages and a set $\mathcal{V}$ of validation scenarios assess feasibility and objective values. The ideal setting essentially corresponds the case $|\mathcal{O}|=|\mathcal {V}|=\infty$, so that in practice we expect APS to work increasingly well as $|\mathcal{O}|$ and $|\mathcal {V}|$ increase. Our experiments in Section~\ref{sec:experimental_evaluation} indicate good practical performance for the ranges of $|\mathcal{O}|$ and $|\mathcal {V}|$ that we consider.

\smallskip\noindent\textbf{Multiple risk constraints.} In general the set $R$ of risk constraints appearing in $Q$ satisfies $|R|>1$, so that quantities such as $V$ and $\alpha$ are vectors; the function \textsc{GetParams} parses the query $Q$, extracts the values $V_r$ and $\alpha_r$ for each constraint $r\in R$, and organizes the values into the vectors $V$ and $\alpha$ (line~\ref{li:getparams}). The \textsc{QuickSolve}$(Q,S)$ function works basically as described above. Assuming that qsSuccess $=$ False, so that the full RCL procedure is needed, the linearization process starts by setting $\alpha'_r=1$ and $V'=V_r$ for each $r\in R$, so that one or more of the risk constraints $r\in Q$ are validation-violated; denote by $R^*\subseteq R$ the set of problematic risk constraints. The search then decreases the problematic $\alpha'_r$ values via individual $\alpha$-searches until all the SPQ constraints are validation-satisfied. These $\alpha$-searches are synchronized in that, at each search step, a bisection operation is executed for each $\alpha'_r$ value with $r\in R^*$ and then the resulting overall set of risk constraints is checked for validation-satisfaction. The $\alpha$-search terminates when bisection has terminated for all of the problematic constraints due to convergence.\footnote{In theory, an initially non-problematic constraint might become problematic during the $V$-search, but we did not observe this behavior in any of our experiments. In any case, one can modify the algorithm slightly to deal with this rare situation.} 
%\azza{adjusting via bisection and "as minimally as possible" seem rather contradictory to me.}. I.e., at each bisection step, the individual $V'$ values are adjusted up or down \azza{Do we ever go down? Now I'm confused! or are you referring to the ranges} as appropriate, until all of them converge: $\Vert V_U-V_L\Vert_\infty\le\delta$. \azza{actually what is appropriate here?} Note that after a $V'$ value for a given constraint converges, it is no longer adjusted during this phase of the search. After all $V'$ values converge,
When the $\alpha$-search terminates, the RCL procedure next decreases each $V'_r$ value by $\delta$ and commences a set of synchronized $V$-searches, and the two types of search alternate as before until a solution is produced.
%no further adjustments to the $\alpha'$ or $V'$ values is possible.

%and then executing an , as before, adding an increment $\Delta$increasing first doing a minimal increment to incorporate an additional scenario, causing one or more of the constraints to be validation-violated, then the $V'$ values get adjusted, and so on, until all values converge.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/CVaRification - Staircase Search .jpg}
%     \caption{\cvarif's staircase-like search finds the appropriate ($\alpha', V'$) combination. It repeatedly finds the minimal $V'$ for which the resulting package is validation-feasible keeping $\alpha'$ fixed, and then, the maximal $\alpha'$ for which the resulting package remains feasible, keeping $V'$ unchanged. Here, an ``X'' or an ``O'' denotes an ($\alpha', V'$) combination resulting in a feasible or infeasible package respectively.}
%     \label{fig:cvarif-intuition}
% \end{figure}

% The search procedure, as shown out in Figure~\ref{fig:cvarif-intuition}, charts out a staircase-like path, where all points above the staircase have more restrictive values of $V'$ than packages considered within the staircase, and hence result in more sub-optimal packages. All points below the staircase are bounded to the left by a point in the staircase that has a more-restrictive value of $\alpha'$, yet resulted in an infeasible package. Thus, the ($\alpha'$, $V'$) combinations in these points will also result in infeasible packages, owing to less  restrictive $\alpha'$-s.

\smallskip\noindent\textbf{Increasing the number of optimization scenarios.} \looseness-1
We have been assuming that the initial number $m$ of scenarios is sufficiently large so that the SAA ILP well approximates the true SPQ, but this may not be the case in general. Therefore, right after each (synchronized) bisection step during an $\alpha$-search or $V$-search, the RCL process examines the intermediate package corresponding to the new set of constraints just produced. If there is a significant relative difference between any VaR, CVaR, or expected value
%, or expected objective valu
when computed over the optimization scenarios and when computed over the validation scenarios,
%with respect to any stochastic attribute among the optimization scenarios has a large relative difference with those metrics among the validation scenarios,
then it follows that SAA approximation is poor.
%the set of optimization scenarios we currently have is not accurately representing the larger set of validation scenarios.
If any relative difference is larger than $\epsilon$, then
%a specified parameter $\beta$ (equal to $\epsilon$ in our experiments)\azza{Why not just say $\epsilon$ then rather than introduce $\beta$ Is there an occasion where we want $\beta$ to not be $\epsilon$? --- If so then it becomes a parameter that we have to justify how we set. If not, then we can just live with less parameters.}, 
the $\alpha$-search or $V$-search terminates immediately and sets \textsf{NeedScenarios} to \textsf{True} (lines~\ref{li:needScenariosalpha} and \ref{li:needScenariosV}). We then increase the number of scenarios (line~\ref{li:genscenariosA}) and restart the RCL process. We also increase the number of scenarios if the values of both $\alpha'$ and $V'$ stop changing and a solution package has not yet been found (line~\ref{li:noprogress}). If the number of optimization scenarios starts to exceed the number of validation scenarios, we terminate the algorithm and return the best solution so far (line~\ref{li:genscenariosA}).


\smallskip\noindent\textbf{Termination and guarantees.}
Assuming that the set $\mathcal{V}$ of validation scenarios is sufficiently large and that the upper bound $\omega_0$ is sufficiently tight, \lcsolve will terminate at line~\ref{li:quickreturn}, \ref{li:donealpha}, or \ref{li:doneV} with a near-optimal solution to $Q(S)$ or will terminate at line~\ref{li:quickreturn} with a \textsf{NULL} solution indicating that the problem is unsolvable. This is the behavior we observed in all of our experiments. Otherwise, \lcsolve will terminate at line~\ref{li:genscenariosB} and return the best package found so far, but with no guarantees on optimality. In this case, the user can increase the number of validation scenarios and try again. \reva{We did not encounter this case in any of our experiments.}

%Furthermore, if any intermediate package satisfies all constraints in $Q(S)$ and is near-optimal, then we return the package immediately instead of continuing with the RCL search, setting the variable status.Done to True. To determine if a package is near-optimal, we find out if its objective value (as measured using the validation scenarios) equals or exceeds $(1-\epsilon)\omega$, where $\omega$ is the objective value of the optimal package. Since $\omega$ cannot be determined exactly, we use an upper bound $\omegaU\ge \omega$, so that any package with objective value above $(1-\epsilon)\omegaU$ will have an objective value above $(1-\epsilon)\omega$. One simple choice for $\omegaU$ is $\omega_0$---the objective value of the probabilistically unconstrained package $X^{\text{D}}$. Since the feasible region for $Q^{\text{D}}(S)$ is at least as large as that for $Q(S)$, we have $\omega_0 \geq \omega$. We use heuristics as in \cite[Sec.~5.4]{BrucatoYAHM20} to tighten (i.e., decrease) $\omegaU$. For example, whenever we encounter a package $X'$ during the RCL process that is validation-infeasible with respect to all the constraints, we compute the corresponding upper bound $\omega'$ and set $\omegaU\gets\min(\omega',\omegaU)$. This works because any validation-feasible package, including the optimal package, would be obtained by tightening every constraint in $X'$, and hence would have a lower objective value than $\omega'$, so that $\omega'$ is indeed an upper bound. Interestingly, in our experiments, we found that the simple upper bound $\omega_0$ would usually be the tightest \anh{Also this is counter-intuitive as if you are saying your $X'$ objective has better objective than $X^D$ assuming that you include all the deterministic constraints when solving for $X'$.} bound.\anh{Counter-example \includegraphics[width=0.5\textwidth]{figures/counter.drawio.png}}\azza{To eliminate yet another variable that we are searching over, can we move this exposition to the appendix and simply state that we set omega to the unconstrained version.}

% \azza{We have 4 reasons to terminate: we hit $\alpha = 1$ or $\alpha$ converges --- honestly it isn't clear, $V_u - V_l < \delta$, optimization = validation scenarios, we are near optimal. Which of these do we always hit first?! If it is the optimality one as it ideally should be, can we simplify the complexity of RCL-solve? Or at least the complexity of how we explain how it works? After reading this a number of times, it is dense ... and one can easily get lost in the details as I might be now. }

% \azza{Also, are the 3 conditions excluding (optimization=validation) always tested at every search and that triggers status.Done?}\azza{After reading the summary, it appears so but is the expectation that we don't look at the pseudocode until the summary? }

% \azza{I tried to refer to the line numbers from within the text. I was only successful doing line 1 in the quicksolve paragraph... Can we try and refer to line numbers where appropriate from the text above. }

% \azza{Again as with Alg 1, in Alg 2, we can either use $|O|$ for $m$ with it as an explicit input and $|V|$ for $\hat m$. }

% \azza{I know the intention was to hide much of the complexity under V-Search and $\alpha$ search, I worry we may have gone too far...}

% \smallskip\noindent\textbf{Summary.} Algorithm~\ref{alg:lcsolve} summarizes the \lcsolve method at a high level---the algorithm returns a . In general the set of risk constraints $R$ appearing in $Q$ satisfies $|R|>1$, so that quantities such as $V$ and $\alpha$ are vectors; indeed, the function \textsc{GetParams} parses the query $Q$, extracts the values $V_r$ and $\alpha_r$ for each constraint $r\in R$, and organizes the values into the vectors $V$ and $\alpha$. With $\alpha'$ fixed, the \textsc{V-Search} function implements the search for the smallest values (component-wise)  of $V'\in[V_L,V_U]$ for which each constraint in the resulting SPQ is validation-satisfied. After a bisection step, it immediately terminates if either (i) it detects the need for more optimization scenarios, in which case it sets the variable status.NeedScenarios equal to True, and (ii) if the package solution $X$ corresponding to the SPQ with the current values of $V'$ and $\alpha'$ is validation-feasible and near-optimal, in which case it sets the variable status.Done equal to True. Otherwise the algorithm terminates when all of the $V'$ values have converged as defined above, and proceeds to the search for $\alpha'$. The function \textsc{$\alpha$-Search} behaves similarly, but, for $V'$ fixed, implements the search for the largest values of $\alpha'\in[\alpha,1]$ (component-wise) for which each constraint in the resulting SPQ is validation-satisfied. For simplicity, our pseudocode assumes that we use the simplest upper bound $\omegaU=\omega_0$ as described above, which is computed via the \textsc{OmegaUpperBound} function in line~\ref{li:EstObjVal}. In more complex versions of the algorithm, the value of $\omegaU$ would be updated by the \textsc{V-Search} and \textsc{$\alpha$-Search} functions.

% \begin{algorithm}[t]
% \caption{\textsc{GetMinimalV}}\label{alg:minV}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Statex $S :=$ A set of tuples tuples
% \Statex scenarios $:=$ A set of optimization scenarios
% \Statex $\alpha' :=$ List of $\alpha'$ paremeters for \LCVaR constraints
% \Statex $V_l :=$ Lower bounds of $V'$ parameters for \LCVaR constraints
% \Statex $\delta :=$ Bisection termination distance
% \Statex $\epsilon :=$ Error Approximation Bound
% \Statex $\omega_0 :=$ Objective value of probabilistically unconstrained package
% \Statex \textsf{MoreScenarios} $:=$ True if more optimization scenarios can be generated
% \Ensure \textsf{Package} $:=$ A near-optimal and validation-feasible package for $Q(S)$, if found
% \Statex \textsf{NeedsScenarios} $:=$ True if more optimization scenarios are needed, False by default
% \Statex \textsf{MinV} $:=$ The minimal $V'$ for feasibility, in no near-optimal package is returned
% \State $V_u :=$ List of $V$ in each VaR/CVaR constraint
% \While{$||V_u - V_l||_{\infty} \geq \delta$}
% \State $V_m := (V_u + V_l)/2$
% \State $Q_m :=$ \textsf{ReplaceRiskConstraints}($\alpha', V_m$)
% \State $X :=$ \textsf{IlpSolver}($Q_m$).\textsf{Solve}()
% \If{\textsf{ValidationFeasible}($X$) and \textsf{Is$\_\epsilon\_$Optimal}($X$, $\omega_0$)}
% \State \Return $\{$\textsf{Package}$= X\}$
% \EndIf
% \If{\textsc{HighDiffOptimizationAndValidation}($X$, $\epsilon$) and \textsf{MoreScenarios}$=$\textsf{True}}
% \State \Return $\{$\textsf{NeedScenarios}$=$\textsf{True}$\}$
% \EndIf
% \For{each risk constraint $r \in Q$}
% \If{$r.$\textsc{ValidationFeasible}($X, \epsilon$)}
% \State $V^{r}_u = V^{r}_m$
% \Else
% \State $V^{r}_l = V^{r}_m$
% \EndIf
% \EndFor
% \EndWhile
% \State \Return $\{$\textsf{MinV}$=V_{m}\}$
% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}[t]
% \caption{\textsc{\lcsolve}}\label{alg:cvarification}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Statex $S :=$ Set of stochastic tuples in the SPQ
% \Statex $m :=$ Initial number of optimization scenarios
% \Statex $\hat{m} :=$ Number of optimization scenarios
% \Statex $\delta :=$ Bisection termination distance
% \Statex $\epsilon :=$ Approximation bound

% \State \textsf{qsSuccess}, $X^{\text{D}} \gets $\textsf{QuickSolve}(Q, S)
% \If{\textsf{qsSuccess} is \textsf{True}}
% \State \Return $X^{\text{D}}$ \Comment{Either $Q(S)$ solution or NULL}
% \EndIf

% \State $V_l \gets \textsf{ComputeLowestBoundValues}(Q, X^{\text{D}})$

% \State $\alpha_l \gets \textsc{GetProbabilityValues}(Q)$

% % \State $d_e \gets 1$ \Comment{{\color{gray}\textit{Exponential search's initial distance}}}
% % \While{true} \Comment{{\color{gray}\textit{Exponential search}}}
% %     \State $L \gets V-d_e$
% %     \State $Q'' \gets \textsc{SetBoundValues}(Q', L)$
% %     \If{\textsc{IsUnsolvable}($Q''$)}
% %         \State \textbf{break}
% %     \EndIf
% %     \State $d_e \gets 2d_e$
% % \EndWhile

% \State $X^* \gets \text{NULL}$
% \State $\text{scenarios} \gets \emptyset$

% \While{\textsc{Is\_$\epsilon$\_Optimal}($Q, X^*, \epsilon$) \textbf{and} \textsc{IsFeasible}($Q, X^*, \hat{m}$)}
%     \State $\text{scenarios} \gets \text{scenarios} \cup \textsc{GenerateScenarios}(\text{tuples}, m)$
%     \State $Q' \gets \textsc{SetCoefficients}(Q,L_P,\text{scenarios})$
%     \State $R_V \gets \textsc{GetBoundValues}(Q)$
%     \State $L_V, R_V, X_V \gets \textsc{BinarySearchOnV}(Q', \delta, L_V, R_V)$
%     \If{$X_V$ != \text{NULL}}
%         \State $X^* \gets X_V$
%     \EndIf
    
%     % \While{$\max |R_V-L_V| > \delta$} \Comment{{\color{gray}\textit{Binary search on $V$}}}
%     %     \State $M_V \gets (R_V+L_V)/2$
%     %     \State $Q'' \gets \textsc{SetBoundValues}(Q', M_V)$
%     %     \If{\textsc{IsUnsolvable}($Q''$)}
%     %         \State $R_V \gets M_V$
%     %     \Else
%     %         \State $X \gets \textsc{ILPSolver}(Q'')$
%     %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
%     %             \State $X^* \gets X$
%     %             \State $R_V \gets M_V$
%     %         \Else
%     %             \State $L_V \gets M_V$
%     %         \EndIf
%     %     \EndIf
%     % \EndWhile

%     \State $Q' \gets \textsc{SetBoundValues}(Q, L_V)$
%     \State $R_P \gets 1$
%     \State $L_P, R_P, X_P \gets \textsc{BinarySearchOnP}(Q', \delta, L_P, R_P)$
%     \If{$X_P$ != \text{NULL}}
%         \State $X^* \gets X_P$
%     \EndIf
%     % \While{$\max |R_P-L_P| > \delta$} \Comment{{\color{gray}\textit{Binary search on $P$}}}
%     %     \State $M_P \gets (R_P+L_P)/2$
%     %     \State $Q'' \gets \textsc{SetCoefficients}(Q',M_P,\text{scenarios})$
%     %     \If{\textsc{IsUnsolvable}($Q''$)}
%     %         \State $L_P \gets M_P$
%     %     \Else
%     %         \State $X \gets \textsc{ILPSolver}(Q'')$
%     %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
%     %             \State $X^* \gets X$
%     %             \State $L_P \gets M_P$
%     %         \Else
%     %             \State $R_P \gets M_P$
%     %         \EndIf
%     %     \EndIf
%     % \EndWhile

%     \State $m \gets 2m$
%     \If{$m > \hat{m}$}
%         \State \textbf{break}
%     \EndIf
    
% \EndWhile
% \State \Return $X^*$

% \end{algorithmic}
% \end{algorithm}

% Letting $\alpha'$ and $V'$ denote the adjusted parameters, observe that each \LCVaR constraint is linear w.r.t. the $x_i$'s, and remains so in the SAA approximation when each $\text{CVaR}_{\alpha'}(t_i.A)$ is approximated by averaging over scenarios with the lowest values (as is done in Algorithm~\ref{alg:estCVaR}). Because all other types of SPaQL constraints, along with their SAA approximations, are also linear w.r.t. the $x_i$'s, \cvarif leads to an ILP formulation whose size is independent of the number of scenarios, as desired. The approximation proceeds by converting all VaR and CVaR constraints to \LCVaR constraints. We next describe this process in detail, and Section~\ref{sec:experimental_evaluation} demonstrate the performance improvements over \ssearch due to \cvarif.

==> sections/06-theory.tex <==
\section{Approximation Guarantees} \label{sec:theory}

% Given an SPQ $Q$, by construction, the sketch package produced by \lcsolve will---almost always---have objective value $\Bar{omega}\geq (1-\epsilon)\omega^*_{sk}$, where $\omega^*_{sk}$ is the objective value of the optimal sketch solution to $Q$.  This guarantee is violated only if \lcsolve reaches the maximum number of scenarios, in which case, we allow it to terminate with a feasible package, even if the guarantee is not met.  Similarly, the refine phase by construction produces a feasible package with objective value $\omega\geq (1-\epsilon)\Bar{omega}$.  This guaranteed is violated only if a refined partition continues to fail after the inter-tuple correlation reaches 1.

For any SPQ $Q(S)$, the size and diameter constraints used by \dpart ensure that the objective value $\Bar{\omega}$ of the returned sketch solution is ``close'' to the true objective value $\omega^*$ for $Q(S)$. \lcsolve-R then ensures that the returned objective value at each step of the refine phase is ``close'' to $\Bar{\omega}$. We now formalize this intuition. An execution of \sskr over $Q(S)$ is \emph{successful} if (i)~\textsc{SolveSketch} returns a non-NULL result and (ii)~a refine order is found such that each call to \lcsolve-R returns a non-NULL result; otherwise, \sskr fails and returns NULL. (We did not observe any \sskr failures in our experiments.) In the case of success, we show that for maximization problems, the sketch package produced by \textsc{SolveSketch} will have objective value $\Bar{\omega}\geq (1-\epsilon)\omega^*_{sk}$, where $\omega^*_{sk}$ is the objective value of the optimal sketch solution to $Q(S_0)$. Moreover, as discussed in Section~\ref{subsec:refine}, \textsc{Refine} produces a feasible package with objective value $\omega\geq (1-\epsilon)\Bar{\omega}$. Theorem~\ref{th:opt_sskr} combines these observations to provide an approximation guarantee on the objective value of a non-NULL package $x^*$ produced by \sskr.
%; see \appref{appendix:APSproof} for a proof.

%Given an SPQ $Q(S)$, by construction, the sketch package produced by \lcsolve will have objective value $\Bar{\omega}\geq (1-\epsilon)\omega^*_{sk}$, where $\omega^*_{sk}$ is the objective value of the optimal sketch solution to $Q$. Similarly, the refine phase by construction produces a feasible package with objective value $\omega\geq (1-\epsilon)\Bar{\omega}$.\footnote{The guarantees of the quality of the sketch and refine packages are only violated if \lcsolve reaches the maximum number of scenarios during sketch, and if a refined partition continues to fail after the inter-tuple correlation reaches 1, respectively.  In such cases, we allow the algorithms to terminate with a feasible package, even if the guarantee is not met.  However, such corner cases were never encountered in our experiments, and one can simply set the algorithms to terminate unsuccessfully in these cases to maintain the theoretical guarantees.} Given this, we can bound the overall approximation guarantee of \sskr with the following theorem; see \appref{appendix:APSproof} for a proof.

%To prepare for the theorem,
We first define ``sketch feasibility''. For a sketch $S_0=\{r_1,\ldots,r_d\}$ of a set $S=\{t_1,\ldots,t_n\}$, denote by $\Lambda$ the set of all functions $\lambda:S\mapsto S_0$ such that, for each $i\in[1..n]$, the element $r_j=\lambda(t_i)$ is one of the duplicate representatives in $t_i$'s partition. For a package $x\in\mathbb{Z}_0^n$ and mapping $\lambda\in\Lambda$ define the package $\lambda(x)=(y_1,\ldots,y_d)\in \mathbb{Z}_0^d$ by setting $y_j=\sum_{i\in I_j}x_i$ for $j\in[1..d]$, where $I_j=\{i: \lambda(t_i)=r_j\}$. A package $x$ for $Q(S)$ is said to be \emph{sketch feasible} if there exists $\lambda\in\Lambda$ such that $y=\lambda(x)$ is a feasible package for $Q(S_0)$.

%Consider a modified set $S'$ of tuples with $|S'|=|S|$ that is obtained by replacing each tuple $t_i\in S$ by a distinct duplicate of $\text{rep}(t_i)$, where $\text{rep}(t_i)$ is the representative of $t_i$ in the sketch $S_0$ of $S$; duplicates of a given representative are independent. A solution package $x^*$ of $Q(S)$ is said to be \emph{sketch feasible} for $Q(S)$ if it is feasible for $Q(S')$.
%, whose proof is given in \cite[Appendix~\ref{appendix:APSproof}]{haque2024stochastic}.

\begin{theorem}[Approximation Guarantee]\label{th:opt_sskr}
Suppose that \sskr returns a non-NULL solution package $x^*$ for a query $Q(S)$. If $x^*$ is sketch feasible, then 
%Let $Q(S)$ be an SPQ that aims to find a package $P$ that maximizes $\mathbb{E}[\sum_{i\in P}t_i.O]$ for an attribute $O$, and suppose that the solution package $x^* = (x^*_1, \dots, x^*_n)$ is sketch feasible for $Q(S)$.
%(i.e., it is feasible for the sketch query if each tuple is replaced with a stochastically distinct duplicate of its representative). Then 
the objective value $\omega$ corresponding to $x^*$ satisfies
\begin{equation}\label{ex:opt_lb}
\omega\ge (1-\epsilon)^2(\omega^* - d_o P_\text{max}),
\end{equation}
where $\omega^*$ is the objective value  of the optimal package solution to $Q(S)$, the quantity $P_\text{max}$ is the maximum allowable package size, and $d_o$ is the diameter threshold of the objective attribute $O$.
\end{theorem}

\reva{Intuitively, \dpart allows us to replace each tuple with their partition's representative with an at most $d_0$ reduction in the objective value of the package. The optimal package with objective value $\omega^*$ will thus have an objective value of at least $(\omega^*-d_o P_{\text{max}})$ when all the tuples are replaced by their representatives. Assuming this sketch package is feasible, \lcsolve will generate a package with an objective value of at least $(1-\epsilon)^2$ times that, where the $(1-\epsilon)^2$-factor comes from the fact that we use \lcsolve to get an $(1-\epsilon)$-optimal sketch package, and Refine returns a package with an objective value of at least $(1-\epsilon)$ times that.}

% Theorem~\ref{th:opt_sskr} provides an approximation guarantee for \sskr. 
% %guarantees on the relation between the objective values of the optimal package and the package produced by \sskr.
% %We prepare for the theorem by introducing the notion of ``sketch feasibility''.
% We call a package \emph{sketch feasible} if the package formed by replacing each tuple in it with a stochastically distinct duplicate of its representative is also feasible w.r.t the sketch query.
% %\peter{This definition is unclear: can a tuple be replaced by any representative? A representative from its original partition?}
% The theorem can be straightforwardly adapted for minimization problems.
% %only considers SPQs whose objective values need to be maximized but can be modified to derive approximation guarantees for minimization problems.

% \begin{theorem}[Approximation Guarantee]\label{th:opt_sskr}
% \sloppy Let $Q$ be an SPQ that aims to find a package $P$ that maximizes $\mathbb{E}[\sum_{i\in P}t_i.O]$ for an attribute $O$, and suppose that the solution package $x^* = \{x^*_1, \dots, x^*_n\}$ is sketch feasible. If the call to \lcsolve during sketch terminates with a $(1-\epsilon)$-guarantee on the quality of the resulting package, and if refine produces a feasible package whose objective value is within a $(1-\epsilon)$-factor of the sketch package, the objective value $\omega$ of the refined package satisfies
% \begin{equation}\label{ex:opt_lb}
% \omega\ge (1-\epsilon)^2(\omega^* - d_o P_{max}),
% \end{equation}
% where

% $\epsilon:=$ error bound for \lcsolve.

% $\omega^*:=$ objective value of the optimal package ($=\sum_{i=1}^{n}\mathbb{E}[t_i.O]x^*_i$),

% $d_o:=$ diameter threshold of the objective attribute $O$,

% $P_{max}:=$ Maximum possible number of tuples in the optimal package, ($\ge \sum_{i=1}^{n} x^*_i$),

% \end{theorem}


%As long as the diameter constraints are reasonably small, we have $\Bar{s} \approx s^*$ \anh{Intuitive reason why this is the case?}. Thus the user can use the total number of tuples in the sketch package to derive the approximation guarantee and get a sense of how close the refined package's objective value is to that of the optimal package.

% If Refine does not find a package solution whose objective value is within a $(1-\epsilon)$-factor of that of the sketch package, but finds a feasible package nonetheless, under the otherwise same assumptions, it can be shown with analogous reasoning as that of Theorem~\ref{th:opt_sskr} that the objective value of the feasible refined package will be at least $\omega\ge (1-\epsilon)(\omega^* - d_o P_{max}) - d_o P_{max}$.

The probability that the optimal package is sketch feasible increases as the diameter thresholds for the attributes in the query constraints become
%sufficiently
small. Small diameter thresholds ensure that a package's sum for any attribute does not change significantly when switching to the sketch problem; see 
\appref{appendix:sketch_feasibility}
%\cite[Appendix~\ref{appendix:sketch_feasibility}]{haque2024stochastic}
for details. We can obtain similar guarantees on minimization problems.
%Whether the second assumption holds for a given SPQ can be easily checked by seeing whether \sskr returns a package.
%The first assumption is highly probable when the diameter thresholds for the attributes in the query constraints are sufficiently small, since this ensures that the optimal package's sum for each constraint attribute does not change by large amounts when passing to the sketch, hence decreasing the probability that the constraint will be violated. 
%\textbf{Effect of Sketching on Constraints} We now consider the effect sketching can have on the risk and expected sums of stochastic attributes and the sums of deterministic attributes of a package, since changes to them can effect whether a package stays feasible after sketching. Suppose, the $j$-th constraint is a risk constraint. Since $Q$ is perfectly linearizeable, it can be losslessly replaced by an \LCVaR constraint with tail probability $\alpha'=\alpha'_{j}$. Then, for any tuple $i$, given the diameter constraint $d_{C_{j}}$ limiting its MAD with its representative, $\alpha'_j(|CVaR_{\alpha'_{j}}(t_i.C_j) - CVaR_{\alpha'_{j}}(rep(t_i.C_j))|) \le \mathbf{E}[|t_i.C_j - rep(t_i.C_j)|] \le d_{C_{j}}$. Hence, the CVaR difference between a tuple and its representative is upper bounded. $$|CVaR_{\alpha'_{j}}(t_i.C_j) - CVaR_{\alpha'_{j}}(rep(t_i.C_j))| \le \frac{d_{C_{j}}}{\alpha'_{j}}$$

%  \anh{I assume that you are talking about $CVaR_{\alpha'_{j}}$ rather than $\LCVaR_{\alpha'_{j}}$ since $\LCVaR$ is a function of package and attribute (not a function of tuple). Then $\alpha'_j(|CVaR_{\alpha'_{j}}(t_i.C_j) - CVaR_{\alpha'_{j}}(rep(t_i.C_j))|)=$} 
% \anh{$ \alpha'_j(|\mathbb{E}[t_i.C_j| t_i.C_j \leq F_{t_i.C_j}^{-1}(\alpha'_{j})] - \mathbb{E}[rep(t_i.C_j))| rep(t_i.C_j)) \leq F_{rep(t_i.C_j))}^{-1}(\alpha'_{j})] =$} 
% \anh{$ \mathbb{E}[\mathbf{1}_{t_i.C_j \leq F_{t_i.C_j}^{-1}(\alpha'_{j})} t_i.C_j]-\mathbb{E}[\mathbf{1}_{rep(t_i.C_j)) \leq F_{rep(t_i.C_j))}^{-1}(\alpha'_{j})} rep(t_i.C_j))]$} \anh{I don't see how the difference of the sum taken from the tail can be bounded by the difference of the expected sum} \riddho{We are taking absolute differences. The minimum difference from the upper $(1-\alpha)$-tail is $0$. If all of the difference is concentrated in the lower $\alpha$ tail, then in the worst case, every scenario will have an $\frac{d_{C}}{\alpha}$ difference (the tuple in the optimal solution will have higher values, and the representative will have lower values in all of them). Let me rethink this a little bit} \anh{Looking good for now with your new reasoning but it is a little bit of a subtle jump in the inequality.}  
% \riddho{Initially, I had a line in between $\alpha'_j(|CVaR_{\alpha'_{j}}(t_i.C_j) - CVaR_{\alpha'_{j}}(rep(t_i.C_j))|) \le |\mathbf{E}[t_i.C_j] - \mathbf{E}[rep(t_i.C_j)]|$ the two where I added the upper $(1-\alpha)$-tail CVaRs, but it seemed too complicated to look at.} \anh{Good for now!}

%For $\hat{X}$, the difference in \LCVaR for the $j$-th constraint is as follows:

%\[
%\begin{split}
%    &\sum_{i=1}^{n} |CVaR_{\alpha'_j}(t_i.C_j) \hat{x_i} - CVaR_{\alpha'_j}(rep(t_i.C_j)) \hat{x_i}|\\
%    = & \sum_{i=1}^{n} |(CVaR_{\alpha'_j}(t_i.C_j) - CVaR_{\alpha'_j}(rep(t_i.C_j)))| \hat{x_i}\\
%    \le & \sum_{i=1}^{n} \frac{d_{C_{j}}}{\alpha'_{j}} \hat{x_i} = \frac{d_{C_{j}}}{\alpha'_{j}} \sum_{i=1}^{n} \hat{x_i} = \frac{d_{C_{j}}\hat{s}}{\alpha'_{j}} \le \frac{d_{C_j}\hat{s}}{\alpha_j}
%\end{split}
%\]
%\sloppy Here, $\alpha_j$ is the tail probability of the risk constraint, and the final inequality follows from the fact that \lcsolve conducts the $\alpha$-search for \LCVaR constraints within $[\alpha, 1]$, implying $\alpha'_j \ge \alpha_j$. A constraint like $\sum_{i=1}^{n}CVaR_{\alpha_j}(t_i.C_j)x_i \ge V_j$, when sketched, becomes

%\[
%\begin{split}
% &\sum_{i=1}^{n} CVaR_{\alpha'_j}(rep(t_i.C_j))x_i \ge V_j\\
% \succcurlyeq_{R} &\sum_{i=1}^{n}CVaR_{\alpha'_j}(t_i.C_j)x_i - \frac{d_{C_j}\hat{s}}{\alpha'_j} \ge V_j\\
% \succcurlyeq_{R} &\sum_{i=1}^{n}CVaR_{\alpha'_j}(t_i.C_j)x_i \ge V_j + \frac{d_{C_j}\hat{s}}{\alpha'_j}\\
% \succcurlyeq_{R} &\sum_{i=1}^{n}CVaR_{\alpha_j}(t_i.C_j)x_i \ge V_j + \frac{d_{C_j}\hat{s}}{\alpha_j}
%\end{split}
%\]

%\noindent Here, $\succcurlyeq_{R}$ denotes the  prior constraint is at least as restrictive as the latter. This result similarly generalizes to non-risk constraints when $\alpha_{j}=1$.

%\anh{In the worst-case the L1-distance is changed by $\frac{d_{C_{j}}*s}{\alpha'_{j}}$. Then the change in L2-distance is bounded between $\frac{d_{C_{j}}*s}{\alpha'_{j}\sqrt{n}}$ and $\frac{d_{C_{j}}*s}{\alpha'_{j}}$}.

%\textbf{Effect of increasing restrictiveness of constraints} Changes in the sum of certain attributes in the package affect its feasibility. In the worst case, each constraint's sum can change by $\frac{d_{C_j}\hat{s}}{\alpha_j}$. In the worst case, constraints like $\sum_{i=1}^{n}c_{ij}x_i \le \tau$ can hence translate to $\sum_{i=1}^{n} rep(c_{ij})x_i \le \tau - \frac{d_{C_j}\hat{s}}{\alpha_j}$, and those like $\sum_{i=1}^{n}c_{ij}x_i \ge \tau$ can   This can render sketched $\hat{X}$ infeasible. To understand 


%We define a constraint vector, $\Vec{L(C)}$, as the vector formed from coefficients of a constraint defined on attribute $C$. Similarly, $\Vec{\mathbf{E}[O]}$ is a vector consisting of the coefficients of each variable in the objective function. The projection of $\Vec{L(C)}$ on $\mathbf{E}[O]$ is $\frac{\Vec{L(C)} \cdot \Vec{\mathbf{E}[O]}}{||\Vec{L(C)}||_2 ||\Vec{\mathbf{E}[O]}||_2}$ \anh{I don't see how the projection is related to the reduction in objective. A possible counter-example is to construct vectors L and E originally perpendicular i.e. its dot product is 0 then no matter how big the changes in L2-distance $\frac{d_{C_{j}}*s}{\alpha'_{j}}$. The reduction is 0?\includegraphics[width=0.5\textwidth]{figures/hyperplane.png}}. For a $\frac{d_{C}p_s}{\alpha'}$ change in the length of the constraint vector, the reduction in the length of the objective vector is, thus, $|\frac{L(C) \cdot \mathbf{E}[O]}{||L(C)||_2 ||\mathbf{E}[O]||_2}|\frac{d_{C}s}{\alpha'}$. For $j$ constraints, the objective value of the linear program formed by removing all integrality constraints from the sketch ILP is lower bounded by \anh{It should not be maximum since the reasoning about the reduction of objective value for each constraint $j$ relies on the fact that other constraints are fixed.}:
%\[
%\begin{split}
%  (1-\max_{j=1, \dots, c}|\frac{\Vec{L(rep(C_j))} \cdot \Vec{\mathbf{E}[rep(O)]}}{||\Vec{L(rep(C_j))}||_2 ||\Vec{\mathbf{E}[rep(O)]}||_2}|\frac{d_{C_j}p_s}{\alpha'_j})\sum_{i=1}^{n}\Vec{\mathbf{E}[rep(O)]}\hat{x_i}  
%\end{split}
%\]

%Due to the diameter threshold $d_O$, 
%\[
%\begin{split}
%    &\Vec{\mathbf{E}[rep(O)]}\hat{x_i} = \sum_{i=1}^{n} \mathbf{E}[rep(t_i.O)] \hat{x_i} \geq \sum_{i=1}^{n} (\mathbf{E}[t_i.O]-d_O) \hat{x_i}\\
%    =& \sum_{i=1}^{n} \mathbf{E}[t_i.O] \hat{x_i} - d_O \sum_{i=1}^{n} \hat{x_i} = \hat{\omega} - d_Op_s 
%\end{split}
%\]

%\anh{$\sum_{i=1}^{n} \mathbf{E}[t_i.O] x_i$ is different from $\sum_{i=1}^{n} \mathbf{E}[t_i.O] \hat{x}_i = \hat{\omega}$. I assume that you are reasoning over any packages $\{x_i\}$ and not reasoning over just the optimal package $\hat{X} = \{\hat{x_1}, \dots, \hat{x_n}\}$} \riddho{Yup, I should just write it for $\hat{x_i}$}

%Hence, the objective value of the optimal solution to the sketch LP is at least
%\[
%\begin{split}
%  \omega^{sk}_{lp} \ge (1-\max_{j=1, \dots, c}[|\frac{\Vec{L(rep(C_j))} \cdot \Vec{\mathbf{E}[rep(O)]}}{||\Vec{L(rep(C_j))}||_2 ||\Vec{\mathbf{E}[rep(O)]}||_2}|\frac{d_{C_j}p_s}{\alpha'_j}])(\hat{\omega} - d_Op_s)  
%\end{split}
%\]

%$r_l = \frac{\omega^{sk}_{lp}}{\omega^{sk}_{ilp}}$, represents the ratio of objective values between the LP relaxation and the sketch ILP. Hence, $\omega^{sk}_{ilp} = r_l*\omega^{sk}_{lp}$. The solution found by \lcsolve will have an objective value $\omega^{sk} \ge (1-\epsilon)\omega^{sk}_{ilp}$.

%\sloppy For a total of $d$ duplicates, let the sketch package be $X^{sk} = \{x^{sk}_1, \dots, x^{sk}_d\}$, with the same number of total tuples, i.e. $\sum_{i=1}^{d} x_i^{sk}=s$. During refine, each duplicate of each representative in the sketch package is replaced by a tuple from its partition. Let $ref: \{r_1, \dots, r_d\} \rightarrow \{t_1, \dots, t_n\}$ be a function that maps each duplicate to the tuple it is replaced with. The objective value of the refined package:
%\[
%\begin{split}
%    \omega^{ref}& = \sum_{i=1}^{d} \mathbf{E}[ref(r_i).O]x^{sk}_i\\
%                & \ge \sum_{i=1}^{d} (\mathbf{E}[r_i.O] -d_O)x^{sk}_i\\
%                & = \sum_{i=1}^{d} \mathbf{E}[r_i.O]x_i - d_O \sum_{i=1}^{d}x^{sk}_i\\
%                & = \omega^{sk} - d_Op_s
%\end{split}
%\]

%Putting it all together, the objective value of the refined package is lower bounded by
%\[
%\begin{split}
%    &((1-\epsilon)r_l(1-\max_{j=1,\dots, c}[|\frac{\Vec{L(rep(C_j))} \cdot \Vec{\mathbf{E}[rep(O)]}}{||L(rep(C_j)||||\Vec{\mathbf{E}[rep(O)]}||}|\frac{d_{C_j}s}{\alpha'_j}]))\\
%    &*(\hat{\omega}-d_{O}p_s)-d_{O}p_s
%\end{split}
%\]

 
%\section{Optimality Guarantee For \sskr}

%\cvarif ensures the returned packages are $(1 \pm \epsilon)$-approximate. For a maximization problem, if the optimal package $\hat{P}$ has an objective value $\hat{\omega}$, a package returned by \cvarif is guaranteed to have an objective value of at least $(1 - \epsilon) \hat{\omega}$. We show that under certain assumptions, we can bound the objective values of the packages returned by \sskr.

%We assume that the sketched version of $\hat{P}$ is feasible. That is, by replacing each tuple in $\hat{P}$ with their representative, we get a feasible package \textsc{Sketched}($\hat{P}$). $\hat{P}$ can have at most $P_{max}$ tuples, where $P_{max}$ represents the maximum number of distinct tuples in a feasible package. Each tuple in $\hat{P}$ can have a MAD of at most $d_{A}$ from the optimal package, where $A$ is the attribute on which the objective is defined and $d_A$ is its diameter threshold. In the worst case, each representative's objective value will be lower than that of its corresponding tuple in $\hat{P}$ by an average of $d_{A}$ over all the scenarios. For $P_{max}$ tuples, the total deviation will be $P_{max}*d_A$. The objective value of \textsc{Sketched}($\hat{P}$) is thus lower bounded by $\hat{\omega} - P_{max}*d_{A}$. Sketch returns a package whose objective value is within $(1-\epsilon)$ times the objective value of the optimal sketch package. If \textsc{Sketched}($\hat{P}$) is feasible, the objective value of the optimal sketch package cannot be lower than $(\hat{\omega} - P_{max}*d_A)$. The objective value of the sketch package will thus be at least $(1-\epsilon)(\hat{\omega} - P_{max}*d_A)$. During Refine, each representative is replaced by a tuple from their partition. Assuming refine completes with a feasible package, the result will be a feasible package all of whose tuples are within a MAD of $d_A$ from their corresponding representative in the sketch package. The refined package's objective value will be lower bounded by:

%\begin{align*}
%    (1-\epsilon)*(\hat{\omega} - P_{max}*d_{A}) - P_{max}*d_A\\
%    \implies (1-\epsilon)\hat{\omega} - (2-\epsilon) P_{max}*d_A
%\end{align*}

%In packages that do not have too many tuples (as is the case in most applications where package queries are intended to be used), $P_{max}$ is small. If the user sets low values for the parameter $\epsilon$ and the diameter threshold $d_A$, the packages generated by \sskr are expected to be near-optimal.

%This bound is based on two assumptions:~(i)~the sketched version of the optimal package $P_{0}$ is feasible, and~(ii)~A valid package is found by refining the sketch package. If sketch uses enough duplicates, which can be ensured by setting the risk tolerance ratio $\alpha$ to $0$, the former assumption is highly probably if the diameter threshold $d_A$ is small for every attribute, that is, all tuples are sufficiently similar to their representatives. The latter assumption is fairly probable since once a valid sketch package is found, refine backtracks through all possible orders in which the partitions having tuples in it can be refined, and readjusts correlation among duplicates if a particular partition cannot be refined in any order.

==> sections/experiments-old.tex <==
\section{Experimental Results} \label{sec:experimental_evaluation}

We designed our experiments to answer the following questions:

\begin{itemize}
    \item Does \sskr scale better than \lcsolve and \ssearch in relations with millions of tuples? To what extent do the objective values of the packages generated by \sskr differ from those generated by \lcsolve and \ssearch?
    \item Is \lcsolve faster than \ssearch and does it produce packages of comparable objective value, especially when stochastic attributes have higher variances?
    \item \skr used KD-Trees to partition relations in the deterministic setting. If we partitioned relations with stochastic attributes using the expected values of the stochastic attributes of each tuple, ignoring the stochasticity in the data, would the objective values of packages produced be worse than our stochasticity-aware partitioning approach, \dpart?
    %\item Can expressing CVaR constraints in SPQs potentially help users get packages with similar objective value but lower risks?
\end{itemize}

%We conducted our experimental evaluation on two datasets:~(i) The Lineitem relation from the TPC-H benchmark, and~(ii)~The portfolio dataset, based on historical stock data. Workloads for both datasets consisted of $5$ queries each. We report the results from our query executions after sorting the queries based on ascending order of their estimated query hardness. We conducted three main sets of experimental comparisons---~(i)~Comparing the runtimes and quality of packages produced by \cvarif with \ssearch in the face of increasing variance in the stochastic attributes.~(ii)~Comparing the runtimes and quality of packages produced by \ssearch with \cvarif and \ssearch in the face of an increasing number of tuples in the dataset.~(iii)~Comparing \dpart with a baseline partitioning approach that partitions tuples based on their mean values across scenarios using KD-trees, to demonstrate the impact of our partitioning approach on the quality of packages produced in large datasets with highly variant data. We observed that~(i)~\cvarif worked much faster than \ssearch especially in high variance datasets, while producing packages of better/similar quality, by~(a)~taking less time to solve the optimization problems on average, and~(b)~solving fewer optimization problems.~(ii)~\sskr produced results in much quicker time than both \cvarif and \ssearch while not sacrificing much in terms of quality of results.~(iii)~In exchange for paying a slightly higher one-time offline partitioning cost than the KD-tree based partitioning approach, packages produced after partitioning using \dpart have significantly better quality than those produced after KD-Tree based partitioning.

\textbf{Environment} We implemented all approaches using Python 3.12.14, used Postgres 16.1 as the supporting DBMS and Gurobi Optimizer to solve the optimization problems. We ran our experiments on a machine with a 2.66 GHz 16-core processor with 16 GB of RAM, 1 TB HDD running on the Ubuntu 22.04 operating system. To account for any variability in results due to inconsistencies in system and optimizer performances, and stochasticity in the data and algorithms, all results we present were executed for 16 iterations each, and we report average results along with an error bar whose height corresponds to the standard variance of the runtimes of all the executions.

\textbf{Datasets} We present evaluations on the TPC-H Decision-Support benchmark~\cite{poess2000new} and the Portfolio dataset, generated from historical stock prices of NASDAQ, NYSE and S\&P-500 listed companies. We used the Lineitem relation from TPC-H, using the open source DBGen script to populate the relation with 6 million tuples. We synthetically made the price and quantity items stochastic by adding gaussian noises. The mean of the noise of each tuple was sampled from a standard normal distribution, while the variance was sampled from an underlying exponential distribution with $\lambda=2$, meaning fewer tuples would have higher variances. The portfolio dataset mimicked the Stock$\_$Investments relation in Figure~\ref{fig:portfolio-builder}, with gains modelled using Geometric Brownian Motion (GBM). GBM uses the drift and volatility of each company to generate future stock price trajectories. We calculated the drift and volatility using historical prices of 3457 companies. We varied witholding periods from half a day to 730 days, with half day increments. We provide details on how we varied the datasets to support different types of experimental comparisons in Appendix~\ref{appendic:datasets}.


\textbf{Workloads} For both datasets, we created workloads consisting of 5 queries each. All queries required producing packages with maximum objective values. This helps make the visualizations of the objective value comparisons of the packages produced by different approaches uniform across queries. Note that, maximizing any function $f(x)$ is equivalent to minimizing the negative function $-f(x)$. Thus, minimizing objective values instead would not change the difficulty of processing an SPQ and does not effect the performance of our approaches. For TPC-H, the queries centred around maximizing expected total prices from supplies with limitations on total taxes to be paid, expected quantities that can be shipped and risks of quantities exceeding limits. For portfolio, the queries centered around risk and budget constrained portfolio optimization. All queries set $P_{max}$, the maximum number of tuples allowed in the package, to 30, with the constraint \mintinline{sql}{COUNT(P.*)<=30}. The full set of queries from both datasets are listed in Appendix~\ref{appendix:workload}.

%\azza{From experience with past submissions, reviewers want to see the actual form of the queries. Just stating the count and a high-level description isn't sufficient. Table 1 takes too much space for the information it provides. It can be two lines or annotated on the other plots or combined with the exact SQL queries.}

\textbf{Hardness} We ensured the queries in our workload were of diverse \emph{hardnesses}. We call a query hard if the probability of a random package satisfying its constraints is small. We estimate this probability similar to the method introduced in~\cite{mai2023scaling}. The probability that a package with $\mathbf{s}$ tuples satisfies a constraint of the form $\sum_{i=1}^{n} A_{i}x_i \le V$, where the values of $A$ are normally distributed with mean $\mu$ and variance $\sigma^2$, is equivalent to the probability of $\sum_{i=1}^{s} N(\mu, \sigma^2) \le V$, or $N(\mu*n, \sigma^2*n) \le V$ according to the central limit theorem. This probability is given by the CDF of the normal distribution $N(\mu*n, \sigma^2*n)$ at $V$. For any given query, we make the simplifying assumption that the probability of each constraint being satisfied is mutually independent. Hence, if a query has $C$ constraints $C_1$, $C_2$, $\dots$, $C_C$ with satisfaction probabilities $P(C_1), \dots, P(C_C)$, the probability of the query being satisfied is $\prod_{i=1}^{C}P(C_i)$. We define hardness as the negative log likelihood of this probability, i.e., $H(Q)=-\log{\prod_{i=1}^{C}P(C_i)}$. Given an SPQ, we first relax it by removing all integrality constraints from it, solve it using \lcsolve and measure the hardness of the ILP that finds a feasible and near-optimal package.

%We estimate the size of the feasible region in the query using \emph{random walks}. We start a random walk from a feasible package found using any SPQ solver. During the walk, each step consists of creating a new package by either inserting a new tuple in the package (this could be done by either adding a new tuple, or increase the multiplicity of an existing one), deleting an existing tuple from the package, or replacing a tuple in the package with another. If the new package is feasible, we have taken a step inside the feasible region. During a walk, we take a sequence of steps in random directions, i.e. we randomly choose to insert/delete/replace a tuple at each step. To prevent looping around the same region during the walk, we perform a step if the direction of the step is not in a `backward' direction with reference to any of the previous steps. The process is illustrated in Figure~\ref{fig:fw-walk}, where each solid arrow represents a step inside the feasible region (the polygon). The red dotted arrow in the end is a backward step, since its `angle' with a previous step (represented by a purple arrow) is over 90 degrees. In high dimensional settings, a step is backward if the step vector's dot product with any of the previous steps is negative. %\azza{Ok, so you have a different definition of backward, in this sense. The above description of backward was not clear at all and you need to be explicit about it.}

%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.15]{figures/Backward-Step.jpg}
%    \caption{Forward Walk From the initial package (In Blue)}
%    \label{fig:fw-walk}
%\end{figure}

%Random walks proceed as long as they can inside the feasible region, taking steps in random directions. If a random modification to the package is detected to be a backward step, the modification is ignored, and alternative modifications are done until a valid step is found. Random walks that never go outside the feasible region are disadvantaged when their initial starting points are close to a tight corner in the feasible region. In such cases, most walks will overstep the boundaries and produce infeasible packages very soon, potentially leaving large portions of the feasible region unexplored. We thus allow random walks to `roam' in infeasible regions for a few steps. This is known as the foraging period, where a walk is given a certain number of steps to walk back into the feasible region. If it cannot find a feasible package within those steps, we give up on the walk and start another one from any of the feasible packages found thus far. If it can find a feasible package within the allotted number of steps, the walk continues as usual, with the foraging period restarting if it again finds itself out of the feasible region at some point.

%To satisfactorily explore a feasible region, for a given query, we conduct 10,000 forwards walks, allowing each a foraging period of 10 steps. We rank the queries based on the average number of feasible packages found per walk, or the average step count ($E_s$). Longer walks imply larger feasible regions. Hence, queries with longer average step counts are generally easier to satisfy. For both datasets, we order queries in ascending order of hardness, i.e. average step count reduces from Q1 to Q5.

%\azza{At this point, as a reader I'm left with "huh?" what is the point of this entire description. You don't map it back to how it measures hardness at all. You need to state the intuition clearly that longer walks imply larger feasible regions and hence easier queries. You also need to give some intuition as to why it is 10,000 random walks, and why forage if you are averaging over 10,000 walks! I suspect foraging is not necessary at all if the goal is simply ranking queries and the measure's only purpose is to rank queries. The other concern I have is that the plots don't seem to be impacted at all by increasing hardness! all runtimes across q1-q5 are somewhat on par. Perhaps we need larger changes in step counts? Also the plots need to visually indicate increasing hardness across the plots e.g. step count = 100, step count = 90, ... etc on the top of each plot.}

%\azza{Also not clear is how did you end up with queries with such precise step (multiples of 5 or 10) counts especially if the hardness measure you use is descriptive and not generative?}

%\input{experiments/query-hardness/hardness}

\textbf{Hyperparameters} For both \ssearch and \lcsolve, we set $m=100$ as the initial number of optimization scenarios, $\hat{m} = 10^6$ as the number of validation scenarios, $\epsilon = 0.05$ as the approximation error bound. Since all queries in our workloads require maximizing objectives, the generated packages are guaranteed to have an objective value at least $0.95$ times that of the optimal package. For \lcsolve, we set $\delta=10^{-3}$ as the bisection termination threshold.

For \dpart, we set the size threshold $\tau=100,000$. Before setting this threshold, we ran 100 randomly generated satisfiable ILPs with 6 constraints and $50,000$ integer variables each and verified the Gurobi Solver took no longer than a minute to solve any of them in our experimental setup. For the TPC-H dataset, we set the diameter threshold for the attributes price, quantity and tax to $5000$, $5$ and $5000$ each. For the portfolio dataset, we set the diameter theshold for price and gain to $0.5$ and $5$ respectively.

\sloppy For \sskr, we set $P_{max}$ to 30, since all queries in the workload have the package size constraint \mintinline{sql}{COUNT(P.*) <= 30}. During Sketch, we decrease the relative risk tolerance by $0.01$ in each iteration, i.e. set $\Delta\alpha = 0.01$.


\textbf{Comparisons} We present experimental comparisons under~(i)~increasing relation sizes,~(ii)~increasing variances,~(iii)~alternative partitioning schemes.

\textbf{Increasing Relation Size} 

We ran all three approaches --- \ssearch, \cvarif and \sskr over datasets of increasing sizes. At their full size, the TPC-H dataset consisted of 1.2 million tuples, while the Portfolio dataset consisted of 6.57 million tuples. Neither \ssearch nor \cvarif can produce packages at such large scales, with their processes either suffering from solver crashes, or being terminated after running for hours. Even for much smaller relations containing around 300,000 tuples, \cvarif and \ssearch took close to an hour to produce results. As Figure~\ref{fig:inc_tuples_rt_cmp} shows, \sskr outperformed the non-partition based approaches, showing orders of magnitude improvement for even the smaller datasets, and produced packages from the full-sized relations in the order of hundreds of seconds. \cvarif outperformed \ssearch in the smaller relations, owing to its convex optimization problems being solved in quicker time than \ssearch's often non-convex optimization problems.

\begin{figure*}[htb]
    \centering
    \input{experiments/increasing_tuples/runtime/combined-figure}
    \begin{center}
        \ref{named}
    \end{center}
    \caption{Runtime Comparisons over increasing number of tuples}
    \label{fig:inc_tuples_rt_cmp}
\end{figure*}


\begin{figure*}[htb]
    \centering
    \input{experiments/increasing_tuples/quality/combined-figure}
    \caption{Comparing Quality of Packages created by \sskr with those created by \cvarif and \ssearch}
    \label{fig:inc_tuples_obj_cmp}
\end{figure*}

We then compared the approaches in terms of the quality of packages produced. Since the divide and conquer approach can cause \sskr to produce packages that are worse in terms of objective value than those produced by \cvarif and \ssearch, we present our results in Fig~\ref{fig:inc_tuples_obj_cmp} in terms of the optimality ratio. We define the optimality ratio as the ratio of the objective value produced by \sskr and the best package produced by either \ssearch or \cvarif. For relation sizes to which neither \ssearch nor\cvarif can scale, we use the objective value of the package found using the highest number of tuples that \cvarif could scale to. We observe that when the relation size is around 20,000 for the TPC-H dataset, or equivalent to the size threshold, the optimality ratio is almost $1$. In such small scales, \sskr only contains a few or just one partition, making its workflow very similar to \cvarif. For slightly higher relation sizes, the objective values of packages produced by \cvarif and \ssearch are unsurprisingly higher than those produced by \sskr. The optimality ratio thus goes below $1$, but never going below $0.9$, indicating that packages produced by \sskr are still of comparable quality. Once we cross the $300,000$ tuple mark, beyond which \cvarif struggles to generate packages, we see a marked increase in the optimality ratio. This is because while \cvarif cannot generate packages that are any better, more tuples gives \sskr more options, from which it can create better packages. This drives the ratio over 1.00, taking it up to around 1.10 as the number of tuples increases.

Together, the two figures show that \sskr can create overall better packages in much shorter time than the time taken by \cvarif and \ssearch to create packages from subsets of those tuples.


\textbf{Increasing Variances} Through these experiments, we take a closer look into the comparative performance between \ssearch and \cvarif. Since neither  approach can handle millions of tuples, we run these experiments over smaller versions of the datasets containing $20,000$ tuples. We test the approaches over varying variances of the stochastic attributes. For the TPC-H dataset, where stochasticity is added via gaussian noises, we multiple by the variance of every tuple by a fixed factor that we call the variance coefficient. We apply the same concept to the portfolio dataset, where the volatility of the gains from each stock investment are multiplied by the variance coefficient.

\begin{figure*}[t]
    \input{experiments/increasing_variance/tpc-h/combined-fig}
    \input{experiments/increasing_variance/portfolio/combined-fig}
    \begin{center}
        \ref{named}
    \end{center}
    \caption{Runtime Comparisons over increasing variances}
    \label{fig:inc_var_rt_cmp}
 \end{figure*}

\begin{figure*}[t]
    \input{experiments/increasing_variance/tpc-h/quality-combined-fig}
    \input{experiments/increasing_variance/portfolio/quality-combined-fig}
    \caption{Quality of Packages over increasing variances}
    \label{fig:inc_var_obj_cmp}
\end{figure*}

Increasing variances has two general effects on SPQ processing:~(i)~Packages have overall greater variance of outcomes, and thus greater risks. Queries with the same risk constraints thus become harder to satisfy.~(ii)~A greater number of optimization scenarios are required to overcome the optimizer's curse, and create packages that are both feasible and near-optimal.

Aside from increased solver times due to harder queries, \ssearch suffers from a setback due to the second effect. If the packages that are created from a few optimization scenarios are feasible but not $(1 \pm \epsilon)$-approximate, it first keeps on increasing the number of summaries in hopes of making the summarized integer program less conservative. This increases the number of optimization problems \ssearch needs to solve. Our implementation of \ssearch somewhat improves Brucato et. al.'s approach in that it doubles the number of optimization scenarios during each iteration just like \cvarif instead of the linear increment proposed in the original paper~\cite{BrucatoYAHM20}.

As seen in Figure~\ref{fig:inc_var_rt_cmp}, \cvarif works much faster than \ssearch, producing results in almost an order of magnitude faster time when the variance coefficient approaches 20.

Both \ssearch and \cvarif only terminate when they are guaranteed to have found $(1+\epsilon)$-approximate packages. As such, their final packages have similar objective values. This is seen in Figure~\ref{fig:inc_var_obj_cmp}, where the optimality ratio is defined as the ratio between the objective values of packages generated by \cvarif and \ssearch respectively. \cvarif searches for the optimal package by bisecting over the CVaR thresholds --- a real-valued continuous interval, whilst \ssearch searches over the appropriate number of summaries to use --- a discrete interval bounded by the number of typically few optimization scenarios. This gives \cvarif more freedom to optimize its results, which can often result in packages with slightly better objective values, as evidenced by the optimality ratios in Figure~\ref{fig:inc_var_obj_cmp} being above 1 more often than not.
\begin{figure*}[htb]
    \input{experiments/increasing_variance/average-optimizer-runtimes/tpc-h/combined-figure}
    \input{experiments/increasing_variance/average-optimizer-runtimes/portfolio/combined-figure}
    \begin{center}
        \ref{named}
    \end{center}
    \caption{Average Time Taken to Solve Optimization Problems}
    \label{fig:inc_var_avg_solver_cmp}
\end{figure*}

To see why \cvarif takes an overall shorter amount of time to solve SPQs, we first look into the average time taken by \cvarif and \ssearch to solve their respective optimization problems. Figure~\ref{fig:inc_var_avg_solver_cmp} shows that this runtime is much lower for \cvarif than \ssearch, which is unsurprising, given that \cvarif's optimization problems are guaranteed to be convex and linear, unlike \ssearch's integer programs.

\begin{figure*}[t]
    \centering
    \input{experiments/increasing_variance/number-of-optimization-problems-solved/tpc-h/combined-figure}
    \input{experiments/increasing_variance/number-of-optimization-problems-solved/portfolio/combined-figure}
    \begin{center}
        \ref{named}
    \end{center}
    \caption{Number of Optimization Problems Solved}
    \label{fig:inc_var_no_of_opt_cmp}
\end{figure*}

Furthermore, due to \ssearch's iterative nature of having to continually increase the number of summaries to find better packages instead of directly increasing the number of optimization scenarios, it ends up with having to solve a lot more optimization scenarios that \cvarif, as seen in Figure~\ref{fig:inc_var_no_of_opt_cmp}.

\textbf{Alternative Partitioning Schemes}

We show the effect of \dpart on the \sskr setup by comparing it with an alternative, simpler baseline partitioning scheme. The alternative scheme has the same size and diameter thresholds, but instead of using other properties of stochasticity, it simply partitions the tuples based on the observed means of each stochastic attribute of each tuple. It uses KD-Trees~\cite{bentley1990k} to perform the partitioning, which hierarchically partitions the dataset until the resulting partitions conform to both size and diameter constraints. This approach is used in deterministic settings to partition relations for \skr. For the largest datasets that contain 6 million tuples each, the KD-Tree based approach requires around 5 minutes (~17\%) lower runtime for partitioning. This result is unsurprising, since KD-Trees do not incur the computational overhead of repeatedly calculating the MAD between pairs of tuples.

\input{experiments/alternative-partitioning/rt-cmp}

However, not taking stochastic properties of the tuples into account results in partitioning together uncorrelated tuples with high variances. This results in high differences between representatives and the respective tuples in a relation. The misrepresenting representatives can produce sketch packages that refine to suboptimal packages.

We observe this when we vary the diversity of variances of tuples in the dataset. We multiply all variances (or volatilities in the portfolio dataset) with different coefficients. The coefficients are sampled from an underlying exponential distribution. We vary the rate parameter $\lambda$ of the distribution. For higher values of $\lambda$, more tuples have higher variances, and the overall variance of the tuples increase.

\begin{figure*}[htb]
    \centering
    \input{experiments/alternative-partitioning/quality/combined-fig}
    \caption{Comparing Quality of Packages After Partitioning By \dpart and \textsc{KD-Trees}}
\end{figure*}

The variance-agnostic KD-Tree approach however does not adjust its partitioning to this change, since the means of every random variable remains the same. As a result, its partitions increasingly consist of tuples with highly contrasting variances, that have very high MADs with each other. Since they cannot be represented effectively by a single representative, the overall quality of packages produced deteriorates. We compare the quality of packages produced in terms of their optimality ratio, i.e. the ratio of the objective value produced by \dpart and \textsc{KD-Trees} respectively. For maximization problems, a higher than 1 optimality ratio indicates that \dpart produces better packages. The results show this to be true, with packages produced by \dpart-based partitioning having 20-70\% higher objective values, with the ratio increasing as diversity in variance increases. Thus, with a nominal 17\% higher one-time offline partitioning cost, partitioning with \dpart helps to produce packages of much better quality for every query.

%\subsubsection{Additional CVaR Constraints}

%\input{experiments/additional_cvar_constraints/quality}

%\azza{The order of presentation of results here (assuming so based on the questions above and the figures) is not the most effective. Fig 11 is the central and most important figure. You start with this primary result. Then Fig 12. I find this figure rather unusual. Why is SS not in the comparison? Why are you baselining SSKR on CVaR? How would you do so given that the number of tuples for CVaR alone doesn't scale to more than $10^6$? Why Fig 8 (only optimizer) and Fig 6. The two don't tell drastically different stories. For Fig 6-10, what is the number of tuples. There is an issue here with the interplay between hardness and variance. Higher variance creates harder queries but as a reader I'm left wondering whether the step counts remain fixed! Fig 13 and perhaps its experiment is better treated as a mini-experiment in the partitioning section.}

==> sections/introduction.tex <==
\section{Introduction}
Decision-making workflows conventionally involve extracting data from warehouses, using them to conceive and train models, and employing in-memory optimizers to prescribe data-driven decisions under uncertain outcomes. The amount of data that can be used for decision-making in such workflows is constrained by the limitations of in-memory optimizers, motivating the need to develop in-database tools for stochastic optimization that can work on enormous volumes of data, and eliminate the need to move data out of databases for prescriptive analytics~\cite{soltanpoor2016prescriptive}. 

\begin{figure}[t]
    \centering
    \resizebox{!}{4.5cm}{\subfloat[A Stock$\_$Investments Relation]{\label{subfig:stock_investments}\input{tables/stock_investments_table}}}
    \hfill
    \resizebox{!}{4.5cm}{\subfloat[Scenarios for `Gain']{\label{subfig:scenarios_for_gain}\input{tables/scenarios_for_gain_table}}}\\
    \vspace{0.2cm}
    \resizebox{!}{1.5cm}{\subfloat[Example \textit{SPaQL} query]{\label{subfig:example_spaql}\includegraphics[scale=0.25]{figures/Example_Spaql.jpg}}}
    \hfill
    \resizebox{!}{1.5cm}{\subfloat[Package generated in response]{\label{subfig:example_package}\input{tables/example_portfolio}}}
    \caption{Creating portfolios using package queries}
    \label{fig:portfolio-builder}
\end{figure}

Suppose an investor attempts to build a portfolio of stock investments. The range of options available to the investor can be represented by the database relation in Fig. \ref{subfig:stock_investments}, where each tuple represents a stock investment that can be bought right away and sold after a certain duration. The gain from such an investment is a stochastic attribute, whose values can be represented by different scenarios (Fig. \ref{subfig:scenarios_for_gain}). Such stochastic attributes can be handled by a Monte Carlo Database System (MCDB)~\cite{JampaniXWPJH11}, where scenarios are generated using modifiable variable generator (VG) functions. For simulating possible future stock prices, a VG function may use Geometric Brownian Motion, which may generate different scenarios on different invocations due to its inherent stochasticity.

Constructing an optimal portfolio is equivalent to choosing a package of tuples from the Stock$\_$Investment relation that maximizes expected gains under risk and budgetary constraints. Brucato et al.\cite{BrucatoYAHM20} propose the \textbf{S}tochastic \textbf{Pa}ckage \textbf{Q}uery \textbf{L}anguage (\textit{SPaQL}), an SQL extension to express such stochastic package queries (Fig. \ref{subfig:example_spaql}), with the resulting package specifying how many and which stocks to buy and when to sell them (Fig \ref{subfig:example_package}). They further show that any SPaQL query can be formulated as a Stochastic Integer Linear Programming (SILP) problem, that can be approximated via Mixed Integer Linear Programming (MILP) over a large number of scenarios.

In database settings, the corresponding MILP formulations can be huge --- too large, in fact, to directly use in-memory optimizers like IBM-CPlex and Gurobi to solve them. This is due to two major reasons: first, the number of scenarios needed to accurately approximate the SILP problem can be in the order of millions. The MILP formulations require one indicator variable for each scenario, making the size of the formulated MILP increase linearly with the number of scenarios used to create packages. Second, each row in the relation corresponds to an integer variable in the MILP formulation. This can make solving queries addressing relations with millions of tuples impossible for in-memory solvers.

Initial efforts for SPQ processing on database relations resulted in \textit{SummarySearch}~\cite{BrucatoYAHM20}, which bundles together multiple scenarios used for generating packages into carefully constructed \textit{summaries}. The corresponding MILP formulations thus have one indicator variable per summary instead of having one for each scenario, which translates to MILP formulations having less indicator variables. However, \textit{SummarySearch} does not handle the problem posed by relations having numerous tuples, and can only solve SPQ-s in a reasonable amount of time when addressed on relations having upto tens of thousands of tuples. Larger relations are not uncommon in stochastic settings. For instance, consider the number of stock investment options in Fig. \ref{subfig:stock_investments}. As of March 2023, the New York Stock Exchange contains 2385 indexed companies. Considering options to sell the stocks either mid-day, or during closing for each day of the following year makes the size of the relation $2,385 X 2 X 365 = 1741050$, approximately 1.74 million tuples. The table can become arbitrarily large when the user wants to exercise more fine-grained control over how many times in the day they can sell their stocks and for how long they are willing to withhold their shares before selling them. Allowing more fine-grained flexibility over selling times and permitting longer horizons for withholding stocks allows for more effective portfolio building, while increasing the number of tuples in the relation. However, this would require scaling up SPQ processing to scales at which the speedups provided by \textit{SummarySearch} alone are insufficient. Furthermore, \textit{SummarySearch's} runtime suffers drastically when stochastic attributes in the relation have large variances. This can happen in various situations, including gains from stock investments in emerging economies, where share prices are known to be more volatile.

In deterministic settings, package queries addressed on large relations are handled using \textit{SketchRefine}~\cite{brucato2018package} \alexandra{the jump into SR is too sudden}. It first conducts an offline partitioning of the tuples in the dataset, splitting them into size-constrained groups of similar tuples. From each partition, it creates a `representative' tuple whose value for each attribute is the mean of the values of all tuples in the partition. Once \textit{SketchRefine} receives a deterministic package query, it first executes the query over only the `representative' tuples, whose number is equal to the number of partitions in the relation. This is known as the `sketch' phase, and is computationally inexpensive compared to executing the package query over the entire relation. The package obtained from the `Sketch' phase is then iteratively `refined'. During each refinement, a representative included in the sketch package is replaced by tuples from its own partition by running a package query over the tuples in the partition, while preserving other representatives included in the sketch package and tuples obtained in the package from previous refinements in the resulting package. The number of distinct tuples included in the package at any point is typically small, and size constraints limit the number of tuples in a partition, meaning that each `refinement' results on the package query being executed over a much smaller number of tuples compared to the tuples in the entire relation. \textit{SketchRefine} thus breaks down a package query addressed over a large relation into a sequence of package queries being executed on subsets of its tuples.

However, adapting \textit{SketchRefine} to stochastic settings is non-trivial. First, for partitioning relations into groups of similar tuples, we need some metric to evaluate how `similar' two tuples with stochastic attributes are with respect to SPQ-s. Second, based on such a similarity metric, we need to develop a method to efficiently partition stochastic relations containing millions of tuples into groups of similar tuples, where the number of tuples in any partition does not exceed a certain size threshold. Third, we need to select a stochastic representative from the tuples in a partition. Fourth, \textit{SketchRefine} assumes that the (possibly distinct) tuples included in any package can be replaced by their corresponding representatives (possibly resulting in different tuples being combined into the same representative) to form a sketch package without violating any constraint with a high probability. This notion is challenged in the stochastic setting, which can include risk constraints. Reducing diversity in packages leads to higher risks, and unifying distinct tuples into the same representative can cause sketch packages to violate risk constraints. This means that the `sketched' versions of optimal packages may be infeasible, and the sketch package will need to include representatives from suboptimal partitions to satisfy risk constraints. These representatives are later refined to include suboptimal tuples in the resulting package, resulting in an overall reduction in the quality of the returned packages. Countering this phenomenon is a major focus of our work. Fifth, we need to account for inter-tuple correlation, and specially, the correlation of each tuples with their representative. 

We address these challenges with our proposed approach, \algname{}. Like its deterministic variant, \algname{} breaks down an SPQ addressed over a large relation into a sequence of more manageable SPQ-s adressing smaller relations. To solve each of these SPQ-s, we propose \cvarmethod{}, a quicker substitute of \textit{SummarySearch}. For \cvarmethod{}, we rethink our approach to handling risk constraints. As in Fig. \ref{subfig:example_spaql}, risk constraints in a \textit{SPaQL} query have the form, `SUM(A)>=V WITH PROBABILITY>=P', where $A$ is an attribute, $V$ is a real value and $P$ represents a probability. In risk evaluation literature, these correspond to Value-at-Risk (VaR) constraints. \cvarmethod{} replaces such constraints in the query with a different type of risk constraint, known as the Conditional Value-at-Risk (CVaR) constraint, which have the form `EXPECTED SUM(A)>=V' IN LOWEST (1-P)-FRACTION OF SCENARIOS', where $A$ refers to the same attribute, $V'$ is a tunable value not exceeding the value $V$ in the original VaR constaint in the query. CVaR constraints restrict the expected sum of the attribute in the package to have an exceeding a minimum threshold. We show that each VaR constraint in the query can be replaced by their \textit{closest approximating CVaR constraint}, while keeping the set of feasible packages unchanged. We further show that CVaR constraints can be translated directly into a single linear constraint involving integer variables only. This improves in-database SPQ processing in three ways.

First, this removes the need to incorporate any indicator variable when SPQ-s are formulated as MILP problems. This is significant, because it removes the nonconvexity introduced as a result of indicator variables, and allows SPQ-s to be formulated purely by Integer Linear Programming (ILP) representations that require less runtime to solve. Second, regardless of the number of scenarios, CVaR constraints are always represented by a single constraint, removing the need to add any additional variables/constraints to ILP formulations when the number of scenarios are increased. This allows us to build packages based on tens of thousands of scenarios. Third, \cvarmethod{} is more robust to attributes having high variances than \textit{SummarySearch}. We demonstrate this in Fig. \ref{fig:cvar_v_summary_search_mini_demo}, where we compare the runtimes and quality of packages generated by \cvarmethod{} and \textit{SummarySearch}, over increasing variances of the `Gain' attribute in the relation of Fig. \ref{subfig:stock_investments} in response to the query in Fig. \ref{subfig:example_spaql}. We increase the variance of `Gain' by multiplying the volatility of each stock by a volatility boost factor. In Geometric Brownian Motion (GBM), the volatility of each company represents to what extent the company's price trajectory may vary from its current trend, or `drift'. Boosting the volatility of each tuple by a constant factor thus increases variance and diversifies the scenarios. Fig. \ref{fig:cvar_v_summary_search_mini_demo} shows that in the face of high volatility, \cvarmethod{} consistently outputs packages of similar quality as \textit{SummarySearch} with much lower runtime. Since neither \cvarmethod{} nor \textit{SummarySearch} can work with millions of tuples, we conduct this experiment over a subset of the `Stock$\_$Investment' relation containing 10,000 tuples.

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
        \caption{Runtime Comparisons}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
        \caption{Objective Value comparisons}
    \end{subfigure}
    \caption{Comparing \cvarmethod{} with \textit{SummarySearch} over increasing tuple variances}
    \label{fig:cvar_v_summary_search_mini_demo}
\end{figure}

Integrating \cvarmethod{} as the core SPQ-processing algorithm for \algname{} allows it to generate high quality packages from millions of tuples with seconds. To demonstrate the superior scalability of \algname{} over \textit{SummarySearch}, we show the result of executing the query in Fig. \ref{subfig:example_spaql} over the Stock\_Investments table in Fig. \ref{subfig:stock_investments} by varying the duration up to which stock withholding is allowed. At full scale, we allow tuples with sell-in dates ranging upto a year (365 days), where there are 1.7 million tuples, a scale at which \textit{SummarySearch} cannot produce results due to its infeasibly large main memory size requirements. Fig. \ref{fig:stochastic_sketchrefine_v_summary_search_mini_demo} shows that \algname{} produces results at significantly faster runtimes than \textit{SummarySearch} even when there is a much lower number of tuples, makes SPQ-processing scalable on million-tuple relations, all while producing packages that are of similar quality as \textit{SummarySearch}.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
        \caption{Runtime Comparisons}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
        \caption{Objective Value comparisons}
    \end{subfigure}
    \caption{Comparing \algname{} with \textit{SummarySearch} over increasing number of tuples}
    \label{fig:stochastic_sketchrefine_v_summary_search_mini_demo}
\end{figure}

We thus present the following key contributions:

\begin{compactitem}
  \item \partioningscheme, an efficient method for partitioning stochastic relations into size-constrained groups of similar tuples.
  \item \algname{}, a framework that converts an SPQ addressed on a large relation into a sequence of SPQ-s on smaller subsets of tuples of the relation to accelerate SPQ-processing while still producing packages having high quality.
  \item \cvarmethod{}, a new SPQ processing method that converts \textit{SPaQL} queries to convex optimization problems, and whose runtime, unlike \textit{SummarySearch}, remains relatively stable when relations have high-variance attributes.
\end{compactitem}

The remainder of this paper covers the syntactic rules of \langname{} (Section \ref{sec:spaql+syntax}), an overview of existing methods for package query processing in both deterministic and stochastic domains (Section \ref{sec:preliminaries_on_package_queries}), detailed descriptions of \cvarmethod{} (Section \ref{sec:cvarification_details}) and \algname{} (Section \ref{sec:stochastic_sketchrefine_details}), experimental evaluation of the methods on real-world datasets (Section \ref{sec:experimental_evaluation}), related literature (Section \ref{sec:related_works}), and our conclusions and directions for future work (Section \ref{sec:conclusion}). 

==> sections/old_files/SSR-old.tex <==
\section{\sskr}\label{section:sskr}


\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-1.jpg}
        \caption{Tuples as points}
        \label{fig:tuple_to_point_vis_hlf}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-2.jpg}
        \caption{Partition tuples}
        \label{fig:partition_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-3.jpg}
        \caption{Select Representatives}
        \label{fig:representative_election_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    %\hfill
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-4.jpg}
        \caption{Form Duplicates}
        \label{fig:representative_duplication_hlf}
    \end{subfigure}\\
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-5.jpg}
        \caption{Sketch: Generate Packages from duplicates}
        \label{fig:sketch_query_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    %\hfill
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-6.jpg}
        \caption{Refine: Replace duplicates with actual tuples}
        \label{fig:first_refinement_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-7.jpg}
        \caption{Second Refinement}
        \label{fig:second_refinement_hlf}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-8 (1).jpg}
        \caption{Final Refinement}
        \label{fig:third_refinement_hlf}
    \end{subfigure}
    \caption{High Level Workflow of \sskr}
    \label{fig:stochastic-sketchrefine-hlf}
\end{figure*}

\cvarif alone cannot scale across the tuple dimension. We address this with a new evaluation mechanism, \sskr. \sskr maintains the high-level workflow of \skr~\cite{brucato2018package}. It partitions the data offline, and employs \cvarif to solve the sketch and refine SPQs. Unlike \skr, it is designed to overcome challenges raised by stochasticity. \sskr revisits \skr's approach to creating sketch packages using a single representative from each partition. When sketching optimal packages with several tuples from the same partition, the single representative strategy will need the sketch solver to include the same representative multiple times. However, we show in Section~\ref{section:sskr} that doing so in stochastic settings increases the risk of a package. To satisfy risk constraints, the solver might be forced to include tuples from suboptimal partitions in sketch packages. Suboptimal sketch packages consequently refined to suboptimal final packages. To overcome this, \sskr duplicates the representatives, and solves the sketch problem over all such duplicates. This allows the sketch solver to include multiple duplicates from each partition without inflating risks. During `Refine', every duplicate in the sketch package is replaced by actual tuples from their partition.

To partition large probabilistic relations offline for \sskr, we propose \dpart, a trivially-parallelizable partitioning scheme. Unlike existing hierarchical stochastic data clustering approaches~\cite{gullo2017information, huang2021robust}, \dpart's time complexity is subquadratic with respect to the number of tuples in the relation. This makes it suitable for partitioning million-tuple relations.  We discuss \dpart in detail in Section~\ref{sec:dpart}.

\peter{Moved \sskr paragraph from former preliminaries section. Needs to be merged (or discarded) to avoid redundancy}

For processing SPQs on large relations, we propose \sskr (Figure~\ref{fig:stochastic-sketchrefine-hlf}). It partitions the data offline into groups of similar tuples (Figure~\ref{fig:partition_hlf}) using \dpart, a novel stochastic partitioning scheme (detailed in Section~\ref{sec:dpart}) that ensures (i) tuples in the same partition are similar with respect to each attribute, and (ii) no partition contains too many tuples. It then selects a representative tuple from each partition (Figure~\ref{fig:representative_election_hlf}). Representative tuples are imaginary tuples whose deterministic attributes are the average of that attribute's values among all the tuples in the partition. Their stochastic attributes each correspond to that of one of the tuples in the partition. Section~\ref{subsec:rep_selection} details the criteria for selecting the corresponding tuple for the stochastic attributes.

Given an SPQ, \sskr first executes a `Sketch' query, solving the query on the combined set of all representatives. The resulting sketch package indicates the number of tuples to be included in the final package from each partition. In deterministic settings, having one decision variable per representative suffices. If a package contains $q$ tuples (each with a multiplicity of 1) from the same partition, its `sketched' version assigns the multiplicity $q$ to the variable corresponding to the representative.

However, under uncertainty, this increases the risks of sketched packages. Suppose, an optimal package has two tuples $t_1$ and $t_2$ from the same partition, whose random variables for a stochastic attribute $A$ have Bernoulli distributions $B(0.5)$. For the package $\{t_1, t_2\}$, the probability of the sum of $A$ being $0$ is 0.25. Yet, if they are represented by  a single tuple $t$ having the same bernoulli distribution, the sketched version of $\{t_1, t_2\}$ would have selected $t$ twice, increasing the probability of the sum of $A$ being $0$ to 0.50. If the SPQ has a VaR constraint limiting the probability of the sum of $A$ being $0$ to 0.30, the sketched version of the optimal package would become infeasible. During Sketch, the solver would be forced to explore alternative options, leading to no package being found or suboptimal packages being generated.

\sskr thus creates stochastically identical duplicates of each representative (Figure \ref{fig:representative_duplication_hlf}). Sketch solves the SPQ over all the duplicates using \cvarif, with the ILP having a decision variable for each duplicate, and assigns a multiplicity to each duplicate (Figure \ref{fig:sketch_query_hlf}). Determining the appropriate number of duplicates for each representative involves a runtime-quality trade-off. The higher the number of duplicates, the better the chances of the sketched version of the optimal package being feasible. With enough duplicates, each tuple in the optimal package can map to a different  duplicate. However, this also means more decision variables in the sketch ILP, i.e., higher runtimes. Fortunately, the number of duplicates needed for any representative is upper bounded by the number of distinct tuples in the optimal package, which is typically much smaller than the number of tuples in a partition. Section \ref{subsec:sketch} discusses Sketch in further detail, including how it determines the appropriate number of duplicates.

Afterwards, each partition whose representatives are included in the sketch package are successively refined by replacing the duplicates with tuples from their own partition (Figures~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}). During each refinement, \cvarif solves the SPQ on all tuples in the partition, the tuples included in the package from previous refinements, and the yet unrefined duplicates of representatives from the sketch package (details in Section~\ref{subsec:refine}). Since no partition consists of too many tuples and the number of distinct tuples in the sketch and refined packages are limited, each refinement can be completed quickly. Once all the refinements are done, all duplicates are replaced by actual tuples, and the final package is obtained.
%Doing the same in \sskr but this would cause the Sketch package to be risk-averse and sub-optimal. To see why, consider a package of two independent Bernoulli random variables $B(0.5)$ and a package that contains the same Bernoulli random variable $B(0.5)$ twice. The former would have a lower probability of getting 0 i.e. $25\%$ chance while the latter would have 50\% chance.\riddho{I feel that this example may not quite work since it might not connect why taking a package with a lower risk is bad, and how this specifically causes issues during sketch seems somewhat ambiguous} Hence, in this case, if we apply the same logic as in \skr, the Sketch query is forced to produce a sketched solution that would inherently risk-averse since multiplying the same random variable would make it riskier than choosing multiple i.i.d. random variables. To overcome this, \sskr uses a novel technique called ``tuple duplication'' (detailed in Section~\ref{subsec:tuple_dup}) to diversify the sketch solution. At a high level, we form stochastically identical duplicates of each representative, as in Figure~\ref{fig:representative_duplication_hlf}. The sketch query runs \cvarif to solve the query over all the duplicates of each representative. As illustrated by Figure~\ref{fig:sketch_query_hlf}, the sketch package will contain only a subset of these duplicates from some of the partitions. Deciding on the number of duplicates for each partition involves a trade-off, since the higher the number of duplicates, the better is the sketch solver's ability to avoid overconstrained sketch packages, but a higher number of decision variables in the sketch problem also means that the solver requires more time to obtain the sketch solution. Details on deciding the appropriate number of duplicates for each representative are provided in Section~\ref{subsec:sketch}. Each partition whose representative's duplicates are included in the sketch package are then successively refined, by replacing them with tuples from their own partition (Figures~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}). To perform each refinement, we use \cvarif to solve the query on all tuples in the partition, the tuples included in the package from previous refinements, and the duplicates of representatives from the yet unrefined partitions of the sketch package (details in Section~\ref{subsec:refine}). Since no partition consists of too many tuples and the number of distinct tuples in the sketch and refined packages are limited, each refinement can be completed quickly. Once all the refinements are done, all duplicates are replaced by actual tuples, and the final package is obtained.
\subsection{The Sketch Phase} \label{subsec:sketch}

Sketch (Algorithm~\ref{alg:sketch}) processes a given SPQ $Q$ on the representatives $R_t$. Like \cvarif, it starts by solving $Q_0$, the version of $Q$ that excludes all the probabilistic constraints (line~1). If $Q_0$ is unsolvable, so is $Q$, since $Q$ has all the constraints that $Q_0$ has and more, so we return a null package (lines~2-3). Otherwise, we solve the ILP for $Q_0$ to get the probabilistically unconstrained optimal package $P_0$ (line~4). We check if $P_0$ satisfies the risk constraints of $Q$ based on $\hat{m}$ validation scenarios, and if so, return it (lines~5-6).

\begin{algorithm}[t]
\caption{\textsc{Sketch}}\label{alg:sketch}
\begin{algorithmic}[1]
\Require $Q:=$ A Stochastic Package Query
\Statex $R_t :=$ A set of representative tuples
\Statex $\tau :=$ Maximum tuples in a partition
\Statex $\Delta\alpha :=$ Change in relative risk tolerance 
\Statex $m :=$ Initial number of optimization scenarios
\Statex $\hat{m} :=$ Max. number of scenarios used
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\Statex $\epsilon :=$ Error approximation bound
\Statex $\delta :=$ Bisection termination distance

\State $Q_0 \gets $\textsc{RemoveProbabilisticConstraints}(Q)
\If{\textsf{IsUnsolvable}($Q_0$)}
\State \Return NULL
\EndIf
\State $X_0 \gets $ \textsf{ILPSolver}($Q_0$)
\If{\textsf{IsFeasible}($Q$, $X_0$, $\hat{m}$)}
\State \Return $X_0$
\EndIf
\State $\alpha \gets$ \textsc{InitialRiskTolerance($\tau$)}
\While{$m \leq \hat{m}$}
      \State tuples $ \gets$ $\emptyset$ 
      \For{$r \in R_t$}
       \State $d \gets $\textsc{NumberOfDuplicates($r, Q, \alpha, m, P_{max}$)}
        \For{$i \in [1, \dots, d]$}
        \State tuples $\gets $ tuples $\cup$ $r$
        \EndFor
      \EndFor
      \State $X \gets $\textsc{CVaRification}($Q$, tuples, $m$, $\hat{m}$, $\delta$)
      \If{\textsf{Is\_$\epsilon$\_Optimal}($Q, X, \epsilon$) \textbf{and} \textsf{IsFeasible}($Q, X, \hat{m}$)}
      \State \Return $X$
      \Else
      \If{$\alpha > 0.0$}
      \State
      $\alpha \gets \max(\alpha - \Delta\alpha, 0.0)$
      \Else
      \State $m \gets min(2m, \hat{m})$
      \EndIf
      \EndIf
\EndWhile
\State \Return \textsc{NULL}
\end{algorithmic}
\end{algorithm}

Otherwise, we use optimization scenarios for each constraint to create packages that satisfy the probabilistic constraints in $Q$. Sketch starts with a relatively small number ($m$, e.g. 100) of optimization scenarios, and doubles their number (line~23) until a validation feasible and $(1 \pm \epsilon)$-approximate package is found (lines~15-16). If no valid package is generated even after using a maximal number ($\hat{m}$, e.g. $10^6$) of optimization scenarios, we return null (line~24).

When creating an appropriate ILP formulation for $Q$, sketch creates duplicates of each representative. The number of duplicates created can vary by representative. To determine the number of duplicates to create, sketch requires $P_{max}$, an upper bound on the number of distinct tuples in a package. This can often be specified in the query itself, by a package size constraint like ``COUNT(*) $\leq$ $P_{max}$''. Alternatively, $P_{max}$ can be derived from deterministic constraints. For instance, if $Q$ has a constraint like ``SUM(A) $\leq$ V'', we can sort all the tuples in ascending order of their values of A and check how many distinct tuples we can include from the beginning until the sum of $A$ exceeds V. $P_{max}$ can also be set based on intuition and domain knowledge, since users may have an estimate of how many tuples they expect to see at most in the generated packages. 

If Sketch creates $P_{max}$ duplicates for every representative, all tuples in the optimal package can be mapped to a distinct representative, even if all $P_{max}$ tuples in the optimal package originate from the same partition. If all tuples are sufficiently similar to the representative, sketched versions of the optimal package would be validation feasible. However, since each duplicate has a corresponding decision variable, this can increase solver runtimes. 

We use $\alpha$, a risk tolerance ratio, to determine an acceptable number of duplicates. If $d<P_{max}$  is the chosen number of duplicates for a representative, the risk of sketched packages can be amplified if all $P_{max}$ tuples in the optimal package are from the representative's partitition.  The sketched version of the package will contain all $d$ duplicates, each having an average multiplicity of $P_{max}/d$. For each risk constraint in $Q$, the VaR/CVaR of this package will be lower than that of the package formed if $P_{max}$ duplicates were used, in which case the sketched version would have each duplicate exactly once. Sketch calculates the relative change in the VaRs/CVaRs between the two packages, and selects the smallest $d$ for which the relative change goes below $\alpha$ for every risk constraint in the query (Details in Section~\ref{subsec:num_dup}).

Sketch initially sets $\alpha$ so as to ensure the total number of duplicates is within a tolerable range for an off-the-shelf solver to solve the ILP in a reasonable amount of time. The number of tolerable decision variables can vary due to underlying hardware attributes of the system, differences in the solver software, runtime versus quality requirements, etc. Recall our partitioning scheme ensures that none of the resulting partitions contain too many tuples. Specifically, no partition contains more than $\tau$ tuples, a size threshold defined by a database administrator. During Refine, the solver solves an ILP that contains all tuples in a partition. Thus, $\tau$ is set so that having $\tau$ decision variables in the ILP does not stress out the solver. Sketch also utilizes this threshold. It sets the initial value of $\alpha$ so that the total number of duplicates across all the representatives does not exceed $\tau$ (line~7) (Details in Section~\ref{subsec:initial_alpha}).

During each iteration, Sketch first calculates the number of duplicates for each representative based on $P_{max}$ and $\alpha$ (lines~10-11). For each stochastic attribute addressed by a constraint or objective in $Q$, it creates $m$ scenarios from these duplicates (lines~12-15). Each scenario consists of a real value for each duplicate of every representative. Details on how these scenarios are constructed are described in Section~\ref{subsec:scenario_gen}.

Once all the scenarios are generated, we use \cvarif to obtain a package $X$ (line~16). Notice the slightly different parameterization as opposed to the \cvarif approach described in Algorithm~\ref{alg:cvarification}. Sketch uses a slightly modified version of the approach. Its \cvarif uses only the given optimization scenarios, running bisections to find the closest linearized CVaR constraint for each risk constraint. It uses $\hat{m}$ validation scenarios to validate the feasibility and optimality of the intermediate packages. However, if the package obtained in the end is not validation feasible or $(1\pm\epsilon)$-optimal, it simply returns the package it found to the Sketch function, instead of attempting to increase the number of optimization scenarios and retry, as was proposed in Algorithm~\ref{alg:cvarification}.

Upon receiving a package $X$, Sketch checks to see if it is $(1 \pm \epsilon)$-optimal and validation feasible (line~17), and returns $X$ if so (line~18). If not, it checks to see if $\alpha$ can be decreased further. Decreasing $\alpha$ results in more duplicates being produced, which can help produce better and more feasible packages. If $\alpha > 0$, we decrease it by $\Delta \alpha$ (lines~20-21), a user-defined hyperparameter that we in our experiments set to be $0.03$. If $\alpha = 0$, we double the number of optimization scenarios and reiterate (line~23).

\subsubsection{Determining the number of duplicates} \label{subsec:num_dup}

The number of duplicates needed by a representative can differ for each constraint. Thus, given a representative $r$ and a query $Q$, we iterate over all the risk constraints in $Q$, and select the maximum number of duplicates of $r$ needed by them (Algorithm~\ref{alg:num_dup}). 

\begin{algorithm}[h]
\caption{\textsc{NumberOfDuplicates}}\label{alg:num_dup}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $Q :=$ A Stochastic Package Query
\Statex $\alpha :=$ Relative risk tolerance
\Statex $m :=$ Number of scenarios
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\State $d \gets 1$
\For{Each risk constraint $c$ in $Q$}
    \If{\textsc{DuplicatesForConstraint}($r$, $c$, $\alpha$, $m$, $P_{max}$) > $d$}
        \State $d \gets $ \textsc{DuplicatesForConstraint}($r$, $c$, $\alpha$, $m$, $P_{max}$) 
    \EndIf
\EndFor
\State \Return $d$
\end{algorithmic}
\end{algorithm}

Duplication aims to ensure that each tuple in the optimal package has a one-to-one correspondence with a duplicate of the representative. When the number of duplicates of a representative $d$ is less than $P_{max}$, this is not ensured. If all $P_{max}$ tuples in the optimal package are from the representative's partition, the sketched version of the optimal package will have to map different tuples to the same duplicate. For any stochastic attribute, in the worst case scenarios for that duplicate, the losses will multiply. This will lead to lower CVaR and VaR values in the sketch package, and make the risk constraints harder to satisfy. 

If a representative has $d$ duplicates, the risk optimal sketched version of a package having $P_{max}$ tuples from the partition will have each of the duplicates included an average of $\frac{P_{max}}{d}$ times. $\frac{P_{max}}{d}$ may not be an integer, so some of the duplicates will have a multiplicity of $\lceil\frac{P_{max}}{d}\rceil$ while the rest are repeated $\lfloor\frac{P_{max}}{d}\rfloor$ times. We create $m$ scenarios from such a package and find the VaR/CVaR of the package among the scenarios. We return the first value of $d$ for which the change in VaR/CVaR relative to that of the package that contains $P_{max}$ duplicates is less than $\alpha$ (lines 7-8 in Algorithm~\ref{alg:dup_count}). 

\begin{algorithm}[h]
\caption{\textsc{DuplicatesForConstraint}}\label{alg:dup_count}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $c :=$ A risk constraint
\Statex $\alpha :=$ Relative risk tolerance
\Statex $m :=$ Number of scenarios
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\State $S_{max} \gets \emptyset$
\For{$i \in [1, \dots, m]$}
    \State $S_{max} \gets S_{max} \cup $ \textsc{CreateScenario}($r$, $c.a$, $P_{max}$)
\EndFor
\For{$d \in [1, \dots, P_{max}]$}
\State $S_d \gets \emptyset$
\For{$i \in [1, \dots, m]$}
    \State $S_d \gets S_d \cup $ \textsc{CreateScenario}($r, c.a, d$)
\EndFor
\If{(\textsc{Risk}($S_{max}$) - \textsc{Risk}($S_{d}$))/|\textsc{Risk}($S_{max}$)| $\leq \alpha$}
\State \Return $d$
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

If the recommended number of duplicates by algorithm~$\ref{alg:dup_count}$ equals or exceeds the number of tuples in a partition, \sskr includes all the tuples from the partition directly during Sketch, instead of having a single representative for them. 


\subsubsection{Determining the initial risk tolerance ratio} \label{subsec:initial_alpha}

To determine an initial value of $\alpha$ that ensures that the total number of duplicates during Sketch in the first iteration is around the size threshold $\tau$, we conduct a bisection over the values of $\alpha$ from $[0, 1]$ (Algorithm~\ref{alg:init_alpha}). If the total number of decision variables is lower than $\tau$ even for $\alpha = 0$, we use $0$ as our initial $\alpha$ (lines 1-2). If the total number of duplicates is too high for $\alpha = 1$, we set $\alpha = 1$ as our initial value of $\alpha$ (lines~3-4). Otherwise, we conduct a bisection from $\alpha_l = 0$ (line~5) to $\alpha_h = 1$ (line~6) that continues until the total number of duplicates used is the same for any value of $\alpha$ within $[\alpha_l, \alpha_h]$ (line~7). During each iteration of the bisection, we check the total number of duplicates produced by setting $\alpha_m = \frac{\alpha_h + \alpha_l}{2}$ using Algorithm~\ref{alg:num_dup}. If the number of duplicates is over $\tau$, we reduce our search interval to $[\alpha_l, \alpha_m]$ (lines~9-10). If the total number of duplicates is below $\tau$, we reduce the search interval to $[\alpha_m, \alpha_h]$. If $\alpha_m$ produces exactly $\tau$ duplicates, we return it immediately and use it as our initial $\alpha$.

\begin{algorithm}[t]
\caption{\textsc{InitialRiskTolerance}}\label{alg:init_alpha}
\begin{algorithmic}[1]
\Require $\tau :=$ Maximum tuples in a partition

\If{\textsc{TotalDuplicates}(0.0) $\leq$ $\tau$}
\State \Return $1.0$
\EndIf
\If{\textsc{TotalDuplicates}(1.0) $\geq$ $\tau$}
\State \Return $0.0$
\EndIf
\State $\alpha_h$ $\gets$ $1.0$
\State $\alpha_l$ $\gets$ $0.0$
\While{\textsc{TotalDuplicates}($\alpha_h$) $>$ \textsc{TotalDuplicates}( $\alpha_l$)}
\State $\alpha_m$ $\gets$ ($\alpha_h$ + $\alpha_l$)/2
\If{\textsc{TotalDuplicates}($\alpha_m$) $> \tau$}
\State $\alpha_h$ $\gets$ $\alpha_m$
\EndIf
\If{\textsc{TotalDuplicates}($\alpha_m$) $< \tau$}
\State $\alpha_l$ $\gets$ $\alpha_m$
\EndIf
\If{\textsc{TotalDuplicates}($\alpha_m$) $= \tau$}
\State \Return $\alpha_m$
\EndIf
\EndWhile
\State \Return $\alpha_l$
\end{algorithmic}
\end{algorithm}

In theory, $\alpha$ may have to be over $1$ to produce around $\tau$ duplicates. In such cases, we still begin from $\alpha=1$, since setting $\alpha$ even higher will worsen the quality of packages produced, if any. We did not encounter this case during our experiments.

\subsubsection{Scenario Generation from Duplicates} \label{subsec:scenario_gen}

During sketch, an optimization scenario can be formed by independently sampling a value from each duplicate of every representative, with \cvarif creating sketch packages based on numerous such scenarios.

However, assuming mutual independence among duplicates ignores inter-tuple correlations within a partition. Positively correlated tuples tend to have lower values in the same scenarios. Thus packages containing positively correlated tuples incur increased losses in the worst-case scenarios and are inherently riskier. As such, constructing a sketch package while being oblivious to inter-tuples correlations within the partition can cause problems while refining the partitions. For instance, if all tuples in the partition are highly correlated with the representative, a sketch package that contains independent duplicates may underestimate the risks incurred by including multiple duplicates of the representative. No feasible solution may be found during refine, when the solver tries to replace independent duplicates with positively correlated tuples. 

Duplicates of each representative should thus be mutually correlated with one another to extents roughly mirroring the correlation between the representative and other tuples in the partition. We use the median of the pairwise Pearson's correlation coefficients between the representative and all other tuples in its partition as the correlation coefficient between each pair of duplicates. For an intuition on why we use the median of the correlation coefficients, note that by duplicating the representatives, we aim to provide a new one-to-one correspondence between duplicates in the sketch package and the tuples included in the package after refining the partition. Using the median ensures that there are as many tuples having a higher correlation with the representative than the duplicates as there are tuples having a lower correlation coefficient. Thus, if one of the duplicates is replaced by a tuple having a higher correlation coefficient than the median, thereby increasing risks compared to the sketch package, the solver will have the chance to balance it out by taking another similarly optimal tuple that has a lower correlation coefficient.

To generate scenarios from duplicates that are mutually correlated by a correlation coefficient $\overline{\rho}$, we propose an accelerated version of the NORTA (NORmal-To-Anything) copula method~\cite{ghosh2003behavior}. Given a set of random variables and their pairwise correlation coefficients, NORTA generates correlated samples from them. It converts values sampled from a multivariate standard normal distribution with a given correlation matrix, to corresponding values at equivalent cumulative densities for arbitrary random variables. Given $d$ correlated random variables $R_1, \dots, R_d$ and their $d \times d$ correlation matrix $\mathbb{\rho}$, where $\mathbb{\rho}_{ij}$ denotes the correlation coefficient between $R_i$ and $R_j$, NORTA first takes $d$ i.i.d. samples a standard normal distribution, forming a $d$-dimensional sample vector $s$. Then, to generate $d$ samples from a multivariate standard normal distribution defined by the correlation matrix $\mathbb{\rho}$, it finds the eigendecomposition of $\mathbb{\rho} = S \Lambda S^{-1}$. Prior literature~\cite{gentle2009computational} shows $s'=S \sqrt{\Lambda} s$ will then reflect a $d$-dimensional sample of the multivariate standard normal distribution with correlation matrix $\mathbb{\rho}$. NORTA then calculates a $d$-dimensional sample vector $s_r$ of the correlated random variables, where the $i$-th element of $s_{r}$, $s^{r}_{i} = F_{i}^{-1}(\Phi(s'))$, with $F_{i}$ denoting the CDF of the $i$-th random variable $R_{i}$, and $\Phi$ denoting the CDF of the standard normal distribution.

In \sskr, the random variables correspond to the stochastic attributes of each duplicate. Given $d$ duplicates for a single representative,  we construct a correlation matrix $\rho$ where $\rho_{ij} = \overline{\rho}$ when $i \neq j$ (typically the median correlation coefficient between a representatives and the tuples it represents), and $\rho_{ii}=1$ for $i,j \in \{1, \dots, d\}$ (Correlation coefficient of any duplicate with itself is 1). Using NORTA, we generate a sample value for each duplicate. An optimization scenario is constructed by appending all sample values of every duplicate of each representative.

\begin{algorithm}[t]
\caption{\textsc{CreateScenario}}\label{alg:scenario_construction}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $a :=$ A stochastic attribute
\Statex $d :=$ The number of duplicates
\Statex $\overline{\rho} :=$ Correlation coefficient between duplicates
\State $s_1, \dots, s_d \gets$ i.i.d. samples from $N(0, 1)$
\State $s'_1 \gets \sqrt{1 + (d-1) \overline{\rho}} s_1 - \sum_{i=2}^{d} \sqrt{1 - \overline{\rho}} s_i$
\For {$i \in \{2, \dots, m\}$}
    \State $s'_i \gets \sqrt{1 - \overline{\rho}} s_i - \sqrt{1 + (d-1) \overline{\rho}} s_1$
\EndFor
\State $F_r \gets$ CDF of $r.a$
\State $s_r = F_r^{-1}(\Phi(s'))$
\State \Return $s_r$

\end{algorithmic}
\end{algorithm}

Eigendecomposing $\mathbb{\rho}$ normally has a computational complexity of $\mathcal{O}(d^3)$. This makes constructing scenarios expensive as we need to perform this decomposition for every representative. Furthermore, the algorithm may iteratively increase the number of duplicates to get better packages, requiring the eigendecomposition to be repeated at each iteration. To remove this bottleneck, we exploit the fact $\rho$ is a matrix where all non-diagonal entries have the same value $\overline{\rho}$. A closed form of the eigenvalues and eigenvectors of this matrix can be trivially computed as $\lambda_1 = 1+(d-1)\overline{\rho}$ with the corresponding eigenvector $[1, 1, \dots, 1]$ and $\lambda_2 = 1-\overline{\rho}$ with $d-1$ corresponding eigenvectors $[-1, 1, 0, \dots, 0]$ $[-1, 0, 1, \dots, 0]$, $\dots$, $[-1, 0, \dots, 1, \dots, 0]$, $\dots$ $[-1, 0, \dots, 1]$. Thus, after generating $d$ independent samples from standard normal distributions, and getting the sample vector $s=[s_1, \dots, s_d]$, the sample vector of $d$ correlated multivariate normal distributions can be found in $\mathcal{O}(d)$ time using $s' = [s_1\sqrt{\lambda_1} - \sqrt{\lambda_2}\sum_{i=2}^{d}s_i, s_2\sqrt{\lambda_2} - s_1\sqrt{\lambda_1}, \dots, s_d\sqrt{\lambda_2} - s_1\sqrt{\lambda_1}]$.

Since all the duplicates of a representative $r$ are stochastically identical, they have the same cdf $F_r$. A scenario can be generated by appending $s_{r} = F_{r}^{-1}(\Phi(s'))$ for every representative $r$. $F_r$ can be precomputed offline from histogram density estimations computed from independent samples~\cite{chan2014near}. Algorithm \ref{alg:scenario_construction} describes our linear time NORTA copula based scenario construction scheme.





\subsection{The Refine Phase} \label{subsec:refine}

Refine iteratively replaces each representative selected in the Sketch Package with tuples from their own partition. In each step, we replace all the selected duplicates from exactly one of the partitions, while preserving the selected duplicates from the yet unrefined partitions and the tuples selected during previous refinements. 

Refine uses the same number of optimization scenarios that were used to derive the Sketch package, and keeps the number of optimization scenarios fixed throughout its execution. The intuition behind keeping the number of scenarios fixed is that if $m$ optimization scenarios were enough to create feasible and near-optimal packages from the duplicates of each partition, they should suffice for doing the same from the actual tuples, since each tuple should be similar enough to their representatives.

Refine needs to find an order in which to refine the partitions included in the sketch package, so that a feasible and near-optimal final package is found. Using an `incorrect' order can lead to failure to find any feasible package. This happens when the ILP used to refine a particular partition does not return a valid package. To find this correct order, we use `Greedy Backtracking', a technique also used in the deterministic \skr algorithm~\cite{brucato2018package}. Intuitively, we backtrack over all possible permutations in which the partitions in the sketch package can be refined until a sequence of refinements results in a feasible and $(1\pm\epsilon)$-approximate package. We begin with a randomly selected permutation of partitions. If any intermediate refinement fails to find a valid package, we `undo' the previous refinement and greedily attempt to refine the failing partition in its place. We keep undoing the previous refinements until the partition can be successfully refined. If a partition cannot be refined even when no other partitions were refined before it, it indicates that the stochastic behaviour of the tuples in it do not coincide sufficiently well with that of the duplicates of the representative. This can happen if the correlations among the duplicates was insufficient, as explained in Section~\ref{subsec:scenario_gen}. In such cases, we increase the correlation coefficient among the duplicates of all such partitions by a tunable extent of 0.1, re-execute the sketch query, and refine the newly obtained sketch package. Greedy backtracking continues to explore different orders in which the partitions may be refined until an acceptable final package is found.

Each refinement involves a partition whose duplicates have a total multiplicity of over $0$ in the sketch package, and solves an ILP. Each refine ILP consists of a decision variable corresponding to each tuple in the partition being refined, one for every duplicate of every partition that were included in the sketch package but have not been refined yet, and one decision variable for every tuple included in the refined package from previous refinements. The constraints of the ILP include all constraints in the query (including the CVaRified VaR constraints), as well as additional constraints that ensure the multiplicities of the tuples obtained from previous refinements and those of duplicates of the yet unrefined representatives remain unchanged. The ILP solver thus needs to find an optimal assignment for decision variables of the tuples in the partition while keeping the multiplicities of all other tuples in the package unchanged. By successfully completing each refinement, duplicates in the sketch package are thus substituted by actual tuples from their partition.    




% \section{CVaR Constraints are all you need} \label{sec:cvarification_details}

% Deterministic constraints, and expected sums in constraints and objectives in SPQs can be represented via linear expressions in ILPs. However, solving SPQs becomes challenging due to risk constraints. \textit{SPaQL} expresses risk constraints via Value-at-Risk (VaR) constraints, whose ILP representations require one indicator variable per optimization scenario. \ssearch improves this by grouping scenarios into summaries and using one indicator variable per summary instead. It increments the number of summaries until an `optimal enough' package is found, while keeping the number of optimization scenarios unchanged. This can be slow when the initial number of optimization scenarios is insufficient, which becomes increasingly likely with higher variances.

% \begin{sloppypar} 
% \textbf{CVaR constraints are linearly representable.} We show that had risk constraints been expressed as Conditional Value-at-Risk (CVaR) constraints instead, they could be represented in ILPs as linear constraints. Consider a CVaR constraint \mintinline{sql}{EXPECTED SUM(A) >= V IN LOWEST T% OF SCENARIOS}, where $A$ is an attribute, $V$ is a real number and $T \in [0, 100]$. We modify the optimization scenarios\footnote{Any package created using modified optimization scenarios can be verified for constraint satisfaction and optimality over the unchanged validation scenarios}, and create `pseudo-scenarios' by sorting scenario values of each tuple in ascending order (Fig. \ref{fig:pseudoscenario-construction}). 
% \end{sloppypar}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.25]{figures/CreatingPseudoScenarios.jpg}
%     \caption{Creating pseudo-scenarios}
%     \label{fig:pseudoscenario-construction}
% \end{figure}

% Observe that the first pseudo-scenario is \textit{at least as bad} as any optimization scenario, i.e. each of its tuples has values that are not greater than their corresponding value in any of the original scenarios. A package $\{x_1, x_2, x_3, ..., x_n\}$ which satisfies the condition $\sum_{j=1}^{n}P_{1j}x_j \geq V$, where $P_{1j}$ represents the value of the $j$-th tuple in the first pseudo-scenario thus also satisfies $\sum_{j=1}^{n}S_{ij}x_j \geq V$ for any scenario $i$, where $S_{ij}$ represents the $j$-th tuple's scenario value, since $S_{ij} \geq P_{1j}$ and $x_j \geq 0$ implies $P_{1j}x_j \leq S_{ij}x_j$ for all $1 \leq j \leq n$.

% In theorem \ref{theorem:conservative_pseudoscenarios}, we generalize this to the first $m$ pseudo-scenarios. If any package has an expected sum of at least $V$ in the first $m'$ pseudo-scenarios, they are guaranteed to have an expected sum of at least $V$ over \emph{any} $m'$ scenarios. Formally, if $L$ is a set of $m'$ scenarios, where $S_{lj}$ represents the value of the $j$-th tuple in scenario $S_{l} \in L$,  

% \begin{equation}
%   \frac{1}{m'}\sum_{i=1}^{m'}\sum_{j=1}^{n}P_{ij}x_{j} \geq V \implies \frac{1}{m'}\sum_{S_{l} \in L} S_{lj}x_{j} \geq V
%   \label{eq:cvar_representation}
% \end{equation}

% For $m' = \frac{T}{100}m$, $m$ being the number of optimization scenarios and $T$ the percentage of scenarios addressed in the CVaR constraint, adding the linear constraint $\frac{1}{m'}\sum_{i=1}^{m'}\sum_{j=1}^{n}P_{ij}x_{j} \geq V$ in the ILP will ensure that the generated package has an expected sum exceeding $V$ over any $m'$ scenarios, and by extension, over the $m'$ scenarios having the lowest sums for the package. Had risks been represented using CVaR constraints, they could be represented in ILPs using such linear constraints, without needing indicator variables.

% \textbf{Converting VaR constraints} In \textit{SPaQL} however, all risk constraints are represented using VaR constraints of the form SUM(A) >= V WITH PROBABILITY>=P. We observe that any package satisfying the CVaR constraint EXPECTED SUM(A)>=V IN LOWEST (1-P)*100\% OF SCENARIOS, will also satisfy the VaR constraint.

% To explain why, suppose $scenario\_score$ refers to the sum of a package $x=\{x_1, ..., x_n\}$ in a scenario $S_i$, i.e. $\sum_{j=1}^{n} S_{ij}x_j$. Any package satisfying the latter CVaR constraint will have an average score of at least $V$ in the (1-P)-fraction of scenarios having the lowest scenario scores, implying the scenario score of at least one of these scenarios must be at least V. All other `better' scenarios must then also have scores of at least $V$. Thus, the package will have a sum of at least $V$ in at least $P$-fraction of the remaining scenarios and the VaR constraint will be satisfied.

% \begin{sloppypar}
%     This provides a method for linearly representing VaR constraints. First, convert the VaR constraint to a CVaR constraint, then create pseudo-scenarios from the optimization scenarios. Using the antecedent of implication~(\ref{eq:cvar_representation}), we generate an ILP whose resulting package satisfies the CVaR constraint, and thus, the original VaR constraint. Disadvantageously, this can overconstrain the ILP, making it unsolvable or have suboptimal solutions. We can, however, account for this by \textit{relaxing} the CVaR constraint. We model a VaR constraint of the form \mintinline{sql}{SUM(A)>=V WITH PROBABILITY P} to a CVaR constraint \mintinline{sql}{EXPECTED SUM(A)>=V' IN LOWEST (1-P)*100% OF SCENARIOS}, where $V' \leq V$. This must be controlled --- if $V'$ is too small, the resulting package may not satisfy the original VaR constraint.
% \end{sloppypar}

% \textbf{Closest Approximating CVaR constraint}: Finding an optimal $V'$ when approximating a VaR constraint by a CVaR constraint can be modeled as a search problem. Setting $V'=V$ results in a possibly overconstrained problem. Smaller values of $V'$ can potentially allow packages with better objective values, but the packages may violate the VaR constraint. Validation scenarios are particularly useful here. Once a package is generated with a CVaR constraint with value $V'$, we check its VaR among the validation scenarios. For instance, if the VaR constraint requires the sum of an attribute for the package to be at least $-10$ with probability $0.95$, and $V'=-20$ meaning the corresponding CVaR constraint will require the expected sum to be at least $-20$ in the lowest $5\%$ of scenarios, the scenario score of the generated package in the $5$-th percentile of validation scenarios is the package's VaR. If this satisfies the VaR constraint, the obtained package is feasible. Suppose for a \textit{low enough} value of $V'=V_{min}$, the generated package has an infeasible VaR. An optimal value of $V'$ can then be found using a bisection over the range $[V_{min}, V]$. From an interval $[V_l, V_u]$ (initially, $V_l=V_{min}$ and $V_u=V$) pick the mid-point, $V' = 0.5(V_{min} + V_{u})$. If this results in a feasible package, we set our new search range to $[V_l, V']$ in search of packages with better objective value. Else, we set the range to $[V', V_u]$ in search of feasible packages. The search terminates when $V_u - V_l \leq \delta$ for a small $\delta \geq 0$. This converges within $\log_2(\frac{V-V_{min}}{\delta})$ iterations.

% A key detail involves finding $V_{min}$ --- a value of $V'$ small enough to guarantee the corresponding VaR constraint is not satisfied when $V'=V_{min}$. Such a lower bound may not exist if the constraint is trivially satisfiable, that is, even without the constraint being imposed, the resulting optimal package has a VaR exceeding the threshold specified in the constraint. Such constraints can be removed from the query, and we do not need the aforementioned bisections for them. To detect if a VaR constraint is satisfied trivially or find $V_{min}$ otherwise, we remove all risk constraints from the query, and obtain the optimal package $P_0$ for this risk-unconstrained SPQ. If removing all risk constraints makes the problem unbounded, we replace the VaR constraints requiring the sum of an attribute $A$ in a package to be at least $V$,  with a typically much easier to satisfy expected value constraint requiring the expected sum of $A$ in the package to be at least $V$. VaR constraints satisfied by $P_0$ are trivial. For others, we use the VaR in the resulting package as the lower bound $V_{min}$.
% %We do this by picking an arbitrary positive number $d>0$, and experimenting to see if setting $V'=V-d$ causes the violation of the VaR constraint. If not, we then try the same with values $V-2d, V-4d, V-8d, ...$. i.e. doubling the difference in each iteration, until a valid lower bound is found. If a lower bound is first found in the $(m+1)$-th iteration, i.e. setting $V'=V-2^md$ causes constraint violation, while $V'=V-2^{m-1}d$ does not, we begin the succeeding bisection in the range $[V-2^md, V-2^{m-1}d]$. 

% Converting VaR constraints to their closest approximating CVaR constraint means each VaR constraint will have a single corresponding linear constraint in the query --- regardless of how many optimization scenarios are used. In terms of optimizer runtimes, this gives us unlimited scalability across the scenario dimension.

% \textbf{\cvarif} (Alg.~\ref{alg:cvarmethod_query_execution}) conducts a sequence of parallelly executed bisections to get the closest approximating CVaR constraint for each risk constraint in the query. It begins with a relatively small number (e.g. 100) of optimization scenarios, as generating too many optimization scenarios with values for every tuple would be time consuming. The algorithm runs an outer loop (Lines 1-21) where it creates a package with the selected number of optimization scenarios (Lines 2-15), returning the package if it is feasible and $(1\pm\epsilon)$-approximate (Lines 16-17).

% To find an optimal package, \cvarif first creates a set of optimization scenarios for each constraint and objective (Lines 2-4). If multiple constraints and the objective share the same attribute, their optimization scenarios can be shared, i.e. we do not need to generate distinct optimization scenarios for each of them. It then gets the optimal package $P_0$ produced in response to the risk unconstrained version of the SPQ using an in-memory ILP solver like Gurobi Optimizer. As mentioned earlier, the VaRs of $P_0$ over the validation scenarios for the risk constraints in $Q$ can be used as the lower bounds for the respective bisections of those risk constraints. Furthermore, the objective value of $P_0$ over the validation scenarios can be used as an upper bound for the objective value of the optimal package for $Q$, which can be used to determine if any package generated by \cvarif is $(1\pm \epsilon)$-approximate. Details on determining $(1\pm\epsilon)$-approximation is described in prior work~\cite{BrucatoYAHM20}.

% %We then find the lower bound for the bisections of each risk constraint (Line 6). In our experiments, we set $d$ to $100$, but we also observed that changing this value will not greatly impact latency since the range of the interval grows exponentially with each iteration. If $V-d$ is smaller than the CVaR of $P_0$ for any constraint, we simply use $P_0$'s CVaR value as the lower bound for the constraint's bisection. 

% \begin{algorithm}[tb]
% \caption{\textit{\cvarmethod{} Query Execution}}\label{alg:cvarmethod_query_execution}
% \begin{algorithmic}[1]

% \Require $Q$, Stochastic package query
% \Statex $m$, initial number of optimization scenarios (e.g. $100$)
% \Statex $\hat{m}$, number of validation scenarios (e.g. $10^6$)
% \Statex $\epsilon$, user-defined approximation error bound
% \While{True}
%   \For{every stochastic constraint and objective in $Q$}
%     \State Generate $m$ scenarios and their pseudo-scenarios
%   \EndFor
%   \State $P_0 \gets$ Package returned for the risk unconstrained SPQ
%   \State Get bounds for bisecting all non-trivial risk constraints
%   \While{All bisections are not complete}
%     \For{each risk constraint $C$}
%      \State $V'_{C} \gets$ Midpoint of search interval for $C$\
%     \EndFor
%     \State Create $ilp\_formulation$ with all values of $V'_C$
%     \State $p \gets SolveILP(ilp\_formulation)$
%     \State Validate $p$ among validation scenarios for all constraints
%     \State Update bounds for bisection
%   \EndWhile
%   \If{$p.is\_feasible(Q) \And p.is\_1\pm\epsilon\_approx(\epsilon)$}
%     \State \Return p %\Comment{{\color{gray} \textit{A feasible and ($1+\epsilon$)-approximate package is returned if found}}}
%   \Else
%     \State $m \gets \min(2m, \hat{m})$ %\Comment{{\color{gray}\textit{Double the number of optimization scenarios and try again}}}
%   %\Else
%   %  \If{not $p.is\_feasible(Q)$}
%   %    \State \Return "No package found"
%   %  \Else
%   %    \State \Return $p$
%   %  \EndIf
%   \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}


% Bisections are then run between the respective bounds of each constraint. At each iteration, for a VaR constraint $C$ requiring the sum of $A$ to exceed $V$ with at least probability $p$, if $[V_l, V_u]$ is the interval of possible CVaR values, we include the linear constraint $\sum_{i=1}^{(1-p)m} \sum_{j=1}^{n} P_{ij}x_{j} \geq (1-p)m*0.5(V_{l}+V_{u})$ into the ILP. Here, $P$ is the set of pseudo-scenarios. $(1-p)m$ represents the number of pseudo-scenarios considered ($(1-p)$-fraction of pseudo-scenarios are considered to correspond with the `IN THE LOWEST $(1-p)*100\%$ OF SCENARIOS' part of the  CVaR constraint) and $0.5*(V_{l}+V_{u})$ is the midpoint of the search interval. Note that, setting $m'=(1-p)m$ and $V=0.5(V_l+V_u)$ makes this linear constraint a simple algebraic manipulation of the antecedent of implication~(\ref{eq:cvar_representation}).

% %If using a limited number of optimization scenarios leads us to constructing a package that can be verified to be feasible among the validation scenarios (i.e. is validation feasible), \textit{and} whose objective value is guaranteed to be within $(1 \pm \epsilon)O_{opt}$, where $O_{opt}$ is the objective value of the optimal package (i.e. is $(1\pm\epsilon)$-approximate), the package is returned. For queries that require maximizing an objective value, the returned package will have an objective value of at least $(1 - \epsilon) O_{opt}$, while for minimization problems, the objective value will be capped at $(1+\epsilon) O_{opt}$. Detecting validation feasibility is trivial, while methods to determine if a package is $(1 \pm \epsilon)$-approximate have been proposed for \textit{SPaQL} in prior literature~\cite{BrucatoYAHM20}.

% Once linear constraints are included in the ILP for all risk constraints (lines 8-11), we use an in-memory solver to solve the ILP and find its optimal package $p$ . We validate constraint satisfaction of $p$ among all the validation scenarios, and update the bounds of each constraint independently (lines 13 and 14). If the ILP has no solution, we perform the same actions that we would if a suboptimal package was generated, which leads to more relaxed bounds for every constraint in later iterations. Once all bisections converge to intervals smaller than $\delta$, which can be an arbitrarily small preset value that we in our experiments set to be $0.1$, we check if the package finally obtained is validation feasible and $(1\pm\epsilon)$-approximate, and if so, return it (lines 16-17). If either of these conditions are violated, or if no package is returned by the solver, we double the number of optimization scenarios and try again (lines 18-19).

% Doubling the number of scenarios at each iteration is possible since \cvarif makes solver runtimes agnostic to the number of optimization scenarios. This allows aggressively increasing the number of optimization scenarios as the only penalty paid is in terms of scenario generation runtime. We ensure the number of optimization scenarios ($m$) never goes beyond the number of validation scenarios ($\hat{m}$). In the worst case, if we begin with $m=100$ optimization and $\hat{m}=10^6$ validation scenarios, there will still be no feasible and $(1\pm\epsilon)$-approximate solution after 13 iterations, after which $m$ will equal $\hat{m}$. Then, if a package is created from the optimization scenarios, it is guaranteed to be validation feasible since the set of optimization and validation scenarios are identical, and will be considered $(1\pm\epsilon)$-approximate. If no package is produced, the query is infeasible and has no solutions.

% Unconditionally increasing the number optimization scenarios is an improvement over \ssearch. If the generated package is not $(1\pm\epsilon)$-approximate, and the number of summaries is lower than the number of optimization scenarios, \ssearch incrementally increases the number of summaries. The number of optimization scenarios is only increased after the number of summaries equals the number of optimization scenarios. This results in a wasted inner loop over the number of summaries if the number of optimization scenarios is initially insufficient. Since this inner loop's complexity depends on the number of optimization scenarios, \ssearch remains much more conservative when increasing the number of optimization scenarios, and increases the number linearly instead of doubling it at each iteration like \cvarif.

% The sequence of ILPs solved during the bisection for the risk constraints is logarithmic to the size of the largest search range for any constraint. \ssearch needs a similar sequence to determine how many scenarios to use for creating each summary. 

% \cvarif updates the intervals of the CVaR approximations for each VaR constraint independently. Treating the problem of finding the closest CVaR approximations for multiple VaR constraints as a multi-dimensional search and updating the intervals co-dependently remains scope for future work.

% Implementation-wise, if the entire set of optimization scenarios, having size $m*n$ where $m$ is the number of optimization scenarios and $n$ is the number of tuples, fits into main memory, we store it entirely in the main memory to enable scenario sharing for other constraints and stochastic objectives addressed on the same attribute. If not, note that expected value constraints and stochastic objectives only require the sum of all scenario values for every tuple in their corresponding ILP expressions. So, we generate one scenario at a time, add its values to the respective sums for each variable, and erase the scenario from main memory. For converting risk constraints to CVaR constraints, we need the sum of the lowest $p$-fraction of scenario values for each tuple to construct the pseudo-scenario based linear constraint. We determine this by using max heaps containing at most $pm$ elements for each tuple. Every time a scenario is generated, we insert the values into each tuple's heap only if the heap has less than $pm$ elements or the scenario value for the tuple is smaller than the maximum value in the heap, in which case the max value is replaced by the value. Once all scenarios are generated, all heaps are erased and the sum of their elements are used for representing the CVaR constraints. Heap insertions and replacements can be parallelized across tuples. This is only possible if $n$ heaps with $pm$ elements fit into main memory. Otherwise, we divide the tuples into blocks of size $b$, such that $b$ heaps of size $pm$ fit into main memory, and generate scenario values for only tuples in the same block at a time.

% Note that while we describe handling VaR constraints that require the sum of an attribute to be higher or equal to a certain value, the methods can be trivially modified to handle VaR constraints that require the sum to not exceed given values.

% Finally, we prove implication (\ref{eq:cvar_representation}), which is the basis of using pseudo-scenarios to linearly represent CVaR constraints.

% \begin{theorem}
%     For any package $x=\{x_1, x_2, ..., x_n\}$ and a set of pseudo-scenarios $P$ formed from a set of scenarios $S$, if the expected scenario$\_$score of $S$ exceeds $V$ in the first $p$ pseudo-scenarios, the expected sum of $x$ in any $p$ scenarios of $S$ will also exceed V.
%     \label{theorem:conservative_pseudoscenarios}
% \end{theorem}

% \begin{proof}
% We define $L$ to be a set of indexes of $p$ scenarios and a one-to-one function $f([1, n], [1, m]): \rightarrow [1, m]$, which takes a tuple $i$ and a scenario $j$, and returns the position of $S_{ij}$ in the $i$-th row of the pseudo-scenario matrix $P$ after sorting. Then:

% $\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} = \sum_{j=1}^{n} x_{j} \sum_{i=1}^{p} P_{ij} \leq \sum_{i=1}^{n} x_{i} \sum_{j \in \bigcup_{t \in L} f(i, t)} P_{ij}$

% The last inequality holds since each element in $\bigcup_{t \in L} f(i, t)$ is either in $[1, p]$, meaning it contributes to both sides of the inequality equally, or is greater than $p$, which means they are being replaced by a value from $P_{i1}, P_{i2}, P_{i3}, ... P_{ip}$ in the left side of the inequality, where the replaced value on the left cannot be larger than the original value on the right since $P$ is row-wise sorted. From the definition of $f$, for all tuples $j$, $\sum_{i \in \bigcup_{t \in L} f(j, t)} P_{ij} = \sum_{i \in L} S_{ij}$.

% Thus, $\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \sum_{j=1}^{n} x_{j} \sum_{i \in L} S_{ij}$

% $\implies \sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i}$

% $\implies \frac{1}{p}\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \frac{1}{p}\sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i}$

% Thus, $\frac{1}{p}\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \geq V \implies \frac{1}{p}\sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i} \geq V$
% \end{proof}

\section{Stochastic partitioning}\label{sec:partitioning}

We describe the offline computation for \sskr by answering three questions:~(i)~How do we quantify similarity between tuples with respect to stochastic attributes? (Section~\ref{subsec:stoch_similarity})~(ii)~How do we partition the tuples? (Section~\ref{sec:dpart})~(iii)~How do we create representatives from the partitions? (Section~\ref{subsec:rep_selection}) %\azza{Perhaps conclude with we answer the first question in section ... and the second question in section... or something of that sort.}

\subsection{Distance between stochastic tuples}
\label{subsec:stoch_similarity}
The value of a tuple for a stochastic attribute is a random variable. To differentiate between such random variables, we consider two important criteria: their distributional shapes (i.e. their pdfs) and mutual correlation. Similar distributional shapes ensures the random variables demonstrate similar tail behaviors while positively correlated tuples demonstrate similar risk profiles --- they tend to have lower values during the same scenarios. Statistical distances/divergences such as Wasserstein metric or KL divergence typically quantify only the dissimilarity between distributional shapes. Therefore, they can group uncorrelated tuples with the same distribution together. Correlation measures such as Pearson's correlation coefficient only quantify correlations without taking distributional shape into account. Thus, we use Mean Absolute Difference (MAD), a distance measure that considers both the distributional shape and detect positive correlations among tuples:

$$\textsc{MAD}(X,Y)=\mathbb{E}[|X-Y|]$$

For deterministic attributes, the MAD of two tuples is simply the absolute difference of their values. For stochastic attributes, we take the mean of the absolute value of the differences of the value of the tuples over $\hat{m}$ scenarios. Tuples that have similar underlying pdfs for a stochastic attribute and are positively correlated with each other exhibit similar values across scenarios, and thus have lower \textsc{MAD}s. Our partitioning scheme groups together tuples that have small pairwise \textsc{MAD}s for all the attributes. We show in Section~\ref{sec:theory} that if all pairs of tuples in the partitions have small \textsc{MAD}s from each other over all the attributes, we can provide theoretical guarantees on the quality of packages produced.

\subsection{\dpart}\label{sec:dpart}

\begin{figure*}[h]
    \centering
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-1.jpg}
        \caption{Run a \textit{PivotScan} from a randomly selected pivot}
        \label{fig:pivotscan_from_random_tuple}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-2.jpg}
        \caption{From the farthest tuple, run a second \textit{PivotScan}}
        \label{fig:farthest_tuple_pivotscan}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-3.jpg}
        \caption{Sort all tuples by increasing distance, and partition every consecutive $s$ tuples}
        \label{fig:size_based_partitioning}
    \end{subfigure}\\
    %\hfill
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-4.jpg}
        \caption{For diameter-based partitioning, run \textit{PivotScan} from any tuple in all partitions}
        \label{fig:random_tuple_pivotscan_for_wide_partitions}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-5.jpg}
        \caption{From the farthest tuples found, run another \textit{PivotScan}}
        \label{fig:farthest_tuple_pivotscan_for_wide_partitions}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[h]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/DistPartition-6.jpg}
        \caption{In wide partitions, group tuples having similar distances separately}
        \label{fig:diameter_based_repartitioning}
    \end{subfigure}
    \caption{High Level Workflow of \partioningscheme{}}
    \label{fig:partitioning-hlf}
\end{figure*}

\dpart partitions the tuples in the relation while satisfying:~(i)~a size constraint: no partition may contain more than $\tau$ tuples and~(ii)~diameter constraints: no two tuples in a partition can have MAD more than $d_A$, where $d_A$ is a diameter threshold defined for attribute $A$. These thresholds can be defined by a user or a database administrator based on the number of decision variables ILP solvers can handle in a reasonable amount of time (this differs due to differences in the underlying hardware and solver software) and application requirements on runtime and quality of results. 

Existing uncertain data clustering algorithms do not ensure the resulting clusters will satisfy such constraints~\cite{ chau2006uncertain, gullo2008clustering, gullo2012uncertain, gullo2013minimizing}. Hierarchical partitioning approaches can be trivially modified to satisfy these constraints, but their runtime complexities are super-quadratic with respect to the number of tuples in the relation, making them unsuitable for fast partitioning of large relations ~\cite{gullo2008hierarchical, zhang2017novel}.



We propose \dpart (Fig.~\ref{fig:partitioning-hlf}) for quickly splitting large relations into partitions satisfying all size and diameter constraints.

It uses \pvscan, an operation that finds the mean absolute difference of a chosen tuple (\textit{pivot}) with all other tuples in its partition with respect to a specified attribute. \dpart has two phases --- (i)~Size-based partitioning and (ii)~Distance-based partitioning.

First, \dpart runs \pvscan from a randomly chosen tuple and finds the distance of all other tuples in the relation from it (Fig.~\ref{fig:pivotscan_from_random_tuple}). For the farthest tuple found, it runs a second \pvscan (Fig.~\ref{fig:farthest_tuple_pivotscan}) and lists all tuples in the relation in ascending order of their distances from the second pivot. We group every consecutive $s$-tuples in this list into the same partition, thereby ensuring no resulting partition has more than $s$ tuples (Fig.~\ref{fig:size_based_partitioning}).

The resulting partitions may be wide and violate diameter constraints for certain attributes. To check this, we randomly select a tuple from each partition, and run a \pvscan from them over all other tuples in the partition for each attribute (Fig.~\ref{fig:random_tuple_pivotscan_for_wide_partitions}).

From the farthest tuples found for each attribute, we run another \pvscan, finding the distance of all other tuples in their partition from them (Fig.~\ref{fig:farthest_tuple_pivotscan_for_wide_partitions}). If any tuple is found to have a distance exceeding $d_{A}$ during this \pvscan, the partition is considered `wide'. All tuples in the partition are again sorted in ascending order of distances, and tuples having distances within intervals $[0, d_A], ]d_A, 2d_A], ... ](k-1)d_A, kd_A]$ are grouped into separate partitions (Fig.~\ref{fig:diameter_based_repartitioning}). The resulting partitions may still be wide with respect to some of the attributes, so distance-based partitioning is recursively applied on each resulting non-empty partition until there are no wide partitions remaining.

\pvscan is embarassingly parallel. Furthermore, after the initial size-based partitioning, diameter-based partitioning can be conducted in parallel for each partition, thus accelerating \dpart when partitioning large relations on multi-core processors.

% \section{\sskr} \label{sec:stochastic_sketchrefine_details}
% While \cvarif provides scalability across the scenario dimension, in-memory solvers struggle with runtime when the number of integer variables in the ILP goes beyond the order of tens of thousands. Since \cvarif associates each tuple with an integer variable, this bottlenecks SPQ processing on large relations.

% %To scale along the tuple dimension, we propose \sskr. Like its deterministic counterpart, \sskr partitions the relation offline (Fig.~\ref{fig:partition_hlf}). The partitioning algorithm needs to ensure that (i)~tuples in the same partition are mutually similar with respect to all attributes, including stochastic ones, making them virtually interchangeable when forming packages, and (ii)~no partition contains too many tuples to avoid overflooding the solver with too many variables during refinements.%\anh{It may be necessary to talk about how many is "too many" at this point}. Ensuring the latter helps avoid situations where the SPQ solver is flooded with too many tuples during refinements. We then select a tuple from each partition as its representative (Fig.~\ref{fig:representative_election_hlf}).

% %\anh{as a reader, it would be a bit confusing as the Fig. 4d seems to show distinct points but you indicate them as "stochastically identical duplicates"}
% %Query execution during \sskr consists of the Sketch and Refine phases. During sketch, we form stochastically identical duplicates of each representative (Fig.~\ref{fig:representative_duplication_hlf}), and form a sketch package by solving an ILP containing variables only the  (Fig.~\ref{fig:sketch_query_hlf}). 
% %For all its advantages, \cvarmethod{} still shares a key weakness with \textit{SummarySearch}- the number of variables in its ILP formulations is equal to the number of tuples in the relation. For in-memory ILP solvers, this number can be prohibitively large for relations with over a million tuples. To solve this problem we employ the \textit{SketchRefine} paradigm described in Section \ref{subsec:sketchrefine_deterministic} and adopt it for stochastic settings with our proposed approach \algname{}. \algname{} first conducts a one-time offline partitioning of the dataset (Fig. \ref{fig:partition_hlf}), and then elects a representative from each partition (Fig. \ref{fig:representative_election_hlf}).   

% We propose \sskr (Fig.~\ref{fig:stochastic-sketchrefine-hlf}), which achieves greater scalability across the tuple dimension by reducing the number of integer variables in the ILPs. It first partitions the relation offline (Fig.~\ref{fig:partition_hlf}), ensuring that (i)~tuples in the same partition are similar across all attributes, and (ii)~no partition contains \textit{too many} tuples. Ensuring the former means tuples from the same partition are almost interchangeable when forming packages, while the latter prevents solvers from having to deal with too many tuples at once.

% Query execution is split into the \textit{sketch} and \textit{refine} phases. During sketch, we form stochastically identical duplicates of each representative. The number of duplicates can differ by representative based on their stochastic properties, as detailed in Section~\ref{subsec:sketch}. For instance, the representatives in Fig.~\ref{fig:representative_duplication_hlf} have 3, 2, 2, 4 and 2 duplicates respectively. A `sketch package' is produced by solving the SPQ over all duplicates of all the representatives. In Fig.~\ref{fig:sketch_query_hlf}, the sketch package includes 2, 1 and 1 duplicates respectively from three of the partitions. Since the number of representatives is much smaller than the number of tuples in the relation and \sskr ensures the number of duplicates of each representative is low, the total number of tuples scoped within sketch is much smaller than the number of tuples in the relation.

% Representative duplication is a key difference between \sskr and its deterministic counterpart. To see its necessity, suppose an SPQ $Q$ has an optimal package $P_{opt}$, some of whose tuples belong to the same partition. For $P_{opt}$ to be generated by \sskr, the sketched version of $P_{opt}$, i.e. the package formed by replacing each tuple of $P_{opt}$ by its representative, needs to satisfy all the constraints. This is not guaranteed if multiple tuples in $P_{opt}$ are mapped to the same representative, meaning that instead of having distinct tuples as in $P_{opt}$, the sketched version needs to include the same representative multiple times. Grouping distinct tuples into the same representative reduces tuple diversity in the sketch package, thereby increasing risk~\cite{lekovic2018investment}.

% Consider a toy example: $P_{opt}$ contains tuples $t_1$ and $t_2$, both of which output $1$ and $-1$ with probability 0.5 for an attribute $A$. $Q$ has a VaR constraint specifying SUM(A)$\geq -1$ WITH PROBABILITY$\geq 0.7$. If $t_1$ and $t_2$ are mutually independent, $P_{opt}$ satisfies the constraint since it will have a sum of 2 with probability 0.25, 0 with probability 0.5, and -2 with probability 0.25. Suppose both tuples belong to the same partition, with $t_1$ being the unduplicated representative. The sketched version of $P_{opt}$ would contain $t_1$ twice, having SUM(A)=-2 with probability 0.5, hence violating the constraint. \sskr is thus forced to find a different feasible package, whose refined version will be suboptimal.

% %This exposes a general limitation that \sskr would have if it did not duplicate representatives. It connects with the general intuition that having more distinct tuples in a package, i.e. increasing a package's diversity, would reduce risks. During sketch, we essentially limit the solver's opportunities for diversification --- we cluster similar tuples into single representatives, and ask the solver to form a sketch package from a limited number of representatives. In an effort to create feasible packages that do not violate risk constraints, the solver selects a diverse set of representatives and ends up including partitions in the sketch package (and consequently in the refined outputs) whose tuples yield poor objective values. This is where the false impression of diversity created by duplicating representatives becomes helpful.

% %\anh{do you mean "the same probability distributions"? I am not sure what marginal means if there is no conditional probability here} \riddho{Corrected}
% Consider what happens when we form two mutually independent duplicates of $t_1$, $t^1_1$ and $t^2_1$ with the same probability distributions --- returning $-1$ and $1$ with probability $0.5$. In the sketched version of $P_{opt}$, $t_1$ will map to $t^1_1$, and $t_2$ to $t^2_1$. The sketched package containing $\{t^1_1, t^2_1\}$, will have an identical probability distribution over SUM(A) as $P_{opt}$, and will be feasible. This way, having stochastically identical duplicates increases the chances of the sketched version of optimal packages being feasible, making optimal packages discoverable by \sskr.

% Using too many duplicates can make the sketch ILP too large. \sskr controls the number of duplicates used for each partition, balancing the need for diverse selection during sketch while keeping the number of duplicates limited.

% During Refine, duplicates in the sketch package are replaced by actual tuples from the relation. First, we choose any partition with duplicates in the sketch package, and solve the equivalent ILP for the SPQ with all the tuples in the partition, and duplicates from other partitions in the sketch package. The solver preserves the number of unrefined duplicates in the package, and replaces the duplicates in the partition being refined with actual tuples from the partition. Refinements are then sequentially done for each partition in the sketch package until all duplicates are replaced by actual tuples. For all subsequent refinements, the corresponding ILP scopes all tuples in the partition being refined, while preserving the tuples included in the package from prior refinements, and duplicates of representatives of yet unrefined partitions~(Fig.~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}).

% %Once the sketch phase ends, each representative in the sketch package is sequentially refined, and replaced with tuples from the partition in similar fashion to \skr (Fig.~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}).

% The rest of this section provides details on each of these steps.
% %During query execution, we first create stochastically identical duplicates of each representative (Fig. \ref{fig:representative_duplication_hlf}). As we shall explain in further detail later, duplicates help to mitigate the effects of the subadditive property of risks. All duplicates of each representative collectively form the `sketch' table. In the first phase of query execution, we run the query on the `sketch' table. The package formed in response will contain only the representatives from selected partitions (Fig. \ref{fig:sketch_query_hlf}). The second and final phase of query execution consists of the refine phase, where the selected representatives are sequentially replaced by tuples from their respective partitions (Fig. \ref{fig:first_refinement_hlf}, \ref{fig:second_refinement_hlf}, \ref{fig:third_refinement_hlf}), resulting in the final package. The size of the sketch problem is related to the number of partitions formed, and the number of duplicates for each representative, while the size of the refine problems is related to the number of tuples in each partition. Due to the partitions being size-constrained, both the sketch and the refine problems are much smaller than the original problem of running the query directly on the entire relation.

% %Of course, this workflow brings forth a new set of questions that need to be answered for it to work. First, how do we define how similar two tuples are with respect to stochastic package queries? Second, given a definition of the similarity between two tuples, how do we partition a database relation containing stochastic attributes into groups of size-constrained but similar tuples? Third, how do we decide which tuples to elect as a representative from each tuple? Fourth, why exactly do we need duplicates of representatives and how do we decide the number of duplicates of each representative to use while processing the sketch query? Fifth, how do we ensure the scenarios generated from these stochastically identical duplicates demonstrate some degree of correlation between themselves during the sketch phase, so as to mimic the correlation between the representative tuples with the other tuples in their partition that will appear during the refine phase? Finally, given all of the information, how do we put them all together into the concrete \algname{} algorithm and can we provide theoretical guarantees on the quality of results produced?

% \subsection{Similarity between stochastic tuples}
% Partitioning a relation into groups of similar tuples requires quantifying dissimilarities among stochastic tuples. Since all SPQ constraints and objectives address individual attributes, we determine the `distance' among tuples based on each attribute separately.

% For any attribute $A$ and tuples $t_1$ and $t_2$ whose values in the $i$-th validation scenario are $S_{i, t_1}$ and $S_{i, t_2}$ respectively, we define the distance between them as the mean absolute difference of their values in all validation scenarios, i.e. $\frac{1}{\hat{M}}*\sum_{i=1}^{\hat{M}} |S_{i, t_1} - S_{i, t_2}|$.

% Mean absolute difference works better than simply comparing the means of the tuples' values because it accounts for the shape of the underlying probability distributions. Suppose, for three mutually independent tuples $t_1$, $t_2$ and $t_3$, $t_1$ and $t_2$'s scenario values are sampled from an underlying standard normal distribution, while $t_3$'s values are sampled from a zero mean normal distribution with variance 2. Suppose, we need to partition the tuples into groups having at most two tuples each. Such size constraints on partition sizes are imposed in practice to ensure the solver is not flooded with too many tuples during refinements, albeit with larger values.

% Since all tuples have the same mean, they are indifferentiable if we use the difference in means as distance. Potentially, this could pit $t_1$ and $t_3$ into the same partition, keeping $t_2$ separate. Suppose, $t_3$ and $t_2$ are the chosen representatives \anh{It is hard for the readers to know why this can be safely assumed (it could be $t_1$ and $t_2$ chosen) since up to this point, they have no idea how you come up with a representative in the first place.}. Higher variance makes packages containing $t_3$ riskier. If an SPQ asks to create a 2-tuple package with VaR exceeding -2.5 with probability 0.95, the only feasible package would be $(t_1, t_2)$, whose VaR based on 10 million samples is $-2.3$ \anh{ I am not sure if these examples are going to be clear for the readers. How do they know these would be the only feasible package?} \riddho{I can add the VaRs of the others possible packages here}. The sketch package can only be created from the representatives $t_3$ and $t_2$ however, and packages $(t_2, t_3), (t_2, t_2), (t_3, t_3)$ are infeasible. Packages containing the same tuple twice have higher VaRs since losses are doubled in the worst case scenarios. Furthermore, $t_2$ cannot be duplicated since its partition only has a single tuple. Since all representative-based packages violate the risk constraint, no sketch package would be formed, and \sskr would fail to find a solution despite a feasible package actually existing.

% Using mean absolute difference resolves this. The mean absolute difference between the pairs $(t_1, t_2), (t_2, t_3), (t_1, t_3)$ is $1.13$, $1.38$, $1.38$ respectively. $t_1$ and $t_2$ are grouped together due to their smaller distance, keeping $t_3$ separate. If $t_2$ and $t_3$ are the chosen representatives, and if $t_2$ is duplicated to $t^1_2, t^2_2$, the sketch package $\{t^1_2, t^2_2\}$ would be feasible and $\{t_1, t_2\}$ would be obtained by refining it.

% We could estimate the densities of each tuple's underlying probability distribution~\cite{acharya2015fast}, and compare the similarities of these estimates. However, this would ignore inter-tuple correlations. High correlations among tuples increases package risks since a tuple incurring losses implies other correlated ones may follow suit.

% Suppose three tuples $t_1$, $t_2$ and $t_3$ all have their scenario values sampled from underlying standard normal distributions, where $t_1$ and $t_2$ are correlated with a Pearson's correlation coefficient of $0.9$, while $t_3$ is uncorrelated with them. Suppose an SPQ requires forming a 2-tuple package with VaR exceeding $-2.5$ with probability $0.95$. The only feasible packages are $\{t_2, t_3\}$ and $\{t_1, t_3\}$. A correlation-agnostic distance metric might group $t_1$ and $t_3$, and keep $t_2$ separate, picking $t_1$ and $t_2$ as representatives. Since no 2-tuple combination of $t_1$ and $t_2$ satisfies the constraint, the sketch package would be unable to generate any package in response. 

% Mean absolute difference considers the \textit{scenario-wise} difference between the values of two tuples. \anh{"Positive" (If they are negatively correlated then this is the opposite)} \riddho{Thanks for pointing this out, edited} Positively correlated tuples hence have smaller distances than uncorrelated ones, despite having the same underlying probability distributions. In our example, the pairwise mean absolute difference between $\{t_1, t_2\}$, $\{t_2, t_3\}$ and $\{t_3, t_1\}$ are 0.36, 1.13 and 1.13 respectively, based on 10 million samples. Partitioning based on mean absolute difference thus groups $t_1$ and $t_2$, keeping $t_3$ separate. Picking either $t_1$ or $t_2$ as a representative from the first partition, and $t_3$ as the representative from the second partition results in a feasible sketch package being formed.

% Furthermore, limiting the mean absolute difference among tuples in a partition provides theoretical guarantees on the quality of packages produced, as described in section \ref{subsec:theoretical_guarantees}.

% %\anh{First of all, I assume that when you say "correlation" you do not mean "dependence". These two concepts are different but related. When talking about "correlation", we mostly talk about "linear correlation" as a measure of how much a random variable $Y$ can be described by a random variable $X$ as $aX+b$ where $a, b$ is some constants. You can see that the Pearson correlation coefficient (PCC) is the standard way to measure this linear correlation between 2 random variables. So if two variables $X, Y$ are linearly correlated then of course they are dependent. But if two variables $X, Y$ are not linearly correlated then we don't know anything about their dependency. It could be that $X=Y^2$ (which in this case $X$ depends on Y). The standard way to measure the dependency of two random variables is distance correlation with a complicated formula.}
% %\anh{Given this, the mean absolute difference does not account for the correlation between pairs of tuples. It only accounts for tuples that are closely identical i.e. $X=Y$ or $X \approx Y$. One way to see this is to have $X=-Y$ which is perfectly linearly correlated, the mean absolute difference would simply be $2E[X]$ which is large or small depending on the mean of the random variable.}

% %\anh{You need to be consistent with either "mean absolute difference" or "mean absolute distance"} \riddho{Done}

% \subsection{Partitioning stochastic data} \label{subsec:distPartition}



% %The user can specify the value of $s$ (e.g. 5000) and the value of $d_{A}$ for each attribute. For larger diameter thresholds, there are a smaller number of groups, resulting in reduced sketch query execution latencies. However, the quality of results can drop since tuples inside the same partition can become increasingly dissimilar to their representatives. We explore the theoretical connection between diameter constraints and their effect on the objective values of the returned packages in section \ref{subsec:theoretical_guarantees}. A database administrator can set the diameter constraints based on the specific application's need for reduced runtimes while sacrificing the quality of results.

% %For stochastic attributes, a diameter constraint restricts the mean absolute difference between any two tuples within the same partition. For deterministic attributes, they constrain the absolute difference between the values for that attribute between all pairs of tuples in a partition.

% %If the size threshold $s$ is set too low, the number of partitions will increase, which increases the number of representatives, and the size of the sketch problem. If the threshold $s$ is set too high, there might be too many variables in the corresponding ILP formulation when refining the partitions.

% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-1.jpg}
%         \caption{Run a \textit{PivotScan} from a randomly selected pivot}
%         \label{fig:pivotscan_from_random_tuple}
%     \end{subfigure}
%     %\hfill
%     \hspace{0.8cm}
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-2.jpg}
%         \caption{From the farthest tuple, run a second \textit{PivotScan}}
%         \label{fig:farthest_tuple_pivotscan}
%     \end{subfigure}
%     \hspace{0.8cm}
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-3.jpg}
%         \caption{Sort all tuples by increasing distance, and partition every consecutive $s$ tuples}
%         \label{fig:size_based_partitioning}
%     \end{subfigure}\\
%     %\hfill
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-4.jpg}
%         \caption{For diameter-based partitioning, run \textit{PivotScan} from any tuple in all partitions}
%         \label{fig:random_tuple_pivotscan_for_wide_partitions}
%     \end{subfigure}
%     \hspace{0.8cm}
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-5.jpg}
%         \caption{From the farthest tuples found, run another \textit{PivotScan}}
%         \label{fig:farthest_tuple_pivotscan_for_wide_partitions}
%     \end{subfigure}
%     %\hfill
%     \hspace{0.8cm}
%     \begin{subfigure}[t]{0.2\textwidth}
%         \centering
%         \includegraphics[scale = 0.2]{figures/DistPartition-6.jpg}
%         \caption{In wide partitions, group tuples having similar distances separately}
%         \label{fig:diameter_based_repartitioning}
%     \end{subfigure}
%     \caption{High Level Workflow of \partioningscheme{}}
%     \label{fig:partitioning-hlf}
% \end{figure*}

% \sskr performs a one-time offline partitioning of the tuples in a relation. The resulting partitions satisfy: (i)~Size constraints, bounding the number of tuples in a partition to a threshold $s$, and (ii)~Diameter Constraints, bounding the pairwise mean absolute difference in a partition for an attribute $A$ to $d_{A}$.

% Values of $s$ (e.g. 5000) and $d_A$ for each attribute are pre-specified by a user/an administrator. $s$ is set based on the number of integer variables an in-memory solver can handle, which depends on the system's main memory size. Larger diameter thresholds result in fewer partitions, trading off quality of packages produced with reduced sketch runtimes, as explored further in Section~\ref{subsec:theoretical_guarantees}.

% Existing uncertain data clustering algorithms do not ensure the resulting clusters will satisfy such constraints~\cite{ chau2006uncertain, gullo2008clustering, gullo2012uncertain, gullo2013minimizing}. Hierarchical partitioning approaches can be trivially modified to satisfy these constraints, but their runtime complexities are super-quadratic with respect to the number of tuples in the relation, making them unsuitable for fast partitioning of large relations ~\cite{gullo2008hierarchical, zhang2017novel}.

% We propose \dpart (Fig.~\ref{fig:partitioning-hlf}) for quickly splitting large relations into partitions satisfying all size and diameter constraints.

% It uses \pvscan, an operation that finds the mean absolute difference of a chosen tuple (\textit{pivot}) with all other tuples in its partition with respect to a specified attribute. \dpart has two phases --- (i)~Size-based partitioning and (ii)~Distance-based partitioning.

% In the first phase, \dpart runs \pvscan from a randomly chosen tuple, and finds the distance of all other tuples in the relation from it (Fig.~\ref{fig:pivotscan_from_random_tuple}). For the farthest tuple found, it runs a second \pvscan (Fig.~\ref{fig:farthest_tuple_pivotscan}), and lists all tuples in the relation in ascending order of their distances from the second pivot \anh{Should mention clearly which pivot: the first one or the second one} \riddho{Thanks again! Edited}. We group every consecutive $s$-tuples in this list into the same partition, thereby ensuring no resulting partition has more than $s$ tuples (Fig.~\ref{fig:size_based_partitioning}).

% The resulting partitions may be wide and violate diameter constraints for certain attributes. To check this, we randomly selecting a tuple from each partition, and running a \pvscan from them over all other tuples in the partition for each attribute (Fig.~\ref{fig:random_tuple_pivotscan_for_wide_partitions}).

% From the farthest tuples found for each attribute, we run another \pvscan, finding the distance of all other tuples in their partition from them (Fig.~\ref{fig:farthest_tuple_pivotscan_for_wide_partitions}). If any tuple is found to have distance exceeding $d_{A}$ during this \pvscan, the partition is considered `wide'. All tuples in the partition are again sorted in ascending order of distances, and tuples having distances within intervals $[0, d_A], ]d_A, 2d_A], ... ](k-1)d_A, kd_A]$ are grouped into separate partitions (Fig.~\ref{fig:diameter_based_repartitioning}). The resulting partitions may still be wide with respect to some of the attributes, so distance-based partitioning is recursively applied on each resulting non-empty partition, until there are no wide partitions remaining.

% \pvscan is trivially parallelizable. Furthermore, after the initial size-based partitioning, diameter based partitioning can be conducted in parallel for each partition, thus accelerating \dpart when partitioning large relations.

% \subsection{Representative Selection:} \label{subsec:representative_selection}

% From each partition, we select a representative tuple for each attribute. Ideally, we would select the tuple with the least mean distance with other tuples in the partition as our representative. However, doing so would require finding the distance between all pairs of tuples in a partition, which has a per-partition time complexity of $\mathcal{O}(s^2\hat{M})$, $s$ being the maximum number of tuples in a partition and $\hat{M}$ being the number of validation scenarios. This is too expensive in large relations containing thousands of partitions.

% For better runtimes, we find the tuple with the least total \textit{worst case replacement cost}. Duplicates of the representative are replaced during refine. If the values of a representative $r$ and a tuple $t$ in the $i$-th scenario are $S_{ir}$ and $S_{it}$ respectively, the cost of replacing $r$ with $t$ is $|S_{ir} - S_{it}|$. In a single scenario, this cost is highest when replacing the representative with a tuple containing either the maximum or the minimum value among all tuples in the partition. If the highest and lowest scenario values among all tuples in a partition are $S_{i,max}$ and $S_{i,min}$ respectively, the worst case replacement cost for a tuple with value $S_{i,t}$ is $C_{i, t}=max(S_{i,max}-S_{i,t}, S_{i,t}-S_{i,min})$. Across all scenarios, the total worst case replacement cost for $t$ is $\sum_{i=1}^{\hat{M}}C_{i, t}$. For each partition, we thus choose the tuple $t$ with the lowest value of $\sum_{i=1}^{\hat{M}}C_{i, t}$ as the representative. This can be computed in $\mathcal{O}(s\hat{M})$.

% Representatives are selected independently for each attribute. Different tuples can be selected as representatives for different attributes. We create a `representative' relation, consisting of the attributes $(partition\_number, attribute, tuple\_id)$, and a foreign key constraint tying $tuple\_id$ values to tuples in the original relation.

% \subsection{The Sketch Phase:} \label{subsec:sketch}
% During sketch, we need to first determine how many duplicates to use for each representative. Using a high number of duplicates helps make optimal packages identifiable by \sskr.

% We exploit the fact that packages typically do not consist of too many distinct tuples. Suppose the maximum number of distinct tuples expected in a package is $P_{max}$ (e.g. 30). $P_{max}$ may be implied in the query explicitly by package size constraints, or, be specified by a database administrator as a \textit{soft constraint} --- the solver will not be barred from creating packages with more distinct tuples if they have better objective values, but the theoretical guarantees provided in Section \ref{subsec:theoretical_guarantees} may not hold for them.

% If we use $P_{max}$ duplicates for each representative, each tuple in the final package would have a one-to-one correspondence with a duplicate in their sketch representations, ensuring no loss of tuple diversity. However, this would increase the size of the sketch problem by a factor of $P_{max}$, resulting in increased solver runtimes for sketch. We still use $P_{max}$ duplicates when validating packages produced by sketch over the validation scenarios.

% While finding packages, a compromise would be to have $d$ duplicates for a representative, where $d<P_{max}$. This would result in increased projected risks when more than $d$ tuples from the partition belong in the optimal package \anh{Not sure how it would result in "increased projected risks" and what do you mean by "projected risks"} \riddho{Projected risk here refers to the risk of the optimal package among the optimization scenarios, but this should be specified better}. In the worst case, all $P_{max}$ tuples will belong to the same partition. For a concrete example, consider what happens when $d=7$ and $P_{max}=30$. The risk-optimal sketch package would consist of any 2 duplicates being included 5 times in the package, with the other 5 duplicates included 4 times each. Its VaR is expected to be higher than a package where 30 duplicates are included once each. We define $risk\_projection(d, P_{max})$ as the VaR over the optimization scenarios, if a package was formed by taking a total of $P_{max}$ tuples from $d$ duplicates. We define the `compromise ratio' as ratio of risk projection when taking $P_{max}$ duplicates instead of $d$ duplicates.

% \begin{equation*}
%     compromise\_ratio(d) = \frac{risk\_projection(P_{max}, P_{max})}{risk\_projection(d, P_{max})}
% \end{equation*}

% \anh{Who and how to set the initial compromise ratio and the increase in compromise ratio? Obviously, this depends on the percentage of the VaR expression (80\% VaR is different from 99\% VaR) as well as the distributions of the tuples.}

% Since the projected risks are higher when less duplicates are used, for $d \leq P_{max}$, $compromise\_ratio\leq 1$. During sketch, we begin with a predefined compromise ratio threshold, and for each representative, create $d$ duplicates where $d$ is the minimum value for which the compromise ratio exceeds the given threshold \anh{How do you select d when there are multiple VaRs?}. We then use \cvarif to find a package in response to an SPQ over all the duplicates. If the generated package is validation feasible but not $(1 \pm \epsilon)$-approximate, instead of increasing the number of optimization scenarios directly, we first increase the compromise ratio threshold and revise the number of duplicates used, and reiterate the process (Alg.~\ref{alg:sketch}). Note that in Line 4, \cvarif does not modify the number of optimization scenarios as it usually does, an activity that is controlled in lines 5-11 instead.

% \begin{algorithm}[tb]
% \caption{\textit{Sketch}}\label{alg:sketch}
% \begin{algorithmic}[1]

% \Require $Q$, Stochastic package query
% \Statex $m$, initial number of optimization scenarios (e.g. $100$)
% \Statex $\hat{m}$, number of validation scenarios (e.g. $10^6$)
% \Statex $\epsilon$, user-defined approximation error bound
% \Statex $\alpha$, initial compromise ratio (e.g. $0.85)$
% \Statex $\delta$, increase in compromise ratio (e.g. $0.03)$
% \While{True}
%   \State Generate optimization scenarios
%   \State Get required number of duplicates according to $\alpha$
%   \State $p \gets \cvarif(Q, m, \hat{m}, \epsilon)$
%   \If{$p.is\_feasible(Q) \And p.is\_1\pm\epsilon\_approx(\epsilon)$}
%     \State \Return p
%   \ElsIf {$p$ is not $(1\pm\epsilon)$-approximate and $\alpha < 1$}
%     \State $\alpha \gets \min(\alpha + \delta, 1)$    
%   \Else
%     \State $m \gets \min(2m, \hat{m})$
%   \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

% Finally, we look into how to generate scenarios from duplicates. If all duplicates were mutually independent, we would independently invoke the VG functions of the representative $d$ times to get $d$ scenario values, collectively forming a single scenario.

% However, tuples in the partition can be correlated with the representatives by different extents. As previously mentioned, correlations impact risk projections. For accurate one-to-one mapping between tuples and duplicates, the duplicates themselves should be mutually correlated to degrees mirroring the inter-tuple correlations within a partition. Doing so exactly is impossible since the number of duplicates is typically much smaller than the number of tuples in a partition. For simplification, we make the mutual correlation between all pairs of duplicates equivalent to $\overline{\rho}$, where $\overline{\rho}$ is the median of correlations of tuples in the partition with the representative, and generate scenarios from correlated duplicates using the NORTA method~\cite{ghosh2003behavior} \anh{Any particular reason why median over mean?}.

% In the NORTA approach, we first generate one sample from $d$ standard normal distributions \anh{If you assume independent here, please write it out}, forming a $d$-dimensional vector $X$. Given a $d \times d$ matrix $P$, we conduct an eigendecomposition of $P$ to $V\Lambda V^{-1}$. A scenario $Z$ of $d$ correlated standard normal distributions is then generated by calculating $Z=V\sqrt{\Lambda}X$. To create a scenario $S$ of any $d$-correlated random variables, if the cumulative density function of the $i$-th random variable is $C_{i}$, the $i$-th element in the scenario $S_{i}=C^{-1}_{i}(\phi(Z_i))$.

% We accelerate scenario generation via NORTA by exploiting the fact that in our case $P$ is a special correlation matrix where for all $1 \leq i, j \leq d$, $P_{ij}=1$ if $i=j$ and $P_{ij}=\overline{\rho}$ otherwise. As such, the eigenvectors and eigenvalues of $P$ can be calculated apriori, bypassing the general cubic computations. Following the notations above, the first eigenvector of $V$ is $\mathbf{1}^{d}$, with the corresponding eigenvalue $\lambda_{1}=1+(d-1)\overline{\rho}$. For $2 \leq i \leq d$, the $i$-th eigenvector $V_{i}$ has $V_{i1}=-1$, $V_{ii}=-1$ and $V_{ij}=0$ if $j$ is neither 1 or $i$. The corresponding eigenvalue for all these vectors are $\lambda_2=1-\overline{\rho}$. As a result, $Z_{1}=X_{1}\sqrt{\lambda_1}-\sum_{i=2}^{d}X_{i}\sqrt{\lambda_2}$, and for all $2 \leq i \leq d$, $Z_{i}=X_{i}\sqrt{\lambda_2} - X_{1}\sqrt{\lambda_1}$, making $Z$ computable in $\mathcal{O}(d)$. Since all $d$-duplicates have the same underlying stochastic distributions, their cumulative density function $C$ is the same, and can be precalculated using fast histogram approximations~\cite{acharya2015fast}. Using $S=C^{-1}(\phi(Z))$, we can generate the corresponding scenario from correlated duplicates.
% \subsection{The Refine Phase:}\label{subsec:refine}

\subsection{Representative selection}\label{subsec:rep_selection}

Ideally, we would like to come up with a representative that minimizes its maximum \textsc{MAD} with any tuple in the partition. However, to come up with such a representative, we essentially need to compute and store the median `random variable' of each partition for each attribute. This is expensive to compute and store. Therefore, we simply select a tuple in the partition with the least \textsc{MAD} overall with other tuples as our representative. However, doing so would require finding the \textsc{MAD} between all pairs of tuples in the partition which is of quadratic time complexity. Instead, we come up with a cost-model heuristic that gives a linear time complexity by finding the tuple with the least total \textbf{worst-case replacement} cost. 

\begin{algorithm}[t]
\caption{\textsc{RepresentativeSelection}}\label{alg:select}
\begin{algorithmic}[1]
\Require $A :=$ the stochastic attribute
\Statex $t_1,\dots,t_N :=$ N tuples
\Statex $\hat{m} :=$ the number of scenarios to generate 

\For {$j \in \{1,\dots,\hat{m}\}$ \textbf{and} $i \in \{1,\dots,N$\}}
    \State $s_{ij}.A \gets $ the realized value of $t_i.A$ in scenario $j$
\EndFor

\For {$j \in \{1,\dots,\hat{m}\}$}
    \State $\min_{j}.A \gets \min_{i=1}^N s_{ij}.A$
    \State $\max_{j}.A \gets \max_{i=1}^N s_{ij}.A$
\EndFor

\For {$i \in \{1,\dots,N\}$}
    \State $C_{i}.A \gets \sum_{j=1}^{\hat{m}} \max(\max_{j}.A - s_{ij}.A, s_{ij}.A-min_{j}.A)$
\EndFor

\State $i^* \gets \operatorname*{argmin}_{i} C_i.A$

\State \Return $t_{i^*}$

\end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:select}, we first generate $\hat{m}$ scenario values for each tuple $t_i.A$ (line~2). Then for each scenario $j$, we compute $\min_j.A$ and $\max_j.A$ the minimum and maximum scenario values over the $N$ tuples respectively (lines~4-5). Hence, for each scenario $j$, the worst-case replacement cost of a tuple $t_i$ is $\max(\max_{j}.A - s_{ij}.A, s_{ij}.A-min_{j}.A)$, i.e., if you replace this tuple as your representative then in the worst-case, the cost is its maximum distance to either the maximum or minimum of that scenario. The overall cost is simply the sum of the costs over the scenarios (line~7). The representative will share the same random variable for the attribute with the tuple having the least total cost.


% \subsection{Theoretical Guarantees:}\label{subsec:theoretical_guarantees}

==> sections/old_files/cvarif_deprecated.tex <==
\section{\cvarif}\label{sec:cvarif}

\begin{algorithm}[t]
\caption{\textsc{Approximate CVaR}}\label{alg:approx}
\begin{algorithmic}[1]
\Require $p :=$ probability value of the CVaR
\Statex $s_1,\dots,s_m :=$ m sampled values

\Comment{ {\color{gray}\textit{Approximate CVaR of an attribute with probability value $p$ using sampled values}}}

\State $\Tilde{s}_1,\dots,\Tilde{s}_m \gets \textsc{SortAscending}(s_1,\dots,s_m)$
\If{$\lfloor pm \rfloor = 0$}
    \State\Return $\Tilde{s}_1$
\Else
    \State \Return $\sum_{i=1}^{\lfloor pm \rfloor} \Tilde{s}_i/\lfloor pm \rfloor$
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{\textsc{\cvarif}}\label{alg:cvarification}
\begin{algorithmic}[1]
\Require $Q[v_1,\dots,v_K] :=$ An SPQ with $K$ stochastic constraints, with bounds $v_k$ and probability value $p_k$ for $k \in \{1,\dots,K\}$.
\Statex $m :=$ Initial number of scenarios used
\Statex $\hat{m} :=$ maximum number of scenarios used
\Statex $\epsilon :=$ approximation error bound
\Statex $\delta :=$ bisection termination distance

\State $N \gets$ the number of tuples in the relation
\State $I_0 \gets \textsc{FormulateILP}(Q[-\infty,\dots,-\infty], \emptyset)$ \Comment{ {\color{gray}\textit{Remove all stochastic constraints in $Q$ and formulate its ILP}}}
\If{\textsc{IsSolveable}($I_0$)}
    \State \Return 
\EndIf
\State $P_0 \gets \textsc{ILPSolver}(I_0)$
\If{\textsc{IsFeasible}($Q,P_0,\hat{m}$)}
    \State \Return $P_0$
\EndIf
\While{$m < \hat{m}$}
    \For{$k \in \{1,\dots,K\}$} \Comment{ {\color{gray}\textit{For each stochastic constraint $k$}}}
        \For {$j \in \{1,\dots,m\}$ \textbf{and} $i \in \{1,\dots,N$\}}
            \State $s_{ij}.A_k \gets $ the realized value of $t_i.A_k$ in scenario $j$
        \EndFor
        \For {$i \in \{1,...,N\}$}
            \State $M_{ki} \gets \textsc{ApproximateCVaR}(p_k,s_{i1}.A_k,\dots,s_{im}.A_k)$
        \EndFor
        \For {$j \in \{1,\dots,m\}$}
            \State $X_j.A_k \gets \sum_{x_i \in P_0} s_{ij}.A_k x_i$ 
        \EndFor
        \State $l_k \gets \textsc{ApproximateCVaR}(p_k,X_{1}.A_k,\dots,X_{m}.A_k)$
        \State $r_k \gets v_k$
    \EndFor
    \State $M \gets (M_{ki})_{k\in\{1,\dots,K\},i\in\{1,\dots,N\}}$ \Comment{ {\color{gray}\textit{Constraint matrix $M$ to formulate ILP from linearized CVaRs}}}
    \While{exists $k$ such that $r_k-l_k>\delta$}\Comment{ {\color{gray}\textit{Bisection strategy}}}
        \For{$k \in \{1,\dots,K\}$}
            \If{$r_k-l_k > \delta$}
                \State $v'_k \gets (l_k+r_k)/2$
            \Else
                \State $v'_k \gets v_k$
            \EndIf
        \EndFor
        \State $I' \gets \textsc{FormulateILP}(Q[v'_1,\dots,v'_K], M)$
        \State $P' \gets \textsc{ILPSolver}(I')$
        \If{\textsc{IsFeasible}$(Q,P',\hat{m})$ \textbf{or} $P'=NULL$}
            \If{$P' \neq NULL$}
                \State{$P^* \gets P'$}
            \EndIf
            \For{each $k$ such that $r_k-l_k > \delta$}
                \State $r_k \gets v'_k$
            \EndFor 
        \Else
            \For{each $k$ such that $r_k-l_k > \delta$}
                \State $l_k \gets v'_k$
            \EndFor 
        \EndIf
    \EndWhile
    \If{\textsc{Is\_$\epsilon$\_Optimal}$(Q,P^*,\epsilon)$}
        \State \Return $P^*$
    \Else
        \State $m \gets \min(2m,\hat{m})$
    \EndIf
\EndWhile
\State \Return $\text{NULL}$ \Comment{ {\color{gray}\textit{No solution is found}}}
\end{algorithmic}
\end{algorithm}

% \azza{This block of pseudocode is not elegant. It needs to be abstracted into sub-functions, so that we can easily grasp the whole and dive into the parts. Also what IsAccurate?! Feasibility is something we get intuitively and so we don't need code for it, but what isAccurate.}

% \azza{I kept getting tripped by is feasible, in the sense that a non-null package output from ILPSolver must mean it is feasible! But hidden in the notation is the fact that you are solving with $m$ scenarios and testing feasibility with $\hat{m}$ scenarios. This is extremely subtle. Also bothersome is that you use $\hat{m}$ to indicate number of validation scenarios but also max number of optimization scenarios. I'd rather you just have different variables that are different and call one the number of validation scenarios, not max number of optimization scenarios. Your current number of optimization scenarios can just grow to the number of validation scenarios.}

% \azza{Certain things are also not evident at all to a typical DB reader. What is a constrain matrix? why build one? It is an implementation artifact ...}

We parameterize a given SPQ $Q$ with $K$ stochastic constraints, each having their bound values, $v_1,\dots,v_K$, as $Q[v_1,\dots,v_K]$. Our proposed approach, \cvarif, described in Algorithm \ref{alg:cvarification}, finds a near-optimal package in response to such a query using a sequence of ILPs, by modifying the values of $\{v_1, \dots, v_k\}$ in each iteration. The ILPs $I'$ are formulated in line~23 from SPQ where each bound $v_k$ is modified to $v'_k$ for all $k \in \{1,\dots,K\}$. To formulate an ILP of $Q[v'_1,\dots,v'_K]$ using linearized CVaRs as above, we need to compute the so-called ``constraint matrix'' $M$ (line~16) which contains CVaR coefficients $CVaR_{p_k}(t_i.A_k)$ of each stochastic constraint $k$ and each tuple $i$. Intuitively, the matrix $M$ is a compact representation of the LHS of the ILP's constraints where the row dimension is the number of constraints and the column dimension is the number of tuples. In addition, the values $v'_1,\dots,v'_K$ are the RHS of the ILP's constraints. We compute each entry $M_{ki}$ (line~11) by approximating $CVaR_{p_k}(t_i.A_k)$ using $m$ scenarios. \textbf{Algorithm~\ref{alg:approx}} computes this approximation given a probability value $p$ and the values of $t_i.A_k$ across $m$ scenarios by calculating the average of the lowest $\lfloor pm\rfloor$ values. Once the constraint matrix $M$ is approximated, \cvarif uses bisection (line~17) to find the optimal value of $v'_k$ for each stochastic constraint $k$ such that the package $P^*$ found in the ILP of $Q[v'_1,\dots,v'_K]$ (line~23) is feasible w.r.t $Q$ (line~25) and $(1+\epsilon)$-approximate (line~33). 
% \azza{This entire para is difficult to understand or parse. Perhaps start by why a feasible package at line 4 is a good solution. Then if it isn't, how does the bisection proceeds. The more I dwell on this, the more I think it is crucial to spell out the FormulateILP because you pack in it how you deal with 0 scenarios and many sceanrios codified via a constraint matrix, and so on.} \azza{Putting this here as a reminder. In our last meeting, we asked for an example that illustrates how the ILPs are formulated and how the constraint matrix is generated, used, etc. Putting it back on your radar.}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \input{tables/stock_saa}
        \caption{The `Stock\_Investments' Table after Sample-Average-Approximation}
        \label{subfig:stock_investments_saa}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \input{queries/example_spaql_after_cvar}
        \caption{A \spaql Query after converting VaRs to CVaRs}
        \label{subfig:example_spaql_after_cvar}  
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \input{tables/ilp_system}
        \caption{An example ILP formulated using linearized CVaRs}
        \label{subfig:example_ilp}
    \end{subfigure}
\caption{Formulating ILPs using linearized CVaRs}
\label{fig:formulating_ilps}
\end{figure*}

To verify the feasibility of $P'$~(line~25), we generate $\hat{m}$ scenarios on the fly to validate it. Validating if a given package satisfies a constraint based on these validation scenarios is straightforward. For example, to validate if a package satisfies a VaR constraint $F_{A}(v) \leq p$, we compute the percentage of the validation scenarios $j$ for which $\sum_{i=1}^N s_{ij}.A\,x_i \leq v$, and compare this percentage with $p$. Notice that we only need to generate scenario values for tuples that are included in $P'$, so validation takes little time, since the generated packages typically contain much fewer tuples than the relation size. 

In line~33, we determine if a generated package $P^*$ is near-optimal, or $(1+\epsilon)$-approximate. This is assuming the objective requires minimizing the sum of a stochastic attribute. To determine if the objective value of $P^*$ is at most $(1+\epsilon)$ times of that of the optimal solution, we assert that $\omega^*/\omega_0 \leq 1+\epsilon$ where $\omega_0$ is the objective value of the risk-unconstrained package $P_0$ obtained in line~3 and $\omega^*$ is the objective value of $P^*$. $P_0$ is generated by removing all risk constraints from a query. Since a risk-unconstrained solution is guaranteed to be more optimal than any package that satisfies the risk constraints, $w_0$ is guaranteed to be a lower bound on the objective value $\overline{\omega}$ of the optimal package $\overline{P}$. That is, $\omega_{0} \leq \overline{\omega}$, which implies $\omega^*/\overline{\omega} \leq \omega^*/\omega_0$. Hence, ensuring $\omega^*/\omega_0 \leq 1+\epsilon$ ensures $\omega^*/\overline{\omega} \leq 1+\epsilon$  or $\omega^{*} \leq (1+\epsilon)  \overline{\omega}$.  Note that, $\omega_{0}$ can be any lower bound of the optimal objective value $\overline{\omega}$.  While we describe the objective value of the risk unconstrained package as our lower bound here, alternative methods of finding this lower bound have been explored in~\cite{BrucatoYAHM20}. When multiple lower bounds can be found using these methods, we use the maximum among them as the value of $\omega_0$. Modifying this method for queries that require maximizing the objective value is straightforward.

Bisecting for the optimal bound value $v'_k$ requires identifying an initial search interval $(l_k,r_k]$ for each stochastic constraint $k$. We compute this interval by setting the right endpoint $r_k$ as the original bound value $v_k$ (line~15) since we know that if $P^*$ satisfies the ILP of $Q[v_1,\dots,v_K]$ then it also satisfies each of the original VaR constraints in $Q$ by Theorem~\ref{theorem:var} and \ref{theorem:cvar}. For the left endpoint $l_k$, we simply require that the solution of the ILP of $Q[l_1,\dots,l_K]$ does not satisfy $Q$. One way to find this is to compute the solution $P_0$ of the ILP of $Q[-\infty,\dots,-\infty]$ (lines~2,3) which is a deterministic package query since we remove all the stochastic constraints by setting their bounds $v_k$ to $-\infty$. If $P_0$ is feasible w.r.t $Q$ or $P_0$ cannot be found (line~4), then either $P_0$ is the optimal solution or there is no solution. In either case, we can return the result as it is. When $P_0$ cannot be found only because the ILP is unbounded, i.e., the ILP has solutions but the solutions can be improved indefinitely without violating any constraints, we simply find the extreme ray at which the solution is unbounded and use it as the replacement for our $P_0$. Otherwise, using $P_0$, we can compute the realized values $X_j.A_k$ of each attribute $A_k$ in each scenario $j$ (line~13) and approximate its CVaR coefficient which is set to $l_k$ (line~14). 

The bisection continues as long as there exists an interval $(l_k,r_k]$ of length greater than an arbitrarily small real-value $\delta$ (line~17). We only do bisection on such intervals (line~20) and keep the original bound value for other intervals (line~22). If the bisected solution $P'$ from the ILP of $Q[v'_1,\dots,v'_K]$ is feasible w.r.t $Q$ or is not found (line~25) then the right endpoints are set to the midpoint (lines~29) to expand the feasible region of the linearized CVaRs which allows us to either find a better feasible solution or to find a solution at all. On the other hand, the left endpoints are set to the midpoint (lines~32) to shrink the feasible region of the linearized CVaRs to find a solution that is within the feasible region of $Q$. By the end of bisection, if the feasible solution $P^*$ exists and is $(1+\epsilon)$-approximate then it is the optimal solution. Otherwise, we keep doubling the number of optimization scenarios (line~36) until we find $P^*$ or declare that no solution is found if a maximal number of optimization scenarios (e.g. a million) had already been used (line~37).

\cvarif (as detailed in Algorithm~\ref{alg:cvarification}) uses the approximation error bound $\epsilon$ to determine if a generated package is near optimal. Therefore, setting lower values of $\epsilon$ gives near-optimal results in exchange for higher runtimes. Experts can take into account the trade-off between performance and optimality, and can use the indifference-zone formulation to rank and select values of $\epsilon$ \cite{Indif}.

\cvarif provides scalability across the scenario dimension. Its ILP formulations have constraint matrices of size $\mathcal{O}(K \times N)$ which is independent of the number of scenarios ($N$ is the number of tuples and $K$ is the number of constraints). However, when the number of tuples scales beyond hundreds of thousands, solving the ILP becomes a bottleneck given the exponential time complexity of ILP solvers with respect to the number of decision variables. 

\section{\sskr}\label{section:sskr}


\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-1.jpg}
        \caption{Tuples as points}
        \label{fig:tuple_to_point_vis_hlf}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-2.jpg}
        \caption{Partition tuples}
        \label{fig:partition_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-3.jpg}
        \caption{Select Representatives}
        \label{fig:representative_election_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    %\hfill
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-4.jpg}
        \caption{Form Duplicates}
        \label{fig:representative_duplication_hlf}
    \end{subfigure}\\
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-5.jpg}
        \caption{Sketch: Generate Packages from duplicates}
        \label{fig:sketch_query_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    %\hfill
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-6.jpg}
        \caption{Refine: Replace duplicates with actual tuples}
        \label{fig:first_refinement_hlf}
    \end{subfigure}
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-7.jpg}
        \caption{Second Refinement}
        \label{fig:second_refinement_hlf}
    \end{subfigure}
    %\hfill
    \hspace{0.8cm}
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale = 0.2]{figures/Stochastic SketchRefine Workflow-8 (1).jpg}
        \caption{Final Refinement}
        \label{fig:third_refinement_hlf}
    \end{subfigure}
    \caption{High Level Workflow of \sskr}
    \label{fig:stochastic-sketchrefine-hlf}
\end{figure*}

For processing SPQs on large relations, we propose \sskr (Figure~\ref{fig:stochastic-sketchrefine-hlf}). It partitions the data offline into groups of similar tuples (Figure~\ref{fig:partition_hlf}) using \dpart, a novel stochastic partitioning scheme (detailed in Section~\ref{sec:dpart}) that ensures (i) tuples in the same partition are similar with respect to each attribute, and (ii) no partition contains too many tuples. It then selects a representative tuple from each partition (Figure~\ref{fig:representative_election_hlf}). Representative tuples are imaginary tuples whose deterministic attributes are the average of that attribute's values among all the tuples in the partition. Their stochastic attributes each correspond to that of one of the tuples in the partition. Section~\ref{subsec:rep_selection} details the criteria for selecting the corresponding tuple for the stochastic attributes.

Given an SPQ, \sskr first executes a `Sketch' query, solving the query on the combined set of all representatives. The resulting sketch package indicates the number of tuples to be included in the final package from each partition. In deterministic settings, having one decision variable per representative suffices. If a package contains $q$ tuples (each with a multiplicity of 1) from the same partition, its `sketched' version assigns the multiplicity $q$ to the variable corresponding to the representative.

However, under uncertainty, this increases the risks of sketched packages. Suppose, an optimal package has two tuples $t_1$ and $t_2$ from the same partition, whose random variables for a stochastic attribute $A$ have Bernoulli distributions $B(0.5)$. For the package $\{t_1, t_2\}$, the probability of the sum of $A$ being $0$ is 0.25. Yet, if they are represented by  a single tuple $t$ having the same bernoulli distribution, the sketched version of $\{t_1, t_2\}$ would have selected $t$ twice, increasing the probability of the sum of $A$ being $0$ to 0.50. If the SPQ has a VaR constraint limiting the probability of the sum of $A$ being $0$ to 0.30, the sketched version of the optimal package would become infeasible. During Sketch, the solver would be forced to explore alternative options, leading to no package being found or suboptimal packages being generated.

\sskr thus creates stochastically identical duplicates of each representative (Figure \ref{fig:representative_duplication_hlf}). Sketch solves the SPQ over all the duplicates using \cvarif, with the ILP having a decision variable for each duplicate, and assigns a multiplicity to each duplicate (Figure \ref{fig:sketch_query_hlf}). Determining the appropriate number of duplicates for each representative involves a runtime-quality trade-off. The higher the number of duplicates, the better the chances of the sketched version of the optimal package being feasible. With enough duplicates, each tuple in the optimal package can map to a different  duplicate. However, this also means more decision variables in the sketch ILP, i.e., higher runtimes. Fortunately, the number of duplicates needed for any representative is upper bounded by the number of distinct tuples in the optimal package, which is typically much smaller than the number of tuples in a partition. Section \ref{subsec:sketch} discusses Sketch in further detail, including how it determines the appropriate number of duplicates.

Afterwards, each partition whose representatives are included in the sketch package are successively refined by replacing the duplicates with tuples from their own partition (Figures~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}). During each refinement, \cvarif solves the SPQ on all tuples in the partition, the tuples included in the package from previous refinements, and the yet unrefined duplicates of representatives from the sketch package (details in Section~\ref{subsec:refine}). Since no partition consists of too many tuples and the number of distinct tuples in the sketch and refined packages are limited, each refinement can be completed quickly. Once all the refinements are done, all duplicates are replaced by actual tuples, and the final package is obtained.
%Doing the same in \sskr but this would cause the Sketch package to be risk-averse and sub-optimal. To see why, consider a package of two independent Bernoulli random variables $B(0.5)$ and a package that contains the same Bernoulli random variable $B(0.5)$ twice. The former would have a lower probability of getting 0 i.e. $25\%$ chance while the latter would have 50\% chance.\riddho{I feel that this example may not quite work since it might not connect why taking a package with a lower risk is bad, and how this specifically causes issues during sketch seems somewhat ambiguous} Hence, in this case, if we apply the same logic as in \skr, the Sketch query is forced to produce a sketched solution that would inherently risk-averse since multiplying the same random variable would make it riskier than choosing multiple i.i.d. random variables. To overcome this, \sskr uses a novel technique called ``tuple duplication'' (detailed in Section~\ref{subsec:tuple_dup}) to diversify the sketch solution. At a high level, we form stochastically identical duplicates of each representative, as in Figure~\ref{fig:representative_duplication_hlf}. The sketch query runs \cvarif to solve the query over all the duplicates of each representative. As illustrated by Figure~\ref{fig:sketch_query_hlf}, the sketch package will contain only a subset of these duplicates from some of the partitions. Deciding on the number of duplicates for each partition involves a trade-off, since the higher the number of duplicates, the better is the sketch solver's ability to avoid overconstrained sketch packages, but a higher number of decision variables in the sketch problem also means that the solver requires more time to obtain the sketch solution. Details on deciding the appropriate number of duplicates for each representative are provided in Section~\ref{subsec:sketch}. Each partition whose representative's duplicates are included in the sketch package are then successively refined, by replacing them with tuples from their own partition (Figures~\ref{fig:first_refinement_hlf},~\ref{fig:second_refinement_hlf},~\ref{fig:third_refinement_hlf}). To perform each refinement, we use \cvarif to solve the query on all tuples in the partition, the tuples included in the package from previous refinements, and the duplicates of representatives from the yet unrefined partitions of the sketch package (details in Section~\ref{subsec:refine}). Since no partition consists of too many tuples and the number of distinct tuples in the sketch and refined packages are limited, each refinement can be completed quickly. Once all the refinements are done, all duplicates are replaced by actual tuples, and the final package is obtained.
\subsection{The Sketch Phase} \label{subsec:sketch}

Sketch (Algorithm~\ref{alg:sketch}) processes a given SPQ $Q$ on the representatives $R$. Like \cvarif, it starts by solving $Q_0$, the version of $Q$ that excludes all the probabilistic constraints (line~1). If $Q_0$ is unsolvable, so is $Q$, since $Q$ has all the constraints that $Q_0$ has and more, so we return a null package (lines~2-3). Otherwise, we solve the ILP for $Q_0$ to get the probabilistically unconstrained optimal package $P_0$ (line~4). We check if $P_0$ satisfies the risk constraints of $Q$ based on $\hat{m}$ validation scenarios, and if so, return it (lines~5-6).

\begin{algorithm}[t]
\caption{\textsc{Sketch}}\label{alg:sketch}
\begin{algorithmic}[1]
\Require $Q:=$ A Stochastic Package Query
\Statex $R :=$ A set of representative tuples
\Statex $\tau :=$ Maximum tuples in a partition
\Statex $\Delta\alpha :=$ Change in relative risk tolerance 
\Statex $m :=$ Initial number of optimization scenarios
\Statex $\hat{m} :=$ Max. number of scenarios
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\Statex $\epsilon :=$ Error approximation bound
\Statex $\delta :=$ Bisection termination distance

\State $Q_0 \gets $\textsc{RemoveProbabilisticConstraints}(Q)
\If{\textsc{IsUnsolvable}($Q_0$)}
\State \Return NULL
\EndIf
\State $P_0 \gets $ \textsc{ILPSolver}($Q_0$)
\If{\textsc{IsFeasible}($Q$, $P_0$, $\hat{m}$)}
\State \Return $P_0$
\EndIf
\State $\alpha \gets$ \textsc{InitialRiskTolerance($\tau$)}
\While{$m \leq \hat{m}$}
      \State scenarios$ \gets \emptyset$ 
      \For{$r \in R$}
       \State $d \gets $\textsc{NumberOfDuplicates($r, Q, \alpha, m, P_{max}$)}
        \For{$a \in $ \textsc{StochasticAttributes(Q)}}
        \For{$i \in [1, \dots, m]$}
        \State $values$ $\gets$ \textsc{CreateScenario}($r, a, d$)
        \State scenarios$_i \gets $ scenarios$_i \cup values$
        \EndFor
        \EndFor
      \EndFor
      \State $P \gets $\textsc{CVaRification}($Q$, scenarios, $\hat{m}$, $\epsilon$, $\delta$)
      \If{\textsc{Is\_$\epsilon$\_Optimal}($Q, P, \epsilon$) \textbf{and} \textsc{IsFeasible}($Q, P, \hat{m}$)}
      \State \Return $P$
      \Else
      \If{$\alpha > 0.0$}
      \State
      $\alpha \gets \max(\alpha - \Delta\alpha, 0.0)$
      \Else
      \State $m \gets min(2m, \hat{m})$
      \EndIf
      \EndIf
\EndWhile
\State \Return \textsc{NULL}
\end{algorithmic}
\end{algorithm}

Otherwise, we use optimization scenarios for each constraint to create packages that satisfy the probabilistic constraints in $Q$. Sketch starts with a relatively small number ($m$, e.g. 100) of optimization scenarios, and doubles their number (line~23) until a validation feasible and $(1 \pm \epsilon)$-approximate package is found (lines~15-16). If no valid package is generated even after using a maximal number ($\hat{m}$, e.g. $10^6$) of optimization scenarios, we return null (line~24).

When creating an appropriate ILP formulation for $Q$, sketch creates duplicates of each representative. The number of duplicates created can vary by representative. To determine the number of duplicates to create, sketch requires $P_{max}$, an upper bound on the number of distinct tuples in a package. This can often be specified in the query itself, by a package size constraint like ``COUNT(*) $\leq$ $P_{max}$''. Alternatively, $P_{max}$ can be derived from deterministic constraints. For instance, if $Q$ has a constraint like ``SUM(A) $\leq$ V'', we can sort all the tuples in ascending order of their values of A and check how many distinct tuples we can include from the beginning until the sum of $A$ exceeds V. $P_{max}$ can also be set based on intuition and domain knowledge, since users may have an estimate of how many tuples they expect to see at most in the generated packages. 

If Sketch creates $P_{max}$ duplicates for every representative, all tuples in the optimal package can be mapped to a distinct representative, even if all $P_{max}$ tuples in the optimal package originate from the same partition. If all tuples are sufficiently similar to the representative, sketched versions of the optimal package would be validation feasible. However, since each duplicate has a corresponding decision variable, this can increase solver runtimes. 

We use $\alpha$, a risk tolerance ratio, to determine an acceptable number of duplicates. If $d<P_{max}$  is the chosen number of duplicates for a representative, the risk of sketched packages can be amplified if all $P_{max}$ tuples in the optimal package are from the representative's partitition.  The sketched version of the package will contain all $d$ duplicates, each having an average multiplicity of $P_{max}/d$. For each risk constraint in $Q$, the VaR/CVaR of this package will be lower than that of the package formed if $P_{max}$ duplicates were used, in which case the sketched version would have each duplicate exactly once. Sketch calculates the relative change in the VaRs/CVaRs between the two packages, and selects the smallest $d$ for which the relative change goes below $\alpha$ for every risk constraint in the query (Details in Section~\ref{subsec:num_dup}).

Sketch initially sets $\alpha$ so as to ensure the total number of duplicates is within a tolerable range for an off-the-shelf solver to solve the ILP in a reasonable amount of time. The number of tolerable decision variables can vary due to underlying hardware attributes of the system, differences in the solver software, runtime versus quality requirements, etc. Recall our partitioning scheme ensures that none of the resulting partitions contain too many tuples. Specifically, no partition contains more than $\tau$ tuples, a size threshold defined by a database administrator. During Refine, the solver solves an ILP that contains all tuples in a partition. Thus, $\tau$ is set so that having $\tau$ decision variables in the ILP does not stress out the solver. Sketch also utilizes this threshold. It sets the initial value of $\alpha$ so that the total number of duplicates across all the representatives does not exceed $\tau$ (line~7) (Details in Section~\ref{subsec:initial_alpha}).

During each iteration, Sketch first calculates the number of duplicates for each representative based on $P_{max}$ and $\alpha$ (lines~10-11). For each stochastic attribute addressed by a constraint or objective in $Q$, it creates $m$ scenarios from these duplicates (lines~12-15). Each scenario consists of a real value for each duplicate of every representative. Details on how these scenarios are constructed are described in Section~\ref{subsec:scenario_gen}.

Once all the scenarios are generated, we use \cvarif to obtain a package $P$ (line~16). Notice the slightly different parameterization as opposed to the \cvarif approach described in Algorithm~\ref{alg:cvarification}. Sketch uses a slightly modified version of the approach. Its \cvarif uses only the given optimization scenarios, running bisections to find the closest linearized CVaR constraint for each risk constraint. It uses $\hat{m}$ validation scenarios to validate the feasibility and optimality of the intermediate packages. However, if the package obtained in the end is not validation feasible or $(1\pm\epsilon)$-optimal, it simply returns the package it found to the Sketch function, instead of attempting to increase the number of optimization scenarios and retry, as was proposed in Algorithm~\ref{alg:cvarification}.

Upon receiving a package $P$, Sketch checks to see if it is $(1 \pm \epsilon)$-optimal and validation feasible (line~17), and returns $P$ if so (line~18). If not, it checks to see if $\alpha$ can be decreased further. Decreasing $\alpha$ results in more duplicates being produced, which can help produce better and more feasible packages. If $\alpha > 0$, we decrease it by $\Delta \alpha$ (lines~20-21), a user-defined hyperparameter that we in our experiments set to be $0.03$. If $\alpha = 0$, we double the number of optimization scenarios and reiterate (line~23).

\subsubsection{Determining the number of duplicates} \label{subsec:num_dup}

The number of duplicates needed by a representative can differ for each constraint. Thus, given a representative $r$ and a query $Q$, we iterate over all the risk constraints in $Q$, and select the maximum number of duplicates of $r$ needed by them (Algorithm~\ref{alg:num_dup}). 

\begin{algorithm}[h]
\caption{\textsc{NumberOfDuplicates}}\label{alg:num_dup}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $Q :=$ A Stochastic Package Query
\Statex $\alpha :=$ Relative risk tolerance
\Statex $m :=$ Number of scenarios
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\State $d \gets 1$
\For{Each risk constraint $c$ in $Q$}
    \If{\textsc{DuplicatesForConstraint}($r$, $c$, $\alpha$, $m$, $P_{max}$) > $d$}
        \State $d \gets $ \textsc{DuplicatesForConstraint}($r$, $c$, $\alpha$, $m$, $P_{max}$) 
    \EndIf
\EndFor
\State \Return $d$
\end{algorithmic}
\end{algorithm}

Duplication aims to ensure that each tuple in the optimal package has a one-to-one correspondence with a duplicate of the representative. When the number of duplicates of a representative $d$ is less than $P_{max}$, this is not ensured. If all $P_{max}$ tuples in the optimal package are from the representative's partition, the sketched version of the optimal package will have to map different tuples to the same duplicate. For any stochastic attribute, in the worst case scenarios for that duplicate, the losses will multiply. This will lead to lower CVaR and VaR values in the sketch package, and make the risk constraints harder to satisfy. 

If a representative has $d$ duplicates, the risk optimal sketched version of a package having $P_{max}$ tuples from the partition will have each of the duplicates included an average of $\frac{P_{max}}{d}$ times. $\frac{P_{max}}{d}$ may not be an integer, so some of the duplicates will have a multiplicity of $\lceil\frac{P_{max}}{d}\rceil$ while the rest are repeated $\lfloor\frac{P_{max}}{d}\rfloor$ times. We create $m$ scenarios from such a package, and find the VaR/CVaR of the package among the scenarios. We return the first value of $d$ for which the change in VaR/CVaR relative to that of the package that contains $P_{max}$ duplicates is less than $\alpha$ (lines 7-8 in Algorithm~\ref{alg:dup_count}). 

\begin{algorithm}[h]
\caption{\textsc{DuplicatesForConstraint}}\label{alg:dup_count}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $c :=$ A risk constraint
\Statex $\alpha :=$ Relative risk tolerance
\Statex $m :=$ Number of scenarios
\Statex $P_{max} :=$ Max. number of distinct tuples in a package
\State $S_{max} \gets \Phi$
\For{$i \in [1, \dots, m]$}
    \State $S_{max} \gets S_{max} \cup $ \textsc{CreateScenario}($r$, $c.a$, $P_{max}$)
\EndFor
\For{$d \in [1, \dots, P_{max}]$}
$S_d \gets \Phi$
\For{$i \in [1, \dots, m]$}
    \State $S_d \gets S_d \cup $ \textsc{CreateScenario}($r, c.a, d$)
\EndFor
\If{(\textsc{Risk}($S_{max}$) - \textsc{Risk}($S_{d}$))/|\textsc{Risk}($S_{max}$)| $\leq \alpha$}
\State \Return $d$
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

If the recommended number of duplicates by algorithm~$\ref{alg:dup_count}$ equals or exceeds the number of tuples in a partition, \sskr includes all the tuples from the partition directly during Sketch, instead of having a single representative for them. 


\subsubsection{Determining the initial risk tolerance ratio} \label{subsec:initial_alpha}

To determine an initial value of $\alpha$ that ensures that the total number of duplicates during Sketch in the first iteration is around the size threshold $\tau$, we conduct a bisection over the values of $\alpha$ from $[0, 1]$ (Algorithm~\ref{alg:init_alpha}). If the total number of decision variables is lower than $\tau$ even for $\alpha = 0$, we use $0$ as our initial $\alpha$ (lines 1-2). If the total number of duplicates is too high for $\alpha = 1$, we set $\alpha = 1$ as our initial value of $\alpha$ (lines~3-4). Otherwise, we conduct a bisection from $\alpha_l = 0$ (line~5) to $\alpha_h = 1$ (line~6) that continues until the total number of duplicates used is the same for any value of $\alpha$ within $[\alpha_l, \alpha_h]$ (line~7). During each iteration of the bisection, we check the total number of duplicates produced by setting $\alpha_m = \frac{\alpha_h + \alpha_l}{2}$ using Algorithm~\ref{alg:num_dup}. If the number of duplicates is over $\tau$, we reduce our search interval to $[\alpha_l, \alpha_m]$ (lines~9-10). If the total number of duplicates is below $\tau$, we reduce the search interval to $[\alpha_m, \alpha_h]$. If $\alpha_m$ produces exactly $\tau$ duplicates, we return it immediately and use it as our initial $\alpha$.

\begin{algorithm}[t]
\caption{\textsc{InitialRiskTolerance}}\label{alg:init_alpha}
\begin{algorithmic}[1]
\Require $\tau :=$ Maximum tuples in a partition

\If{\textsc{TotalDuplicates}(0.0) $\leq$ $\tau$}
\State \Return $1.0$
\EndIf
\If{\textsc{TotalDuplicates}(1.0) $\geq$ $\tau$}
\State \Return $0.0$
\EndIf
\State $\alpha_h$ $\gets$ $1.0$
\State $\alpha_l$ $\gets$ $0.0$
\While{\textsc{TotalDuplicates}($\alpha_h$) $>$ \textsc{TotalDuplicates}( $\alpha_l$)}
\State $\alpha_m$ $\gets$ ($\alpha_h$ + $\alpha_l$)/2
\If{\textsc{TotalDuplicates}($\alpha_m$) $> \tau$}
\State $\alpha_h$ $\gets$ $\alpha_m$
\EndIf
\If{\textsc{TotalDuplicates}($\alpha_m$) $< \tau$}
\State $\alpha_l$ $\gets$ $\alpha_m$
\EndIf
\If{\textsc{TotalDuplicates}($\alpha_m$) $= \tau$}
\State \Return $\alpha_m$
\EndIf
\EndWhile
\State \Return $\alpha_l$
\end{algorithmic}
\end{algorithm}

In theory, $\alpha$ may have to be over $1$ to produce around $\tau$ duplicates. In such cases, we still begin from $\alpha=1$, since setting $\alpha$ even higher will worsen the quality of packages produced, if any. We did not encounter this case during our experiments.

\subsubsection{Scenario Generation from Duplicates} \label{subsec:scenario_gen}

During sketch, an optimization scenario can be formed by independently sampling a value from each duplicate of every representative, with \cvarif creating sketch packages based on numerous such scenarios.

However, assuming mutual independence among duplicates ignores inter-tuple correlations within a partition. Positively correlated tuples tend to have lower values in the same scenarios. Thus packages containing positively correlated tuples incur increased losses in the worst-case scenarios and are inherently riskier. As such, constructing a sketch package while being oblivious to inter-tuples correlations within the partition can cause problems while refining the partitions. For instance, if all tuples in the partition are highly correlated with the representative, a sketch package that contains independent duplicates may underestimate the risks incurred by including multiple duplicates of the representative. No feasible solution may be found during refine, when the solver tries to replace independent duplicates with positively correlated tuples. 

Duplicates of each representative should thus be mutually correlated with one another to extents roughly mirroring the correlation between the representative and other tuples in the partition. We use the median of the pairwise Pearson's correlation coefficients between the representative and all other tuples in its partition as the correlation coefficient between each pair of duplicates. For an intuition on why we use the median of the correlation coefficients, note that by duplicating the representatives, we aim to provide a new one-to-one correspondence between duplicates in the sketch package and the tuples included in the package after refining the partition. Using the median ensures that there are as many tuples having a higher correlation with the representative than the duplicates as there are tuples having a lower correlation coefficient. Thus, if one of the duplicates is replaced by a tuple having a higher correlation coefficient than the median, thereby increasing risks compared to the sketch package, the solver will have the chance to balance it out by taking another similarly optimal tuple that has a lower correlation coefficient.

To generate scenarios from duplicates that are mutually correlated by a correlation coefficient $\overline{\rho}$, we propose an accelerated version of the NORTA (NORmal-To-Anything) copula method~\cite{ghosh2003behavior}. Given a set of random variables and their pairwise correlation coefficients, NORTA generates correlated samples from them. It converts values sampled from a multivariate standard normal distribution with a given correlation matrix, to corresponding values at equivalent cumulative densities for arbitrary random variables. Given $d$ correlated random variables $R_1, \dots, R_d$ and their $d \times d$ correlation matrix $\mathbb{\rho}$, where $\mathbb{\rho}_{ij}$ denotes the correlation coefficient between $R_i$ and $R_j$, NORTA first takes $d$ i.i.d. samples a standard normal distribution, forming a $d$-dimensional sample vector $s$. Then, to generate $d$ samples from a multivariate standard normal distribution defined by the correlation matrix $\mathbb{\rho}$, it finds the eigendecomposition of $\mathbb{\rho} = S \Lambda S^{-1}$. Prior literature~\cite{gentle2009computational} shows $s'=S \sqrt{\Lambda} s$ will then reflect a $d$-dimensional sample of the multivariate standard normal distribution with correlation matrix $\mathbb{\rho}$. NORTA then calculates a $d$-dimensional sample vector $s_r$ of the correlated random variables, where the $i$-th element of $s_{r}$, $s^{r}_{i} = F_{i}^{-1}(\Phi(s'))$, with $F_{i}$ denoting the CDF of the $i$-th random variable $R_{i}$, and $\Phi$ denoting the CDF of the standard normal distribution.

In \sskr, the random variables correspond to the stochastic attributes of each duplicate. Given $d$ duplicates for a single representative,  we construct a correlation matrix $\rho$ where $\rho_{ij} = \overline{\rho}$ when $i \neq j$ (typically the median correlation coefficient between a representatives and the tuples it represents), and $\rho_{ii}=1$ for $i,j \in \{1, \dots, d\}$ (Correlation coefficient of any duplicate with itself is 1). Using NORTA, we generate a sample value for each duplicate. An optimization scenario is constructed by appending all sample values of every duplicate of each representative.

\begin{algorithm}[t]
\caption{\textsc{CreateScenario}}\label{alg:scenario_construction}
\begin{algorithmic}[1]
\Require $r :=$ A representative tuple
\Statex $a :=$ A stochastic attribute
\Statex $d :=$ The number of duplicates
\Statex $\overline{\rho} :=$ Correlation coefficient between duplicates
\State $s_1, \dots, s_d \gets$ i.i.d. samples from $N(0, 1)$
\State $s'_1 \gets \sqrt{1 + (d-1) \overline{\rho}} s_1 - \sum_{i=2}^{d} \sqrt{1 - \overline{\rho}} s_i$
\For {$i \in \{2, \dots, m\}$}
    \State $s'_i \gets \sqrt{1 - \overline{\rho}} s_i - \sqrt{1 + (d-1) \overline{\rho}} s_1$
\EndFor
\State $F_r \gets$ CDF of $r.a$
\State $s_r = F_r^{-1}(\Phi(s'))$
\State \Return $s_r$

\end{algorithmic}
\end{algorithm}

Eigendecomposing $\mathbb{\rho}$ normally has a computational complexity of $\mathcal{O}(d^3)$. This makes constructing scenarios expensive as we need to perform this decomposition for every representative. Furthermore, the algorithm may iteratively increase the number of duplicates to get better packages, requiring the eigendecomposition to be repeated at each iteration. To remove this bottleneck, we exploit the fact $\rho$ is a matrix where all non-diagonal entries have the same value $\overline{\rho}$. A closed form of the eigenvalues and eigenvectors of this matrix can be trivially computed as $\lambda_1 = 1+(d-1)\overline{\rho}$ with the corresponding eigenvector $[1, 1, \dots, 1]$ and $\lambda_2 = 1-\overline{\rho}$ with $d-1$ corresponding eigenvectors $[-1, 1, 0, \dots, 0]$ $[-1, 0, 1, \dots, 0]$, $\dots$, $[-1, 0, \dots, 1, \dots, 0]$, $\dots$ $[-1, 0, \dots, 1]$. Thus, after generating $d$ independent samples from standard normal distributions, and getting the sample vector $s=[s_1, \dots, s_d]$, the sample vector of $d$ correlated multivariate normal distributions can be found in $\mathcal{O}(d)$ time using $s' = [s_1\sqrt{\lambda_1} - \sqrt{\lambda_2}\sum_{i=2}^{d}s_i, s_2\sqrt{\lambda_2} - s_1\sqrt{\lambda_1}, \dots, s_d\sqrt{\lambda_2} - s_1\sqrt{\lambda_1}]$.

Since all the duplicates of a representative $r$ are stochastically identical, they have the same cdf $F_r$. A scenario can be generated by appending $s_{r} = F_{r}^{-1}(\Phi(s'))$ for every representative $r$. $F_r$ can be precomputed offline from histogram density estimations computed from independent samples~\cite{chan2014near}. Algorithm \ref{alg:scenario_construction} describes our linear time NORTA copula based scenario construction scheme.





\subsection{The Refine Phase} \label{subsec:refine}

Refine iteratively replaces each representative selected in the Sketch Package with tuples from their own partition. In each step, we replace all the selected duplicates from exactly one of the partitions, while preserving the selected duplicates from the yet unrefined partitions and the tuples selected during previous refinements. 

Refine uses the same number of optimization scenarios that were used to derive the Sketch package, and keeps the number of optimization scenarios fixed throughout its execution. The intuition behind keeping the number of scenarios fixed is that if $m$ optimization scenarios were enough to create feasible and near-optimal packages from the duplicates of each partition, they should suffice for doing the same from the actual tuples, since each tuple should be similar enough to their representatives.

Refine needs to find an order in which to refine the partitions included in the sketch package, so that a feasible and near-optimal final package is found. Using an `incorrect' order can lead to failure to find any feasible package. This happens when the ILP used to refine a particular partition does not return a valid package. To find this correct order, we use `Greedy Backtracking', a technique also used in the deterministic \skr algorithm~\cite{brucato2018package}. Intuitively, we backtrack over all possible permutations in which the partitions in the sketch package can be refined until a sequence of refinements results in a feasible and $(1\pm\epsilon)$-approximate package. We begin with a randomly selected permutation of partitions. If any intermediate refinement fails to find a valid package, we `undo' the previous refinement and greedily attempt to refine the failing partition in its place. We keep undoing the previous refinements until the partition can be successfully refined. If a partition cannot be refined even when no other partitions were refined before it, it indicates that the stochastic behaviour of the tuples in it do not coincide sufficiently well with that of the duplicates of the representative. This can happen if the correlations among the duplicates was insufficient, as explained in Section~\ref{subsec:scenario_gen}. In such cases, we increase the correlation coefficient among the duplicates of all such partitions by a tunable extent of 0.1, re-execute the sketch query, and refine the newly obtained sketch package. Greedy backtracking continues to explore different orders in which the partitions may be refined until an acceptable final package is found.

Each refinement involves a partition whose duplicates have a total multiplicity of over $0$ in the sketch package, and solves an ILP. Each refine ILP consists of a decision variable corresponding to each tuple in the partition being refined, one for every duplicate of every partition that were included in the sketch package but have not been refined yet, and one decision variable for every tuple included in the refined package from previous refinements. The constraints of the ILP include all constraints in the query (including the CVaRified VaR constraints), as well as additional constraints that ensure the multiplicities of the tuples obtained from previous refinements and those of duplicates of the yet unrefined representatives remain unchanged. The ILP solver thus needs to find an optimal assignment for decision variables of the tuples in the partition while keeping the multiplicities of all other tuples in the package unchanged. By successfully completing each refinement, duplicates in the sketch package are thus substituted by actual tuples from their partition.    




% \section{CVaR Constraints are all you need} \label{sec:cvarification_details}

% Deterministic constraints, and expected sums in constraints and objectives in SPQs can be represented via linear expressions in ILPs. However, solving SPQs becomes challenging due to risk constraints. \textit{SPaQL} expresses risk constraints via Value-at-Risk (VaR) constraints, whose ILP representations require one indicator variable per optimization scenario. \ssearch improves this by grouping scenarios into summaries and using one indicator variable per summary instead. It increments the number of summaries until an `optimal enough' package is found, while keeping the number of optimization scenarios unchanged. This can be slow when the initial number of optimization scenarios is insufficient, which becomes increasingly likely with higher variances.

% \begin{sloppypar} 
% \textbf{CVaR constraints are linearly representable.} We show that had risk constraints been expressed as Conditional Value-at-Risk (CVaR) constraints instead, they could be represented in ILPs as linear constraints. Consider a CVaR constraint \mintinline{sql}{EXPECTED SUM(A) >= V IN LOWEST T% OF SCENARIOS}, where $A$ is an attribute, $V$ is a real number and $T \in [0, 100]$. We modify the optimization scenarios\footnote{Any package created using modified optimization scenarios can be verified for constraint satisfaction and optimality over the unchanged validation scenarios}, and create `pseudo-scenarios' by sorting scenario values of each tuple in ascending order (Fig. \ref{fig:pseudoscenario-construction}). 
% \end{sloppypar}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.25]{figures/CreatingPseudoScenarios.jpg}
%     \caption{Creating pseudo-scenarios}
%     \label{fig:pseudoscenario-construction}
% \end{figure}

% Observe that the first pseudo-scenario is \textit{at least as bad} as any optimization scenario, i.e. each of its tuples has values that are not greater than their corresponding value in any of the original scenarios. A package $\{x_1, x_2, x_3, ..., x_n\}$ which satisfies the condition $\sum_{j=1}^{n}P_{1j}x_j \geq V$, where $P_{1j}$ represents the value of the $j$-th tuple in the first pseudo-scenario thus also satisfies $\sum_{j=1}^{n}S_{ij}x_j \geq V$ for any scenario $i$, where $S_{ij}$ represents the $j$-th tuple's scenario value, since $S_{ij} \geq P_{1j}$ and $x_j \geq 0$ implies $P_{1j}x_j \leq S_{ij}x_j$ for all $1 \leq j \leq n$.

% In theorem \ref{theorem:conservative_pseudoscenarios}, we generalize this to the first $m$ pseudo-scenarios. If any package has an expected sum of at least $V$ in the first $m'$ pseudo-scenarios, they are guaranteed to have an expected sum of at least $V$ over \emph{any} $m'$ scenarios. Formally, if $L$ is a set of $m'$ scenarios, where $S_{lj}$ represents the value of the $j$-th tuple in scenario $S_{l} \in L$,  

% \begin{equation}
%   \frac{1}{m'}\sum_{i=1}^{m'}\sum_{j=1}^{n}P_{ij}x_{j} \geq V \implies \frac{1}{m'}\sum_{S_{l} \in L} S_{lj}x_{j} \geq V
%   \label{eq:cvar_representation}
% \end{equation}

% For $m' = \frac{T}{100}m$, $m$ being the number of optimization scenarios and $T$ the percentage of scenarios addressed in the CVaR constraint, adding the linear constraint $\frac{1}{m'}\sum_{i=1}^{m'}\sum_{j=1}^{n}P_{ij}x_{j} \geq V$ in the ILP will ensure that the generated package has an expected sum exceeding $V$ over any $m'$ scenarios, and by extension, over the $m'$ scenarios having the lowest sums for the package. Had risks been represented using CVaR constraints, they could be represented in ILPs using such linear constraints, without needing indicator variables.

% \textbf{Converting VaR constraints} In \textit{SPaQL} however, all risk constraints are represented using VaR constraints of the form SUM(A) >= V WITH PROBABILITY>=P. We observe that any package satisfying the CVaR constraint EXPECTED SUM(A)>=V IN LOWEST (1-P)*100\% OF SCENARIOS, will also satisfy the VaR constraint.

% To explain why, suppose $scenario\_score$ refers to the sum of a package $x=\{x_1, ..., x_n\}$ in a scenario $S_i$, i.e. $\sum_{j=1}^{n} S_{ij}x_j$. Any package satisfying the latter CVaR constraint will have an average score of at least $V$ in the (1-P)-fraction of scenarios having the lowest scenario scores, implying the scenario score of at least one of these scenarios must be at least V. All other `better' scenarios must then also have scores of at least $V$. Thus, the package will have a sum of at least $V$ in at least $P$-fraction of the remaining scenarios and the VaR constraint will be satisfied.

% \begin{sloppypar}
%     This provides a method for linearly representing VaR constraints. First, convert the VaR constraint to a CVaR constraint, then create pseudo-scenarios from the optimization scenarios. Using the antecedent of implication~(\ref{eq:cvar_representation}), we generate an ILP whose resulting package satisfies the CVaR constraint, and thus, the original VaR constraint. Disadvantageously, this can overconstrain the ILP, making it unsolvable or have suboptimal solutions. We can, however, account for this by \textit{relaxing} the CVaR constraint. We model a VaR constraint of the form \mintinline{sql}{SUM(A)>=V WITH PROBABILITY P} to a CVaR constraint \mintinline{sql}{EXPECTED SUM(A)>=V' IN LOWEST (1-P)*100% OF SCENARIOS}, where $V' \leq V$. This must be controlled --- if $V'$ is too small, the resulting package may not satisfy the original VaR constraint.
% \end{sloppypar}

% \textbf{Closest Approximating CVaR constraint}: Finding an optimal $V'$ when approximating a VaR constraint by a CVaR constraint can be modeled as a search problem. Setting $V'=V$ results in a possibly overconstrained problem. Smaller values of $V'$ can potentially allow packages with better objective values, but the packages may violate the VaR constraint. Validation scenarios are particularly useful here. Once a package is generated with a CVaR constraint with value $V'$, we check its VaR among the validation scenarios. For instance, if the VaR constraint requires the sum of an attribute for the package to be at least $-10$ with probability $0.95$, and $V'=-20$ meaning the corresponding CVaR constraint will require the expected sum to be at least $-20$ in the lowest $5\%$ of scenarios, the scenario score of the generated package in the $5$-th percentile of validation scenarios is the package's VaR. If this satisfies the VaR constraint, the obtained package is feasible. Suppose for a \textit{low enough} value of $V'=V_{min}$, the generated package has an infeasible VaR. An optimal value of $V'$ can then be found using a bisection over the range $[V_{min}, V]$. From an interval $[V_l, V_u]$ (initially, $V_l=V_{min}$ and $V_u=V$) pick the mid-point, $V' = 0.5(V_{min} + V_{u})$. If this results in a feasible package, we set our new search range to $[V_l, V']$ in search of packages with better objective value. Else, we set the range to $[V', V_u]$ in search of feasible packages. The search terminates when $V_u - V_l \leq \delta$ for a small $\delta \geq 0$. This converges within $\log_2(\frac{V-V_{min}}{\delta})$ iterations.

% A key detail involves finding $V_{min}$ --- a value of $V'$ small enough to guarantee the corresponding VaR constraint is not satisfied when $V'=V_{min}$. Such a lower bound may not exist if the constraint is trivially satisfiable, that is, even without the constraint being imposed, the resulting optimal package has a VaR exceeding the threshold specified in the constraint. Such constraints can be removed from the query, and we do not need the aforementioned bisections for them. To detect if a VaR constraint is satisfied trivially or find $V_{min}$ otherwise, we remove all risk constraints from the query, and obtain the optimal package $P_0$ for this risk-unconstrained SPQ. If removing all risk constraints makes the problem unbounded, we replace the VaR constraints requiring the sum of an attribute $A$ in a package to be at least $V$,  with a typically much easier to satisfy expected value constraint requiring the expected sum of $A$ in the package to be at least $V$. VaR constraints satisfied by $P_0$ are trivial. For others, we use the VaR in the resulting package as the lower bound $V_{min}$.
% %We do this by picking an arbitrary positive number $d>0$, and experimenting to see if setting $V'=V-d$ causes the violation of the VaR constraint. If not, we then try the same with values $V-2d, V-4d, V-8d, ...$. i.e. doubling the difference in each iteration, until a valid lower bound is found. If a lower bound is first found in the $(m+1)$-th iteration, i.e. setting $V'=V-2^md$ causes constraint violation, while $V'=V-2^{m-1}d$ does not, we begin the succeeding bisection in the range $[V-2^md, V-2^{m-1}d]$. 

% Converting VaR constraints to their closest approximating CVaR constraint means each VaR constraint will have a single corresponding linear constraint in the query --- regardless of how many optimization scenarios are used. In terms of optimizer runtimes, this gives us unlimited scalability across the scenario dimension.

% \textbf{\cvarif} (Alg.~\ref{alg:cvarmethod_query_execution}) conducts a sequence of parallelly executed bisections to get the closest approximating CVaR constraint for each risk constraint in the query. It begins with a relatively small number (e.g. 100) of optimization scenarios, as generating too many optimization scenarios with values for every tuple would be time consuming. The algorithm runs an outer loop (Lines 1-21) where it creates a package with the selected number of optimization scenarios (Lines 2-15), returning the package if it is feasible and $(1\pm\epsilon)$-approximate (Lines 16-17).

% To find an optimal package, \cvarif first creates a set of optimization scenarios for each constraint and objective (Lines 2-4). If multiple constraints and the objective share the same attribute, their optimization scenarios can be shared, i.e. we do not need to generate distinct optimization scenarios for each of them. It then gets the optimal package $P_0$ produced in response to the risk unconstrained version of the SPQ using an in-memory ILP solver like Gurobi Optimizer. As mentioned earlier, the VaRs of $P_0$ over the validation scenarios for the risk constraints in $Q$ can be used as the lower bounds for the respective bisections of those risk constraints. Furthermore, the objective value of $P_0$ over the validation scenarios can be used as an upper bound for the objective value of the optimal package for $Q$, which can be used to determine if any package generated by \cvarif is $(1\pm \epsilon)$-approximate. Details on determining $(1\pm\epsilon)$-approximation is described in prior work~\cite{BrucatoYAHM20}.

% %We then find the lower bound for the bisections of each risk constraint (Line 6). In our experiments, we set $d$ to $100$, but we also observed that changing this value will not greatly impact latency since the range of the interval grows exponentially with each iteration. If $V-d$ is smaller than the CVaR of $P_0$ for any constraint, we simply use $P_0$'s CVaR value as the lower bound for the constraint's bisection. 

% \begin{algorithm}[tb]
% \caption{\textit{\cvarmethod{} Query Execution}}\label{alg:cvarmethod_query_execution}
% \begin{algorithmic}[1]

% \Require $Q$, Stochastic package query
% \Statex $m$, initial number of optimization scenarios (e.g. $100$)
% \Statex $\hat{m}$, number of validation scenarios (e.g. $10^6$)
% \Statex $\epsilon$, user-defined approximation error bound
% \While{True}
%   \For{every stochastic constraint and objective in $Q$}
%     \State Generate $m$ scenarios and their pseudo-scenarios
%   \EndFor
%   \State $P_0 \gets$ Package returned for the risk unconstrained SPQ
%   \State Get bounds for bisecting all non-trivial risk constraints
%   \While{All bisections are not complete}
%     \For{each risk constraint $C$}
%      \State $V'_{C} \gets$ Midpoint of search interval for $C$\
%     \EndFor
%     \State Create $ilp\_formulation$ with all values of $V'_C$
%     \State $p \gets SolveILP(ilp\_formulation)$
%     \State Validate $p$ among validation scenarios for all constraints
%     \State Update bounds for bisection
%   \EndWhile
%   \If{$p.is\_feasible(Q) \And p.is\_1\pm\epsilon\_approx(\epsilon)$}
%     \State \Return p %\Comment{{\color{gray} \textit{A feasible and ($1+\epsilon$)-approximate package is returned if found}}}
%   \Else
%     \State $m \gets \min(2m, \hat{m})$ %\Comment{{\color{gray}\textit{Double the number of optimization scenarios and try again}}}
%   %\Else
%   %  \If{not $p.is\_feasible(Q)$}
%   %    \State \Return "No package found"
%   %  \Else
%   %    \State \Return $p$
%   %  \EndIf
%   \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}


% Bisections are then run between the respective bounds of each constraint. At each iteration, for a VaR constraint $C$ requiring the sum of $A$ to exceed $V$ with at least probability $p$, if $[V_l, V_u]$ is the interval of possible CVaR values, we include the linear constraint $\sum_{i=1}^{(1-p)m} \sum_{j=1}^{n} P_{ij}x_{j} \geq (1-p)m*0.5(V_{l}+V_{u})$ into the ILP. Here, $P$ is the set of pseudo-scenarios. $(1-p)m$ represents the number of pseudo-scenarios considered ($(1-p)$-fraction of pseudo-scenarios are considered to correspond with the `IN THE LOWEST $(1-p)*100\%$ OF SCENARIOS' part of the  CVaR constraint) and $0.5*(V_{l}+V_{u})$ is the midpoint of the search interval. Note that, setting $m'=(1-p)m$ and $V=0.5(V_l+V_u)$ makes this linear constraint a simple algebraic manipulation of the antecedent of implication~(\ref{eq:cvar_representation}).

% %If using a limited number of optimization scenarios leads us to constructing a package that can be verified to be feasible among the validation scenarios (i.e. is validation feasible), \textit{and} whose objective value is guaranteed to be within $(1 \pm \epsilon)O_{opt}$, where $O_{opt}$ is the objective value of the optimal package (i.e. is $(1\pm\epsilon)$-approximate), the package is returned. For queries that require maximizing an objective value, the returned package will have an objective value of at least $(1 - \epsilon) O_{opt}$, while for minimization problems, the objective value will be capped at $(1+\epsilon) O_{opt}$. Detecting validation feasibility is trivial, while methods to determine if a package is $(1 \pm \epsilon)$-approximate have been proposed for \textit{SPaQL} in prior literature~\cite{BrucatoYAHM20}.

% Once linear constraints are included in the ILP for all risk constraints (lines 8-11), we use an in-memory solver to solve the ILP and find its optimal package $p$ . We validate constraint satisfaction of $p$ among all the validation scenarios, and update the bounds of each constraint independently (lines 13 and 14). If the ILP has no solution, we perform the same actions that we would if a suboptimal package was generated, which leads to more relaxed bounds for every constraint in later iterations. Once all bisections converge to intervals smaller than $\delta$, which can be an arbitrarily small preset value that we in our experiments set to be $0.1$, we check if the package finally obtained is validation feasible and $(1\pm\epsilon)$-approximate, and if so, return it (lines 16-17). If either of these conditions are violated, or if no package is returned by the solver, we double the number of optimization scenarios and try again (lines 18-19).

% Doubling the number of scenarios at each iteration is possible since \cvarif makes solver runtimes agnostic to the number of optimization scenarios. This allows aggressively increasing the number of optimization scenarios as the only penalty paid is in terms of scenario generation runtime. We ensure the number of optimization scenarios ($m$) never goes beyond the number of validation scenarios ($\hat{m}$). In the worst case, if we begin with $m=100$ optimization and $\hat{m}=10^6$ validation scenarios, there will still be no feasible and $(1\pm\epsilon)$-approximate solution after 13 iterations, after which $m$ will equal $\hat{m}$. Then, if a package is created from the optimization scenarios, it is guaranteed to be validation feasible since the set of optimization and validation scenarios are identical, and will be considered $(1\pm\epsilon)$-approximate. If no package is produced, the query is infeasible and has no solutions.

% Unconditionally increasing the number optimization scenarios is an improvement over \ssearch. If the generated package is not $(1\pm\epsilon)$-approximate, and the number of summaries is lower than the number of optimization scenarios, \ssearch incrementally increases the number of summaries. The number of optimization scenarios is only increased after the number of summaries equals the number of optimization scenarios. This results in a wasted inner loop over the number of summaries if the number of optimization scenarios is initially insufficient. Since this inner loop's complexity depends on the number of optimization scenarios, \ssearch remains much more conservative when increasing the number of optimization scenarios, and increases the number linearly instead of doubling it at each iteration like \cvarif.

% The sequence of ILPs solved during the bisection for the risk constraints is logarithmic to the size of the largest search range for any constraint. \ssearch needs a similar sequence to determine how many scenarios to use for creating each summary. 

% \cvarif updates the intervals of the CVaR approximations for each VaR constraint independently. Treating the problem of finding the closest CVaR approximations for multiple VaR constraints as a multi-dimensional search and updating the intervals co-dependently remains scope for future work.

% Implementation-wise, if the entire set of optimization scenarios, having size $m*n$ where $m$ is the number of optimization scenarios and $n$ is the number of tuples, fits into main memory, we store it entirely in the main memory to enable scenario sharing for other constraints and stochastic objectives addressed on the same attribute. If not, note that expected value constraints and stochastic objectives only require the sum of all scenario values for every tuple in their corresponding ILP expressions. So, we generate one scenario at a time, add its values to the respective sums for each variable, and erase the scenario from main memory. For converting risk constraints to CVaR constraints, we need the sum of the lowest $p$-fraction of scenario values for each tuple to construct the pseudo-scenario based linear constraint. We determine this by using max heaps containing at most $pm$ elements for each tuple. Every time a scenario is generated, we insert the values into each tuple's heap only if the heap has less than $pm$ elements or the scenario value for the tuple is smaller than the maximum value in the heap, in which case the max value is replaced by the value. Once all scenarios are generated, all heaps are erased and the sum of their elements are used for representing the CVaR constraints. Heap insertions and replacements can be parallelized across tuples. This is only possible if $n$ heaps with $pm$ elements fit into main memory. Otherwise, we divide the tuples into blocks of size $b$, such that $b$ heaps of size $pm$ fit into main memory, and generate scenario values for only tuples in the same block at a time.

% Note that while we describe handling VaR constraints that require the sum of an attribute to be higher or equal to a certain value, the methods can be trivially modified to handle VaR constraints that require the sum to not exceed given values.

% Finally, we prove implication (\ref{eq:cvar_representation}), which is the basis of using pseudo-scenarios to linearly represent CVaR constraints.

% \begin{theorem}
%     For any package $x=\{x_1, x_2, ..., x_n\}$ and a set of pseudo-scenarios $P$ formed from a set of scenarios $S$, if the expected scenario$\_$score of $S$ exceeds $V$ in the first $p$ pseudo-scenarios, the expected sum of $x$ in any $p$ scenarios of $S$ will also exceed V.
%     \label{theorem:conservative_pseudoscenarios}
% \end{theorem}

% \begin{proof}
% We define $L$ to be a set of indexes of $p$ scenarios and a one-to-one function $f([1, n], [1, m]): \rightarrow [1, m]$, which takes a tuple $i$ and a scenario $j$, and returns the position of $S_{ij}$ in the $i$-th row of the pseudo-scenario matrix $P$ after sorting. Then:

% $\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} = \sum_{j=1}^{n} x_{j} \sum_{i=1}^{p} P_{ij} \leq \sum_{i=1}^{n} x_{i} \sum_{j \in \bigcup_{t \in L} f(i, t)} P_{ij}$

% The last inequality holds since each element in $\bigcup_{t \in L} f(i, t)$ is either in $[1, p]$, meaning it contributes to both sides of the inequality equally, or is greater than $p$, which means they are being replaced by a value from $P_{i1}, P_{i2}, P_{i3}, ... P_{ip}$ in the left side of the inequality, where the replaced value on the left cannot be larger than the original value on the right since $P$ is row-wise sorted. From the definition of $f$, for all tuples $j$, $\sum_{i \in \bigcup_{t \in L} f(j, t)} P_{ij} = \sum_{i \in L} S_{ij}$.

% Thus, $\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \sum_{j=1}^{n} x_{j} \sum_{i \in L} S_{ij}$

% $\implies \sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i}$

% $\implies \frac{1}{p}\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \leq \frac{1}{p}\sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i}$

% Thus, $\frac{1}{p}\sum_{i=1}^{p}\sum_{j=1}^{n} P_{ij}x_{j} \geq V \implies \frac{1}{p}\sum_{i \in L} \sum_{j=1}^{n} S_{ij}x_{i} \geq V$
% \end{proof}

==> sections/old_files/cvarif_old.tex <==
\section{\cvarif}\label{sec:cvarif}
\peter{the following paragraph should be moved to the next secion and modified appropriately.} \riddho{Pasting this here in case we need this paragraph later on}
\smallskip\noindent\textbf{CVaRification.} Theorem~\ref{th:constraintCompare} implies that, for a given stochastic attribute $A$, an L-CVaR constraint with parameters $\alpha$ and $V$ is more restrictive than a VaR or CVaR constraint with the same parameters. Note that the L-CVaR constraint becomes less and less restrictive as either $V$ decreases or $\alpha$ increases, until it is not restrictive at all. It is therefore possible, by judicious  choice of $V$ and $\alpha$ to relax the L-CVaR constraint until it is approximately as restrictive as the original VaR or CVaR constraint; the algorithm is given in the following section. Letting $\alpha'$ and $V'$ denote the adjusted parameters, observe that each L-CVaR constraint is linear in the $x_i$'s, and remains so in the SAA approximation when each $\text{CVaR}_{\alpha'}(t_i.A)$ is approximated via averaging over scenarios with the lowest values (Algorithm~\ref{alg:approx}). Because all other types of SPaQL constraint types are also linear in the $x_i$'s (see the definitions at the beginning of the section) and their SAA approximations are linear as well, \cvarif leads to an ILP formulation whose size is independent of the number of scenarios, as desired. The approximation proceeds by converting all VaR and CVaR constraints to L-CVaR constraints. We next describe this process in detail, and Section~\ref{sec:experimental_evaluation} demonstrate the performance improvements over \ssearch due to \cvarif.
% \begin{algorithm}[t]
% \caption{\textsc{Approximate CVaR}}\label{alg:approx}
% \begin{algorithmic}[1]
% \Require $p :=$ probability value of the CVaR
% \Statex $s_1,\dots,s_m :=$ m sampled values

% \Comment{ {\color{gray}\textit{Approximate CVaR of an attribute with probability value $p$ using sampled values}}}

% \State $\Tilde{s}_1,\dots,\Tilde{s}_m \gets \textsc{SortAscending}(s_1,\dots,s_m)$
% \If{$\lfloor pm \rfloor = 0$}
%     \State\Return $\Tilde{s}_1$
% \Else
%     \State \Return $\sum_{i=1}^{\lfloor pm \rfloor} \Tilde{s}_i/\lfloor pm \rfloor$
% \EndIf
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
\caption{\textsc{\cvarif}}\label{alg:cvarification}
\begin{algorithmic}[1]
\Require $Q :=$ A Stochastic Package Query
\Statex $\text{tuples} :=$ Stochastic tuples in the SPQ
\Statex $m :=$ Initial number of optimization scenarios
\Statex $\hat{m} :=$ Max. number of scenarios used
\Statex $\delta :=$ Bisection termination distance

\State $Q_0 \gets $\textsc{RemoveProbabilisticConstraints}(Q)
\If{\textsc{IsUnsolvable}($Q_0$)}
\State \Return NULL
\EndIf
\State $X_0 \gets $ \textsc{ILPSolver}($Q_0$)
\If{\textsc{IsFeasible}($Q$, $X_0$, $\hat{m}$)}
\State \Return $X_0$
\EndIf

\State $L_V \gets \textsc{ComputeLowestBoundValues}(Q, X_0)$

\State $L_P \gets \textsc{GetProbabilityValues}(Q)$

% \State $d_e \gets 1$ \Comment{{\color{gray}\textit{Exponential search's initial distance}}}
% \While{true} \Comment{{\color{gray}\textit{Exponential search}}}
%     \State $L \gets V-d_e$
%     \State $Q'' \gets \textsc{SetBoundValues}(Q', L)$
%     \If{\textsc{IsUnsolvable}($Q''$)}
%         \State \textbf{break}
%     \EndIf
%     \State $d_e \gets 2d_e$
% \EndWhile

\State $X^* \gets \text{NULL}$
\State $\text{scenarios} \gets \emptyset$

\While{\textsc{Is\_$\epsilon$\_Optimal}($Q, X^*, \epsilon$) \textbf{and} \textsc{IsFeasible}($Q, X^*, \hat{m}$)}
    \State $\text{scenarios} \gets \text{scenarios} \cup \textsc{GenerateScenarios}(\text{tuples}, m)$
    \State $Q' \gets \textsc{SetCoefficients}(Q,L_P,\text{scenarios})$
    \State $R_V \gets \textsc{GetBoundValues}(Q)$
    \State $L_V, R_V, X_V \gets \textsc{BinarySearchOnV}(Q', \delta, L_V, R_V)$
    \If{$X_V$ != \text{NULL}}
        \State $X^* \gets X_V$
    \EndIf
    
    % \While{$\max |R_V-L_V| > \delta$} \Comment{{\color{gray}\textit{Binary search on $V$}}}
    %     \State $M_V \gets (R_V+L_V)/2$
    %     \State $Q'' \gets \textsc{SetBoundValues}(Q', M_V)$
    %     \If{\textsc{IsUnsolvable}($Q''$)}
    %         \State $R_V \gets M_V$
    %     \Else
    %         \State $X \gets \textsc{ILPSolver}(Q'')$
    %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
    %             \State $X^* \gets X$
    %             \State $R_V \gets M_V$
    %         \Else
    %             \State $L_V \gets M_V$
    %         \EndIf
    %     \EndIf
    % \EndWhile

    \State $Q' \gets \textsc{SetBoundValues}(Q, L_V)$
    \State $R_P \gets 1$
    \State $L_P, R_P, X_P \gets \textsc{BinarySearchOnP}(Q', \delta, L_P, R_P)$
    \If{$X_P$ != \text{NULL}}
        \State $X^* \gets X_P$
    \EndIf
    % \While{$\max |R_P-L_P| > \delta$} \Comment{{\color{gray}\textit{Binary search on $P$}}}
    %     \State $M_P \gets (R_P+L_P)/2$
    %     \State $Q'' \gets \textsc{SetCoefficients}(Q',M_P,\text{scenarios})$
    %     \If{\textsc{IsUnsolvable}($Q''$)}
    %         \State $L_P \gets M_P$
    %     \Else
    %         \State $X \gets \textsc{ILPSolver}(Q'')$
    %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
    %             \State $X^* \gets X$
    %             \State $L_P \gets M_P$
    %         \Else
    %             \State $R_P \gets M_P$
    %         \EndIf
    %     \EndIf
    % \EndWhile

    \State $m \gets 2m$
    \If{$m > \hat{m}$}
        \State \textbf{break}
    \EndIf
    
\EndWhile
\State \Return $X^*$

\end{algorithmic}
\end{algorithm}

\azza{I very much like the brevity of this section and it gets to the intuition much faster than before but you lose the reader when you try to connect to the algorithms and especially the relationship between Algo 1 and 2.}

\azza{A better name for Alg 1 is LinearizeCVaR} \peter{I would say EstimateCVaR. It is simply using scenarios to empirically estimate a CVaR. Presumably the CVaR is of the form $\text{CVaR}_p(t_i.A)$ if the function is being invoked during linearization.}
\azza{For each algorithm, I'd like you to put Output the same way you have input which describes what the output would be. I'd also reorder because LinearizeCVaR is a sub-module of CVarify.}

\azza{Alg 2 is called cvarification but "cvarification" feels like a process to convert VaR to CVaR rather than the solving process. This is a big change to make so I'm fine keeping things as they are but I do want to make this comment because it may be a bit of a reading block for some, perhaps we can call the algorithm CVarify\&Solve, rather than just "CVarification" }

\azza{Also, all algorithms should be "verbs" not "nouns" ... NumberOfDuplicates, InitialRiskTolerance, etc don't quite fit with the other naming convention of "CreateScenario" or "Sketch" ...}

Theorems~\ref{theorem:var}~and~\ref{theorem:cvar} show that if a package $X$ satisfies the linearized CVaR constraints with bound values $V$ then it should satisfy the corresponding VaR/CVaR constraints. Hence, such package $X$ can also be sub-optimal w.r.t the original SPQ. To find more optimal packages, one can relax the linearized CVaR constraints by decreasing the bound values $V$, i.e., finding the lowest $V^*$ such that the package $X^*$ found by setting bound values $V^*$ satisfies the original SPQ. This allows us to use binary search to find $V^*$ between an interval $(L,R]=(V_0,V]$ where $V_0$ are particular bound values such that the package $X_0$ found by setting bound values $V_0$ does not satisfy the original SPQ. In Algorithm~\ref{alg:cvarification}, to find such $V_0$ (line~1), we choose $X_0$ as the ILP solution when we remove all probabilistic constraints from $Q$ (line~1,4 Algorithm~\ref{alg:sketch}) \azza{blech! this is bad to call something a function that is then the first 4 lines of a different algorithm. Why not just make it a submodule? - you can put these in the appendix if they take too much space and then have both Sketch and Algorithm 2 refer to it?} and compute $V_0=CVaR_P(X_0)$ using Algorithm~\ref{alg:approx}. \azza{Where is this anywhere in any of the algorithms?}

To formulate $Q$ as an ILP using linearized CVaR constraints, we compute $CVaR_P(t_i.A)$ \azza{Is this a reference to Algorithm 1?} for each tuple $t_i$ in each risk constraint of attribute $A$ (line~3). \cvarif then proceeds with binary search as long as one of the bound value intervals is longer than $\delta$ (line~5). If the formulated ILP $Q''$ with "mid-point" bound values $M$ has no solution (line~8), then it means that the constraints are too tight and we need to relax them by setting the right-end point $R$ to $M$ (line~9). Otherwise, depending on whether the solution $X$ of $Q''$ satisfies the original SQP $Q$ (line~12), we would either relax or tighten the constraints to find $V^*$.

\azza{Using module names like IsUnsolvable or IsFeasible makes us anticipate that these modules are somewhere to be found (possibly in the appendix), especially because they are not immediately obvious. If these are meant to be pseudo statements like sort ascending then use "sf" rather than "sc" to format. I can buy set coefficients, get bound values, maybe ILPSolve as "sf" but the rest may need actual submodules defined in the appendix.}

==> sections/old_files/cvarification-old.tex <==
\section{\cvarmethod{}: CVaR Constraints are all you need} \label{sec:cvarification_details}

We first show how to solve queries containing CVaR constraints. We then show how each VaR constraint in a query can be substituted by its \textit{closest approximating CVaR constraint} to produce feasible high-quality packages in quicker time than \textit{SummarySearch}, allowing us to generalize our method of handling CVaR constraints to dealing with queries having VaR constraints. The resulting method, \cvarmethod{}, can be used to solve any \langname{} query having any number of risk constraints of any type.

\subsection{Handling CVaR constraints} \label{subsec:handling_cvar_constraints}

Given a CVaR constraint and a corresponding set of validation scenarios, it is computationally easy to verify if a package satisfies the constraint. Suppose, we have $\hat{M}$ validation scenarios for a particular attribute, for the $j-th$ of which the $i-th$ tuple in a relation containing $n$ tuples has the value $v_{ij}$. If $x_i$ denotes the number of instances of the $i-th$ tuple included in a package, the sum of the package for that attribute in the $j-th$ scenario is $scenario\_score(j) = \sum_{i=1}^{n} v_{ij}x_{i}$.

The CVaR (Conditional Value-at-Risk) of a package in the lowest $p\%$ of scenarios refers to the average scenario\_score of the package in $\frac{p\hat{M}}{100}$ scenarios in which its scenario\_scores are the lowest. Thus, validating if a package satisfies the constraint in the validation scenarios involves the following:
 
\begin{compactitem}
 \item For all validation scenarios $j \in [1, n]$, we determine the $scenario\_score(j)$ for the corresponding scenario.
 \item Sort the validation scenarios in ascending (descending) order of their $scenario\_scores$ for CVaR constraints that address scenarios for the lowest (highest) $p\%$ of scenarios.
 \item Compute the average $scenario\_score$ in the first $p\%$ of scenarios. If this average is not less (more) than the value $V$ indicated in the constraint specifying `$\leq V$' (`$\geq V$'), the constraint is satisfied.
\end{compactitem}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{figures/ValidatingCVaRConstraints.jpg}
    \caption{Validating a Sample CVaR constraint}
    \label{fig:cvar_validation}
\end{figure}

Fig. \ref{fig:cvar_validation} shows an example where a CVaR query is validated over 6 validation scenarios. In practical settings, we expect the number of validation scenarios to be numerous (e.g. $~10^6$). What makes CVaR constraint verification tractable is that once we know what the package is, we can determine in polynomial time what the best and worst case scenarios for it are. However, coming up with a package to validate is more challenging since the set of scenarios with the lowest/highest scenario scores will differ for different packages.

The fact that validation scenarios and optimization scenarios are two different sets provides some flexibility to \textit{modify} the optimization scenarios and generate a potentially \textit{imperfect} solution from them. If the generated package does not satisfy the CVaR constraint(s) in the validation scenarios, or is not $(1 \pm \epsilon)$-approximate, we can tune our approach for generating the package from the optimization scenarios, create new packages and re-validate them.

In \cvarmethod{}, we first replace the optimization scenarios with `pseudo-scenarios'. In our descriptions, we assume we are faced with a CVaR constraint in the form of `EXPECTED SUM(A) >= V IN LOWEST P \% OF SCENARIOS'. Modifying our approach for handling other types of CVaR constraints supported by \langname{} (e.g. replacing `LOWEST' with `HIGHEST' and `$\geq$' with `$\leq$') is trivial. First, we imagine all the optimization scenarios to collectively form an $n \times m$-sized scenario matrix $S$, where $S_{ij}$ denotes the value of the i-th tuple in the j-th scenario, for $n$ tuples and $m$ optimization scenarios. To create a set of pseudo-scenarios, denoted by a pseudo-scenario matrix $P$, where $P_{ij}$ denotes the value of the i-th tuple in the j-th pseudo-scenario, we first assign $S$ to $P$, that is for all $1 \leq i \leq n, 1 \leq j \leq m$, we ensure $P_{ij} = S_{ij}$. Then, we sort the rows of P in ascending order from left to right, as shown in Fig. \ref{fig:pseudoscenario-generation}.
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.25]{figures/CreatingPseudoScenarios.jpg}
    \caption{Creating pseudo-scenarios}
    \label{fig:pseudoscenario-generation}
\end{figure}

Sorting the rows in a tuple-wise manner ensures that we now know exactly what the pseudo-scenarios with the lowest scenario scores are, regardless of the nature of the package. The pseudo-scenario for which \textit{any} package will yield the lowest scenario score will be the first scenario in the pseudo-scenario matrix. By extension, the first $p'=\lceil\frac{pm}{100}\rceil$ pseudo-scenarios will yield the lowest $p'$ scenario scores, representing the lowest $p\%$ of scenarios referred to in the query's constraint. The expected sum of the attribute for a package $\{x_1, x_2, x_3, ..., x_n\}$ in these scenarios is $\dfrac{\sum_{j=1}^{p'} \sum_{i=1}^{n} P_{ij}x_{i}}{p'}$. Since the constraint requires this expected sum to be $\geq v$, we can write the constraint with the expression $\dfrac{\sum_{j=1}^{p'} \sum_{i=1}^{n} P_{ij}x_{i}}{p'} \geq v$, or:

\begin{equation}
    \sum_{j=1}^{p'} \sum_{i=1}^{n} P_{ij}x_{i} \geq p'v
    \label{eq:cvar_expression}
\end{equation}

Since Eq. \ref{eq:cvar_expression} is linear, we can directly add it into the ILP formulation, in addition to the expressions for the other constraints and objective as outlined in section \ref{subsec:spqs_to_silps}. Readers may observe that for any package, the first few pseudo-scenarios are typically harder to satisfy than the set of worst-case optimization scenarios. For instance, all tuples in the first pseudo-scenario are guaranteed to have values that are smaller than or equal to the values of the corresponding tuples in any scenario in the original optimization set. Any package that satisfies the CVaR constraint over the first $p'$ pseudo-scenarios is guaranteed to satisfy the same constraint over at least $p'$ optimization scenarios as well.

Formally, we first prove that the scenario scores for any package are sorted in ascending order over pseudo-scenarios $1$ to $n$, and, by extension, the first $p'$ pseudo-scenarios are indeed the scenarios where the sum of the attribute for the tuples in the package are the lowest. We then prove that if any package satisfies the constraint over the first $p'$ pseudo-scenarios, it is guaranteed to satisfy the constraint over the original set of optimization constraints.

\begin{lemma}
For any pseudo-scenario matrix P, for any package $x=\{x_1, x_2, x_3, ..., x_n\}$, for any pair of integers $(l, r)$ such that $1 \leq l \leq r \leq m$, $scenario\_score(l) \leq scenario\_score(r)$.
\label{lemma:scenario_scores_are_monotonic}
\end{lemma}
\begin{proof}
For any position $1 \leq p \leq m$, $scenario\_score(p)=\sum_{i=1}^{n} P_{ip}x_{i}$. Since pseudo-scenario matrices are sorted in ascending order horizontally, $P_{il} \leq P_{ir}$. Since for all $1 \leq i \leq n$, $x_i \geq 0$, $P_{il}x_{i} \leq P_{ir}x_{i}$. Thus, $\sum_{i=1}^{n} P_{il}x_{i} \leq \sum_{i=1}^{n} P_{ir}x_{i}$, which implies $scenario\_score(l) \leq scenario\_score(r)$.
\end{proof}


\begin{theorem}
For any pseudo-scenario matrix $P$, for any package $x=\{x_1, x_2, x_3, ..., x_n\}$, for any $1 \leq p' \leq m$ the scenario scores in the first $p'$ pseudo-scenarios will be lower than those in the remaining $m-p'$ pseudo-scenarios.
\label{theorem:first_few_pseudoscenarios_suffice}
\end{theorem}
\begin{proof}
For any pair of pseudo-scenarios $(i, j)$, where $1 \leq i \leq p'$, and $p'+1 \leq j \leq m$ (i.e. $i$ is among the first $p'$ pseudo-scenarios while $j$ is any one of the remaining $m-p'$ pseudo-scenarios), $i < j$. From lemma \ref{lemma:scenario_scores_are_monotonic}, $scenario\_score(i) \leq scenario\_score(j)$.
\end{proof}

From theorem \ref{theorem:first_few_pseudoscenarios_suffice}, only the first $p'$ scenarios need to be considered when creating the corresponding linear expression with the scenarios having the lowest scenario scores for a CVaR constraint as seen in eq. \ref{eq:cvar_expression}. Next, we prove that if a package satisfies eq. \ref{eq:cvar_expression}, it is guaranteed to satisfy the CVaR constraint over the original set of optimization scenarios. Suppose that for any package $x=\{x_1, x_2, x_3, ..., x_n\}$, $Low(x, p', S)$ represents the column indices of the set of optimization scenarios with the lowest scenario scores in the scenario matrix $S$. The package's expected sum in these scenarios will be $\frac{\sum_{j \in Low(x, p', s)}\sum_{i=1}^{n} S_{ij}x_{i}}{p'}$, whereas the expected sum in the first $p'$ pseudo-scenarios is $\frac{\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i}}{p'}$.  If the constraint requires the expected sum to be not lower than $v$, then $\frac{\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i}}{p'} \geq v$ will imply $\frac{\sum_{j \in Low(x, p', s)}\sum_{i=1}^{n} S_{ij}x_{i}}{p'} \geq v$ if $\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i} \leq \sum_{j \in Low(x, p', s)}\sum_{i=1}^{n} S_{ij}x_{i}$.

\begin{theorem}
For any scenario matrix $S$ with a corresponding pseudo-scenario matrix $P$, if for any package $x = \{x_1, x_2, x_3, ..., x_n\}$, $Low(x, p', S)$ represents the column indices of the set of optimization scenarios with the lowest scenario scores in the scenario matrix, then: 
\begin{equation}
\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i} \leq \sum_{j \in Low(x, p', s)}\sum_{i=1}^{n} S_{ij}x_{i}   
\end{equation}
\label{theorem:pseudo-scenarios_are_conservative}
\end{theorem}
\begin{proof}
Let us define a one-to-one function $f([1, n], [1, m]): \longrightarrow [1, m]$ that takes a tuple $i$ and a scenario $j$, and returns the corresponding position of $S_{ij}$ in the $i-th$ row of the pseudo-scenario matrix $P$ after sorting. For example, in Fig. \ref{fig:pseudoscenario-generation}, f(1, 2) will return 1, since the value -3 for the first tuple in the second scenario is transferred to the first pseudo-scenario. Now, consider the following:

$\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i} = \sum_{i=1}^{n} x_{i} \sum_{j=1}^{p'} P_{ij}$

$\sum_{i=1}^{n} x_{i} \sum_{j=1}^{p'} P_{ij} \leq \sum_{i=1}^{n} x_{i} \sum_{j \in \bigcup_{t \in Low(x, p', S)} f(i, t)} P_{ij}$

To understand why the above is true, observe that each of the $p'$ elements in $\bigcup_{t \in Low(x, p', S)} f(i, t)$ are either in $[1, p']$, meaning their contributions on both sides of the inequality is equal, or is greater than $p'$, which means they are being replaced by a value from $P_{i1}, P_{i2}, P_{i3}, ... P_{ip'}$ in the left side of the inequality, where the value on the left cannot be larger than the value on the right since since $P$ is row-wise sorted. From the definition of $f$, for all tuples $i$, $\sum_{j \in \bigcup_{t \in Low(x, p', S)} f(i, t)} P_{ij} = \sum_{j \in Low(x, p', s)} S_{ij}$.

Thus, $\sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i} \leq \sum_{i=1}^{n} x_{i} \sum_{j \in Low(x, p', s)} S_{ij}$

$\implies \sum_{j=1}^{p'}\sum_{i=1}^{n} P_{ij}x_{i} \leq \sum_{j \in Low(x, p', s)} \sum_{i=1}^{n} S_{ij}x_{i}$
\end{proof}

\anh{I appreciate how you describe CVaRification in terms of pseudo scenarios but it could be much more concise and understandable if you describe it mathematically. Your theorem 4.3 can be described as: Let $X_i$ be random variables and $m_i \geq 0$. Let $X$ be a linear combination of $X_i$ i.e. $X=\sum_i m_iX_i$. Then $$\sum_i m_i \mathbb{E}[X_i | X_i \leq F_{X_i}^{-1}(p)] \leq \mathbb{E}[X|X \leq F_X^{-1}(p)]$$ where $F_X^{-1}(p)$ is the quantile function of random variable $X$ at percentile $p$. Also this is the "subadditive property of risk" that you mention above and you should mention again here.} 

Theorem \ref{theorem:pseudo-scenarios_are_conservative} implies that considering the first $p'$ pseudo-scenarios while building the corresponding ILP makes the problem conservative, and guarantees CVaR constraint satisfaction. However, this risks making the ILP formulation overly conservative, resulting in suboptimal packages. Suppose, that the package derived from considering the first $p'$ pseudo-scenarios is overly conservative. Now, consider that we replace the $ p'$-pseudo-scenario-based constraint with a $(p'+1)$-pseudo-scenario-based constraint in the ILP. In other words, instead of ensuring that the expected sum of the attribute is over $v$ in the worst $p'$ scenarios, we need to ensure the expected sum of the attribute is over the same value $v$ in the worst $(p'+1)$ scenarios. Intuitively, we are adding a scenario that is strictly \textit{not worse} than any of the previously considered scenarios. For any package, this means that the expected sum of any attribute in the lowest $(p'+1)$-scenarios will be potentially greater (and certainly not less) than the expected sum in the lowest $p'$ scenarios. This leads to an important observation - the higher the number of pseudo-scenarios considered, the more relaxed the corresponding constraint potentially gets in the ILP formulation. Thus, if considering the first $p'$ pseudo-scenarios leads to a package that satisfies the constraint in the validation scenarios, but whose objective value does not make it $(1+\epsilon)$-approximate, we could increase the number of pseudo-scenarios considered to some value $\alpha$, such that $p' \leq \alpha \leq m$, and include in the corresponding ILP formulation the linear constraint:

\begin{equation}
    \sum_{j=1}^{\alpha} \sum_{i=1}^{n} P_{ij}x_{i} \geq \alpha*v
    \label{eq:cvar_expression_alpha_pseudoscenarios}
\end{equation}

The parameter $\alpha$ thus provides a means to tune the hardness of our pseudo-scenario-based constraint. If $\alpha = p'$, the constraint is guaranteed to be satisfied among the validation scenarios, but risks being overly conservative. On the other extreme, we could set $\alpha = m$, meaning all the pseudo-scenarios will be considered.
This would make eq. \ref{eq:cvar_expression_alpha_pseudoscenarios} equivalent to $\sum_{j=1}^{m} \sum_{i=1}^{n} P_{ij}x_{i} \geq m*v$. This can be written as $\sum_{i=1}^{n} x_{i} \sum_{j=1}^{m} P_{ij} \geq m*v$. Since the i-th row in the pseudo-scenario matrix $P$ contains all the elements in the i-th row of the scenario matrix $S$ exactly once, $\sum_{j=1}^{m} P_{ij} = \sum_{j=1}^{m} S_{ij}$. Hence,

$\sum_{i=1}^{n} x_{i} \sum_{j=1}^{m} P_{ij} \geq m*v \implies \sum_{i=1}^{n} x_{i} \sum_{j=1}^{m} S_{ij} \geq m*v$

$\implies \sum_{j=1}^{m} \sum_{i=1}^{n} S_{ij}x_{i} \geq m*v \implies \frac{\sum_{j=1}^{m} \sum_{i=1}^{n} S_{ij}x_{i}}{m} \geq v$

Thus, setting $\alpha = m$ is equivalent to a CVaR constraint that considers 100\% of the scenarios scenarios, or equivalently an expected value constraint over all of the scenarios. If the resulting package still satisfies the original CVaR constraint in the validation scenarios, we can replace the CVaR constraint with an expected value constraint of the form `EXPECTED SUM(A)>=V'.

In most cases, however, setting $\alpha = m$ will result in packages that do not satisfy the constraint, while setting $\alpha = p'$ will produce packages that are guaranteed to satisfy the CVaR constraint among the optimization scenarios, but with potentially suboptimal objective values. We thus run a binary search to find the highest value of $\alpha$ for which the resulting package satisfies the CVaR constraint among the validation scenarios. During each iteration of the search, we modify the value of $\alpha$ considered for each CVaR constraint independently of each other. For a particular constraint, if a given value of $\alpha$ results in a package that is validation feasible (i.e. satisfies the constraint in the validation scenarios), we set the lower bound of the binary search for that constraint to $\alpha$, otherwise, we set the upper bound to $\alpha-1$. The search terminates when both bounds converge to the same value, requiring at most $\mathcal{O}(\lg{m})$ iterations.

\subsection{CVaR Approximations for VaR constraints}\label{subsec:cvar_approxating_var}

In this section, we describe how VaR constraints in the form of \texttt{`SUM(A) >= V WITH PROBABILITY >= P'} can be solved by approximating them using CVaR constraints. Consider replacing all such constraints in the query with a CVaR constraint of the form \texttt{`EXPECTED SUM(A) >= V IN LOWEST (1-P)*100\% OF SCENARIOS'}. Note that VaR constraints in the form of  \texttt{`SUM(A) <= V WITH PROBABILITY >= P'} can be similarly replaced with CVaR constraints of the form \texttt{`EXPECTED SUM(A) <= V IN HIGHEST (1-P)*100\% OF SCENARIOS'}. We also note that `(1-P)*100\% OF SCENARIOS' covers the most extreme (1-P) fraction of scenarios. We first prove the following:

\begin{theorem}
    A package that satisfies the constraint \texttt{`EXPECTED SUM(A) >= V IN LOWEST (1-P)*100\% OF SCENARIOS'} is guaranteed to satisfy the constraint \texttt{`SUM(A) >= V WITH PROBABILITY >= P'}.
    \label{theorem:cvar_approximation_is_conservative_enough}
\end{theorem}
\begin{proof}
    For m optimization scenarios, a package that satisfies the CVaR constraint \texttt{`EXPECTED SUM(A) >= V IN LOWEST (1-P)*100\% OF SCENARIOS'} will have an average scenario\_score that is not less than $V$ in the lowest $(1-P)*m$ scenarios. In a list containing every optimization scenario sorted in the ascending order of their scenario scores for the package, the $(1-P)*m$-th scenario must have a scenario score $\geq V$ (since its scenario score is the maximum among the lowest $(1-P)*m$ scenarios). This means that the remaining $P*m$ scenarios, whose scenario scores are more than or equal to that of the $(1-P)*m$-th scenario, and whose combined probability mass is $P$, must have scenario scores $\geq V$ as well. Thus, with probability $\geq P$, the sum of attribute A in the package will be $\geq V$, that is, the VaR constraint will be satisfied. 
\end{proof}

Theorem \ref{theorem:cvar_approximation_is_conservative_enough} shows that the suggested CVaR alternatives to the VaR constraints are guaranteed to be conservative enough, that is, all packages that satisfy the CVaR alternative will satisfy the VaR constraint in the original query. To generate packages that satisfy the CVaR alternative, we can impute the pseudo-scenario-based linear constraint in eq. \ref{eq:cvar_expression} into the corresponding ILP formulation, which per Theorem \ref{theorem:pseudo-scenarios_are_conservative}, will generate a package that is guaranteed to satisfy the CVaR alternative.

While the generated packages should satisfy the VaR constraint among the optimization scenarios, this method risks making the corresponding ILP formulations overly conservative. Thus, the packages may have suboptimal objective values. A tempting workaround for this may be to tune $\alpha$, the number of pseudo-scenarios considered, as we do for CVaR constraints. However, for CVaR constraints, a package generated using $\alpha = m$ being validation feasible implies the constraint is trivial. This may not necessarily be true in the case of VaR constraints. Thus, instead of tuning $\alpha$, we tune the value of $V'$, and run a bisection to find the lowest value of $V'$ for which satisfying the CVaR constraint \texttt{`EXPECTED SUM(A) >= V' IN LOWEST (1-P)*100\% OF SCENARIOS'} leads to creating a package that satisfies the original VaR constraint \texttt{`SUM(A) >= V WITH PROBABILITY >= P'} among the validation scenarios. To create a package that satisfies the CVaR constraint for a value of $V'$, we use the following linear constraint in the ILP formulations, where $P$ denotes the pseudo-scenario matrix for a given set of optimization scenarios $S$:

\begin{equation}
    \sum_{j=1}^{(1-P)*m} \sum_{i=1}^{n} P_{ij}*x_{i} \geq (1-P)*m*V'
    \label{eq:cvar_approximation_expression}
\end{equation}

\begin{figure}[b]
    \centering
    \includegraphics[scale=0.26]{figures/Replacing_VaR_Constraints_With_CVaR.jpg}
    \caption{Visualizing how making $V'$ too high or too low results in suboptimal or infeasible packages respectively}
    \label{fig:cvar_tuning}
\end{figure}
To run a bisection, we first need to find a lower bound for the value of $V'$ for which the generated package is not validation feasible. To initially find this lower bound $V_{low}$, we first set $V' = V - d$, where $V$ is the value specified in the VaR constraint, and $d$ can be any positive real value (e.g. 100). If the generated package is validation feasible for $V' = V - d$, we proceed to test the values $V - 2*d$, $V - 4*d$, $V - 8*d$ and so on, doubling the difference each time. We set $V_{low} = V - 2^{i}*d$ for the minimum value of $i$ for which the generated package is not validation feasible. Furthermore, we set $V_{up} = V - 2^{i-1}*d$ as the upper bound for the bisection, since it is a value for which the generated package was validation feasible. To prevent the search for $V_{low}$ from turning into an infinite loop in case of a trivial VaR constraint, we need a lower bound $\underline{V}$ of the VaR of the attribute for the optimal package. To determine $\underline{V}$, we can use the VaR of that attribute in the optimal package produced in response to the query with all risk constraints removed from it. Recall that we already use the objective score of the package produced in response to such a query to determine if the final package we get is $(1 \pm \epsilon)$. We simply need to use the VaR of that package for the corresponding attribute of the VaR constraint as $\underline{V}$. If, after $i$-iterations, $V - 2^{i}*d$ goes below $\underline{V}$, we conclude that the VaR constraint is trivial. If not, we run the bisection starting with the range $\{V_{low}, V_{up}\}$. During each iteration of the bisection, the value $V'$ is selected as the mid-point between the two bounds. If the generated package is validation feasible, we set the upper bound to $V'$, and set the lower bound to $V'$ otherwise. The bisection terminates when the two bounds become almost equal, in which case we return the package generated during the last iteration.

\anh{As before, you can describe all these concepts if the formulation has been mathematically defined. For example, one way to do this is to define the CVaR and VaR inequalities as: $$CVaR_m(X,v,p) \iff \sum_i m_i \mathbb{E}[X_i | X_i \leq F_{X_i}^{-1}(p)] \geq v$$ and $$CVaR(X,v,p) \iff \mathbb{E}[X|X \leq F_X^{-1}(p)] \geq v$$ and $$VaR(X,v,p) \iff Pr(X \leq v) \leq p$$}

\subsection{SPQ Processing with \cvarmethod{}}\label{subsec:spq_processing_with_cvarification}

Section \ref{subsec:handling_cvar_constraints} shows how CVaR constraints in SPQ-s can be handled using a single linear constraint in the corresponding ILP formulation, while section \ref{subsec:cvar_approxating_var} shows the same for VaR constraints. To find an optimal linear constraint that generates a package that satisfies all the constraints and whose objective value is as optimal as possible, we run bisections for each constraint to tune their corresponding linear constraints. Thus for a given set of optimization and validation scenarios, a solution to the stochastic package query can be found using a sequence of ILP formulations.

However, even after tuning all risk constraints to their optimal pseudo-scenario-based linear constraints, that is, after the bisections for each constraint terminate, the resulting package may not be validation-feasible or may not have an objective value that is $(1 \pm \epsilon)$-approximate. In such cases, we double the number of optimization scenarios used, and try again. We observe that the size of the ILP formulations in our proposed method is independent of the number of optimization scenarios. No matter how many optimization scenarios there are, the corresponding ILP formulations only contain a single linear constraint for each constraint in the query, and the number of variables in the ILP formulation is equal to the number of tuples. This allows us to aggressively increase the number of optimization scenarios, doubling up the value in each iteration. Algorithm \ref{alg:cvarmethod_query_execution} shows the overall query execution flow for \cvarmethod{}, our proposed approach. 

\begin{algorithm}[tb]
\caption{\textit{\cvarmethod{} Query Execution}}\label{alg:cvarmethod_query_execution}
\begin{algorithmic}[1]

\Require $Q$, Stochastic package query
\Statex $M$, initial number of optimization scenarios (e.g. $100$)
\Statex $\hat{M}$, number of validation scenarios (e.g. $10^6$)
\Statex $\epsilon$, user-defined approximation error bound
\While{True}
  \State Find upper and lower bounds for the bisection for each VaR constraint and remove trivial ones
  \While{Bisection of all VaR and CVaR constraints are not complete}
    \State Modify $\alpha$ for each CVaR constraint
    \State Modify $V'$ for each VaR constraint
    \State Create corresponding $ilp\_formulation$ with all values of $\alpha$ and $V'$
    \State $p \gets SolveILP(ilp\_formulation)$
    \State Validate resulting package $p$ for all constraints
    \State Update bounds for bisection
  \EndWhile
  \If{$p.is\_feasible(Q) \And p.is\_1+\epsilon\_approx(\epsilon)$}
    \State \Return p \Comment{{\color{gray} \textit{A feasible and ($1+\epsilon$)-approximate package is returned if found}}}
  \Else
    \State $M \gets 2*M$ \Comment{{\color{gray}\textit{Double the number of optimization scenarios and try again}}}
  \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

There are several advantages that \cvarmethod{} provides over \textit{SummarySearch}. First, it does not need to tune anything like the number of summaries, as \textit{SummarySearch} does in Algorithm \ref{alg:summarysearch_query_execution}. Thus, in cases where the number of optimization scenarios initially selected is not enough, \cvarmethod{} detects the problem just after it finishes optimizing the values of $\alpha$ and $V'$ for its CVaR and VaR constraints via a logarithmic number of steps using binary search, instead of running an entire inner linear loop first to increase the number of summaries like \textit{SummarySearch} does. Since optimizing the linear constraints for CVaR and VaR constraints is done using bisection, this process finishes within a logarithmic number of iterations, after which the number of optimization scenarios can be increased right away. Second, unlike the ILP formulations for \textit{SummarySearch}, which contains one indicator variable per summary, \cvarmethod{} solves the SILP using a series of indicator-variable free ILP formulations containing linear constraints only. Third, since the size of the ILP formulations by \cvarmethod{} is independent of the number of optimization scenarios, we can aggressively double up the number of optimization scenarios used in each iteration. Fourth, \cvarmethod{} is less parametric than \textit{SummarySearch}, in that the user does not need to define the number of summaries, the increment in the number of summaries and scenarios, as they need to do for \textit{SummarySearch}.

\begin{expbox}{Given the same set of optimization scenarios, which methods finds better results quicker?}
\includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
\tcblower
Given the same set of optimization scenarios, we show that \cvarmethod{} can find more optimal packages with lower runtime than \textit{SummarySearch}, by experimenting with both methods on the query in Fig. \ref{fig:example_spaql}, after removing the CVaR constraint. We observed that for 100 optimization scenarios, due to the absence of indicator variables, \cvarmethod{} generates its results in X seconds, while \textit{SummarySearch} takes Y seconds, Furthermore, due to \cvarmethod{}'s ability to flexibly tune the value of $V'$ for the VaR constraint to generate more optimal results, its generated package has an objective value of X, which is better than that of the package generated by \textit{SummarySearch} (Y).
\end{expbox}

==> sections/old_files/cvarification_9-11.tex <==
\section{\lcsolve: Solving Small SPQs}\label{sec:cvarif}

Our new \sskr algorithm (discussed in Section~\ref{section:sskr}) solves a large-scale SPQ with many tuples, by solving a sequence $Q(S_0), Q(S_1),\ldots$ of relatively small SPQ problems, where the query $Q$ is fixed but the set $S$ of tuples varies.
%with $S_0$ representing a small ``sketch'' comprising a set of ``representatives'', and subsequent sets being generated via a ``refinement'' process where representative tuples are replaced by actual tuples.
In this section we describe \lcsolve (Algorithm~\ref{alg:lcsolve}), our scenario-scalable algorithm for solving each SPQ encountered during the sketch-and-refine process. We assume henceforth that the set $\mathcal{V}$ of validation scenarios is large enough so that a package is validation-feasible if and only if it is feasible for the original SPQ, and that the objective function for a feasible package is essentially equal to its approximation based on $\mathcal{V}$; this assumption typically holds in practice.

\begin{algorithm}[t]
\caption{\textsc{\lcsolve}}\label{alg:lcsolve}
\begin{algorithmic}[1]
\Require $Q :=$ A Stochastic Package Query
\Statex $S :=$ Set of stochastic tuples in the SPQ
\Statex $m :=$ Initial number of optimization scenarios
%\Statex $\mathcal{O}$ $:=$ Initial set of optimization scenarios
\Statex $\mathcal{V}$ $:=$ Set of validation scenarios
\Statex $\delta :=$ Bisection termination distance
\Statex $\epsilon :=$ Approximation bound

\Ensure $X :=$ A validation-feasible and $\epsilon$-optimal package for $Q(S)$ \\ \makebox[17pt]{} (or NULL if unsolvable)
%or too few opt. scenarios)

\State $\mathcal{O} \gets \textsc{GenerateScenarios}(m)$ \Comment{Initial optimization scenarios}
\State \textsf{qsSuccess}, $X^{\text{D}} \gets $\textsf{QuickSolve}(Q, S) \Comment{Check if solution is ``easy''}\label{li:quicksolve}
\If{\textsf{qsSuccess} $=$ \textsf{True}}
\State \Return $X^{\text{D}}$ \Comment{Either $Q(S)$ solution or NULL}\label{li:quickreturn}
\EndIf

\State $\alpha, V\gets \textsc{GetParams}(Q)$ \Comment{Extract $(\alpha_r,V_r)$ for each $r\in Q$}
\State $\omega_0\gets \textsc{OmegaUpperBound}(Q,S,X^{\text{D}},\mathcal{V})$\label{li:EstObjVal}
\While{True}
\State $\alpha' \gets\alpha$, $\omegaU\gets\omega_0$
\State Compute $V_L$ as in \eqref{eq:defVL}
and set $V_U\gets V$, $\alpha_L\gets \alpha$, $\alpha_U\gets 1$
\While{True}
\State \textcolor{gray}{$\triangleright$ \textit{Search for V}}
\State  status, $V', X\gets \textsc{V-Search}(\alpha', V_L,V_U,Q,S,\epsilon,\delta,\mathcal{O},\mathcal{V},\omegaU)$
\State \algorithmicif\ status.NeedScenarios $=$ True \algorithmicthen\ \textbf{break}
\State \algorithmicif\ status.Done $=$ True \algorithmicthen\ \textbf{return} $X$
\State $V_U\gets V'$
\State \textcolor{gray}{$\triangleright$ \textit{Search for $\alpha$}}
\State  status, $\alpha', X\gets \textsc{$\alpha$-Search}(V', \alpha_L,\alpha_U,Q,S,\epsilon,\delta,\mathcal{O},\mathcal{V},\omegaU)$
\State \algorithmicif\ status.NeedScenarios $=$ True \algorithmicthen\ \textbf{break}
\State \algorithmicif\ status.Done $=$ True \algorithmicthen\ \textbf{return} $X$
\State $\alpha' \gets \min\bigl(1,\alpha'+(\lfloor\alpha' m\rfloor+1)/m\bigr)$
\State $\alpha_L\gets \alpha'$
\EndWhile
\State $\mathcal{O} \gets \mathcal{O} \cup \textsc{GenerateScenarios}(m)$
\State $m\gets 2m$
\State \algorithmicif\ $m>|\mathcal{V}|$ \algorithmicthen\ \textbf{return} NULL%$X$
\EndWhile

\end{algorithmic}
\end{algorithm}

\smallskip\noindent\textbf{Overview.} The basic idea is to replace each \emph{risk constraint} (VaR or CVaR constraint) in an SPQ with an approximating \LCVaR constraint such that the resulting problem size is independent of the number of scenarios and can be solved using an ILP solver. We leverage Theorem~\ref{th:constraintCompare}, which implies that, for a given stochastic attribute $A$, an \LCVaR constraint with parameters $\alpha$ and $V$ is more restrictive than a risk constraint with the same parameters. Note that an \LCVaR constraint of the form $\LCVaR_\alpha(X\cdot A) \ge V$ becomes less restrictive as either $V$ decreases or $\alpha$ increases. It is therefore possible, by judicious choice of $V$ and $\alpha$, to replace each risk constraint by an \LCVaR constraint that is approximately just as restrictive. The SAA approximation to the SPQ then becomes an ILP, and we can apply an ILP solver to compute the desired package.

%\cvarif refers to the process of replacing all risk constraints by linear \LCVaR constraints of similar restrictiveness. This replacement 
\emph{Risk-constraint linearization} (RCL), i.e., replacing all risk constraints in a query $Q(S)$ by \LCVaR constraints of similar restrictiveness, is accomplished via a search over potential $(\alpha,V)$ values for every \LCVaR constraint. For each choice of values, we solve the resulting SPQ via SAA approximation using the optimization scenarios and then check whether the returned package satisfies the original risk constraints in the query with respect to the validation scenarios. Packages that satisfy the risk constraints are deemed ``validation-feasible''. \lcsolve aims to compute a package that is both~(i)~validation-feasible, and~(ii)~near-optimal, i.e., whose objective values are $\ge (1-\epsilon)\omega$ for maximization and $\le (1+\epsilon)\omega$ for minimization problems, with $\omega$ being the optimal package's objective value and $\epsilon$ being an application-specific error tolerance.

\smallskip\noindent\textbf{Quick solution in special cases.}
Sometimes a query $Q(S)$ can be solved quickly, without going through the entire RCL process. Specifically, denote by $Q^{\text{D}}(S)$ the deterministic package query obtained by removing all probabilistic constraints, i.e., all VaR, CVaR and expected sum constraints, from $Q(S)$. If the ILP solver can find a package solution $X^{\text{D}}$ and if this solution is validation-feasible for $Q(S)$, then $X^{\text{D}}$ is the solution to $Q(S)$, since it satisfies all constraints, including the probabilistic ones, and the objective value is as high as possible since the probabilistic constraints have been completely relaxed, thereby maximizing the feasible region.
%and adding back any further constraints to the query will only shrink the feasible region, hence lowering the objective value.
On the other hand, if no feasible solution can be found for $Q^{\text{D}}(S)$, then $Q(S)$ is also unsolvable, since $Q$ has all the constraints that $Q^{\text{D}}$ has, and more. We denote by \textsc{QuickSolve}$(Q,S)$ the subroutine that detects these two possible outcomes (line~\ref{li:quicksolve}). \textsc{QuickSolve}$(Q,S)$ returns a pair $(\text{qsSuccess},X^{\text{D}})$. If $\text{qsSuccess}= \text{TRUE}$, then $X^{\text{D}}$ either is the package solution to $Q(S)$ or $X^{\text{D}}=$ NULL, which indicates that $Q(S)$ is unsolvable, and \lcsolve terminates and returns one of these values (line~\ref{li:quickreturn}). If $\text{qsSuccess}= \text{FALSE}$ then $X^{\text{D}}$ solves $Q^{\text{D}}(S)$ but is validation-infeasible for $Q(S)$ and the full RCL process is needed.

% If \textsc{QuickSolve}$(Q,S)$.Success = TRUE, then the subroutine returns either an optimal package \textsc{QuickSolve}$(Q,S)$.Package = $X^{\text{D}}$ or returns a null package (i.e.,\textsc{QuickSolve}$(Q, S)$.Package = NULL), indicating that the problem is unsolvable. Otherwise, \textsc{QuickSolve}$(Q,S)$.Success = FALSE is returned, along 
% with the package $X^{\text{D}}$ that solves $Q^{\text{D}}(S)$---this package is validation-infeasible for $Q(S)$ 
% %with the probabilistically unconstrained package $X^{\text{D}}$
% and the full RCL process is needed.

% \begin{algorithm}[t]
% \caption{\textsc{QuickSolve}}\label{alg:qSolve}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Ensure \textsf{Success} $:=$ True if \textsf{Package} solves $Q(S)$, False otherwise
% \Statex \textsf{Package} $:=$ The returned package

% \State $Q^{\text{D}} :=$ \textsc{RemoveProbabilisticConstraints}($Q$)
% \State $X^{\text{D}} :=$ \textsc{IlpSolver}($Q^{\text{D}}$).\textsc{Solve}()
% \If{\textsc{ValidationFeasible}($X^{\text{D}}$)}
%     \State \Return \{\textsf{Success} $=$ \textsc{True}, \textsf{Package} $= X^{\text{D}}$\}
% \ElsIf{$X^{\text{D}}$ is NULL}
%     \State \Return \{\textsf{Success} $=$ \textsc{True}, \textsf{Package} $= NULL$\}
% \Else
%     \State \Return \{\textsf{Success} $=$ \textsc{False}, \textsf{Package} $= X^{\text{D}}$\}
% \EndIf
% \end{algorithmic}
% \end{algorithm}

\smallskip\noindent\textbf{The case of a single risk constraint.} To understand how RCL works, first consider an SPQ having a single risk constraint---on a random attribute $A$ with parameters $(\alpha,V)$---that will be replaced by an \LCVaR constraint. If the \LCVaR constraint is too stringent, the package solution will be validation-feasible, but sub-optimal, whereas if the constraint is too relaxed, the package solution will be validation-infeasible. A package solution may also be validation-infeasible or sub-optimal if the number of optimization scenarios is too small so that the SAA approximation is not accurate. We will discuss how RCL deals with this latter issue shortly, but suppose for now that the initial number $m$ of optimization scenarios is adequate.
%in which case the package's VaR, CVaR or objective value among the optimization scenarios will differ sharply from its VaR/CVaR among the validation scenarios.

Let $\alpha'$ and $V'$ denote the adjusted parameters of the \LCVaR constraint. Recall that, for any risk constraint with parameters $\alpha$ and $V$, setting $\alpha'=\alpha$ and $V'=V$ will cause the corresponding \LCVaR constraint to be overly restrictive. The parameter $\alpha'$ can be set as high as $1$, in which case each coefficient $\hat C_i=\LCVaR_{\alpha'}(t_i.A)$ will be the average of the $t_i.A$ values across \emph{all} the optimization scenarios. On the other hand, for a given value of $\alpha$, the parameter $V'$ can be set as low as $V_0$, where $V_0=\sum_{i=1}^n \text{CVaR}_\alpha(t_i.A)*x_{0,i}$ and $X^{\text{D}}=(x_{0,1},\ldots,x_{0,n})$ is the package solution to the probabilistically unconstrained problem $Q^D(S)$. 
%$ is the \LCVaR of the probabilistically unconstrained package $X^{\text{D}}$, in the lower $\alpha$ tail.
We thus need to search for the ideal values of $\alpha'$ and $V'$ between the limits $[\alpha, 1]$ and $[V_0, V]$ respectively. Note that, given a set $\mathcal{O}$ of optimization scenarios, we can approximate $V_0$ using Algorithm~\ref{alg:estCVaR}: 
\begin{equation}\label{eq:defVL}
\hat V_0=\sum_{i=1}^n \textsc{EstimateCVaR}(\alpha,t_i.A,\mathcal{O})*x_{0,i},
%\widehat{\text{CVaR}}_\alpha(t_i.A)*x_{0,i}.
\end{equation}
% where $\widehat{\text{CVaR}}_\alpha$ is an estimate of $\text{CVaR}_\alpha$ computed as in Algorithm~\ref{alg:estCVaR}.
% \azza{What if to avoid yet another CVaR notation and to make the reference super clear we just state: \\
%$\hat V_0 = \sum_{i=1}^n \textsc{EstimateCVaR}(\alpha, m, t_i.A)*x_{0, i}$
%}

%Figure~\ref{fig:cvarif-intuition} shows how \lcsolve finds the appropriate $(\alpha', V')$ combination. 
\smallskip\noindent\textbf{Alternating parameter search.} The RCL process works as follows. The first package generated by \textsc{QuickSolve}, $X^{\text{D}}$, can be viewed as being formed from a query having the trivial \LCVaR constraint with parameters $(\alpha, V_0)$. If \lcsolve is not terminated early by \textsc{QuickSolve}, then $X^{\text{D}}$ is validation-infeasible, meaning that we need a more restrictive \LCVaR constraint. This is done via a \emph{$V$-search}, that is, by increasing $V'$, via bisection, up to the minimum value for which the corresponding package is validation-feasible, while keeping $\alpha'$ unchanged. (Increasing $V'$ further would reduce the objective value.) To get better objective values, we then make the \LCVaR constraint less restrictive via an \emph{$\alpha$-search}, that is, by increasing $\alpha'$, via bisection, up to the maximum value for which the resulting package remains validation-feasible. Note that the search interval $[V_0,V]$ for $V'$ is a continuous interval, so that the bisection process terminates when the bisection bounds $V_L$ and $V_U$ satisfy $V_U-V_L\le\delta$ for a small positive constant $\delta$. (In our experiments we found that $\delta=10^{-3}$ was an effective and robust choice. \peter{Fix as needed.}) In contrast, the $\alpha$-search examines a discrete set of values $\alpha=\alpha_1<\alpha_2<\cdots<\alpha_q=1$ in the interval $[\alpha,1]$, where $\alpha_j=\min\{y:\lfloor y|\mathcal{O}|\rfloor=\lfloor \alpha_{j-1}|\mathcal{O}|\rfloor+1\}$ for $j>1$. These are the successive values at which exactly one additional optimization scenario is used to create the estimated \LCVaR coefficients for each tuple, hence changing the approximating ILP. Equivalently, we can write $\alpha_j=(\lfloor \alpha_{j-1}\rfloor+1)/|\mathcal{O}|$.

After the above $\alpha$-search terminates at some value $\alpha'=\alpha_j$, we pivot back to adjusting $V'$---specifically, we increase the value of $\alpha'$ to $\alpha_{j+1}$.
%increase $\alpha'$ by the smallest amount possible to ensure that exactly one additional optimization scenario is used to create the estimated \LCVaR coefficients for each tuple. Specifically, we have been using $\lfloor \alpha' m\rfloor$ scenarios to estimate the coefficients, and we now increase $\alpha'$ by the smallest amount $\Delta$ such that $\lfloor (\alpha'+\Delta)m\rfloor= \lfloor\alpha' m\rfloor+1$; that is, $\Delta=(\lfloor\alpha' m\rfloor+1)/m$.
%\azza{I'm also having a hard time placing this with the logic that triggers NeedScenarios in the pseudocode and what follows from there.}\peter{Note that $m$ is not changing, only the fraction of the $m$ scenarios that are used to define the $\alpha'$-tail when estimating CVaR.}
Since $\alpha_j$ was the largest confidence value to produce a validation-feasible package, the new value of $\alpha'=\alpha_{j+1}$ leaves us with an \LCVaR constraint that is too relaxed---the package resulting from it is necessarily validation-infeasible. We then increase $V'$ via a $V$-search (using the new value of $\alpha'$) to regain validation-feasibility, then increase $\alpha$ via an $\alpha$-search to improve the objective value as much as possible while retaining validation-feasibility, and so on. The process is repeated until either we cannot increase $\alpha'$ further, i.e., $\alpha'=\alpha_q=1$, or we cannot increase $V'$ further, i.e., $V'\ge V-\delta$, where for simplicity we use the same value of $\delta$ as for the bisection termination parameter. 

%both $V'$ and $\alpha'$ ``converge''---i.e., the distances $|V_u-V_l|$ and $|\alpha_u-\alpha_l|$ between upper and lower bisection bounds are both less than or equal to a specified tolerance $\delta$. \peter{Riddho: Is this correct?}\azza{how to set this threshold parameter?} \riddho{This is correct for $V$-searches, for $\alpha$-search, we simply find the largest $\alpha$, such that for any $\alpha' > \alpha$, $\lfloor \alpha' m \rfloor > \lfloor \alpha m \rfloor$, which will cause the corresponding package to be infeasible. $\alpha$-search is occurring over a discrete domain, while $V$-search is along a continuous one, so we still need to specify this threshold $\delta$ for $V$. We don't quite have a systematic method for setting this parameter. I wonder if we should change the definition of $\delta$ to be some multiple of the initial search range. That is, our search terminates when $|V_u-V_l| \leq \delta * |V^0_u-V^0_l|$, [$V^0_l$,$V^0_u$] being the initial search range, and show experimental results with a small $\delta$, e.g. $10^{-3}$}. 


%---or if a bisection along either parameter does not result in an increased objective value.
%This happens if $V'$ equals $V$ in the original risk constraint being replaced, or if $\alpha'$ equals $1$,

\smallskip\noindent\textbf{Multiple risk constraints.} In the case of multiple risk constraints, the search starts with the non-NULL package $X^{\text{D}}$ returned by \textsc{QuickSolve}, for which one or more of the risk constraints $r\in Q$ are validation-violated. The search then increases these problematic $V'$ values via individual $V$-searches until all the SPQ constraints are validation-satisfied. These $V$-searches are synchronized in that, at each search step, a bisection step is executed for each $V'$ value and then the resulting set of risk constraints are checked for validation-satisfaction. The $V$-search terminates when bisection has ceased for all of the problematic constraints due to convergence.\footnote{In theory, an initially non-problematic constraint might become problematic during the $V$-search, but we did not observe this behavior in any of our experiments. In any case, one can modify the algorithm slightly to deal with this rare situation; see Appendix~X.} 
%\azza{adjusting via bisection and "as minimally as possible" seem rather contradictory to me.}. I.e., at each bisection step, the individual $V'$ values are adjusted up or down \azza{Do we ever go down? Now I'm confused! or are you referring to the ranges} as appropriate, until all of them converge: $\Vert V_U-V_L\Vert_\infty\le\delta$. \azza{actually what is appropriate here?} Note that after a $V'$ value for a given constraint converges, it is no longer adjusted during this phase of the search. After all $V'$ values converge,
When the $V$-search terminates, the RCL procedure next increases each of the $\alpha'$ values as described above, and commences a set of synchronized $\alpha$-searches, and the two types of search alternate as before until no further adjustments to the $\alpha'$ or $V'$ values is possible.


%and then executing an , as before, adding an increment $\Delta$increasing first doing a minimal increment to incorporate an additional scenario, causing one or more of the constraints to be validation-violated, then the $V'$ values get adjusted, and so on, until all values converge.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/CVaRification - Staircase Search .jpg}
%     \caption{\cvarif's staircase-like search finds the appropriate ($\alpha', V'$) combination. It repeatedly finds the minimal $V'$ for which the resulting package is validation-feasible keeping $\alpha'$ fixed, and then, the maximal $\alpha'$ for which the resulting package remains feasible, keeping $V'$ unchanged. Here, an ``X'' or an ``O'' denotes an ($\alpha', V'$) combination resulting in a feasible or infeasible package respectively.}
%     \label{fig:cvarif-intuition}
% \end{figure}

% The search procedure, as shown out in Figure~\ref{fig:cvarif-intuition}, charts out a staircase-like path, where all points above the staircase have more restrictive values of $V'$ than packages considered within the staircase, and hence result in more sub-optimal packages. All points below the staircase are bounded to the left by a point in the staircase that has a more-restrictive value of $\alpha'$, yet resulted in an infeasible package. Thus, the ($\alpha'$, $V'$) combinations in these points will also result in infeasible packages, owing to less  restrictive $\alpha'$-s.

\smallskip\noindent\textbf{Increasing the number of optimization scenarios.} 
We have been assuming that the initial number $m$ of scenarios is sufficiently large so that the SAA ILP well approximates the true stochastic package query, but this may not be the case in general.  Therefore, right after each (synchronized) bisection step during a $V$-search or $\alpha$-search, the RCL process examines the intermediate package corresponding to the new set of constraints just produced. If there is a significant relative difference between any VaR, CVaR, or expected sum
%, or expected objective value when computed over the optimization scenarios and
when computed over the validation scenarios,
%with respect to any stochastic attribute among the optimization scenarios has a large relative difference with those metrics among the validation scenarios,
then it follows that SAA approximation is poor.
%the set of optimization scenarios we currently have is not accurately representing the larger set of validation scenarios.
Specifically, if any relative difference is larger than a specified parameter $\beta$, the bisection and the staircase search terminates immediately, with the boolean flag \textsf{NeedsScenarios} set to true. (In our experiments, we take $\beta=\epsilon$.) We then increase the number of scenarios and restart the RCL process. If the number of optimization scenarios becomes equal to the number of validation scenarios, we terminate the algorithm and return the best solution so far.

\smallskip\noindent\textbf{Termination.} Furthermore, if any intermediate package satisfies all constraints in $Q(S)$ and is near-optimal, then we return the package immediately instead of continuing with the RCL search, setting the variable status.Done to \texttt{True}. To determine if a package is near-optimal, we find out if its objective value (as measured using the validation scenarios) equals or exceeds $(1-\epsilon)\omega$, where $\omega$ is the objective value of the optimal package. Since $\omega$ cannot be determined exactly, we use an upper bound $\omegaU\ge \omega$, so that any package with objective value above $(1-\epsilon)\omegaU$ will have an objective value above $(1-\epsilon)\omega$. One simple choice for $\omegaU$ is $\omega_0$---the objective value of the probabilistically unconstrained package $X^{\text{D}}$. Since the feasible region for $Q^{\text{D}}(S)$ is at least as large as that for $Q(S)$, we have $\omega_0 \geq \omega$. We use heuristics as in \cite[Sec.~5.4]{BrucatoYAHM20} to tighten (i.e., decrease) $\omegaU$. For example, whenever we encounter a package $X'$ during the RCL process that is validation-infeasible with respect to all the constraints, we compute the corresponding upper bound $\omega'$ and set $\omegaU\gets\min(\omega',\omegaU)$. This works because any validation-feasible package, including the optimal package, would be obtained by tightening every constraint in $X'$, and hence would have a lower objective value than $\omega'$, so that $\omega'$ is indeed an upper bound. Interestingly, in our experiments, we found that the simple upper bound $\omega_0$ would usually be the tightest \anh{Also this is counter-intuitive as if you are saying your $X'$ objective has better objective than $X^D$ assuming that you include all the deterministic constraints when solving for $X'$.} bound.\anh{Counter-example \includegraphics[width=0.5\textwidth]{figures/counter.drawio.png}}\azza{To eliminate yet another variable that we are searching over, can we move this exposition to the appendix and simply state that we set omega to the unconstrained version.}

\azza{We have 4 reasons to terminate: we hit $\alpha = 1$ or $\alpha$ converges --- honestly it isn't clear, $V_u - V_l < \delta$, optimization = validation scenarios, we are near optimal. Which of these do we always hit first?! If it is the optimality one as it ideally should be, can we simplify the complexity of RCL-solve? Or at least the complexity of how we explain how it works? After reading this a number of times, it is dense ... and one can easily get lost in the details as I might be now. }

\azza{Also, are the 3 conditions excluding (optimization=validation) always tested at every search and that triggers status.Done?}\azza{After reading the summary, it appears so but is the expectation that we don't look at the pseudocode until the summary? }

\azza{I tried to refer to the line numbers from within the text. I was only successful doing line 1 in the quicksolve paragraph... Can we try and refer to line numbers where appropriate from the text above. }

\azza{Again as with Alg 1, in Alg 2, we can either use $|O|$ for $m$ with it as an explicit input and $|V|$ for $\hat m$. }

\azza{I know the intention was to hide much of the complexity under V-Search and $\alpha$ search, I worry we may have gone too far...}

\smallskip\noindent\textbf{Summary.} Algorithm~\ref{alg:lcsolve} summarizes the \lcsolve method at a high level---the algorithm returns a . In general the set of risk constraints $R$ appearing in $Q$ satisfies $|R|>1$, so that quantities such as $V$ and $\alpha$ are vectors; indeed, the function \textsc{GetParams} parses the query $Q$, extracts the values $V_r$ and $\alpha_r$ for each constraint $r\in R$, and organizes the values into the vectors $V$ and $\alpha$. With $\alpha'$ fixed, the \textsc{V-Search} function implements the search for the smallest values (component-wise)  of $V'\in[V_L,V_U]$ for which each constraint in the resulting SPQ is validation-satisfied. After a bisection step, it immediately terminates if either (i) it detects the need for more optimization scenarios, in which case it sets the variable status.NeedScenarios equal to True, and (ii) if the package solution $X$ corresponding to the SPQ with the current values of $V'$ and $\alpha'$ is validation-feasible and near-optimal, in which case it sets the variable status.Done equal to True. Otherwise the algorithm terminates when all of the $V'$ values have converged as defined above, and proceeds to the search for $\alpha'$. The function \textsc{$\alpha$-Search} behaves similarly, but, for $V'$ fixed, implements the search for the largest values of $\alpha'\in[\alpha,1]$ (component-wise) for which each constraint in the resulting SPQ is validation-satisfied. For simplicity, our pseudocode assumes that we use the simplest upper bound $\omegaU=\omega_0$ as described above, which is computed via the \textsc{OmegaUpperBound} function in line~\ref{li:EstObjVal}. In more complex versions of the algorithm, the value of $\omegaU$ would be updated by the \textsc{V-Search} and \textsc{$\alpha$-Search} functions.

% \begin{algorithm}[t]
% \caption{\textsc{GetMinimalV}}\label{alg:minV}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Statex $S :=$ A set of tuples tuples
% \Statex scenarios $:=$ A set of optimization scenarios
% \Statex $\alpha' :=$ List of $\alpha'$ paremeters for \LCVaR constraints
% \Statex $V_l :=$ Lower bounds of $V'$ parameters for \LCVaR constraints
% \Statex $\delta :=$ Bisection termination distance
% \Statex $\epsilon :=$ Error Approximation Bound
% \Statex $\omega_0 :=$ Objective value of probabilistically unconstrained package
% \Statex \textsf{MoreScenarios} $:=$ True if more optimization scenarios can be generated
% \Ensure \textsf{Package} $:=$ A near-optimal and validation-feasible package for $Q(S)$, if found
% \Statex \textsf{NeedsScenarios} $:=$ True if more optimization scenarios are needed, False by default
% \Statex \textsf{MinV} $:=$ The minimal $V'$ for feasibility, in no near-optimal package is returned
% \State $V_u :=$ List of $V$ in each VaR/CVaR constraint
% \While{$||V_u - V_l||_{\infty} \geq \delta$}
% \State $V_m := (V_u + V_l)/2$
% \State $Q_m :=$ \textsf{ReplaceRiskConstraints}($\alpha', V_m$)
% \State $X :=$ \textsf{IlpSolver}($Q_m$).\textsf{Solve}()
% \If{\textsf{ValidationFeasible}($X$) and \textsf{Is$\_\epsilon\_$Optimal}($X$, $\omega_0$)}
% \State \Return $\{$\textsf{Package}$= X\}$
% \EndIf
% \If{\textsc{HighDiffOptimizationAndValidation}($X$, $\epsilon$) and \textsf{MoreScenarios}$=$\textsf{True}}
% \State \Return $\{$\textsf{NeedScenarios}$=$\textsf{True}$\}$
% \EndIf
% \For{each risk constraint $r \in Q$}
% \If{$r.$\textsc{ValidationFeasible}($X, \epsilon$)}
% \State $V^{r}_u = V^{r}_m$
% \Else
% \State $V^{r}_l = V^{r}_m$
% \EndIf
% \EndFor
% \EndWhile
% \State \Return $\{$\textsf{MinV}$=V_{m}\}$
% \end{algorithmic}
% \end{algorithm}




% \begin{algorithm}[t]
% \caption{\textsc{\lcsolve}}\label{alg:cvarification}
% \begin{algorithmic}[1]
% \Require $Q :=$ A Stochastic Package Query
% \Statex $S :=$ Set of stochastic tuples in the SPQ
% \Statex $m :=$ Initial number of optimization scenarios
% \Statex $\hat{m} :=$ Number of optimization scenarios
% \Statex $\delta :=$ Bisection termination distance
% \Statex $\epsilon :=$ Approximation bound

% \State \textsf{qsSuccess}, $X^{\text{D}} \gets $\textsf{QuickSolve}(Q, S)
% \If{\textsf{qsSuccess} is \textsf{True}}
% \State \Return $X^{\text{D}}$ \Comment{Either $Q(S)$ solution or NULL}
% \EndIf

% \State $V_l \gets \textsf{ComputeLowestBoundValues}(Q, X^{\text{D}})$

% \State $\alpha_l \gets \textsc{GetProbabilityValues}(Q)$

% % \State $d_e \gets 1$ \Comment{{\color{gray}\textit{Exponential search's initial distance}}}
% % \While{true} \Comment{{\color{gray}\textit{Exponential search}}}
% %     \State $L \gets V-d_e$
% %     \State $Q'' \gets \textsc{SetBoundValues}(Q', L)$
% %     \If{\textsc{IsUnsolvable}($Q''$)}
% %         \State \textbf{break}
% %     \EndIf
% %     \State $d_e \gets 2d_e$
% % \EndWhile

% \State $X^* \gets \text{NULL}$
% \State $\text{scenarios} \gets \emptyset$

% \While{\textsc{Is\_$\epsilon$\_Optimal}($Q, X^*, \epsilon$) \textbf{and} \textsc{IsFeasible}($Q, X^*, \hat{m}$)}
%     \State $\text{scenarios} \gets \text{scenarios} \cup \textsc{GenerateScenarios}(\text{tuples}, m)$
%     \State $Q' \gets \textsc{SetCoefficients}(Q,L_P,\text{scenarios})$
%     \State $R_V \gets \textsc{GetBoundValues}(Q)$
%     \State $L_V, R_V, X_V \gets \textsc{BinarySearchOnV}(Q', \delta, L_V, R_V)$
%     \If{$X_V$ != \text{NULL}}
%         \State $X^* \gets X_V$
%     \EndIf
    
%     % \While{$\max |R_V-L_V| > \delta$} \Comment{{\color{gray}\textit{Binary search on $V$}}}
%     %     \State $M_V \gets (R_V+L_V)/2$
%     %     \State $Q'' \gets \textsc{SetBoundValues}(Q', M_V)$
%     %     \If{\textsc{IsUnsolvable}($Q''$)}
%     %         \State $R_V \gets M_V$
%     %     \Else
%     %         \State $X \gets \textsc{ILPSolver}(Q'')$
%     %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
%     %             \State $X^* \gets X$
%     %             \State $R_V \gets M_V$
%     %         \Else
%     %             \State $L_V \gets M_V$
%     %         \EndIf
%     %     \EndIf
%     % \EndWhile

%     \State $Q' \gets \textsc{SetBoundValues}(Q, L_V)$
%     \State $R_P \gets 1$
%     \State $L_P, R_P, X_P \gets \textsc{BinarySearchOnP}(Q', \delta, L_P, R_P)$
%     \If{$X_P$ != \text{NULL}}
%         \State $X^* \gets X_P$
%     \EndIf
%     % \While{$\max |R_P-L_P| > \delta$} \Comment{{\color{gray}\textit{Binary search on $P$}}}
%     %     \State $M_P \gets (R_P+L_P)/2$
%     %     \State $Q'' \gets \textsc{SetCoefficients}(Q',M_P,\text{scenarios})$
%     %     \If{\textsc{IsUnsolvable}($Q''$)}
%     %         \State $L_P \gets M_P$
%     %     \Else
%     %         \State $X \gets \textsc{ILPSolver}(Q'')$
%     %         \If{\textsc{IsFeasible}($Q,X,\hat{m}$)}
%     %             \State $X^* \gets X$
%     %             \State $L_P \gets M_P$
%     %         \Else
%     %             \State $R_P \gets M_P$
%     %         \EndIf
%     %     \EndIf
%     % \EndWhile

%     \State $m \gets 2m$
%     \If{$m > \hat{m}$}
%         \State \textbf{break}
%     \EndIf
    
% \EndWhile
% \State \Return $X^*$

% \end{algorithmic}
% \end{algorithm}

% Letting $\alpha'$ and $V'$ denote the adjusted parameters, observe that each \LCVaR constraint is linear w.r.t. the $x_i$'s, and remains so in the SAA approximation when each $\text{CVaR}_{\alpha'}(t_i.A)$ is approximated by averaging over scenarios with the lowest values (as is done in Algorithm~\ref{alg:estCVaR}). Because all other types of SPaQL constraints, along with their SAA approximations, are also linear w.r.t. the $x_i$'s, \cvarif leads to an ILP formulation whose size is independent of the number of scenarios, as desired. The approximation proceeds by converting all VaR and CVaR constraints to \LCVaR constraints. We next describe this process in detail, and Section~\ref{sec:experimental_evaluation} demonstrate the performance improvements over \ssearch due to \cvarif.

==> sections/old_files/spq-old.tex <==
\section{Scaling stochastic package queries: Overview and preliminaries}
\label{sec:prob}
%\azza{After discussion, we agreed to remove prelim entirely. We will merge in the SPQ para into here. What I'd like very clearly done here is a clear definition of every type of constraint and clarity that all probabilistic constraints are VaR constraints. For each of these definitions, please include the equivalent SPaQL clause that captures it. In the clause use $v, p$ so that it is easy to grasp.}

% \cprotect\azza{Please use {\verb!\mintinline{sql}{spaql clauses}!} when inlining spaql code/phrases.} \anh{done}

In this section, we review the syntax for \spaql constraints
%constraint constructs, 
and introduce language extensions to handle CVaR constraints.  We discuss the relationship between CVaR and VaR constraints, and provide the main insights for transforming VaR constraints to CVaR (\cvarif).  We also describe the challenges and insights for scaling stochastic package evaluation through the combination of \cvarif and \sskr. 

\smallskip\noindent\textbf{\spaql constraint modeling.}
We assume a relation with $n$ tuples. In SPQ evaluation, each tuple $t_i$ is associated with an integer variable $x_i$ that represents the tuple's multiplicity in the package result. A \emph{feasible package} is an assignment of the variables $\{x_1, \dots, x_n\}$, such that all query constraints are satisfied; as in the introductory example, we typically want to find a feasible package that maximizes or minimizes a given objective function.
% SPQ processing assigns a multiplicity $x_i$ to each tuple $t_i$ in a relation, with $x_i \geq 0$ denoting how many times a package includes $t_i$. In an $n$-tuple relation, processing an SPQ requires finding an optimal assignment of $\{x_1, \dots, x_n\}$ such that all constraints in the query are satisfied. 
We review here the different types of \spaql constraints and their mathematical semantics; see translations; see~\cite{BrucatoYAHM20} for a full SpaQL language description. 
%\matteo{maybe use ``semantics'' rather than mathematical translations?}, and refer the reader to the original work for the full language specification~\cite{BrucatoYAHM20}:

% \alexandra{Not sure this level of detail is necessary. How much do we need to review here?}

% \anh{Two issues: (1) Overloaded notation of $P$ here: $P$ as Package in COUNT(P.*) or $P$ as LOWEST $P\%$ (2) Inconsistency: $V$ as notation for bound value in SPAQL language but we use $v$ as bound value in description of theorems and algorithms.}
\begin{itemize}[leftmargin=*]
    \item {\small\mintinline[breaklines,bgcolor=bg]{sql}{REPEAT R}}: \emph{Repeat constraints}  cap the multiplicities of every tuple to $1+R$, i.e., $x_i \leq (1+R)$, $\forall 1 \leq i \leq n$.
    \item {\small\mintinline[breaklines,bgcolor=bg]{sql}{COUNT(Package.*) <= S}}: \emph{Package size constraints} bound the total number of tuples, i.e., $\sum_{i=1}^{n} x_i \leq S$.
    \item {\small\mintinline[breaklines,bgcolor=bg]{sql}{SUM(A) <= V}}: \emph{Deterministic constraints} bound the sum of the values of a deterministic attribute  $A$ in the package. If $t_i.A$ represents the value of $A$ in tuple $t_i$, the constraint translates to $\sum_{i=1}^{n}  t_i.A * x_i \leq V$.
    \item {\small\mintinline[breaklines,bgcolor=bg]{sql}{EXPECTED SUM(A) <= V}}: \emph{Expected sum constraints} bound the expected sum of a \emph{stochastic} attribute $A$ in the package. If $t_i.A$ represents the random variable for $A$ in a tuple $t_i$, the constraint becomes $\mathbb{E}[\sum_{i=1}^{n} t_i.A*x_i] \leq V$.
    \item \frbox{\small \lstinline!SUM(A) <= V WITH PROBABILITY <= P!}:
    %{\small\mintinline[breaklines,bgcolor=bg]{sql}{SUM(A) <= V WITH PROBABILITY <= P}}: 
    \emph{VaR constraints} bound the probability that the sum of $A$ is below or above a value, i.e., $\Prob(\sum_{i=1}^{n} t_i.A * x_i \leq V) \leq P$.
\end{itemize}

\smallskip\noindent\textbf{Increasing risk expressivity with CVaR constraints.}
VaR constraints cannot sufficiently express different forms of risk tolerance.  In the example \spaql query of Figure~\ref{fig:portfolio-builder}, the VaR constraint bounds the probability that the loss will be more than \$10, but it does not bound the expected loss in worst-case scenarios. So, while it makes the loss less likely, the amount of loss is unbounded in unfavorable scenarios.\matteo{It would be good to tie this to the example query. For example, in the event the investor loses more than \$10, which only happens with a 5\% probability, they can lose much more than just \$10, without any way to control how much is lost on average} \anh{For example, 1\% I lose $a$\$ while 99\% I gain $b$\$. So CVaR of the lower 5\% is simply $(-0.01a+0.04b)/0.05=-0.2a+0.8b$. I can make the CVaR unbounded by increasing the loss $a$. However, $\Pr(Gain < 0)$ is always 1\%}.  We propose\matteo{We should first acknowledge that CVar constraints are a known approach (not our proposal) for this exact problem. We are merely extending the language to allow them in package queries} the following language extension:
\begin{itemize}[leftmargin=*]
    \item {\small\mintinline[breaklines,bgcolor=bg]{sql}{EXPECTED SUM(A) >= V IN LOWER P TAIL}}\matteo{I'm not a fan of referring to ``scenarios'' in the language. Not super declarative, in the sense that, so far, nothing in the language made any reference to ``scenarios''. Var says ``with probability'' not ``fraction of scenarios''. Also, we say ``EXPECTED'', not ``AVERAGE'', for the same reasons. I'd suggest something like IN LOWEST D\% [[OF?] CASES]. I'd also not use P again since it's not a probability value like in Var. Also, does the language allow for ``HIGHEST D\% CASES''? Also, what would this constraint look like in the portfolio query?}:\\
    \emph{Conditional Value at Risk (CVaR) constraints} bound the average sum of $A$ in the package in the lower $P$ fraction of the values in the sum distribution.
\end{itemize}

% VaR constraints alone may not be enough to comprehensively express a user's risk tolerance. Consider the \spaql query in Figure~\ref{subfig:example_spaql}. The VaR constraint in it prohibits the resulting package from having losses of more than $10\$$ in more than $5\%$ of scenarios. This, however, does not bound the potential financial damage in the $5\%$ of worst-case scenarios. A CVaR constraint limiting the average losses in these scenarios would prevent packages with high tail-losses from being returned.
% \spaqlp, our \spaql extension, allows specifying \emph{Conditional Value-At-Risk} (CVaR) constraints as: \\
% \noindent\mintinline[breaklines]{sql}{EXPECTED SUM(A) >= V IN LOWEST P FRACTION OF SCENARIOS}

CVaR constraints add important expressivity to \spaql, as they allow users to control \anh{the expected} risk over worst-case scenarios that lie beyond the coverage of VaR constraints~\cite{alexander2004comparison, krokhmal2002portfolio, Sarykalin2008}.
Mathematically, they translate to $\mathbb{E}[S | S \leq F_S^{-1}(P)] \leq V$, where $S=\sum_{i=1}^{n} t_i.A * x_i$ is the sum of $A$ in the package and $F_S^{-1}$ is its inverse CDF. Users can specify each type of constraint with alternative inequalities (i.e., $\geq$ instead of $\leq$).

\smallskip
\noindent
\textbf{VaR constraints increase complexity.}
If all constraints and the objective\footnote{SPQ objectives maximize (or minimize) sums of deterministic or stochastic attributes: \mintinline[breaklines]{sql}{MAXIMIZE SUM(A)} and \mintinline[breaklines]{sql}{MAXIMIZE EXPECTED SUM(A)}, respectively, with mathematical formulations: $\argmax_{x_1, \dots, x_n} \sum_{i=1}^{n} t_i.A * x_i$ and $\argmax_{x_1, \dots, x_n}\mathbb{E}[\sum_{i=1}^{n} t_i.A * x_i]$, respectively.} in an SPQ can be expressed as linear combinations of the decision variables $\{x_1, \dots, x_n\}$, the optimization problems can be solved using off-the-shelf ILP solvers like Gurobi. This is good news, as ILPs take less time to solve than non-convex integer programs~\cite{Hong2014}. Repeat, package size, and deterministic constraints, and objectives on deterministic attributes are all readily expressed as linear combinations. Expected sum constraints and objectives can also be expressed as linear combinations using the linearity of expectation, that is, $\mathbb{E}[\sum_{i=1}^N t_i.A*x_i]=\sum_{i=1}^N\mathbb{E}[ t_i.A]x_i$. During Sample Average Approximation (SAA), we use $m$-scenarios, and use the average of $t_i.A$ across these scenarios as coefficients for the expected sum constraints and objectives. 

% SPQs can maximize the sums of both deterministic and stochastic attributes. For deterministic attributes, objectives like `\mintinline[breaklines]{sql}{MAXIMIZE SUM(A)}' are formulated as $\argmax_{x_1, \dots, x_n} \sum_{i=1}^{n} t_i.A * x_i$. Objective on stochastic attributes are expressed as `\mintinline[breaklines]{sql}{MAXIMIZE EXPECTED SUM(A)}' and formulated as $\argmax_{x_1, \dots, x_n}\mathbb{E}[\sum_{i=1}^{n} t_i.A * x_i]$. Objectives can also require minimizing the (expected) sums. 



%\riddho{Placing the following passage from the previous preliminary section, need to edit it}
%\textbf{Stochastic Package Queries} (SPQs)~\cite{BrucatoYAHM20} extend PQs by allowing probabilistic constraints and objectives. In a probabilistic relation of $N$ tuples, we denote $t_i.\mathbf{A}$ as the random variable of stochastic attribute $\mathbf{A}$ of tuple $t_i$ ($i \in \{1,\dots,N\}$), for example, the gain of a particular stock are particular period of time. An example of a probabilistic constraint with respect to this gain could be: $\Pr(\sum_{i=1}^N t_i.\mathbf{A}\, x_i \leq -10) \leq 0.05$, i.e., the probability of an at-least-ten-dollar loss of the stock portfolio is at most $5\%$. Here $x_i \geq 0$ is the multiplicity of tuple $t_i$, i.e., how many stocks one would purchase and sell after a given number of dates. Therefore, an SPQ requires finding a package $\{x_1,\dots,x_N\}$ that satisfies:~(i)~all deterministic constraints such as the investment budget being capped at one thousand dollars, i.e., $\sum_{i=1}^N t_i.P\, x_i \leq 1000$ ($P$ denoting price of a tuple)~(ii)~all probabilistic constraints such as the aforementioned Value-at-Risk (VaR) constraint. \azza{aforementioned ... this is too stuffy! but more importantly, where was it aforementioned? You don't actually say that the probabilistic constraint is in fact a Value at Risk constraint. This needs to be explicitly stated!} In this paper, we introduce a new type of risk constraint in SPQs called Conditional Value-at-Risk (CVaR) constraints~\cite{Sarykalin2008} (Section~\ref{sec:prob}) which constrain tail risks for packages and can conveniently be used to solve SPQs containing VaR constraints quickly, as we show in Section~\ref{sec:cvarif}.


%Packages formed in response to SPQs optimally assign a multiplicity $x_i$ to each tuple $t_i$ in an $N$-tuple relation, subject to all constraints being satisfied \azza{Its important to say that $x_i$ is the decision variable}. The types of probabilistic constraints supported by \spaqlp are~(i)~Expected sum constraints,~(ii)~Value-at-Risk (VaR) constraints, and~(iii)~Conditional Value-at-Risk (CVaR) constraints. An expected sum constraint limits the expected sum of a stochastic attribute (say $\textbf{A}$) to being above (or below) a given threshold (say $v$)\azza{Why say A or say v? Just be precise!}. Such constraints can be trivially expressed as linear combinations of the values of $x_i$ using the linearity of expectation, that is, $\mathbb{E}[\sum_{i=1}^N t_i.\textbf{A} \,x_i]=\sum_{i=1}^N\mathbb{E}[ t_i.\textbf{A}]x_i \leq (\geq) v$ where $t_i.\textbf{A}$ denotes the random variable corresponding to attribute \textbf{A} in tuple $t_i$. In the remainder of this section, we discuss how we handle VaR and CVaR constraints in SPQs. \azza{$x_i$ preceding $t_i$ is clearer as in many ways $x_i$ is the decision variable. As notation, a bold \textbf{A} is very distracting especially since it just represents the coefficient brought in by the tuple. Please use a softer symbol}

VaR constraints, however, are trickier to linearize. Without loss of generality, let's assume all VaR constraints have the form\footnote{Appendix~\ref{appendix:interchangeable} shows how to convert other VaR forms to this.}:\\
\noindent
{\small\mintinline[breaklines]{sql}{SUM(A)<=V WITH PROBABILITY <= P}},
which is equivalent to $\Pr(\sum_{i=1}^N t_i.A*x_i \leq V) \leq P$.
VaR constraints are non-linear and non-convex with respect to the multiplicities $x_i$ and are thus harder to optimize~\cite{xi2012gradual} (more details in Appendix~\ref{appendix:non-linearity}).

% and all CVaR constraints have the form: \\
% \noindent\mintinline[breaklines]{sql}{EXPECTED SUM(A)>=V IN LOWEST P FRACTION OF SCENARIOS},
% which is equivalent to $\mathbb{E}[S| S\leq F_S^{-1}(P)] \geq V$. 

% Appendix~\ref{appendix:interchangeable} shows how to convert risk constraints of other forms to these forms. VaR constraints are non-linear and non-convex w.r.t. the multiplicities $x_i$ and are thus harder to optimize~\cite{xi2012gradual}. Appendix ~\ref{appendix:non-linearity} explains why. 

\smallskip
\noindent
\textbf{Decreasing complexity\matteo{[of Var constraints]} with \cvarif.}
In contrast with VaR constraints, CVaR constraints \emph{can} be linearized.\footnote{Existing approaches to CVaR-constrained optimization are iterative processes. The number of iterations and the cost per iteration both scale linearly with the number of decision variables, resulting in an overall quadratic time complexity wrt the number of tuples~\cite{bubeck2015convex}. These techniques are thus impractical for processing SPQs addressed on million-tuple relations.}   \azza{The switch from $\geq V$ to $\leq V$ is disorienting.}
With slight abuse of notation, let us use $CVaR_{P}(X) \leq V$ to denote the CVaR constraint {\small\mintinline[breaklines]{sql}{EXPECTED SUM(A) <= V IN LOWEST P FRACTION OF SCENARIOS}}. A linearization of this constraint breaks down the left-hand side: $\sum_{i=1}^{n}CVaR_{P}(t_i.A)*x_i \geq V$. Since $CVaR_{P}(t_i.A)$ is a real-number, this results in a linear constraint in the optimization problem, regardless of how many scenarios there are. Unlike VaR constraints, no indicator variables are needed.  As the following theorem shows, 
any package that satisfies the linearized constraint, also satisfies the original CVaR constraint.\footnote{We provide proofs of all theorems in the Appendix.}
\begin{theorem}[Subadditivity of CVaR]
    For any package $X=\{x_1, \dots, x_n\}$ and $P \in (0, 1]$, the following holds:
    $$\sum_{i=1}^{n} \text{CVaR}_{P}(t_i.A)*x_i \geq V \implies \text{CVaR}_{P}(X) \geq V$$
    \label{theorem:cvar}
\end{theorem}
\azza{Without making any edits here in case Alexandra has a major rewrite in mind. The same comment from 2.1 holds, the statement of the theorem should match the goal. You want somehow to state Linearized CVaR is more "conservative" than CVaR and you want those terms to be in it.}
\alexandra{I kept the notation and theorem statement unchanged, because I don't have a better alternative right now, but I don't find them great.  Since we don't have a definition of ``linearized CVaR'', rather a description of the process, I am not sure we can reference it this way in the statement.} \azza{The more  I read throught these the more important it is to define linearized CVaR and CVaR and have the distinction/differences be crystal clear.}

We exploit the linearizability of CVaR constraints to remove the complexity of VaR constraints through a novel \cvarif process.  
\cvarif reformulates the SPQ by replacing any VaR constraints with CVaR. Consider the following VaR constraint in the \spaql query of Figure \ref{fig:portfolio-builder}:
{\small
\begin{minted}{sql}
SUM(Gain) >= -10 WITH PROBABILITY >= 0.95
\end{minted}
}
This VaR constraint tolerates more risk than the following CVaR constraint:
% \\
% \resizebox{\linewidth}{!}{\mintinline[breaklines]{sql}{EXPECTED SUM(Gain) >= -10 IN LOWEST 0.05 FRACTION OF SCENARIOS}}
{\small
\begin{minted}{sql}
EXPECTED SUM(Gain) >= -10 IN LOWEST 0.05 FRACTION OF SCENARIOS
\end{minted}
}

As the following theorem states, any package that satisfies the CVaR constraint, also satisfies the VaR constraint.
\begin{theorem}
\label{theorem:var}
    Any package that satisfies the CVaR constraint {\small\mintinline[breaklines]{sql}{EXPECTED SUM(A) <= V IN LOWEST P FRACTION OF SCENARIOS}}, also satisfies the VaR constraint \small\mintinline[breaklines]{sql}{SUM(A) <= V WITH PROBABILITY >= 1-P}.
\end{theorem}


% The above \emph{Conditional Value at Risk (CVaR)} constraint~\cite{alexander2004comparison} caps the expected loss in the worst cases (here, the scenarios with  profits in the lowest 5 percentile). A package satisfying this CVaR constraint also satisfies the former VaR constraint. Importantly, solving an optimization problem having only CVaR constraints requires less time than solving one with VaR constraints. We show in Section~\ref{sec:prob} that we can express each CVaR constraint with one linear constraint in the optimization problem, regardless of how many scenarios there are. Unlike VaR constraints, no indicator variables are needed. The optimization problems are thus integer linear programs (ILPs) that take less time to solve than non-convex problems~\cite{burer2012non}.


Of course, restricting risk via these conservative reformulations can over-constrain the problem, making it unsolvable or resulting in suboptimal solutions. We compensate by appropriately relaxing the CVaR bound ({\small\mintinline{sql}{EXPECTED SUM(Gain) >= ??}}). We use bisection to find the optimal bound value, which we describe in Section \ref{sec:cvarif}\matteo{Something that is missing is why we think there is a value for ??, in its search space (0 to P?), that can satisfy the Var constraints via a CVar constraint. Maybe there is no such ?? for some cases? Also, what do we mean by ``optimal'' bound value here?}.
Together, Theorems~\ref{theorem:cvar}~and~\ref{theorem:var} show that we can represent all risk constraints in a query as linear constraints with two sets of conversions. First, we convert all VaR constraints to CVaR constraints. Second, we convert all CVaR constraints to linearized CVaR constraints that can be solved quickly by in-market solvers. 
% The coefficients of linearized CVaR constraints are the values of $CVaR_P(t_i.A)$, the expected value of the random variables $t_i.A$ corresponding to the stochastic attribute $A$ of the tuples $t_i$ in the $P$-lower fractile of their distributions. Using SAA, this can be found trivially for a given tuple $t_i$ and attribute $A$ --- we sort all $m$ scenario values of $t_i.A$ in ascending order, and take the average of the lowest $\lfloor pm \rfloor$ values (Algorithm~\ref{alg:approx}).
Section~\ref{sec:experimental_evaluation} shows its performance improvements over \ssearch.

% To overcome non-linearity and non-convexity, we replace VaR constraints with convex CVaR constraints, i.e. we replace `\mintinline[breaklines]{sql}{SUM(A)<=V WITH PROBABILITY<=P}' with `\mintinline[breaklines]{sql}{EXPECTED SUM(A)>=V IN LOWEST P FRACTION OF SCENARIOS}'. Theorem \ref{theorem:var} proves that any package satisfying the CVaR constraint will also satisfy the VaR constraint.
% \begin{theorem}
% \label{theorem:var}
%     Let $S$ be any random variable, $F_{S}$ its cdf and $p$ be a probability value within  $(0,1]$. Then $$\mathbb{E}[S|S \leq F_{S}^{-1}(P)] \geq V \implies \Pr(S \leq V) \leq P$$
% \end{theorem}
% \begin{proof}
%     \sloppy By definition of conditional expectation, we have $$V \leq \mathbb{E}[S|S \leq F_{S}^{-1}(P)] \leq F_{S}^{-1}(P) \implies F_{S}(V) \leq P$$ $$\implies \Pr(S \leq V) \leq P$$
% \end{proof}
% \azza{The statement of the theorem should match the main goal: "A package satisfying a CVaR constraint (the form of it) satisfies the VaR constraint (the form of it)" Right now there is no context for where $S$ comes from or $F_S$, etc (even if you describe those 3 paras before, it is not held in a reader's main memory when they flit back to this theorem). You are not writing for an audience that is familiar with CVaR or stochastic package queries, and later when you refer back to these theorems, you want the readers to quickly get what they show.}

% \azza{I went over Alexandra's pass and made some minor typo fixes and edits and removed frameboxes to give us better control on spacing and replicated the style of introducing spaql constraints. I am assuming Alexandra's has a plan with what follows. So I'm jumping to 3 instead.}


\smallskip
\noindent
\textbf{SPQ evaluation.}
\cvarif alone cannot scale across the tuple dimension. We address this with a new evaluation mechanism, \sskr. \sskr maintains the high-level workflow of \skr~\cite{brucato2018package}. It partitions the data offline, and employs \cvarif to solve the sketch and refine SPQs. Unlike \skr, it is designed to overcome challenges raised by stochasticity. \sskr revisits \skr's approach to creating sketch packages using a single representative from each partition. When sketching optimal packages with several tuples from the same partition, the single representative strategy will need the sketch solver to include the same representative multiple times. However, we show in Section~\ref{section:sskr} that doing so in stochastic settings increases the risk of a package. To satisfy risk constraints, the solver might be forced to include tuples from suboptimal partitions in sketch packages. Suboptimal sketch packages consequently refined to suboptimal final packages. To overcome this, \sskr duplicates the representatives, and solves the sketch problem over all such duplicates. This allows the sketch solver to include multiple duplicates from each partition without inflating risks. During `Refine', every duplicate in the sketch package is replaced by actual tuples from their partition.  

To partition large probabilistic relations offline for \sskr, we propose \dpart, a trivially-parallelizable partitioning scheme. Unlike existing hierarchical stochastic data clustering approaches~\cite{gullo2017information, huang2021robust}, \dpart's time complexity is subquadratic with respect to the number of tuples in the relation. This makes it suitable for partitioning million-tuple relations.  We discuss \dpart in detail in Section~\ref{sec:dpart}.


 




% This key insight shows that packages satisfying SPQs containing VaR constraints can be found by solving convex optimization problems by first converting all VaR constraints to CVaR constraints. However, existing approaches to CVaR-constrained optimization are iterative processes. The number of iterations and the cost per iteration in them both scale linearly with the number of decision variables --- resulting in an overall quadratic time complexity w.r.t. the number of tuples~\cite{bubeck2015convex}. These techniques are thus impractical for processing SPQs addressed on million-tuple relations. 

% We overcome this by converting all CVaR constraints in an SPQ to a third form--- `linearized CVaR' constraints. Suppose, for a stochastic attribute $A$, a CVaR constraint requires the expected sum of a package $X=\{x_1, \dots, x_n\}$ to be over $V$ in the $P$-lower fraction of outcomes. With a slight abuse of notation, let us denote this constraint as $CVaR_{P}(X) \geq V$. A linearized CVaR constraint breaks down the left-hand side of this constraint into the sum of its parts. It adds up the individual CVaRs of each tuple in the package, $\sum_{i=1}^{n}CVaR_{P}(t_i.A)*x_i \geq V$, where $t_i.A$ represents the random variable for $A$ in the tuple $t_i$. The CVaR of each tuple $t_i$, $CVaR_{P}(t_i.A)$ is a real-number. Thus, the linearized CVaR constraint is a linear combination of the decision variables $\{x_1, \dots, x_n\}$, making it particularly useful when we try to formulate the SPQ as an ILP. We show in Theorem~\ref{theorem:cvar}, that the conversion from CVaR constraints to linearized CVaR constraints is conservative.

%We address this by `linearizing' all CVaR constraints in the query. We convert a CVaR constraint of the form $\mathbb{E}[X|X \leq F_{X}^{-1}(p)] \geq v$ to the `linearized CVaR constraint', $\sum_{i=1}^N \mathbb{E}[t_i.\textbf{A}|t_i.\textbf{A} \leq F^{-1}_{t_i.\textbf{A}}(p)]\,x_i \geq v$, where $X = \sum_{i=1}^N t_i.\textbf{A}\, x_i$. During sample average approximation, where we attempt to create packages from $m$ optimization scenarios, a linearized CVaR constraint is represented in an ILP by setting the average of the lowest $\lfloor pm \rfloor$ values of a tuple $t_i$ as the coefficient of its decision variable $x_i$. Thus, linearized CVaR constraints have the advantage of being representable in ILPs by single linear constraints, regardless of the number of scenarios used. Theorem \ref{theorem:cvar} shows that the conversion of CVaR constraints to linearized CVaR constraints is conservative, i.e., a package satisfying a linearized CVaR constraint is guaranteed to satisfy the corresponding CVaR constraint.

%\azza{I dislike the wrapping and unwrapping of X. We will use linearized CVaR from now on, so why represent the sum as a new random variable and then break it up later during linearization. } \anh{if we go with the consistency of not using X, then all the proofs and statements of writing $F_X^{-1}(p)$, $F_X(v)$, $E[X|X \leq F_X^{-1}(p)]$ are very verbose.}\azza{That's not entirely true. If you move 3.1 to appendix, then you can introduce that shorthand there and contain it to 3.1 where it matters the most. What's left is (1) of 3.3 that is again only if we keep it in the main paper, but even so using the fleshed out form does not cause verbosity!}

%Many convex optimization algorithms efficiently handle CVaRs but most of them are iterative methods with the number of iterations and the cost of each iteration scaling linearly with the number of tuples resulting in a quadratic complexity~\cite{bubeck2015convex}. This is not practical in SPQs addressed on relations having millions tuples. To overcome this, we further approximate CVaR by making it linearly separable using its subadditivity property \riddho{Should we provide some intuition as to what we mean by ``linear separability'' here, and why it helps?}, which states:
% \azza{Without making any edits here in case Alexandra has a major rewrite in mind. The same comment from 2.1 holds, the statement of the theorem should match the goal. You want somehow to state Linearized CVaR is more "conservative" than CVaR and you want those terms to be in it.}
% \begin{theorem}[Subadditivity of CVaR]
%     For any package $X=\{x_1, \dots, x_n\}$ and $P \in (0, 1]$, the following holds:
%     $$\sum_{i=1}^{n} CVaR_{P}(t_i.A)*x_i \geq V \implies CVaR_{P}(X) \geq V$$
%     \label{theorem:cvar}
% \end{theorem}

% We prove Theorem~\ref{theorem:cvar} in Appendix Section~\ref{appendix:subadditivity}. Together, Theorems~\ref{theorem:var}~and~\ref{theorem:cvar} show that we can represent all risk constraints in a query as linear constraints with two sets of conversions. First, we convert all VaR constraints to CVaR constraints. Second, we convert all CVaR constraints to linearized CVaR constraints. The coefficients of linearized CVaR constraints are the values of $CVaR_P(t_i.A)$, the expected value of the random variables $t_i.A$ corresponding to the stochastic attribute $A$ of the tuples $t_i$ in the $P$-lower fractile of their distributions. Using SAA, this can be found trivially for a given tuple $t_i$ and attribute $A$ --- we sort all $m$ scenario values of $t_i.A$ in ascending order, and take the average of the lowest $\lfloor pm \rfloor$ values (Algorithm~\ref{alg:approx}).



% In summary, we are ready to formulate any SPQ as an ILP. Every tuple $t_i$ in the relation is associated with an integer decision variable $x_i$. These decision variables represent multiplicities and are hence non-negative ($x_i \geq 0$ is implied). Repeat, package size and deterministic constraints are added to the ILP using their linear representations. Expected sum constraints are linearized using the linearity of expectation. VaR constraints are converted to CVaR constraints, and CVaR constraints are converted to linearized CVaR constraints, whose linear constraints contain the CVaR of every tuple $t_i$ as the coefficients of $t_i$. Objectives can be denoted as linear combinations of the values of $x_i$. Wherein required, we approximate expected values and CVaRs of stochastic attributes of individual tuples using $m$ optimization scenarios.

%Theorem~\ref{theorem:var} and theorem~\ref{theorem:cvar} imply that any package $\{x_1,...,x_N\}$, satisfying a ``linearized CVaR'' constraint, $\sum_{i=1}^N\mathbb{E}[t_i.\textbf{A}|t_i.\textbf{A} \leq F^{-1}_{t_i.\textbf{A}}(p)]\,x_i \geq v$ will also satisfy the VaR constraint $\Pr(\sum_{i=1}^N t_i.\mathbf{A}\, x_i \leq v) \leq p$. Linearized CVaR constraints are linear combinations of the multiplicities of each tuple in a package and their coefficients. The coefficients, which are the CVaRs of each tuple, can be computed before assigning values to $x_i$. Thus, by using linearized CVaRs to approximate VaRs, we effectively convert an SPQ into an ILP. Our proposed approach \cvarif thus converts each VaR constraint in a \spaqlp query to a CVaR constraint, and then converts each CVaR constraint to their linearized versions. However, linearized CVaR constraints, being conservative approximations of VaR constraints, can make the problem harder to satisfy, meaning the corresponding ILPs can be infeasible or have sub-optimal solutions. To overcome this,  our proposed approach \cvarif gradually relaxes the thresholds of the linearized CVaR constraints by appropriately adjusting their bounds, i.e., the values of $v$.

%\azza{More issues with algorithm 2:
%\begin{itemize}
%    \item You don't define $X$ anywhere. What is X?
%    \item What exactly is the output of Algorithm 1? Can you term it or explain it?
%    \item What exactly does a constraint matrix reprsent. How does interact with the Query in Formulate ILP? Why is it not directly changing the Query, which we then pass to Formulate ILP. Why is the output of FormulateILP another Query? The notation of Q is so overloaded and its interaction with M is confusing.
%\end{itemize}
%}
%\section{\cvarif}\label{sec:cvarif}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[scale=0.20]{figures/Original Feasible Region.jpg}
        \caption{Non-convex Feasible region with VaR constraint}
        \label{subfig:spq-with-var}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[scale=0.20]{figures/Over-constrained Feasible Region.jpg}
        \caption{Over-constrained Region, Suboptimal Package}
        \label{subfig:overconstrained}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[scale=0.20]{figures/Underconstrained Feasible Region.jpg}
        \caption{Underconstrained Region, Infeasible Package}
        \label{subfig:underconstrained}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[scale=0.20]{figures/Appropriately Constrained Feasible Region.jpg}
        \caption{Appropriate Approximation of Feasible Region}
        \label{subfig:appropriate}
    \end{subfigure}
    \caption{CVaR approximation of VaR Constraint}
    \label{fig:cvar-approx}
\end{figure*}

%Formulating ILPs from SPQs makes the optimization problems convex. However, the conversions of all risk constraints to linearized CVaR constraints we propose in Section~\ref{sec:prob} are conservative. The generated packages may be risk-averse. While they satisfy the original risk constraints, they may not be near-optimal since the conservative constraints can shrink the feasible region of the ILP too much.


==> sections/old_files/spq_syntax.tex <==
\section{The \langname{} syntax} \label{sec:spaql+syntax}
\langname{} extends \textit{SPaQL} by allowing users to specify CVaR constraints. Fig \ref{fig:spaql+_syntax} demonstrates the syntax of \langname{}. The \textit{PACKAGE} keyword (Line 1) differentiates the package query from traditional SQL ones. An alias for the package name can be optionally provided. The user then specifies the relation being addressed in the query (Line 2). We focus on single relation queries in this paper, and processing SPQ-s that address joins of multiple-relations remains a scope for future work. Optionally, the user can specify a repeat constraint, which limits the number of times the same tuple can be included in a package. Repeat 0 indicates that no tuple can be repeated, meaning each tuple can appear at most once in the package. Setting the repeat value to any non-negative integer $R$ indicates that a tuple can be included at most $R+1$ times in a package. In the absence of a repeat constraint, any tuple can be repeated any number of times. The user can express selection predicates specifying specific attribute values they want in the tuples included in the package with the WHERE clause as in traditional SQL queries (Line 3). Constraints on aggregates of the tuples included in a package can be of several types. Package size constraints specify the minimum/maximum number of tuples in a package (Line 5), deterministic constraints express the minimum/maximum value of the sum for a deterministic attribute (Line 6), expected value constraints constrain the minimum/maximum expected sum for a stochastic attribute (Line 7), while VaR and CVaR constraints (Lines 8 and 9) constrain the risks involved with the package. A \langname{} query can contain any number of package size, deterministic, expected value and risk constraints grouped together with a `SUCH THAT' clause (Line 4), and will always end a line specifying the objective, which can be either minimizing or maximizing the sum (expected sum for stochastic attributes) of an attribute (Line 10). 

\begin{figure}[t]
    \begin{flushleft}
        \texttt{\footnotesize 1. SELECT PACKAGE(*) [AS alias\_name]\\
        2. FROM table\_name [REPEAT R]\\
        3. WHERE [predicate\_clause]\\
        4. SUCH THAT\\
        5. \hspace{0.2cm}  [COUNT(alias\_name.*) [$\leq$ | $\geq$] S] AND\\
        6. \hspace{0.2cm}  [SUM($A_{1}$) [$\leq$ | $\geq$] $V_{1}$] AND\\
        7. \hspace{0.2cm}  [EXPECTED SUM($A_{2}$) [$\leq$ | $\geq$] $V_{2}$] AND\\
        8. \hspace{0.2cm}  [SUM($A_{3}$) [$\leq$ | $\geq$] $V_{3}$ WITH PROBABILITY >= $p_3$] AND\\
        9. \hspace{0.2cm}  [EXPECTED SUM($A_4$) [$\leq$ | $\geq$] $V_4$ IN [LOWEST | HIGHEST] $p_4$\% OF SCENARIOS]\\
        10.[MAXIMIZE | MINIMIZE] [EXPECTED] SUM($A_5$)
        }
    \end{flushleft}
    \caption{Syntax of \langname{}}
    \label{fig:spaql+_syntax}
\end{figure}


==> sections/preliminaries.tex <==
\section{Preliminaries} \label{sec:preliminaries}

Stochastic Package Queries (SPQs) are extensions of (deterministic) Package Queries that allow specifying constraints and objectives over stochastic attributes and provide opportunities for risk control by constraining Values-at-Risk (VaRs) and Conditional Values-at-Risk (CVaRs). This section overviews Package Queries, \skr --- the scalable approach for solving them, and preliminary concepts related to SPQ processing. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{Package_Queries_To_ILPs.jpg}
    \caption{A package query and its equivalent ILP formulation}
    \label{fig:deterministic_package_query_to_ilp}
\end{figure}

A \textbf{Package Query} (PQ)~\cite{brucato2018package} is a database specification of an Integer Linear Program (ILP) that returns a package - a multiset of tuples in the relation that satisfies local and global predicates. A local predicate requires each tuple in the package to individually satisfy boolean conditions. In Figure~\ref{fig:deterministic_package_query_to_ilp} for instance, the package query requires only gluten-free recipes, a condition that each tuple in the package must satisfy. A global predicate requires all tuples to collectively satisfy a linear constraint, such as finding a meal with at most 3 dishes, which constrains packages to having at most 3 tuples. Among packages satisfying all the predicates, we attempt to find one that optimizes a linear objective, for instance, finding a meal with the least total fat content.\azza{I do not like multiple illustrative examples. Stick with the one example of stocks. Also, I don't immediately see the value add to what was said about PQs in the intro.}

\textbf{\skr} proposes a divide-and-conquer approach to efficiently solve PQs in large relations \cite{brucato2018package} by partitioning the relation offline into small groups of similar tuples. After partitioning, \skr formulates a much smaller relation containing one representative tuple per partition whose value for each attribute is the mean of the values of all the tuples in the partition. During query execution, \skr first solves the ``sketch'' query over the representative tuples. During the `refine' phase, \skr iteratively replaces each representative selected during sketch with tuples from their partition by solving an ILP in each step. The final package is obtained when all refinements are done. \azza{This is just a longer repeat of what you already say in the intro. It doesn't add much and can be removed entirely.}

\textbf{Stochastic Package Queries} (SPQs)~\cite{BrucatoYAHM20} extend PQs by allowing probabilistic constraints and objectives. In a probabilistic relation of $N$ tuples, we denote $t_i.\mathbf{A}$ as the random variable of stochastic attribute $\mathbf{A}$ of tuple $t_i$ ($i \in \{1,\dots,N\}$), for example, the gain of a particular stock are particular period of time. An example of a probabilistic constraint with respect to this gain could be: $\Pr(\sum_{i=1}^N t_i.\mathbf{A}\, x_i \leq -10) \leq 0.05$, i.e., the probability of an at-least-ten-dollar loss of the stock portfolio is at most $5\%$. Here $x_i \geq 0$ is the multiplicity of tuple $t_i$, i.e., how many stocks one would purchase and sell after a given number of dates. Therefore, an SPQ requires finding a package $\{x_1,\dots,x_N\}$ that satisfies:~(i)~all deterministic constraints such as the investment budget being capped at one thousand dollars, i.e., $\sum_{i=1}^N t_i.P\, x_i \leq 1000$ ($P$ denoting price of a tuple)~(ii)~all probabilistic constraints such as the aforementioned Value-at-Risk (VaR) constraint. \azza{aforementioned ... this is too stuffy! but more importantly, where was it aforementioned? You don't actually say that the probabilistic constraint is in fact a Value at Risk constraint. This needs to be explicitly stated!} In this paper, we introduce a new type of risk constraint in SPQs called Conditional Value-at-Risk (CVaR) constraints~\cite{Sarykalin2008} (Section~\ref{sec:prob}) which constrain tail risks for packages and can conveniently be used to solve SPQs containing VaR constraints quickly, as we show in Section~\ref{sec:cvarif}.\azza{This section has value. I wonder though if it is just part of the next section and it has no place here.}

\textbf{Optimization and Validation}: In SPQs, optimization and validation procedures use scenarios to approximate probabilistic constraints. A scenario is simply a realization of all the random variables in one instance. We usually rely on a predefined number (say $m$) of scenarios to accurately optimize or validate a probabilistic constraint. For example, given $s_{ij}.\mathbf{A}$ the realized value of stochastic attribute $\mathbf{A}$ of tuple $t_i$ in scenario $j$, then let $y_j=\mathbbm{1}({\sum_{i=1}^N s_{ij}.\mathbf{A}\,x_i \leq -10})$ be the indicator function of whether the stock portfolio has at least 10 dollars of loss in scenario $j$. To optimize or validate is simply to make sure that $\sum_{i=1}^m y_i \leq 0.05m$.\azza{Again, I'm inclined to say that this was touched upon in the intro when you described how SAA works ... there are no further details here that add more to what you said in the intro, to merits its own place in a prelim section.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We first overview package queries, their equivalence with ILPs, \skr, and provide preliminaries of SPQ processing.
% %This section discusses deterministic package queries, and their equivalence with Integer Linear Programming (ILP) problems, before briefly reviewing \textit{SketchRefine}, which helps scale package queries on large deterministic relations. We then discuss SPQ-s, and their equivalent SILP formulations, before explaining how \textit{SummarySearch} generates packages in response to them.

% %\subsection{Deterministic Package Queries}\label{subsec:det_package_queries}

% \textbf{Deterministic Package Queries:}~Suppose we want $3$ gluten-free meals with minimal fat content while avoiding too many repetitions and keeping calorie consumption within acceptable bounds.

% Fig.~\ref{fig:deterministic_package_query_to_ilp} shows a package query for this, and its equivalent ILP formulation. If $x_i$ is the number of times the $i$-th tuple in an $n$-tuple relation is included in the package, package building becomes equivalent to finding an optimal assignment of $\{x_1, x_2, x_3,$ ..., $x_n\}$ such that $\forall 1 \leq i \leq n$, $x_i \geq 0$, and $\sum_{i=1}^{n} A_i * x_i$ is optimized subject to all constraints in the query, where $A$ is the attribute whose sum is to be optimized, and $A_i$ is its value in the $i$-th tuple. If the $i$-th tuple does not satisfy the query's base predicate, we add the constraint $x_i = 0$, keeping the tuple away from the package. For repetition constraints that restrict the number of repetitions of a tuple in the package to $R$, we add constraints $x_{i} \leq (1+R)$ for all $i \in \{1, ..., n\}$. A package size constraint limiting the number of tuples in the package to at most (least) $s$ can be expressed as $\sum_{i=1}^{n}x_{i} \leq s$ ($\geq s$). A constraint limiting the sum of an attribute $C$ in the package to at most (least) $L$ can be expressed as $\sum_{i=1}^{n} C_i * x_i \leq L$ ($\geq L$).

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.4]{Package_Queries_To_ILPs.jpg}
%     \caption{A package query and its equivalent ILP formulation}
%     \label{fig:deterministic_package_query_to_ilp}
% \end{figure}

% %\subsection{Scaling Deterministic Package Query Processing: \textit{SketchRefine}} \label{subsec:sketchrefine_deterministic}
% \textbf{\skr:}~Such ILP formulations contain as many variables as tuples in the relation, making them infeasible to be solved by in-memory solvers for large relations~\cite{brucato2018package}. \skr solves this by breaking down the problem into a series of more manageable subqueries on subsets of tuples of the relation. 

% It first partitions the relation offline, splitting the tuples into size-constrained groups containing tuples with similar values for every attribute. For each resulting partition, a representative is constructed by taking the mean of all tuples in the partition for each attribute, collectively forming a new `representative' relation.

% Query execution in \skr consists of the Sketch and Refine phases. During sketch, the query is executed on the representative relation. The size of the representative relation equalling the number of partitions, is much smaller than the actual relation. Hence, executing queries on it requires much lower runtime than executing the query on the whole relation. Once the `sketch package' is obtained, `refine' starts. Each representative included in the sketch package is sequentially `refined' --- the representative is replaced by tuples from its partition. Each refinement solves an ILP consisting of all the tuples included in the partition of the representative being replaced, the yet unrefined representatives from the sketch solution, and the tuples obtained from any previous refinements. Since the number of tuples in each partition is bounded, and the number of tuples in a package is typically small, the total number of tuples scoped within each refinement is also low. The final package is obtained when all refinements are done.

% %\subsection{Stochastic Package Queries as SILP-s:}\label{subsec:spqs_to_silps}

% \textbf{Problem Formulation:}~SPQ can have objectives defined on probabilistic attributes, where the expected sum of the attribute in the package is to be optimized. Suppose, $x_i$ again represents the number of times the i-th tuple is included in the package. If an SPQ requires maximizing the expected sum over a stochastic attribute $A$, we generate $m$ scenarios for $A$. If the value of the $i$-th tuple in the $j$-th scenario is $S^{A}_{ij}$, finding an optimal package translates to finding an optimal assignment of $\{ x_1, x_2, x_3, ..., x_n \}$, such that $\frac{1}{m} \sum_{j=1}^{m} \sum_{i=1}^{n} S^{A}_{ij}x_i$ is maximized, subject to the constraints specified. In addition to all forms of constraints in deterministic package queries, SPQs may have constraints based on expected sums and risks. If the expected sum of a package for an attribute $C$ cannot exceed $v$, we add the ILP constraint $\frac{1}{m} \sum_{j=1}^{m} \sum_{i=1}^{n} S^{C}_{ij}x_i \leq v$.

% \textbf{Value-at-Risk (VaR)}~constraints restrict the probability with which the sum of the values of the tuples in the package can exceed a given threshold. The VaR constraint in the query of Fig.~\ref{subfig:example_spaql} requires the sum of the resulting package's tuples' gains to be greater than $-10\$$ with at least 0.95 probability. For $m$ scenarios, the total losses of the resulting package should not exceed $10\$$ in at least $0.95 * m$ scenarios. A VaR constraint that restricts the sum of an attribute $B$ to at least $v$ is satisfied by a package $\{ x_1, x_2, x_3, ..., x_n \}$ in the $j$-th scenario iff $\sum_{i=1}^{n} S^{B}_{ij}x_{i} \geq v$. To ensure constraint satisfaction, we use indicator variables, a type of variable whose value can be conditionally set. For the j-th scenario, an indicator variable $I_{j}$ is 1 iff the VaR constraint is satisfied for the scenario (i.e. $\sum_{i=1}^{n} S^{B}_{ij}x_{i} \geq v$) and 0 otherwise. A VaR constraint that needs to be satisfied with a probability of $p$ is then satisfied over $m$ scenarios iff $\sum_{i=1}^{m} I_i \geq p*m$.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[scale=0.27]{figures/Solve-And-Validate Paradigm.jpg}
%     \caption{Separating optimization and validation scenarios}
%     \label{fig:solve-and-validate-paradigm}
% \end{figure}

% \textbf{Optimization \& Validation Scenarios}: Generating many scenarios for every tuple is time consuming, as is solving a mixed ILP with millions of indicator variables. Existing approaches~\cite{BrucatoYAHM20} thus generate packages based on few \textit{optimization} scenarios using SPQ solvers and validate the package's constraint satisfaction (i.e. validation feasibility) using numerous \textit{validation} scenarios (Fig.~\ref{fig:solve-and-validate-paradigm}). Validation scenarios need to generate values only for the few tuples in a package, thus needing little time for scenario generation.
% \iffalse
% \begin{expbox}{How does an ILP solver's runtime evolve with the number of optimization scenarios?}
% \includegraphics[height=0.5in, width=1.0in]{empty_square.jpg}
% \tcblower
% Adding one indicator variable for every optimization scenario results in increased runtimes for off-the-shelf ILP solvers. This plot demonstrates the effect of this on the runtime of Gurobi's ILP solver, in response to the query mentioned in Fig. \ref{fig:example_spaql} after omitting the CVaR constraint.
% \end{expbox}

% \subsection{\textit{SummarySearch}: Handling Hundreds of Optimization Scenarios}

% To overcome the problem of handling numerous optimization scenarios, prior work proposes \textit{SummarySearch}, where several optimization scenarios are bundled together to create one single modified scenario known as a summary. Summaries are designed to be conservative, in that if a package satisfies a constraint for a particular summary, it also satisfies all the scenarios used in constructing the summary. Since the number of summaries is much lower than the number of optimization scenarios considered, the number of indicator variables fed into the ILP solver is much lower than the number of variables that would be included in the solver if the one-indicator-variable-per-optimization-scenario approach was followed, resulting in lower ILP solver runtimes.

% We refer interested readers to Brucatto et al for details on the methods for constructing summaries, and formulating ILP problems using them. Here we focus on what \textit{SummarySearch} needs to do to find a package that is both feasible in that it satisfies all the constraints in the query, and whose objective score $\omega$ is near-optimal, i.e. is guaranteed to be within $(1 \pm \epsilon)\hat{\omega}$, where $\hat{\omega}$ is the objective score of the optimal package. For maximization problems, \textit{SummarySearch} is guaranteed to return a package that is at least $(1-\epsilon)\hat{\omega}$, while for minimization problems, the result is at most $(1+\epsilon)\hat{\omega}$. We call such a solution $(1 \pm \epsilon)$ approximate. \textit{SummarySearch} starts with a predefined number of optimization scenarios (e.g. 100), and incrementally increases this number until a feasible and $(1 \pm \epsilon)$-approximate solution is found. 

% For a fixed number of optimization scenarios, \textit{SummarySearch} tries to search for a suitable number of summaries. The lower the number of summaries, the lower the number of indicator variables used in the ILP formulation, resulting in lower ILP solver runtimes. If one summary is used, all optimization scenarios are bundled into a single group, and a subset of them are used to construct the summaries. On the other extreme, if the number of summaries is equal to the number of optimization scenarios, each optimization scenario becomes a summary itself, and \textit{SummarySearch} effectively becomes equivalent to the baseline approach of adding one indicator variable per optimization scenario.

% Due to their conservative nature, using a small number of summaries results in over-constrained ILP formulations, which in turn results in suboptimal packages. If the initial number of summaries used does not result in a $(1 \pm \epsilon)$ approximate package, \textit{SummarySearch} increases the number of summaries, and tries again. This continues iteratively until a $(1 \pm \epsilon)$-approximate solution is found. Algorithm \ref{alg:summarysearch_query_execution} shows an overview of how \textit{SummarySearch} controls the number of summaries and optimization scenarios used during its query evaluation.

% \begin{algorithm}[t]
% \caption{\textit{SummarySearch Query Execution}}\label{alg:summarysearch_query_execution}
% \begin{algorithmic}[1]

% \Require $Q$, stochastic package query w/o CVaR constraints
% \Statex $M$, initial number of optimization scenarios (e.g. $100$)
% \Statex $m$, increment in number of optimization scenarios (e.g. $100$)
% \Statex $\hat{M}$, number of validation scenarios (e.g. $10^6$)
% \Statex $Z$, initial number of summaries (e.g. $1$)
% \Statex $z$, increment in number of summaries (e.g. $1$)
% \Statex $\epsilon$, user defined approximation error bound
% \State $\overline{\omega} \gets $ Upper bound of the objective value of the optimal package
% \While{True}
%   \State $p \gets SolveWithSummaries(Q, M, \hat{M}, Z, \epsilon)$ \Comment{{\color{gray} \textit{Get a candidate package}}}
%   \If{$p.is\_feasible(Q) \And p.is\_1+\epsilon\_approx(\epsilon, \overline{\omega})$}
%     \State \Return p
%   \EndIf
%   \If{not $p.is\_feasible(Q)$}
%     \State $M \gets M + m$ \Comment{{\color{gray}\textit{Increase the number of scenarios if a feasible solution could not be found}}}
%   \EndIf
%   \If{not $p.is\_1+\epsilon\_approx(\epsilon, \overline{\omega})$}
%     \If{$Z \leq M$}
%       \State $Z  \gets Z + min(z, M-z)$ \Comment{{\color{gray}\textit{If possible, increase the number of summaries to make the corresponding ILP less conservative and potentially get more optimal packages}}}
%     \Else
%       \State $M \gets M + m$ \Comment{{\color{gray}\textit{If the number of summaries is already equal to the number of optimization scenarios, increase the number of optimization scenarios.}}}
%     \EndIf
%   \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}

% The runtime of \textit{SummarySearch} suffers when the initial number of optimization scenarios considered is not sufficient for deriving a $(1 \pm \epsilon)$-approximate solution. Such cases are highly likely to occur when the scenarios greatly vary from each other, which could happen due to high variance in many tuples, meaning that packages produced on the basis of a small number of optimization scenarios do not generalize well to large sets of validation scenarios. In such cases, \textit{SummarySearch} will continually enter the condition in Line 9 of Algorithm \ref{alg:summarysearch_query_execution}, and will increase the number of summaries repeatedly (Line 11) until the number of summaries is equal to the number of optimization scenarios. Only after the number of summaries equals the number of optimization scenarios does \textit{SummarySearch} consider increasing the number of optimization scenarios itself, something that in retrospect, should have been done right from the beginning. When the number of summaries does reach that extent, there is no difference between running \textit{SummarySearch} and running the naive approach suggested in the previous subsection. Thus, the runtime costs of \textit{SummarySearch} is greatly dependent on choosing a sufficient number of optimization scenarios initially, an assumption that becomes increasingly unsure when more tuples in a relation have greater variances.

% \subsection{Approximation Guarantees on the Quality of Packages Produced:} \label{subsec:approximation_guarantees_summary_search}
% \textit{SummarySearch} proposes methods to determine if a formulated package is $(1 \pm \epsilon)$-approximate for \textit{SPaQL} queries. \langname{} queries may additionally contain CVaR constraints, thus requiring tweaks to some of these methods which we explain in this section. Consider a maximization problem whose optimal solution has an objective value of $\hat{\omega}$. Our goal is to find a package with objective value $\omega \geq (1-\epsilon) \hat{\omega}$. If we can efficiently determine an upper bound $\overline{\omega} \geq \hat{\omega}$ and find a package with objective value $\omega \geq (1-\epsilon)\overline{\omega}$, then $\omega \geq (1-\epsilon)\hat{\omega}$ is guaranteed to be satisfied as well, since for all $0 \leq \epsilon \leq 1$, $(1-\epsilon)\overline{\omega} \geq (1-\epsilon)\hat{\omega}$. The following choices, if and when applicable, can be used as values of the upper bound $\overline{\omega}$:
% \begin{compactitem}
%     \item For any query $Q$, the objective value $\omega_{0}$ of the package obtained for a query $Q_{0}$ can be used as the upper bound, where $Q_{0}$ is the same as $Q$, but with all risk constraints removed. Removing any constraint results in a more loosely bounded SILP formulation, yielding optimal packages with greater (or equal) objective values than those of the original query. Removing risk constraints eliminates the need to depend on validation scenarios to ensure constraint satisfaction, meaning that the objective value of the package generated from any initial set of optimization scenarios can be used to determine the upper bound. The expected value of each tuple among the validation scenarios for each stochastic attribute can be precomputed offline, and used for computing the corresponding linear constraints for the expected value constraints. If removing all probabilistic constraints makes the query unbounded, \textit{SummarySearch} provides workarounds to replace the VaR constraints in the query with trivialized versions of them that are easy to satisfy. In \langname{}, a query may potentially only contain CVaR constraints. If one such CVaR constraint requires the expected sum of an attribute $A$ to be over a certain value $V'$ in the lowest $P\%$ of scenarios, we relax the "lowest $P\%$ of scenarios" part of the query, making it an expected value constraint of the form `EXPECTED SUM(A) >= V' that can be satisfied over the full set of validation scenarios using the precomputed expected values of each tuple. Similar treatment can be done for other forms of CVaR constraints.    
%     \item If a query $Q$ contains both a VaR and a CVaR constraint that work \textit{against} the objective, for instance, if, for an attribute $A$ whose expected sum is to be maximized in the objective value, there exists a VaR constraint in the form of \texttt{SUM(A) <= V WITH PROBABILITY >= P} and a CVaR constraint in the form of \texttt{EXPECTED SUM(A) <= $V'$ IN HIGHEST $(1-P)*100$\% OF SCENARIOS} (i.e the constraints limit the sum of the attribute while the objective asks to maximize it), then, the optimal solution's objective value is upper bounded by $P*min(V, V') + (1-P)*V'$. To understand why this is true, we observe the expected sum of the attribute in the extreme $(1-P)$-portion of upper tail scenarios is bounded to $V'$ by the CVaR constraint. For the remaining $P$-portion of scenarios with lower sums, no scenario can have a higher sum than $V$, and the expected sum of the scenarios with lower values cannot be greater than that of the upper tail, and hence is bounded by $V'$ as well. Thus, the expected sum of the attribute in these scenarios cannot be greater than $V'$, making the overall expected sum bounded by $P*min(V, V') + (1-P)*V'$. If there exists only such a CVaR constraint in the query (and not a VaR constraint), the upper bound will become $V'$.
%     \item If the query has a size constraint limiting the number of tuples in a package to within $S$, and the maximum value in any scenario by any tuple for the attribute addressed in the objective is $V_{max}$, the objective value of the optimal package is bounded by $S*V_{max}$.
% \end{compactitem}

% If multiple upper bounds are applicable in a maximization query, we consider the minimum among them to be $\overline{\omega}$. Queries whose objectives involve minimizing sums of an attribute can have their lower bounds defined similarly.

% \fi

==> tables/ilp_system.tex <==
\begin{equation*}
\begin{aligned}
\max_{x_1,x_2... \geq 0} \quad & 0.5x_1+...+3.9x_{730}+1.2x_{731}+...+8.65x_{1460}+...\\
\textrm{s.t.} \quad & 195.71x_1+...+195.71x_{730}+373.04x_{731}+...+373.04x_{1460}+... \leq 1000\\
  & -1.2x_1-...-0.1x_{730}-4.3x_{731}-...-12.4x_{1460}-... \geq -10\\
\end{aligned}
\end{equation*}


==> tables/scenarios_examples.tex <==
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|lcr|}
% \multicolumn{3}{l}{\textbf{Scenario}}\\
\hline
\textbf{ID} & \ldots & \textbf{Gain} \\
% \midrule
1 & \ldots & -1.53                      \\
2 & \ldots & -1.34                       \\
3 & \ldots & 0.78                      \\
%4 & 0.84                    \\
& \ldots &                  \\
730 & \ldots & 23.45                       \\
731 & \ldots & 0.34                       \\
732 & \ldots & 0.23                     \\
%0.18                    \\
& \ldots &                     \\
1460 & \ldots & -13.34                       \\
& \ldots &                      \\
\hline
\end{tabular}
\setlength{\tabcolsep}{6pt}
% 
% \begin{tabular}{lcr}
% \toprule
% \multicolumn{1}{l}{\textbf{ID}} & \multicolumn{1}{c}{\ldots} & \multicolumn{1}{r}{\textbf{Gain}} \\
% \midrule
% 1 & \ldots & 0.45                      \\
% 2 & \ldots & 0.56                       \\
% 3 & \ldots &0.42                      \\
% %0.38                     \\
% \ldots                      \\
% 730 & \ldots & -3.15                       \\
% 731 & \ldots & -1.34                       \\
% 732 & \ldots & -2.23                     \\
% %-1.85                      \\
% \ldots                       \\
% 1460 & \ldots & 11.25                       \\
% \ldots                       \\
% \bottomrule
% \end{tabular}
% \begin{tabular}{lcr}
% \toprule
% \multicolumn{1}{l}{\textbf{ID}} & \multicolumn{1}{c}{\ldots} & \multicolumn{1}{l}{\textbf{Gain}} \\
% \midrule
% 1 & \ldots & 2.45                      \\
% 2 & \ldots & 3.45                       \\
% 3 & \ldots & 3.76                      \\
% %3.91                     \\
% \ldots                      \\
% 730 & \ldots & 31.45                       \\
% 731 & \ldots & 1.56                       \\
% 732 & \ldots & 0.94                     \\
% %1.28                    \\
% \ldots                       \\
% 1460 & \ldots & 8.76                       \\
% \ldots                       \\
% \bottomrule
% \end{tabular}

==> tables/scenarios_for_gain_table.tex <==

\begin{tabular}{lcr}
\toprule
\multicolumn{1}{l}{\textbf{ID}} & \multicolumn{1}{c}{\ldots} & \multicolumn{1}{r}{\textbf{Gain}} \\
\midrule
1 & \ldots & -1.53                      \\
2 & \ldots & -1.34                       \\
3 & \ldots & 0.78                      \\
%4 & 0.84                    \\
\ldots                      \\
730 & \ldots & 23.45                       \\
731 & \ldots & 0.34                       \\
732 & \ldots & 0.23                     \\
%0.18                    \\
 \ldots                       \\
1460 & \ldots & -13.34                       \\
\ldots                       \\
\bottomrule
\end{tabular}
\begin{tabular}{lcr}
\toprule
\multicolumn{1}{l}{\textbf{ID}} & \multicolumn{1}{c}{\ldots} & \multicolumn{1}{r}{\textbf{Gain}} \\
\midrule
1 & \ldots & 0.45                      \\
2 & \ldots & 0.56                       \\
3 & \ldots &0.42                      \\
%0.38                     \\
& \ldots &                      \\
730 & \ldots & -3.15                       \\
731 & \ldots & -1.34                       \\
732 & \ldots & -2.23                     \\
%-1.85                      \\
& \ldots &                      \\
1460 & \ldots & 11.25                       \\
& \ldots &                      \\
\bottomrule
\end{tabular}
\begin{tabular}{lcr}
\toprule
\multicolumn{1}{l}{\textbf{ID}} & \multicolumn{1}{c}{\ldots} & \multicolumn{1}{l}{\textbf{Gain}} \\
\midrule
1 & \ldots & 2.45                      \\
2 & \ldots & 3.45                       \\
3 & \ldots & 3.76                      \\
%3.91                     \\
& \ldots &                      \\
730 & \ldots & 31.45                       \\
731 & \ldots & 1.56                       \\
732 & \ldots & 0.94                     \\
%1.28                    \\
& \ldots &                        \\
1460 & \ldots & 8.76                       \\
& \ldots &                       \\
\bottomrule
\end{tabular}

==> tables/stock_saa.tex <==

\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{l}{\bf ID} & \multicolumn{1}{l}{\bf Stock} & \multicolumn{1}{l}{\bf Price} & \multicolumn{1}{l}{\bf Sell After} & \makecell{\bf Expected \\ \bf Gain} & \makecell{\bf Expected Gain at \\ \bf Lower 5 Percentile} \\
\midrule
1                      & AAPL              & 195.71                       & 0.5 days                       & 0.5 & -1.2                        \\

2                      & AAPL               & 195.71                       & 1 day                     & 0.88 & -1.0                           \\

3                      & AAPL               & 195.71                       & 1.5 days                     & 0.99 & -0.74                           \\
%4                      & AAPL               & 195.71                       & 2 days                     & ?                         \\
...                    & ...                & ...                          & ...                       & ...  & ...                     \\
730                      & AAPL           & 195.71                       & 365 days                      & 3.9 & -0.1                           \\
731                      & MSFT              & 373.04                       & 0.5 days                      & 1.2 & -4.3                           \\
732                      & MSFT             & 373.04                       & 1 day                      & 1.4 & -3.7                           \\
%733                      & MSFT              & 373.04                       & 1.5 days                     & ?                        \\
...                    & ...                & ...                          & ...                       & ...  & ...                     \\
1460                      & MSFT               & 373.04                       & 365 days                      & 8.65 & -12.4    \\
...                    & ...                & ...                          & ...                       & ...  & ...                     \\
\bottomrule
\end{tabular}
